Lectures on Linear Algebra over Division Ring

In this book i treat linear algebra over division ring. A system of linear equations over a division ring has properties similar to properties of a system of linear equations over a field. However, noncommutativity of a product creates a new picture. Matrices allow two products linked by transpose. Biring is algebra which defines on the set two correlated structures of the ring. As in the commutative case, solutions of a system of linear equations build up right or left vector space depending on type of system. We study vector spaces together with the system of linear equations because their properties have a close relationship. As in a commutative case, the group of automorphisms of a vector space has a single transitive representation on a frame manifold. This gives us an opportunity to introduce passive and active representations. Studying a vector space over a division ring uncovers new details in the relationship between passive and active transformations, makes this picture clearer. Considering of twin representations of division ring in Abelian group leads to the concept of D vector space and their linear map. Based on polyadditive map I considered definition of tensor product of rings and tensor product of D vector spaces.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александр Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Aleks Kleyn.\\
Linear Algebra over Division Ring: System of Linear Equations.\\
Create Space, 2012; ISBN-13: 978-1477631812
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
Vol 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\BiblioItem
{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Biring.Russian.tex <==
%auto-ignore
\input{Biring.Eq}
\ifx\PrintBook\undefined
\else
\chapter{Бикольцо матриц}
\label{chapter: Biring of Matrices}
\fi
\section{Концепция обобщённого индекса}
\label{section: Concept of Generalized Index}

Изучая тензорное исчисление, мы начинаем с изучения
одновалентных ковариантного и контравариантного
тензоров. Несмотря на различие свойств, оба эти объекта
являются элементами соответствующих векторных пространств.
Если мы введём обобщённый индекс по правилу
$a^i=a^i$, $b^i=b^\cdot{}^-_i$,
то мы видим, что эти тензоры ведут себя одинаково.
Например, преобразование ковариантного тензора принимает форму
\[b'^i=
b'^\cdot{}^-_i=f^\cdot{}^-_i{}_\cdot{}^j_- b^\cdot{}^-_j
=f^i_j b^j\]

Это сходство идёт
сколь угодно далеко, так как тензоры
также порождают векторное пространство.

Эти наблюдения сходства свойств
ковариантного и контравариантного
тензоров приводят нас к концепции обобщённого
индекса.
Я пользуюсь символом $\cdot$ перед
обобщённым индексом, когда мне необходимо описать его структуру.
Я помещаю символ $'-'$ на месте индекса,
позиция которого изменилась. Например, если исходное
выражение было $a_{ij}$,
я пользуюсь записью $a_i{}^j_-$ вместо записи $a_i^j$.

Хотя структура обобщённого индекса произвольна, мы будем предполагать,
что существует взаимно однозначное отображение отрезка натуральных
чисел $1$, ..., $n$ на множество значений индекса. Пусть $i$ - множество
значений индекса $i$. Мы будем обозначать мощность этого множества
символом $|i|$ и будем полагать $|i|=n$. Если нам надо
перечислить элементы $a_i$, мы будем пользоваться обозначением
$a_1$, ..., $a_n$.

Представление координат вектора в форме матрицы позволяет сделать запись
более компактной. Вопрос о представлении вектора
как строка или столбец матрицы является вопросом соглашения.
Mы можем распространить концепцию обобщённого индекса на элементы матрицы.
Матрица - это двумерная таблица, строки и столбцы которой занумерованы
обобщёнными индексами.
Для представления матрицы мы будем пользоваться
одним из следующих представлений:
\begin{description}
\item [\AddIndex{Стандартное представление}{Standard representation}]
в этом случае мы представляем элементы матрицы $A$ в виде $A^a_b$.
\item [\AddIndex{Альтернативное представление}{Alternative representation}]
в этом случае мы представляем элементы матрицы $A$ в виде ${}^aA_b$
или ${}_bA^a$.
\end{description}
Так как мы пользуемся обобщёнными индексами,
мы не можем сказать, нумерует ли индекс $a$ строки
матрицы или столбцы,
до тех пор, пока мы не знаем структуры индекса.

Мы могли бы пользоваться терминами
$*$\hyph столбец и $*$\hyph строка, которые более близки традиционным.
Однако как мы увидим ниже для нас несущественна форма представления
матрицы.
Для того, чтобы обозначения, предлагаемые ниже,
были согласованы с традиционными,
мы будем предполагать, что матрица представлена в виде
\ShowEq{standard representation of matrix}

\begin{definition}
\label{definition: notation for matrix}
Я использую следующие имена и обозначения различных
\AddIndex{минорных матриц}{minor matrix}
матрицы $A$
\begin{description}
\begin{sloppypar}
\item
[\ShowEq{c row}\ \ ]
\AddIndex{\sups строка}{c row}
с индексом $a$ является обобщением
столбца матрицы. Верхний индекс перечисляет элементы
\sups строки, нижний индекс перечисляет \sups строки.
\end{sloppypar}
\item
[\ShowEq{A from columns T}\ \ ]
минорная матрица, полученная из $A$ выбором
\sups строк с индексом из множества $T$
\item [\ShowEq{A without column a}\ \ ]
минорная матрица, полученный из $A$ удалением
\sups строки $A_a$
\item [\ShowEq{A without columns T}\ \ ]
минорная матрица, полученный из $A$ удалением
\sups строк с индексом из множества $T$
\item [\ShowEq{r row}\ \ ]
\AddIndex{\subs строка}{r row}
с индексом $b$ является обобщением
строки матрицы. Нижний индекс перечисляет элементы
\subs строки, верхний индекс перечисляет \subs строки.
\item [\ShowEq{A from rows S}\ \ ]
минорная матрица, полученный из $A$ выбором \subs строк с индексом
из множества $S$
\item [\ShowEq{A without row b}\ \ ]
минорная матрица, полученный из $A$ удалением
\subs строки ${}^bA$
\item [\ShowEq{A without rows S}\ \ ]
минорная матрица, полученный из $A$ удалением \subs строк с индексом
из множества $S$
\end{description}
\qed
\end{definition}

\begin{remark}
\label{remark: combine the notation of indexes}
Мы будем комбинировать запись индексов. 
Так \ShowEq{A from b a} является $1\times 1$ минорной матрицей.
Одновременно, это обозначение элемента матрицы.
Это позволяет отождествить $1\times 1$ матрицу и её элемент.
Индекс $a$ является номером
\sups строки матрицы и
индекс $b$ является номером \subs строки матрицы.
\qed
\end{remark}

Каждая форма записи матрицы имеет свои преимущества.
Стандартная форма более естественна, когда мы изучаем
теорию матриц. Альтернативная форма записи делает выражения более ясными в теории
векторных пространств. Распространив альтернативную запись индексов
на произвольные тензоры, мы сможем лучше
понять взаимодействие различных геометрических объектов.
Опираясь на принцип двойственности (теорема
\ref{theorem: duality principle for biring of matrices}),
мы можем расширить наши выразительные возможности.

\begin{remark}
\label{remark: pronunciation of rows}
Мы можем договориться, что при чтении мы произносим символ \sups\ как
$c$\hyph\ и символ \subs\ как $r$\hyph, формируя тем самым названия \AddIndex{$c$\hyph строка}{c-row}
и \AddIndex{$r$\hyph строка}{r-row}. В последующем мы распространим это соглашение на другие
элементы линейной алгебры. Я буду пользоваться этим соглашением
при составлении индекса.
\qed
\end{remark}

Так как транспонирование матрицы меняет местами
\subs строки и \sups строки, то мы получаем равенство
\ShowEq{transpose of matrix, 1}

\begin{remark}
\label{remark: transpose of matrix}
Как видно из равенства
\EqRef{transpose of matrix, 1},
для нас несущественно, с какой стороны мы указываем номер
\subs строки и с какой стороны мы указываем номер \sups строки.
Это связано с тем, что мы можем нумеровать элементы матрицы
различными способами. Если мы хотим указывать
номера \subs строки и \sups строки согласно определению
\ref{definition: notation for matrix}, то равенство
\EqRef{transpose of matrix, 1}
примет вид
\ShowEq{transpose of matrix, 2}
В стандартном представлении равенство
\EqRef{transpose of matrix, 1}
примет вид
\ShowEq{transpose of matrix, 3}
\qed
\end{remark}

Мы называем матрицу\footnote{
Запись $({}^\cdot{}^-_iA_\cdot{}^j_-)^{-1}$
означает, что
при обращении Адамара столбцы и строки меняются местами.
\label{footnote: index of inverse element}
Мы можем
формально записать это выражение следующим образом
\[
({}^\cdot{}_i^-A_\cdot{}^j_-)^{-1}=
\frac 1{{}^iA_j}
\]}
\ShowEq{Hadamard inverse of matrix}
\AddIndex{обращением Адамара матрицы}{Hadamard inverse of matrix} $A=({}_bA^a)$
(\citeBib{q-alg-9705026}-\href{http://arxiv.org/PS_cache/q-alg/pdf/9705/9705026.pdf\#Page=4}{page 4}).

Я пользуюсь Эйнштейновским соглашением о суммировании.
Это означает, что, когда индекс присутствует в
выражении дважды и множество индексов известно, у меня есть сумма
по этому индексу.
Я буду явно указывать множество
индексов, если это необходимо. Kроме того, в этой статье
я использую туже корневую букву для матрицы и её элементов.

Мы будем изучать матрицы, элементы которых принадлежат телу $D$.
Мы также будем иметь в виду, что вместо тела $D$ мы можем
в тексте писать поле $F$. Мы будем явно писать поле $F$
в тех случаях, когда коммутативность
будет порождать новые детали.  
Обозначим через $1$ единичный элемент тела $D$.

Пусть $I$, $|I|=n$ - множество индексов.
\AddIndex{Символ Кронекера}{Kronecker symbol}
определён равенством
\ShowEq{Kronecker symbol}
\ShowEq{Kronecker symbol=}

\section{Бикольцо}
\label{section: Biring}

Мы будем рассматривать матрицы, элементы которых принадлежат телу $D$.

Произведение матриц связано с произведением гомоморфизмов
векторных пространств над полем. Согласно традиции произведение
матриц $A$ и $B$ определено как произведение
\subs строк матрицы $A$ и \sups строк матрицы $B$.
Условность этого определения становится очевидной,
если мы обратим внимание, что \subs строка матрицы $A$
может быть столбцом этой матрицы.
В этом случае мы умножаем столбцы матрицы $A$
на строки матрицы $B$.
Таким образом, мы можем определить два вида
произведения матриц.
Чтобы различать эти произведения, мы вводим
новые обозначения.\footnote{Для совместимости
обозначений с существующими мы будем иметь
в виду \RC произведение, когда
нет явных обозначений.}

\begin{definition}
\label{definition: rc-product of matrices}
\AddIndex{\RC произведение матриц}
{rc-product of matrices} $A$ и $B$ имеет вид
\ShowEq{rc-product of matrices}
и может быть выражено как произведение \subs строки матрицы $A$
и \sups строки матрицы $B$.\footnote{В альтернативной форме
операция состоит из двух символов $*$, которые записываются на
месте индекса суммирования. В стандартной форме операция имеет вид
\ShowEq{rc-product of matrices, 1}
и может быть интерпретирована
как символическая запись
\ShowEq{rc-product of matrices, 2}
где мы записываем символ $*$ на месте индекса,
по которому предполагается суммирование.}
\qed
\end{definition}

\begin{definition}
\label{definition: cr-product of matrices}
\AddIndex{\CR произведение матриц}
{cr-product of matrices} $A$ и $B$ имеет вид
\ShowEq{cr-product of matrices}
и может быть выражено как произведение
\sups строки матрицы $A$
на \subs строку матрицы $B$.\footnote{В альтернативной форме
операция состоит из двух символов $*$, которые записываются на
месте индекса суммирования. В стандартной форме операция имеет вид
\ShowEq{cr-product of matrices, 1}
и может быть интерпретирована
как символическую запись
\ShowEq{cr-product of matrices, 2}
где мы записываем символ $*$ на месте индекса,
по которому предполагается суммирование.}
\qed
\end{definition}

\begin{remark}
\label{remark: pronunciation of product}
Мы будем пользоваться символом \RC\  или \CR\  в имени свойств
каждого произведения и в обозначениях. Согласно замечанию
\ref{remark: pronunciation of rows} мы можем читать символы
$\RCstar$ и $\CRstar$ как $rc$\hyph произведение и $cr$\hyph произведение.
Это правило мы распространим на последующую терминологию.
\qed
\end{remark}

\begin{remark}
\label{remark: cr-product of matrices}
Также как и в замечании
\ref{remark: transpose of matrix},
я хочу обратить внимание на то, что я меняю нумерацию элементов
матрицы.
Если мы хотим указывать
номера \subs строки и \sups строки согласно определению
\ref{definition: notation for matrix}, то равенство
\EqRef{cr-product of matrices}
примет вид
\ShowEq{cr-product of matrices, 3}
Однако формат равенства
\EqRef{cr-product of matrices, 3}
несколько необычен.
\qed
\end{remark}

Множество $n\times n$ матриц замкнуто относительно \RC произведения и \CR произведения,
а также относительно суммы, определённой согласно правилу
\[
(A+B)_a^b=A_a^b+B_a^b
\]

\begin{theorem}
\label{theorem: rcstar transpose}
\ShowEq{rcstar transpose, 0}
\end{theorem}
\begin{proof}
Цепочка равенств
\ShowEq{rcstar transpose, 1}
следует из \EqRef{transpose of matrix, 1},
\EqRef{rc-product of matrices} и
\EqRef{cr-product of matrices}.
Равенство \EqRef{rcstar transpose, 0} следует из
\EqRef{rcstar transpose, 1}.
\end{proof}

Матрица $\delta=(\delta_a^c)$
является единицей для обоих произведений.

\begin{definition}
\label{definition: biring}
\AddIndex{Бикольцо}{biring} $\mathcal{A}$ - это множество,
на котором мы определили унарную операцию, называемую транспозицией,
и три бинарных операции,
называемые \RC произведение, \CR произведение и сумма, такие что
\begin{itemize}
\item \RC произведение и сумма определяют структуру кольца на $\mathcal{A}$
\item \CR произведение и сумма определяют структуру кольца на $\mathcal{A}$
\item оба произведения имеют общую единицу $\delta$
\item произведения удовлетворяют равенству
\begin{equation}
\EqLabel{rcstar transpose}
(A\RCstar B)^T=A^T\CRstar B^T
\end{equation}
\item транспозиция единицы есть единица
\begin{equation}
\EqLabel{transpose of identity}
\delta^T=\delta
\end{equation}
\item двойная транспозиция есть исходный элемент
\begin{equation}
\EqLabel{double transpose}
(A^T)^T=A
\end{equation}
\end{itemize}
\qed
\end{definition} 

\begin{theorem}
\label{theorem: cstart transpose}
\begin{equation}
\EqLabel{cstart transpose}
(A\CRstar B)^T=(A^T)\RCstar (B^T)
\end{equation}
\end{theorem}
\begin{proof}
Мы можем доказать \EqRef{cstart transpose} в случае матриц тем же
образом, что мы
доказали \EqRef{rcstar transpose}. Тем не менее для нас более
важно показать, что \EqRef{cstart transpose}
следует непосредственно из \EqRef{rcstar transpose}.

Применяя \EqRef{double transpose} к каждому слагаемому в левой части
\EqRef{cstart transpose}, мы получим
\begin{equation}
\EqLabel{cstart transpose, 1}
(A\CRstar B)^T=((A^T)^T\CRstar (B^T)^T)^T
\end{equation}
Из \EqRef{cstart transpose, 1} и \EqRef{rcstar transpose} следует, что
\begin{equation}
\EqLabel{cstart transpose, 2}
(A\CRstar B)^T=((A^T\RCstar B^T)^T)^T
\end{equation}
\EqRef{cstart transpose} следует из \EqRef{cstart transpose, 2}
и \EqRef{double transpose}.
\end{proof}

\begin{definition}
Мы определим \AddIndex{\RC степень}{rc power} элемента $A$ бикольца $\mathcal{A}$,
пользуясь рекурсивным правилом
\ShowEq{rc power}
\qed
\end{definition} 

\begin{definition}
Мы определим \AddIndex{\CR степень}{cr power} элемента $A$ бикольца $\mathcal{A}$,
пользуясь рекурсивным правилом
\ShowEq{cr power}
\qed
\end{definition} 

\begin{theorem}
\label{theorem: transpose power}
\begin{equation}
\EqLabel{rc transpose power}
(A^T)^{\RCPower n}=(A^{\CRPower n})^T
\end{equation}
\begin{equation}
\EqLabel{cr transpose power}
(A^T)^{\CRPower n}=(A^{\RCPower n})^T
\end{equation}
\end{theorem}
\begin{proof}
Мы проведём доказательство индукцией по $n$.

При $n=0$ утверждение непосредственно следует из равенств
\EqRef{rc power, 0}, \EqRef{cr power, 0} и \EqRef{transpose of identity}.

Допустим утверждение справедливо при $n=k-1$
\begin{align}
\EqLabel{rc transpose power, 0}
(A^T)^{\RCPower {n-1}}=(A^{\CRPower {n-1}})^T
\end{align}
Из \EqRef{rc power, n} следует
\begin{equation}
\EqLabel{rc transpose power, 1}
(A^T)^{\RCPower k}=(A^T)^{\RCPower {k-1}}\RCstar A^T
\end{equation}
Из \EqRef{rc transpose power, 1} и \EqRef{rc transpose power, 0} следует
\begin{equation}
\EqLabel{rc transpose power, 2}
(A^T)^{\RCPower k}=(A^{\CRPower {k-1}})^T\RCstar A^T
\end{equation}
Из \EqRef{rc transpose power, 2} и \EqRef{cstart transpose} следует
\begin{equation}
\EqLabel{rc transpose power, 3}
(A^T)^{\RCPower k}=(A^{\CRPower {k-1}}\CRstar A)^T
\end{equation}
Из \EqRef{rc transpose power, 1} и \EqRef{cr power, n} следует
\EqRef{rc transpose power}.

Мы можем доказать \EqRef{cr transpose power} подобным образом.
\end{proof}

\begin{definition}
Элемент
\ShowEq{rc-inverse element}
бикольца $\mathcal{A}$
- это \AddIndex{\RC обратный элемент}{rc-inverse element}
элемента $A$, если
\begin{equation}
\EqLabel{rc-inverse matrix}
A\RCstar A^{\RCInverse}=\delta
\end{equation}
Элемент
\ShowEq{cr-inverse element}
бикольца $\mathcal{A}$
- это \AddIndex{\CR обратный элемент}{cr-inverse element}
элемента $A$, если
\begin{equation}
\EqLabel{cr-inverse matrix}
A\CRstar A^{\CRInverse}=\delta
\end{equation}
\qed
\end{definition} 

\begin{theorem}
\label{theorem: transpose inverse}
Предположим, что элемент $A\in\mathcal{A}$ имеет \RC обратный элемент. Тогда транспонированный
элемент $A^T$ имеет \CR обратный элемент и эти
элементы удовлетворяют равенству
\begin{equation}
\EqLabel{rcstar transpose inverse}
(A^T)^{\CRInverse}=(A^{\RCInverse})^T
\end{equation}
Предположим, что элемент $A\in\mathcal{A}$ имеет \CR обратный элемент. Тогда транспонированный
элемент $A^T$ имеет \RC обратный элемент и эти
элементы удовлетворяет равенству
\begin{equation}
\EqLabel{cstart transpose inverse}
(A^T)^{\RCInverse}=(A^{\CRInverse})^T
\end{equation}
\end{theorem}
\begin{proof}
Если мы возьмём транспонирование обеих частей \EqRef{rc-inverse matrix}
и применим \EqRef{transpose of identity}, мы получим
\[
(A\RCstar A^{\RCInverse})^T=\delta^T=\delta
\]
Применяя \EqRef{rcstar transpose}, мы получим
\begin{equation}
\EqLabel{cstart transpose inverse, 1}
\delta=A^T\CRstar( A^{\RCInverse})^T
\end{equation}
\EqRef{rcstar transpose inverse} следует из сравнения
\EqRef{cr-inverse matrix} и \EqRef{cstart transpose inverse, 1}.

Мы можем доказать \EqRef{cstart transpose inverse} подобным образом.
\end{proof}

Теоремы \ref{theorem: rcstar transpose},
\ref{theorem: cstart transpose},
\ref{theorem: transpose power}
и \ref{theorem: transpose inverse} показывают,
что существует двойственность
между \RC произведением и \CR произведением.
Мы можем объединить эти утверждения.

\begin{theorem}
[\AddIndex{принцип двойственности для бикольца}
{duality principle for biring}]
\label{theorem: duality principle for biring}
Пусть $\mathfrak{A}$ - истинное утверждение о
бикольце $\mathcal{A}$.
Если мы заменим одновременно
\begin{itemize}
\item $A\in\mathcal{A}$ и $A^T$
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}

\begin{theorem}
[\AddIndex{принцип двойственности для бикольца матриц}
{duality principle for biring of matrices}]
\label{theorem: duality principle for biring of matrices}
Пусть $\mathcal{A}$ является бикольцом матриц.
Пусть $\mathfrak{A}$ - истинное утверждение о матрицах.
Если мы заменим одновременно
\begin{itemize}
\item \sups строки и \subs строки всех матриц
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}
\begin{proof}
Непосредственное следствие
теоремы \ref{theorem: duality principle for biring}.
\end{proof}

\begin{remark}
\label{remark: left and right matrix notation}
В выражении
\[A\RCstar B\RCstar C\]
мы выполняем операцию умножения слева направо.
Однако мы можем выполнять операцию умножения
справа налево. В традиционной записи это выражение примет вид
\[C\CRstar B\CRstar A\]
Мы сохраним правило,
что показатель степени записывается справа от выражения.
Если мы пользуемся стандартным представлением,
то индексы также записываются справа от выражения.
Если мы пользуемся альтернативным представлением,
то индексы читаются в том же порядке, что и символы операции
и корневые буквы.
Например, если исходное выражение имеет вид
\ShowEq{left and right matrix notation, 1}
то выражение, читаемое справа налево, примет вид
\ShowEq{left and right matrix notation, 2}
в стандартном представлении либо примет вид
\ShowEq{left and right matrix notation, 3}
в альтернативном представлении.

Если задать порядок, в котором мы записываем индексы,
то мы можем утверждать, что мы читаем выражение сверху вниз,
читая сперва верхние индексы, потом нижние. Договорившись, что
это стандартная форма чтения, мы можем прочесть выражение снизу вверх.
При этом мы дополним правило, что символы операции также читаются в том же
направлении, что и индексы. Например, выражение
\ShowEq{left and right matrix notation, 4}
прочтённое снизу вверх, в стандартной форме имеет вид
\ShowEq{left and right matrix notation, 5}
Согласно принципу двойственности, если верно одно утверждение,
то верно и другое.
\qed
\end{remark}

\begin{theorem}
\label{theorem: two products equal}
Если матрица $A$ имеет \RC обратную матрицу, то для любых матриц
$B$ и $C$ из равенства
\begin{equation}
\EqLabel{two products equal, 1}
B\RCstar A=C\RCstar A
\end{equation}
следует равенство
\begin{equation}
\EqLabel{two products equal, 2}
B=C
\end{equation}
\end{theorem}
\begin{proof}
Равенство \EqRef{two products equal, 2} следует из
\EqRef{two products equal, 1}, если обе части равенства
\EqRef{two products equal, 1} умножить на $A^{\RCInverse}$.
\end{proof}

\section{Квазидетерминант}
\label{section: Quasideterminant}

\begin{theorem}
\label{theorem: inverse minor}
Предположим, что $n\times n$ матрица $A$
имеет \RC обратную матрицу.\footnote{Это утверждение
и его доказательство основаны
на утверждении 1.2.1 из \citeBib{math.QA-0208146}
(\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=8}{page 8})
для матриц над свободным кольцом с делением.}
Тогда $k\times k$ минорная матрица \RC обратной матрицы 
удовлетворяет равенству
\ShowEq{inverse minor}
\end{theorem}
\begin{proof}
Определение \EqRef{rc-inverse matrix} \RC обратной матрицы
приводит к системе линейных уравнений
\ShowEq{inverse minor, 1}
Мы умножим \EqRef{inverse minor, 11} на
\ShowEq{inverse minor,3}
Теперь мы можем подставить \EqRef{inverse minor,3} в
\EqRef{inverse minor, 12}
\ShowEq{inverse minor,4}
\EqRef{inverse minor} следует из \EqRef{inverse minor,4}.
\end{proof}

\begin{corollary}
\label{corollary: inverse matrix}
Предположим, что $n\times n$ матрица $A$
имеет \RC обратную матрицу.
Тогда элементы \RC обратной матрицы удовлетворяют
равенству\footref{footnote: index of inverse element}
\ShowEq{inverse matrix}
\qed
\end{corollary}

\begin{example}
Рассмотрим матрицу
\ShowEq{inverse matrix 2x2, 0}
Согласно \EqRef{inverse matrix}
\ShowEq{inverse matrix 2x2}
\ePrints{0612.111}
\ifx\Semafor\ValueOn
Рассмотрим произведение матриц
\ShowEq{inverse matrix 2x2, 1}
Из непосредственных вычислений следует
\ShowEq{inverse matrix 2x2, 2}
\fi
\qed
\end{example}

Согласно \citeBib{math.QA-0208146},
\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=3}{page 3}
у нас нет определения
детерминанта в случае тела.
Тем не менее, мы можем определить квазидетерминант,
который в конечном итоге даёт похожую картину.
В определении, данном ниже, мы следуем определению
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=9}{1.2.2}.

\begin{definition}
\label{definition: RC-quasideterminant}
\AddIndex{$(^j_i)$\hyph \RC квазидетерминант}{j i RC-quasideterminant}
$n\times n$ матрицы $A$
- это формальное выражение\footref{footnote: index of inverse element}
\ShowEq{j i RC-quasideterminant definition}
\ShowEq{j i RC-quasideterminant =}
Согласно замечанию \ref{remark: combine the notation of indexes}
мы можем рассматривать $(^j_i)$\hyph \RC квазидетерминант
как элемент матрицы
\ShowEq{RC-quasideterminant definition},
которую мы будем называть
\AddIndex{\RC квазидетерминантом}{RC-quasideterminant}.
\qed
\end{definition}

\begin{theorem}
Выражение для \RC обратной матрицы имеет вид
\begin{equation}
\EqLabel{quasideterminant and inverse}
A^{\RCInverse}=
\mathcal{H}\RCDet{A}
\end{equation}
\end{theorem}
\begin{proof}
\EqRef{quasideterminant and inverse} следует
из \EqRef{j i RC-quasideterminant =}.
\end{proof}

\begin{theorem}
Выражение для
$(^j_i)$\hyph \RC квазидетерминанта
имеет любую из следующих форм\footnote{Мы можем дать подобное
доказательство для
\AddIndex{$(^j_i)$\hyph \CR квазидетерминанта}{j i cr-quasideterminant}.
Однако мы можем записать соответствующие утверждения,
опираясь на принцип двойственности. Так, если прочесть равенство
\EqRef{quasideterminant, 1} справа налево, то мы получим равенство
\ShowEq{CR quasideterminant definition}
}
\ShowEq{quasideterminant, expression}
\end{theorem}
\begin{proof}
Утверждение  следует
из \EqRef{inverse matrix, Hadamard} и
\EqRef{j i RC-quasideterminant =}.
\end{proof}

\begin{example}
Рассмотрим матрицу
\ShowEq{inverse matrix 2x2, 0}
Согласно \EqRef{quasideterminant, 1}
\ShowEq{quasideterminant, matrix 2x2}
\qed
\end{example}

\begin{theorem}
\label{theorem: two quasideterminants}
\ShowEq{CR and RC quasideterminants}
\end{theorem}
\begin{proof}
Согласно \EqRef{j i RC-quasideterminant =}
и \EqRef{Hadamard inverse of matrix}
\ShowEq{CR and RC quasideterminants, 1}
Пользуясь теоремой \ref{theorem: transpose inverse}, мы получим
\ShowEq{CR and RC quasideterminants, 2}
Пользуясь \EqRef{transpose of matrix, 1}, мы имеем
\ShowEq{CR and RC quasideterminants, 3}
Пользуясь \EqRef{CR and RC quasideterminants, 3},
\EqRef{Hadamard inverse of matrix},
\EqRef{j i RC-quasideterminant =}, мы получим
\EqRef{CR and RC quasideterminants}.
\end{proof}

Теорема \ref{theorem: two quasideterminants} расширяет
принцип двойственности, теорема \ref{theorem: duality principle for biring of matrices},
на утверждения о квазидетерминантах и
утверждает, что одно и тоже выражение является \RC квазидетерминантом
матрицы $A$ и \CR квазидетерминантом матрицы $A^T$.
Пользуясь этой теоремой, мы можем
записать любое утверждение о \CR матрице,
опираясь на подобное утверждение о \RC матрице.

\begin{theorem}[принцип двойственности]
\label{theorem: duality principle, quasideterminants}
Пусть $\mathfrak{A}$ - истинное утверждение о бикольце матриц.
Если мы одновременно заменим
\begin{itemize}
\item \subs строку и \sups строку
\item \RC квазидетерминант и \CR квазидетерминант
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}

\begin{theorem}
\begin{align}
\EqLabel{inverse product of matrix over scalar, 1}
(mA)^{\RCInverse}&=A^{\RCInverse}m^{-1}\\
\EqLabel{inverse product of matrix over scalar, 2}
(Am)^{\RCInverse}&=m^{-1}A^{\RCInverse}
\end{align}
\end{theorem}
\begin{proof}
Мы докажем равенство \EqRef{inverse product of matrix over scalar, 1}
индукцией по размеру матрицы.

Для $1\times 1$ матрицы утверждение очевидно, так как
\ShowEq{inverse product of matrix over scalar, 1}

Допустим утверждение справедливо для $(n-1)\times(n-1)$ матрицы. Тогда из равенства
\EqRef{inverse minor} следует
\ShowEq{inverse product of matrix over scalar, 1, 1}
Из равенства \EqRef{inverse product of matrix over scalar, 1, 1}
следует равенство \EqRef{inverse product of matrix over scalar, 1}.
Аналогично доказывается равенство \EqRef{inverse product of matrix over scalar, 2}.
\end{proof}

\begin{theorem}
\label{theorem: RC-inverse matrix, delta}
Пусть
\ShowEq{unit matrix order 2}
Тогда
\ShowEq{inverse matrix, unit}
\end{theorem}
\begin{proof}
Из \EqRef{inverse matrix, 1 1}
и \EqRef{inverse matrix, 2 2} очевидно, что
\ShowEq{inverse matrix, unit 1 1}
и
\ShowEq{inverse matrix, unit 2 2}
Тем не менее выражение для
\ShowEq{inverse matrix, unit 1 2}
и
\ShowEq{inverse matrix, unit 2 1}
не может быть определено из
\EqRef{inverse matrix, 1 2} и \EqRef{inverse matrix, 2 1}
так как
\ShowEq{inverse matrix, unit 01}
Мы можем преобразовать эти выражения. Например
\ShowEq{inverse matrix, unit 02}
Мы непосредственно видим, что
\ShowEq{inverse matrix, unit 03}
Таким же образом мы можем найти, что
\ShowEq{inverse matrix, unit 04}
Это завершает доказательство \EqRef{RC inverse matrix, unit}.

Равенство
\EqRef{CR inverse matrix, unit} следует из
\EqRef{RC inverse matrix, unit}, теоремы \ref{theorem: two quasideterminants}
и симметрии матрицы \EqRef{unit matrix order 2}.
\end{proof}

\ePrints{0612.111}
\ifx\Semafor\ValueOn
\section{Приводимое бикольцо}
\label{section: Reducible Biring}

Если мы рассматриваем бикольцо матриц над полем $F$, то
из коммутативности произведения в поле следует 
\begin{equation}
\EqLabel{reducibility of products}
A\RCstar B
=(A_a^cB_c^b)
=(B_c^bA_a^c)
=B\CRstar A
\end{equation}

\begin{definition}
\AddIndex{Приводимое бикольцо}{reducible biring}
- это бикольцо, в котором выполняется
\AddIndex{условие приводимости произведений}
{condition of reducibility of products}
\EqRef{reducibility of products}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: transpose in reducible biring}
\begin{align}
\EqLabel{transpose star rc product}
(A\RCstar B)^T&=B^T\RCstar A^T\\
\EqLabel{transpose star cr product}
(A\CRstar B)^T&=B^T\CRstar A^T
\end{align}
в приводимом бикольце.
\end{theorem}
\begin{proof}
Из \EqRef{rcstar transpose}
и \EqRef{reducibility of products}
следует, что
\[
(A\RCstar B)^T=A^T\CRstar B^T=B^T\RCstar A^T
\]
Мы можем доказать \EqRef{transpose star cr product}
аналогичным образом.
\end{proof}

\begin{theorem}
\label{theorem: inverse in reducible biring}
\begin{equation}
\EqLabel{inverse in reducible biring}
A^{\CRInverse} =A^{\RCInverse} 
\end{equation}
в приводимом бикольце.
\end{theorem}
\begin{proof}
Из \EqRef{rc-inverse matrix}
и \EqRef{reducibility of products}
следует, что
\begin{equation}
\EqLabel{inverse in reducible biring, 1}
\delta=A\RCstar A^{\RCInverse}= A^{\RCInverse}\CRstar A
\end{equation}
\EqRef{inverse in reducible biring} следует
из сравнения \EqRef{inverse in reducible biring, 1}
и \EqRef{cr-inverse matrix}.
\end{proof}

\section{Квазидетерминант над полем}

\begin{definition}
Для матриц, определённых над полем, мы определим функцию,
называемую \AddIndex{определитель матрицы}{determinant},
\begin{equation}
\EqLabel{determinant, initial value}
\det()=1
\end{equation}
\begin{equation}
\EqLabel{determinant, recursion}
\det a=\sum_a(-1)^{|a|+|b|}
a^b_a\det a^{[a]}_{[b]}
\end{equation}
\qed
\end{definition}

\begin{theorem}
\label{theorem: quasideterminant in reducible biring}
\begin{equation}
\EqLabel{quasideterminant in reducible biring}
\RCDet{a}_b^a=(-1)^{|a|+|b|}
\frac{\det a}
{\det a[^b_a]}
\end{equation}
для матриц, определённых над полем.
\end{theorem}
\begin{proof}
Мы проведём доказательство индукцией по $n$.
Так как умножение в поле коммутативно, мы можем
уточнить выражение \EqRef{quasideterminant, 2}
\begin{equation}
\EqLabel{quasideterminant in reducible biring, 1}
\RCDet{a}_b^a=a_b^a
-\frac{a_b^ca_e^a}
{\RCDet{a^{[b]}_{[a]}}_e^c}
\end{equation}

При $n=1$ мы можем доказать утверждение теоремы непосредственной проверкой.

Пусть утверждение теоремы справедливо при $n=k-1$.
Тогда это утверждение справедливо для всех  минорных матриц $k\times k$ матрицы $a$.
Мы подставим \EqRef{quasideterminant in reducible biring}
в равенство \EqRef{quasideterminant in reducible biring, 1}
\begin{align*}
\RCDet{a}_b^a=a_b^a
  &-\sum_{|c|<|a|}\sum_{|e|<|b|}
\frac{a_b^ca_e^a}
{(-1)^{|c|+|e|}\frac{det\ a[^b_a]}
{det\ a[^{b,e}_{a,c}]}}
\\&+\sum_{|c|>|a|}\sum_{|e|<|b|}
\frac{a_b^ca_e^a}
{(-1)^{|c|+|e|}\frac{det\ a[^b_a]}
{det\ a[^{b,e}_{a,c}]}}
\\&+\sum_{|c|<|a|}\sum_{|e|>|b|}
\frac{a_b^ca_e^a}
{(-1)^{|c|+|e|}\frac{det\ a[^b_a]}
{det\ a[^{b,e}_{a,c}]}}
\\&-\sum_{|c|>|a|}\sum_{|e|>|b|}
\frac{a_b^ca_e^a}
{(-1)^{|c|+|e|}\frac{det\ a[^b_a]}
{det\ a[^{b,e}_{a,c}]}}
\end{align*}
\begin{equation}
\EqLabel{quasideterminant in reducible biring, 2}
\begin{array}{rl}
\RCDet{a}_b^a=a_b^a
  &\displaystyle
  -\sum_{|c|<|a|}\sum_{|e|<|b|}
\frac{(-1)^{|a|+|b|+|e|+|c|}
a_b^ca_e^a
det\ a[^{b,e}_{a,c}]}
{(-1)^{|a|+|b|}det\ a[^b_a]}
\\&\displaystyle
+\sum_{|c|>|a|}\sum_{|e|<|b|}
\frac{(-1)^{|a|+|b|+|e|+|c|}
a_b^ca_e^a
det\ a[^{b,e}_{a,c}]}
{(-1)^{|a|+|b|}det\ a[^b_a]}
\\&\displaystyle
+\sum_{|c|<|a|}\sum_{|e|>|b|}
\frac{(-1)^{|a|+|b|+|e|+|c|}
a_b^ca_e^a
det\ a[^{b,e}_{a,c}]}
{(-1)^{|a|+|b|}det\ a[^b_a]}
\\&\displaystyle
-\sum_{|c|>|a|}\sum_{|e|>|b|}
\frac{(-1)^{|a|+|b|+|e|+|c|}
a_b^ca_e^a
det\ a[^{b,e}_{a,c}]}
{(-1)^{|a|+|b|}det\ a[^b_a]}
\end{array}
\end{equation}
Подставив равенство
\[
\det a[_c^b]=\left\{
\begin{array}{lr}
\displaystyle
\left(\sum_{|e|<|b|}-\sum_{|e|>|b|}\right)
(-1)^{|a|+|e|}
a_e^a
det\ a[^{b,e}_{a,c}]&c>a 
\\
\displaystyle
\left(\sum_{|e|>|b|}-\sum_{|e|<|b|}\right)
(-1)^{|a|+|e|}
a_e^a
det\ a[^{b,e}_{a,c}]&c<a
\end{array}
\right.
\]
в равенство \EqRef{quasideterminant in reducible biring, 2},
мы получим
\[
\RCDet{a}_b^a=a_b^a
+\left(
\sum_{|c|<|a|}+\sum_{|c|>|a|}
\right)
\frac{(-1)^{|b|+|c|}
a_b^c
det\ a[^b_c]}
{(-1)^{|a|+|b|}det\ a[^b_a]}
\]
Сложив дроби, мы получим
\begin{equation}
\EqLabel{quasideterminant in reducible biring, 3}
\RCDet{a}_b^a
=(-1)^{|a|+|b|}
\sum_{c\in M}
\frac{(-1)^{|b|+|c|}
a_b^c\det a[_c^b]}
{det\ a[^b_a]}
\end{equation}
Подставив \EqRef{determinant, recursion} в
\EqRef{quasideterminant in reducible biring, 3},
мы докажем, что утверждение теоремы справедливо при $n=k$.
\end{proof}
\fi


==> Center.Ring.Russian.tex <==
%auto-ignore
\input{Center.Ring.Eq}

\begin{definition}
\label{definition: center of ring}
Пусть $D$ - кольцо.\footnote{\citeBib{Serge Lang},
стр. 84.} Множество \symb{Z(D)}{center of ring}1
элементов $a\in D$ таких, что
\ShowEq{center of ring}
для всех $x\in D$,
называется
\AddIndex{центром кольца $D$}{center of ring}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: center of ring}
Центр $Z(D)$ кольца $D$ является подкольцом кольца $D$.
\end{theorem}
\begin{proof}
Непосредственно следует из определения \ref{definition: center of ring}.
\end{proof}

\begin{definition}
Пусть $D$ - кольцо с единицей $e$.\footnote{Определение
дано согласно
определению из \citeBib{Serge Lang},
стр. 84, 85.} Отображение
\[
l:Z\rightarrow D
\]
для которого $l(n)=ne$ будет гомоморфизмом колец, и его ядро является
идеалом $(n)$, порождённым целым числом $n\ge 0$.
Канонический инъективный гомоморфизм
\[
Z/nZ\rightarrow D
\]
является изоморфизмом между $Z/nZ$ и подкольцом в $D$.
Если $nZ$ - простой идеал, то у нас возникает два случая.
\begin{itemize}
\item $n=0$. $D$ содержит в качестве подкольца
кольцо, изоморфное $Z$ и часто отождествляемое
с $Z$. В этом случае мы говорим, что $D$ имеет
\AddIndex{характеристику $0$}{ring has characteristic 0}.
\item $n=p$ для некоторого простого числа $p$. $D$ имеет
\AddIndex{характеристику $p$}{ring has characteristic p}, и $D$
содержит изоморфный образ $F_p=Z/pZ$.
\end{itemize}
\qed
\end{definition}

\begin{theorem}
\label{theorem: integer subring of ring}
Пусть $D$ - кольцо характеристики $0$ и пусть $d\in D$.
Тогда любое целое число $n\in Z$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Утверждение теоремы доказывается по индукции.
При $n=0$ и $n=1$ утверждение очевидно.
Допустим утверждение справедливо при $n=k$.
Из цепочки равенств
\[
(k+1)d=kd+d=dk+d=d(k+1)
\]
следует очевидность утверждения при $n=k+1$.
\end{proof}

\begin{theorem}
\label{theorem: integer subring of center}
Пусть $D$ - кольцо характеристики $0$.
Тогда кольцо целых чисел $Z$ является подкольцом центра $Z(D)$ кольца $D$.
\end{theorem}
\begin{proof}
Следствие теоремы \ref{theorem: integer subring of ring}.
\end{proof}


==> Complex.Number.Russian.tex <==
%auto-ignore

\input{\FilePrefix Complex.Number.Eq}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\Section{Линейная функция комплексного поля}
\else
\section{Линейная функция комплексного поля}
\fi
\label{section: Linear Function of Complex Field}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: complex field over real field}
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
\fi%Calculus.Paper
Матрица линейной функции
\[
y^{\gi i}=x^{\gi j}f_{\gi j}^{\gi i}
\]
поля комплексных чисел над полем действительных чисел
удовлетворяет соотношению
\begin{align}
\EqLabel{complex field over real field, 0}
f_{\gi 0}^{\gi 0}&=f_{\giA}^{\giA}
\\
\EqLabel{complex field over real field, 1}
f_{\gi 0}^{\giA}&=-f_{\giA}^{\gi 0}
\end{align}
\end{theorem}
\begin{proof}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
Пользуясь равенством
\xEqRef{0812.4763}{linear map over field, division ring, relation}
получаем соотношения
\ShowEq{complex field over real field}
Из равенств
\EqRef{complex field over real field, 0, 0} и
\EqRef{complex field over real field, 0, 1}
следует \EqRef{complex field over real field, 0}.
Из равенств
\EqRef{complex field over real field, 1, 0} и
\EqRef{complex field over real field, 1, 1}
следует \EqRef{complex field over real field, 1}.
\else%Calculus.Paper
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: complex field over real field}.
\fi%Calculus.Paper
\end{proof}

\ePrints{0701.238,1003.1544,8433-5163}
\ifx\Semafor\ValueOff
\begin{theorem}[Уравнения Коши\Hyph Римана]
Если матрица
\ShowEq{Jacobian of map of complex variable}
является матрицей Якоби функции комплексного переменного
\[
x=x^{\gi 0}+x^{\giA}i\rightarrow y=y^{\gi 0}(x^{\gi 0},x^{\giA})+y^{\giA}(x^{\gi 0},x^{\giA})i
\]
над полем действительных чисел,
то
\ShowEq{Cauchy Riemann equations, complex field, 1}
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: complex field over real field}.
\end{proof}

\begin{theorem}
Производная функции комплексного переменного удовлетворяет равенству
\ShowEq{Cauchy Riemann equations, complex field, 2}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{Cauchy Riemann equations, complex field, 2, 1}
следует из равенств
\EqRef{Cauchy Riemann equations, complex field, 1}.
\end{proof}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Равенство \EqRef{Cauchy Riemann equations, complex field, 2}
эквивалентно равенству
\ShowEq{Cauchy Riemann equations, complex field, 3}
\fi
\ifx\texFuture\Defined
Производная Гато функции комплексного переменного является
полным дифференциалом и имеет вид
\ShowEq{Gateaux derivative, complex field}
где $dx$, $dy\in R$.
Поэтому символическое уравнение
\ShowEq{Cauchy Riemann equations, Gateaux derivative, complex field}
не выражает связь производной Гато с уравнения Коши\Hyph Римана.
\fi
\fi

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\Section{Алгебра кватернионов}
\else
\section{Алгебра кватернионов}
\label{section: Quaternion Algebra}
\fi

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
В этой статье я рассматриваю множество кватернионных алгебр,
определённых в \citeBib{Izrail M. Gelfand: Quaternion Groups}.

\begin{definition}
Пусть $F$ - поле.
Расширение $F(i,j,k)$ поля $F$ называется
\AddIndex{алгеброй
\symB{E(F,a,b)}1{quaternion algebra over the field}
кватернионов над полем $F$}{quaternion algebra over the field}\footnote{Я
буду следовать определению из \citeBib{Izrail M. Gelfand: Quaternion Groups}.},
если произведение в алгебре $E$ определено согласно правилам
\ShowEq{product in E(F,a,b), table}
где $a$, $b\in F$, $ab\ne 0$.
\qed
\end{definition}

Элементы алгебры $E(F,a,b)$ имеют вид
\[
x=x^{\gi 0}+x^{\giA}i+x^{\gi 2}j+x^{\gi 3}k
\]
где $x^{\gi i}\in F$, $\gi i=\gi 0$, $\giA$, $\gi 2$, $\gi 3$.
Кватернион
\[
\overline x=x^{\gi 0}-x^{\giA}i-x^{\gi 2}j-x^{\gi 3}k
\]
называется сопряжённым кватерниону $x$.
Мы определим
\AddIndex{норму кватерниона}{norm of quaternion}
$x$ равенством
\ShowEq{norm of quaternion E(F,a,b)}
Из равенства \EqRef{norm of quaternion E(F,a,b)} следует, что
$E(F,a,b)$ является алгеброй с делением только когда $a<0$, $b<0$.
Тогда мы можем пронормировать базис так, что $a=-1$, $b=-1$.

Мы будем обозначать символом
\ShowEq{quaternion division algebra over the field}
алгебру $E(F,-1,-1)$
кватернионов с делением над полем $F$.
\symB{H}0{quaternion algebra over real field}
Мы будем полагать $\ShowSymbol{quaternion algebra over real field}=E(R,-1,-1)$.
\def\EF{E(F)}
\else
\def\EF{H}
\fi
Произведение в алгебре кватернионов $\EF$ определено согласно правилам
\begin{equation}
\begin{array}{c|ccc}
&i&j&k\\
\hline
i&-1&k&-j\\
j&-k&-1&i\\
k&j&-i&-1\\
\end{array}
\EqLabel{product of quaternions}
\end{equation}
В алгебре $\EF$ норма кватерниона имеет вид
\begin{equation}
\EqLabel{norm of quaternion}
|x|^2=x\overline x=(x^{\gi 0})^2+(x^{\giA})^2+(x^{\gi 2})^2+(x^{\gi 3})^2
\end{equation}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
При этом обратный элемент имеет вид
\begin{equation}
\EqLabel{inverce quaternion}
x^{-1}=|x|^{-2}\overline x
\end{equation}

Внутренний автоморфизм алгебры кватернионов $H$\footnote{См.
\citeBib{Hamilton papers 3}, с. 643.}
\ShowEq{Quaternion Rotation}
описывает вращение вектора с координатами $x$, $y$, $z$.
Если $q$ записан в виде суммы скаляра и вектора
\ShowEq{Quaternion Rotation, 1}
то \EqRef{Quaternion Rotation} описывает вращение
вектора $(x,y,z)$ вокруг вектора $(a,b,c)$ на угол $2\alpha$.
\fi


==> Convention.Russian.tex <==
%auto-ignore
\input{\FilePrefix Convention.Eq}

\section{Соглашения}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597}
\ifx\Semafor\ValueOn
\begin{convention}
Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции,
хотя встречается текст, в котором неясно, какому термину надо
отдать предпочтение.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597,1011.3102}
\Items{Calculus.Paper,1211.6965,4910-5816,GJSFRF.Basis,1302.7204,CACAA.02.97}
\Items{4993-2400}
\ifx\Semafor\ValueOn
\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $s$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\begin{convention}
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
\qed
\end{convention}
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\begin{convention}
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,1211.6965,4910-5816,CACAA.01.195,GJSFRF.Basis,1302.7204}
\Items{CACAA.02.97,4993-2400}
\ifx\Semafor\ValueOn
\begin{convention}
\label{convention: we use separate color for index of element}
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,GJSFRF.Basis,1302.7204,CACAA.02.97}
\ifx\Semafor\ValueOn
\begin{convention}
%\label{convention: }
Очень трудно провести границу между модулем и алгеброй.
Тем более, иногда в процессе построения мы должны сперва
доказать, что множество $A$ является модулем,
а потом мы доказываем, что это множество является алгеброй.
Поэтому для записи координат элемента модуля
мы также будем пользоваться соглашением
\ref{convention: we use separate color for index of element}.
\qed
\end{convention}
\fi

\ePrints{1302.7204,CACAA.02.97,1310.5591,MSimplex,MBasis,MAlgebra}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
\ePrints{1302.7204,CACAA.02.97,MSimplex,MAlgebra}
\ifx\Semafor\ValueOn
$D$\Hyph алгебры
\else
$\Omega$\Hyph группы
\fi
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph число, а кватернион называется $H$\Hyph число.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,4993-2400}
\ifx\Semafor\ValueOn
\begin{convention}
Отождествление вектора и матрицы его координат
может привести к неоднозначности в равенстве
\ShowEq{Identification can lead to ambiguity, 1}
где $\Basis e$ - базис векторного пространства.
Поэтому мы будем записывать равенство
\EqRef{Identification can lead to ambiguity, 1}
в виде
\ShowEq{Identification can lead to ambiguity, 2}
чтобы видеть, где записан вектор.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,CACAA.01.195}
\ifx\Semafor\ValueOn
\begin{convention}
Если свободная конечномерная алгебра имеет единицу,
то мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\qed
\end{convention}
\fi

\ePrints{1104.5197,1105.4307}
\ifx\Semafor\ValueOn
\begin{convention}
Хотя алгебра является свободным модулем над некоторым
кольцом, мы не пользуемся векторными обозначениями
при записи элементов алгебры. В тех случаях, когда я рассматриваю
матрицу координат элемента алгебры, я буду пользоваться векторными
обозначениями для записи соответствующего элемента.
Чтобы не возникала неоднозначность при записи сопряжения,
я буду обозначать $a^*$ элемент, сопряжённый элементу $a$.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072,1111.6035,1102.5168}
\ifx\Semafor\ValueOn
\begin{convention}
В \citeBib{Cohn: Universal Algebra}
произвольная операция алгебры обозначена буквой $\omega$,
и $\Omega$ - множество операций некоторой универсальной алгебры.
Соответственно, универсальная алгебра с множеством операций
$\Omega$ обозначается $\Omega$\Hyph алгебра.
Аналогичные обозначения мы видим в
\citeBib{Burris Sankappanavar} с той небольшой разницей,
что операция в алгебре обозначена буквой $f$
и $\mathcal F$ - множество операций.
Я выбрал первый вариант обозначений, так как в этом случае
легче видно, где я использую операцию.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072}
\ifx\Semafor\ValueOn
\begin{convention}
Так как число универсальных алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\Omega_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\Omega}$\Hyph алгебр.
\ePrints{8443-0072}
\ifx\Semafor\ValueOn
Символом
\else
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом
\fi
$\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\Omega}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\VX A,\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.
\qed
\end{convention}

\begin{convention}
Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\qed
\end{convention}
\fi

\ePrints{8443-0072,1111.6035,0906.0135,NewAffine,1102.5168,1305.4547,1310.5591}
\Items{1003.3714,4820-2669,MBasis,4993-2400}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ - $\Omega_1$\Hyph алгебра.
Пусть $B$ - $\Omega_2$\Hyph алгебра.
Запись
\ShowEq{A->*B}
означает, что определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
\qed
\end{convention}
\fi

\ePrints{0702.561,0707.2246,0803.2620}
\ifx\Semafor\ValueOn
\begin{convention}
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
\qed
\end{convention}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\begin{remark}
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\qed
\end{remark}
\fi

\ePrints{1001.4852,1003.1544,1006.2597,1011.3102}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\begin{convention}
Если в некотором выражении используется несколько
операций, среди которых есть операция $\circ$, то предполагается,
что операция $\circ$ выполняется первой.
Ниже приведен пример эквивалентных выражений.
\ShowEq{list circ expressions}
\qed
\end{convention}
\fi

%\ePrints{0906.0135,NewAffine}
%\ifx\Semafor\ValueOn
%\item
%Пусть $\VX X$ - базис башни представлений $(\Vector A,\Vector f)$.
%Мы будем называть $\Omega_n$\Hyph слово
%$w_n(\Vector f,\VX X,x_n)$ координатами $x_n\in A_n$
%относительно базиса $\VX X$.
%\fi

\ePrints{1107.1139}
\ifx\Semafor\ValueOn
\begin{convention}
Для данной $D$\Hyph алгебры $A$
левый сдвиг
\ShowEq{left shift, D algebra}
определён равенством
\ShowEq{left shift 1, D algebra}
и правый сдвиг
\ShowEq{right shift, D algebra}
определён равенством
\ShowEq{right shift 1, D algebra}
\qed
\end{convention}
\fi

\ePrints{MBasis}
\ifx\Semafor\ValueOn
\begin{convention}
Мы будем полагать,
что рассматриваемая мера является полной мерой.
\qed
\end{convention}
\fi

\ifx\PrintPaper\undefined
Без сомнения, у читателя могут быть вопросы,
замечания, возражения. Я буду признателен любому отзыву.
\fi



==> Division.Ring.Russian.tex <==
%auto-ignore
\input{Division.Ring.Eq}
\chapter{Геометрия тела}
\label{chapter: Geometry of Division Ring}

\section{Центр тела}

\Input{Center.Ring}

Пусть $D$ - тело. Если $D$ имеет характеристику $0$,
$D$ содержит в качестве подполя изоморфный образ поля $Q$
рациональных чисел. Если $D$ имеет характеристику $p$,
$D$ содержит в качестве подполя изоморфный образ $F_p$.
В обоих случаях это подполе будет называться простым полем.
Так как простое поле является наименьшим подполем в $D$,
содержащим $1$ и не имеющим автоморфизмов, кроме тождественного,
его обычно отождествляют с $Q$ или $F_p$,
в зависимости от того, какой случай имеет место.

\begin{theorem}
\label{theorem: center of division ring}
Центр $Z(D)$ тела $D$ является подполем тела $D$.
\end{theorem}
\begin{proof}
\begin{sloppypar}
Согласно теореме \ref{theorem: center of ring}
достаточно проверить, что $a^{-1}\in Z(D)$,
если $a\in Z(D)$.
Пусть $a\in Z(D)$.
Многократно применяя равенство \EqRef{center of ring},
мы получим цепочку равенств
\begin{equation}
\EqLabel{center of ring,1}
aa^{-1}x=x=xaa^{-1}=axa^{-1}
\end{equation}
Из \EqRef{center of ring,1} следует
\[
a^{-1}x=xa^{-1}
\]
Следовательно, $a^{-1}\in Z(D)$.
\end{sloppypar}
\end{proof}

\begin{theorem}
Пусть $D$ - тело характеристики $0$ и пусть $d\in D$.
Тогда для любого целого числа $n\in Z$
\ShowEq{inverse integer in division ring}
\end{theorem}
\begin{proof}
Согласно теореме \ref{theorem: integer subring of ring}
справедлива цепочка равенств
\ShowEq{inverse integer in division ring, 1}
Умножив правую и левую части равенства
\EqRef{inverse integer in division ring, 1} на $n^{-1}$,
получим
\ShowEq{inverse integer in division ring, 2}
Из \EqRef{inverse integer in division ring, 2} следует
\EqRef{inverse integer in division ring}.
\end{proof}

\begin{theorem}
\label{theorem: division ring, rational number}
Пусть $D$ - тело характеристики $0$ и пусть $d\in D$.
Тогда любое рациональное число $p\in Q$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Мы можем представить рациональное число $p\in Q$ в
виде $p=mn^{-1}$, $m$, $n\in Z$.
Утверждение теоремы следует из цепочки равенств
\[
pd=mn^{-1}d=n^{-1}dm=dmn^{-1}=dp
\]
основанной на утверждении теоремы \ref{theorem: integer subring of ring}
и равенстве \EqRef{inverse integer in division ring}.
\end{proof}

\begin{theorem}
\label{theorem: rational subring of center}
Пусть $D$ - тело характеристики $0$.
Тогда поле рациональных чисел $Q$ является подполем центра $Z(D)$ тела $D$.
\end{theorem}
\begin{proof}
Следствие теоремы \ref{theorem: division ring, rational number}.
\end{proof}

\section{Геометрия тела над полем}
\label{section: Geometry of Division Ring over Field}

%\begin{remark}
%\label{remark: Geometry of Division Ring over Field}
Мы можем рассматривать тело $D$ как векторное пространство над полем
\ShowEq{division ring over field}
Так как $F$ - поле, то мы можем писать все индексы справа от
корневой буквы.
При этом мы будем пользоваться следующими соглашением
\ref{convention: we use separate color for index of element}.
%\qed
%\end{remark}

\begin{remark}
\label{remark: dimension of division ring}
Пусть $\Basis e$ - базис тела $D$ над полем $F$. Тогда произвольный
элемент $a\in D$ можно представить в виде
\ShowEq{expansion relative to basis, division ring}
Если размерность тела $D$ над полем $F$ бесконечна,
то базис может быть либо счётным, либо его мощность
может быть не меньше, чем мощность континуума.
Если базис счётный, то на коэффициенты $a^{\gi i}$
разложения \EqRef{expansion relative to basis, division ring} накладываются
определённые ограничения. Если мощность множества $I$ континуум,
то предполагается, что на множестве $I$ определена мера и
сумма в разложении \EqRef{expansion relative to basis, division ring}
является интегралом по этой мере.
\qed
\end{remark}

\begin{remark}
\label{remark: Geometry of Division Ring over Field}
Поскольку в теле $D$ определена операция произведения, то мы можем рассматривать
тело как алгебру над полем
\ShowEq{division ring over field}
Для элементов базиса мы положим
\ShowEq{structural constants}
\ShowEq{product, division ring over field, basis}
Коэффициенты $\ShowSymbol{structural constants}{ring}$
разложения \EqRef{product, division ring over field, basis}
называются \AddIndex{структурными константами}{structural constants}
тела $D$ над полем $F$.
\end{remark}

Из равенств \EqRef{expansion relative to basis, division ring},
\EqRef{product, division ring over field, basis} следует
\ShowEq{product, division ring over field}
Из равенства \EqRef{product, division ring over field} следует
\ShowEq{product, division ring over field, associativity, proof}
Из ассоциативности произведения
\[
(ab)c=a(bc)
\]
и равенств \EqRef{product, division ring over field, associativity, proof, 1}
и \EqRef{product, division ring over field, associativity, proof, 2}
следует
\ShowEq{product, division ring over field, associativity, proof, 3}
Так как векторы $a$, $b$, $c$ произвольны, а
векторы $e_{\gik}$ линейно независимы, то из равенства
\EqRef{product, division ring over field, associativity, proof, 3}
следует
\ShowEq{product, division ring over field, associativity}

\begin{theorem}
\label{theorem: division ring over field, change basis}
Координаты $a^{\gi j}$ вектора $a$ являются тензором
\ShowEq{division ring over field, change basis, 3}
\end{theorem}
\begin{proof}
Пусть $\Basis e'$ - другой базис. Пусть
\ShowEq{division ring over field, change basis}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e'$.
Так как вектор $a$ не меняется, то
\ShowEq{division ring over field, change basis, 1}
Из равенств \EqRef{division ring over field, change basis}
и \EqRef{division ring over field, change basis, 1}
следует
\ShowEq{division ring over field, change basis, 2}
Так как векторы $e_{\gi j}$ линейно независимы, то равенство
\EqRef{division ring over field, change basis, 3}
следует
из равенства
\EqRef{division ring over field, change basis, 2}.
Следовательно, компоненты вектора являются тензором.
\end{proof}

\begin{theorem}
Структурные константы тела $D$ над полем $F$ являются тензором
\ShowEq{product, division ring over field, structural constant prim}
\end{theorem}
\begin{proof}
Рассмотрим аналогичным образом преобразование произведения.
Равенство \EqRef{product, division ring over field}
в базисе $\Basis e'$ имеет вид
\ShowEq{product, division ring over field, prim}
Подставив \EqRef{division ring over field, change basis, 3}
и \EqRef{division ring over field, change basis}
в \EqRef{product, division ring over field, prim},
получим
\ShowEq{product, division ring over field, prim, 1}
Из \EqRef{product, division ring over field} и
\EqRef{product, division ring over field, prim, 1}
следует
\ShowEq{product, division ring over field, prim, 2}
Так как векторы $a$ и $b$ произвольны, а
векторы $e_{\gil}$ линейно независимы, то равенство
\EqRef{product, division ring over field, structural constant prim}
следует
из равенства
\EqRef{product, division ring over field, prim, 2}.
Следовательно, структурные константы являются тензором.
\end{proof}

%\section{Сопряжение в теле}

%Пусть ${}_ie$ - базис тела $D$ над полем $F$.
%Положим ${}_ie^*={}_ie$. Будем рассматривать базис,
%для которого ${}_0e=1$. Для произвольного элемента
%$a\in D$, $a=a^0\ {}_0e+a^i\ {}_ie$


==> Group.Representation.Russian.tex <==
%auto-ignore
\input{Group.Representation.Eq}
\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\chapter{Представление группы}
\label{chapter: Representation of Group}
\fi

\section{Представление группы}
\label{section: Representation of Group}

Группа - одна из немногих алгебр, которая позволяет рассматривать
произведение преобразований $\Omega$\Hyph алгебры $M$ таким образом, что если
преобразования принадлежат представлению, то их произведение также
принадлежит представлению.
При этом следует помнить, что порядок отображений при суперпозиции
зависит от порядка отображений на диаграмме и с какой стороны
отображения действуют на элементы множества.

\begin{definition}
\label{definition: left-side representation of group} 
Пусть ${}^*M$ - группа с произведением
\ShowEq{fg *M Tstar}
и $\delta$ - единица группы ${}^\star M$.
Пусть $G$ - группа.
Мы будем называть гомоморфизм групп
\ShowEq{left-side representation of group, map}
\AddIndex{левосторонним представлением группы $G$}{left-side representation of group}
или
\AddIndex{\Ts{G}представлением группы}{A* representation of algebra}
в $\Omega$\Hyph алгебре $M$, если отображение $f$ удовлетворяет условиям
\ShowEq{left-side representation of group}
\qed
\end{definition}

\begin{remark}
Поскольку отображение \EqRef{left-side representation of group, map}
- гомоморфизм, то
\ShowEq{left-side representation of group, map product}
Мы здесь пользуемся соглашением
\[
f(a)f(b)=f(a)\circ f(b)
\]
Таким образом, концепция представления групп состоит в том,
что в каком порядке мы перемножаем элементы группы,
в том же порядке перемножаются соответствующие преобразования представления.
Из равенств \EqRef{left-side representation of group}
и \EqRef{left-side representation of group, map product}
следует
\ShowEq{left-side representation of group, associativity}
Равенство
\EqRef{left-side representation of group, associativity}
совместно с ассоциативностью произведения преобразований
представляет собой
\AddIndex{закон ассоциативности}{associative law}
для \Ts{G}представления.
Это позволяет записывать равенство
\EqRef{left-side representation of group, associativity}
без использования скобок
\[
f(ab)u=f(a)f(b)u
\]
\qed
\end{remark}

\begin{definition}
\label{definition: right-side representation of group} 
Пусть $M^\star$ - группа с произведением
\ShowEq{fg *M starT}
и $\delta$ - единица группы $M^\star$.
Пусть $G$ - группа.
Мы будем называть гомоморфизм групп
\ShowEq{right-side representation of group, map}
\AddIndex{правосторонним представлением группы $G$}{right-side representation of group}
или
\AddIndex{\sT{G}представлением}{*A representation of algebra}
в $\Omega$\Hyph алгебре $M$, если отображение $f$ удовлетворяет условиям
\ShowEq{right-side representation of group}
\qed
\end{definition}

\begin{remark}
Поскольку отображение \EqRef{right-side representation of group, map}
- гомоморфизм, то
\ShowEq{right-side representation of group, map product}
Из равенств \EqRef{right-side representation of group}
и \EqRef{right-side representation of group, map product}
следует
\ShowEq{right-side representation of group, associativity}
Равенство
\EqRef{right-side representation of group, associativity}
совместно с ассоциативностью произведения преобразований
представляет собой
\AddIndex{закон ассоциативности}{associative law}
для \sT{G}представления.
Это позволяет записывать равенство
\EqRef{right-side representation of group, associativity}
без использования скобок
\[
uf(ab)=uf(a)f(b)
\]
\qed
\end{remark}

\begin{definition}
\label{definition: nonsingular transformation} 
Мы будем называть преобразование
\[
t:M\rightarrow M
\]
\AddIndex{невырожденным преобразованием}{nonsingular transformation},
если существует обратное отображение.
\qed
\end{definition}

\begin{theorem}
\label{theorem: inverse transformation}
Для любого $g\in G$ преобразование $f(g)$ является
невырожденным и удовлетворяет равенству
\begin{equation}
\EqLabel{inverse transformation}
f(g^{-1})=f(g)^{-1}
\end{equation}
\end{theorem}
\begin{proof}
На основании \EqRef{left-side representation of group} и
\ShowEq{f(e)=}
мы можем записать
\[
u=\delta (u)=f(gg^{-1})(u)=f(g)(f(g^{-1})(u))
\]
Это завершает доказательство.
\end{proof}

\begin{theorem}
Групповая операция определяет два различных представления на группе:
\begin{itemize}
\item
\AddIndex{Левый сдвиг}{left shift}
\ShowEq{left shift =}
\ShowEq{left shift}
является \Ts{G}представлением на множестве\footnote{Левый сдвиг
не является представлением группы в группе,
так как преобразование $t_\star$ не является гомоморфизмом
группы.
Аналогичное замечание верно для правого сдвига.
} $G$
\ShowEq{left shift, product}
\item
\AddIndex{Правый сдвиг}{right shift}
\ShowEq{right shift =}
\ShowEq{right shift}
является \sT{G}представлением на множестве $G$
\ShowEq{right shift, product}
\end{itemize}
\end{theorem}
\begin{proof}
Равенство \EqRef{left shift, product}
следует из ассоциативности произведения
\[
t_\star(ab)c=(ab)c=a(bc)=t_\star(a)(t_\star(b)c)
=(t_\star(a)\circ t_\star(b))c
\]
Аналогично доказывается равенство \EqRef{right shift, product}.
\end{proof}

\begin{definition}
\label{definition: orbit of left-side representation of group}
Пусть $G$ - группа.
Пусть $f$ - \Ts{G}представление в $\Omega$\Hyph алгебре $M$.
Для любого $v\in M$ мы определим
\AddIndex{орбиту представления группы $G$}
{orbit of representation of group} как множество
\ShowEq{orbit of representation of group}
\qed
\end{definition}

Так как $f(e)=\delta$, то $v\in f(G)v$.

\begin{theorem}
\label{theorem: proper definition of orbit}
Если
\begin{equation}
\EqLabel{orbit, proposition}
v\in f(G)u
\end{equation}
то
\[
f(G)u=f(G)v
\]
\end{theorem}
\begin{proof}
Из \EqRef{orbit, proposition} следует
существование $a\in G$ такого, что
\begin{equation}
v=f(a)u
\EqLabel{orbit, 1}
\end{equation}
Если $w\in f(G)v$, то
существует $b\in G$ такой, что
\begin{equation}
w=f(b)v
\EqLabel{orbit, 2}
\end{equation}
Подставив \EqRef{orbit, 1} в \EqRef{orbit, 2}, мы получим
\begin{equation}
w=f(b)(f(a)u)
\EqLabel{orbit, 3}
\end{equation}
На основании \EqRef{left-side representation of group}
из \EqRef{orbit, 3} следует,
что $w\in f(G)u$.
Таким образом,
\[
f(G)v\subseteq f(G)u
\]

На основании \EqRef{inverse transformation}
из \EqRef{orbit, 1} следует,
что
\begin{equation}
u=f(a)^{-1}v=f(a^{-1})v
\EqLabel{orbit, 4}
\end{equation}
Равенство \EqRef{orbit, 4} означает, что
$u\in f(G)v$ и, следовательно,
\[
f(G)u\subseteq f(G)v
\]
Это завершает доказательство.
\end{proof}

Таким образом, \Ts{G}представление $f$ в $\Omega$\Hyph алгебре $M$
порождает отношение эквивалентности $S$ и
орбита $f(G)u$ является классом эквивалентности.
Мы будем пользоваться обозначением
\symb{M/f(G)}{space of orbits of G* representation}1
для фактор множества $M/S$ и мы будем называть
это множество
\AddIndex{пространством орбит \Ts{G}представления}
{space of orbits of G* representation} $f$.

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: direct product of representations}
Если определены \Ts{G}представление $f_1$ в $\Omega$\Hyph алгебре $M_1$
и \Ts{G}представление $f_2$ в $\Omega$\Hyph алгебре $M_2$,
то мы можем определить
\AddIndex{прямое произведение \Ts{G}представлений}
{direct product of G* representations}
$f_1$ и $f_2$ группы
\begin{align*}
f&=f_1\times f_2:G\rightarrow M_1\otimes M_2\\
f(g)&=(f_1(g),f_2(g))
\end{align*}
\end{theorem}
\begin{proof}
Чтобы показать, что $f$ является представлением,
достаточно показать, что $f$ удовлетворяет определению
\ref{definition: left-side representation of group}.
\[f(e)=(f_1(e),f_2(e))=(\delta_1,\delta_2)=\delta\]
\begin{align*}
f(ab)u&=(f_1(ab)u_1,f_2(ab)u_2)\\
&=(f_1(a)(f_1(b)u_1),f_2(a)(f_2(b)u_2))\\
&=f(a)(f_1(b)u_1,f_2(b)u_2)\\
&=f(a)(f(b)u)
\end{align*}
\end{proof}
\fi

\section{Однотранзитивное правостороннее представление группы}
\label{section: Single Transitive Representation of Group}

\begin{definition}
\label{definition: kernel of inefficiency of representation of group}
Мы будем называть
\AddIndex{ядром неэффективности \Ts{G}представления}
{kernel of inefficiency of G* representation}
множество \[K_f=\{g\in G:f(g)=\delta\}\]
\qed
\end{definition}

\begin{theorem}
\label{theorem: kernel of inefficiency, representation of group}
Ядро неэффективности \Ts{G}представления - это подгруппа группы $G$.
\end{theorem}
\begin{proof}
Допустим
$f(a_1)=\delta$ и $f(a_2)=\delta$. Тогда
\[f(a_1a_2)u=f(a_1)(f(a_2)u)=u\]
\[f(a^{-1})=f^{-1}(a)=\delta\]
\end{proof}

\begin{theorem}
\Ts{G}представление
\AddIndex{эффективно}{effective G* representation}
тогда и только тогда, когда ядро неэффективности $K_f=\{e\}$.
\end{theorem}
\begin{proof}
Утверждение является следствием определений
\ref{definition: effective representation of algebra} и
\ref{definition: kernel of inefficiency of representation of group} и
теоремы \ref{theorem: kernel of inefficiency, representation of group}.
\end{proof}

Если действие не эффективно, мы можем перейти к эффективному
заменив группой $G_1=G|K_f$,
пользуясь факторизацией по ядру неэффективности.
Это означает, что мы можем изучать только эффективное действие.

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{definition}
\label{definition: free representation of group}
Рассмотрим \Ts{G}представление $f$ в $\Omega$\Hyph алгебре $M$.
\AddIndex{Малая группа}{little group} или
\AddIndex{группа стабилизации}{stability group} элемента $x\in M$ -
это множество
\ShowEq{little group}

Мы будем называть \Ts{G}представление $f$
\AddIndex{свободным}{free representation of group},
если для любого $x\in M$ группа стабилизации $G_x=\{e\}$.
\qed
\end{definition}

\begin{theorem}%
\label{theorem: free representation of group}
Если определено свободное \Ts{G}представление $f$ группы $G$ на $\Omega$\Hyph алгебре $A$,
то определено взаимно однозначное соответствие между орбитами представления,
а также между орбитой представления и группой $G$.
\end{theorem}
\begin{proof}
Допустим для точки $a\in A$
существуют $g_1$, $g_2\in G$
\begin{equation}
\EqLabel{free representation of group, 1}
f(g_1)a=f(g_2)a
\end{equation}
Умножим обе части равенства \EqRef{free representation of group, 1}
на $f(g_1^{-1})$
\[
a=f(g_1^{-1})f(g_2)a
\]
Поскольку представление свободное, $g_1=g_2$. Теорема доказана,
так как мы установили взаимно однозначное соответствие между
орбитой и группой $G$.
\end{proof}
\else

\begin{definition}
\label{definition: transitive representation of group}
Мы будем называть представление группы
\AddIndex{транзитивным}{transitive representation of group},
если для любых $a, b \in V$ существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление группы
\AddIndex{однотранзитивным}{single transitive representation of group},
если оно транзитивно и эффективно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
\Ts{G}представление однотранзитивно тогда и только тогда, когда для любых $a, b \in M$
существует одно и только одно $g\in G$ такое, что $a=f(g)(b)$
\end{theorem}
\begin{proof}
Следствие определений \ref{definition: effective representation of algebra}
и \ref{definition: transitive representation of group}.
\end{proof}
\fi

\begin{definition}
Мы будем называть пространство $V$
\AddIndex{однородным пространством группы}{homogeneous space of group} $G$,
если мы имеем однотранзитивное \Ts{G}представление на $V$.
\qed
\end{definition}

\begin{theorem}%
\label{theorem: single transitive representation of group}
Если мы определим однотранзитивное
представление $f$ группы $G$ на $\Omega$\Hyph алгебре $A$,
то мы можем однозначно определить координаты на $A$, пользуясь координатами на группе $G$.

Если $f$ - левостороннее представление,
то $f(a)$ эквивалентно левому сдвигу $t_\star(a)$ на группе $G$.
Если $f$ - правостороннее представление, то $f(a)$ эквивалентно
правому сдвигу ${}_\star t(a)$ на группе $G$.
\end{theorem}
\begin{proof}
Мы выберем точку $v\in A$
и определим координаты точки $w\in A$
как координаты $a\in G$ такого, что $w=f(a) v$.
Координаты, определённые таким образом, однозначны
с точностью до выбора начальной точки $v\in A$,
так как действие эффективно.

Если $f$ - левостороннее представление,
мы будем пользоваться записью
\[f(a)v=av\]
Так как запись
\[f(a)(f(b)v)=a(bv)=(ab)v=f(ab)v\]
совместима с групповой структурой, мы видим, что
левостороннее представление $f$ эквивалентно левому сдвигу.

Если $f$ - правостороннее представление,
мы будем пользоваться записью
\[vf(a)=va\]
Так как запись
\[(vf(b))f(a)=(vb)a=v(ba)=vf(ba)\]
совместима с групповой структурой, мы видим, что
правостороннее представление $f$ эквивалентно правому сдвигу.
\end{proof}

\begin{remark}
Мы будем записывать эффективное
\Ts{G}представление в форме
\[v'=t_\star(a) v=av\]
Орбита этого представления имеет вид
\ShowEq{orbit of effective G* representation}
Мы будем пользоваться обозначением
\ShowEq{space of orbits of effective G* representation}
для пространства орбит эффективного \Ts{G}представления.
\qed
\end{remark}

\begin{remark}
Мы будем записывать эффективное
\sT{G}представление в форме
\[v'=v\ {}_\star t(a)=va\]
Орбита этого представления имеет вид
\ShowEq{orbit of effective *G representation}
Мы будем пользоваться обозначением
\ShowEq{space of orbits of effective *G representation}
для пространства орбит эффективного \sT{G}представления.
\qed
\end{remark}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: Free representation is single transitive}
Свободное \Ts{G}представление эффективно.
Свободное \Ts{G}представление $f$ в $\Omega$\Hyph алгебре $M$
однотранзитивно на орбите.
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: free representation of group}.
\end{proof}
\fi

\begin{theorem}%
\label{theorem: shifts on group commuting}
Правый и левый сдвиги на группе $G$ перестановочны.
\end{theorem}
\begin{proof}
Это следствие ассоциативности группы $G$
\[(t_\star(a)\circ\ {}_\star t(b))c = a(cb)=(ac)b
=({}_\star t(b)\circ t_\star(a))c\]
\end{proof}

Теорема \ref{theorem: shifts on group commuting} может
быть сформулирована следующим образом.

\begin{theorem}%
\label{theorem: shift is automorphism of representation}
Пусть $G$ - группа. Для любого $a\in G$ отображение
$t_\star(a)$ является автоморфизмом представления ${}_\star t$.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: shifts on group commuting}
\begin{equation}
t_\star(a)\circ {}_\star t(b)={}_\star t(b)\circ t_\star(a)
\EqLabel{shifts on group commuting}
\end{equation}
Равенство \EqRef{shifts on group commuting}
совпадает с равенством
\EqRef{morphism of representations of F algebra, definition, 2}
из определения
\ref{definition: morphism of representations of F algebra}
при условии $r=id$, $R=t_\star(a)$.
\end{proof}

\begin{theorem}%
\label{theorem: two representations of group}
Пусть \Ts{G}представление $f$
на $\Omega$\Hyph алгебре $M$ однотранзитивно.
Тогда мы можем однозначно определить однотранзитивное \sT{G}представление $h$
на $\Omega$\Hyph алгебре $M$
такое, что диаграмма
\[
\xymatrix{
M\ar[rr]^{h(a)}\ar[d]^{f(b)} & & M\ar[d]^{f(b)}\\
M\ar[rr]_{h(a)}& &M
}
\]
коммутативна для любых $a$, $b\in G$.\footnote{Это
утверждение можно также найти в \citeBib{Rashevsky}.}
\end{theorem}
\begin{proof}
Мы будем пользоваться групповыми координатами для точек $v\in M$.
Тогда согласно теореме \ref{theorem: single transitive representation of group}
мы можем записать левый сдвиг $t_\star(a)$ вместо преобразования $f(a)$.

Пусть $v_0, v\in M$. Тогда мы можем найти
одно и только одно $a\in G$ такое, что
\[v=v_0 a=v_0\ {}_\star t(a)\]
Мы предположим
\[h(a)=\ {}_\star t(a)\]
Существует $b\in G$ такое, что
\[w_0=f(b)v_0=t_\star (b)v_0\ \ \ \ w=f(b)v=t_\star(b) v\]
Согласно теореме \ref{theorem: shifts on group commuting} диаграмма
\begin{equation}
\xymatrix{
v_0\ar[rr]^{h(a)=\ {}_\star t(a)}\ar[d]^{f(b)=t_\star(b)}
& & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)=\ {}_\star t(a)}& &w
}
\label{Diagram: two representations of group}
\end{equation}
коммутативна.

Изменяя $b$ мы получим, что $w_0$ - это произвольная точка, принадлежащая $M$.

Мы видим из диаграммы, что, если $v_0=v$, то $w_0=w$ и следовательно $h(e)=\delta$.
С другой стороны, если $v_0\neq v$, то $w_0\neq w$ потому, что
\Ts{G}представление $f$ однотранзитивно.
Следовательно \sT{G}представление $h$ эффективно.

Таким же образам мы можем показать, что для данного $w_0$ мы можем найти $a$
такое, что $w=h(a)w_0$. Следовательно \sT{G}представление $h$ однотранзитивно.

В общем случае, произведение преобразований \Ts{G}представления $f$
не коммутативно и следовательно
\sT{G}представление $h$ отлично от \Ts{G}представления $f$.
Таким же образом мы можем создать \Ts{G}представление $f$, пользуясь \sT{G}представлением $h$.
\end{proof}

Мы будем называть представления $f$ и $h$
\AddIndex{парными представлениями группы}{twin representations of group} $G$.

\begin{remark}
\label{remark: one representation of group}
Очевидно, что преобразования $t_\star(a)$ и ${}_\star t(a)$
отличаются, если группа $G$ неабелева.
Тем не менее, они являются отображениями на.
Теорема \ref{theorem: two representations of group} утверждает, что, если оба
представления правого и левого сдвига существуют на множестве $M$,
то мы можем определить два перестановочных представления на множестве $M$.
Только правый или левый сдвиг не может представлять оба типа представления.
Чтобы понять почему это так, мы можем изменить диаграмму \eqref{Diagram: two representations of group}
и предположить $h(a)v_0=t_\star(a) v_0=v$
вместо $h(a)v_0=v_0{}_\star t(a)=v$ и
проанализировать, какое выражение $h(a)$ имеет в
точке $w_0$. Диаграмма
\[\xymatrix{
v_0\ar[rr]^{h(a)=t_\star(a)}\ar[d]^{f(b)=t_\star(b)}
& & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)}& &w
}\]
эквивалентна диаграмме
\[\xymatrix{
v_0\ar[rr]^{h(a)=t_\star(a)} & & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)}\ar[u]_{f^{-1}(b)=t_\star(b^{-1})}& &w
}\]
и мы имеем $w=bv=bav_0=bab^{-1}w_0$. Следовательно
\[h(a)w_0=(bab^{-1})w_0\] Мы видим, что представление $h$
зависит от его аргумента.\qed  
%There is interesting question. Если I имею преобразование $a\star$ in точке $b$
%what is $c$ такое, что $a\star b = R_c b$. Мы можем find it из равенства
%$ab=bc$, so $c=b^{-1}ab$, следовательно
%\[a\star b = R_{b^{-1}ab} b\]?????
\end{remark}

\begin{theorem}%
\label{theorem: twin representations of group, automorphism}
Пусть $f$ и $h$ - парные преставления группы $G$. Для любого $a\in G$ отображение
$h(a)$ является автоморфизмом представления $f$.
\end{theorem}
\begin{proof}
Следствие теорем
\ref{theorem: shift is automorphism of representation} и
\ref{theorem: two representations of group}.
\end{proof}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{remark}
Существует ли морфизм представлений
из $t_\star$ в $t_\star$, отличный от автоморфизма $(\id,{}_\star t(a))$?
Если мы положим
\[
r(g)=cgc^{-1}
\]
\[
R(a)(m)=cmac^{-1}
\]
то нетрудно убедиться, что отображение $(r,R(a))$ является
морфизмом представлений из $t_\star$ в $t_\star$.
Но это отображение не является
автоморфизмом представления $t_\star$,
так как $r\ne\id$.
\qed
\end{remark}
\fi


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\Index%192%*%*D- векторное пространство
   {$*D$\Hyph векторное пространство}%
   {*D vector space}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) mapping}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%660%A%Astar- модуль
   {$A\star$\Hyph модуль}%
   {Astar-module}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%726%N%n алгебра над кольцом
   {$n$\Hyph алгебра над кольцом}%
   {n algebra over ring}%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%600%R%RCcirc вырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph вырожденная матрица $\mathcal A(A)$\Hyph отображений}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph невырожденная матрица $A(A)$\Hyph отображений}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%111%R%rcd аффинный базис
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%735%S%starD аффинное пространство
   {$\star D$\Hyph аффинное пространство}%
   {starD affine space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%197%Б%базис D векторного пространства
   {базис $D$\Hyph векторного пространства}%
   {basis, D vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%727%В%векторное пространство над полем
   {векторное пространство над полем}%
   {vector space over field}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%157%Д%дифференциал Гато отображения
   {дифференциал Гато отображения}%
   {Gateaux differential of map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%680%И%интеграл отображения
   {интеграл отображения}%
   {integral of map}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%177%К%категория левосторонних представлений Omega1 алгебры из категории A
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of left-side representations of Omega1 algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of mappings}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%741%К%кватернионная алгебра
   {кватернионная алгебра}%
   {quaternion algebra}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%737%К%координаты точки rcd аффинного пространства относительно базиса
   {координаты точки \rcd аффинного пространства относительно базиса}%
   {coordinates in rcd affine space}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%228%Л%левое D векторное пространство
   {левое $D$\Hyph векторное пространство}%
   {left vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%184%Л%левостороннее представление группы
   {левостороннее представление группы}%
   {left-side representation of group}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль нaд кольцом
   {левый модуль нaд кольцом $D$}%
   {left module over ring}%
\Index%661%Л%левый модуль над D- алгеброй A
   {левый модуль над $D$\Hyph алгеброй $A$}%
   {left module over algebra}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%88%Л%линейная комбинация векторов
   {линейная комбинация векторов}%
   {linear combination of  vectors}%
\Index%32%Л%линейная оболочка в векторном пространстве
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%688%Л%линейно зависимое множество A- модуля
   {линейно зависимое множество $A$\Hyph модуля}%
   {linear dependent vectors, module}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%21%Л%линейно зависимые векторы
   {линейно зависимые векторы}%
   {linearly dependent vectors}%
\Index%34%Л%линейно независимые векторы
   {линейно независимые векторы}%
   {linearly independent vectors}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%740%Л%линейное преобразование rcd аффинного пространства
   {линейное преобразование \rcd аффинного пространства}%
   {linear transformation, rcd affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие базисов \rcd аффинного пространства
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%738%Н%начало системы координат star D аффинного пространства
   {начало системы координат $\star D$\Hyph аффинного пространства}%
   {origin of coordinate system of starD affine space}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\SetIndexSpace%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен степени
   {однородный многочлен степени $n$}%
   {homogeneous polynomial of power}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг rcd аффинного пространства
   {параллельный сдвиг \rcd аффинного пространства}%
   {parallel shift, rcd affine space}%
\Index%684%П%парные представления D- алгебры
   {парные представления $D$\Hyph алгебры}%
   {twin representations of D algebra}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное *G представление
   {пассивное \sT{G}представление}%
   {passive *G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%353%П%правое D векторное пространство
   {правое $D$\Hyph векторное пространство}%
   {right vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%355%П%правостороннее представление группы
   {правостороннее представление группы}%
   {right-side representation of group}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль нaд кольцом
   {правый модуль нaд кольцом $D$}%
   {right module over ring}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%207%Т%тензорное произведение векторных пространств
   {тензорное произведение векторных пространств}%
   {tensor product of vector spaces}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление Omega- алгебры
   {эффективное представление $\Omega$\Hyph алгебры}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Linear.Map.Russian.tex <==
%auto-ignore
\input{Linear.Map.Eq}
\chapter{Линейное отображение
\texorpdfstring{$\RCstar D$}{Rcd}\hyph векторного пространства}
\label{chapter: rcd Linear Map}

\section{Линейное отображение
\texorpdfstring{$\RCstar D$}{Rcd}\hyph векторного пространства}
\label{section: rcd Linear Map}

В этом разделе мы положим, что $V$, $W$ - это \rcd векторные пространства.

\begin{definition}
Обозначим
\ShowEq{set linear maps, rcd vector space}
множество линейных отображений
\DrawEq{A:V->W}{}
\rcd векторного пространства $V$
в \rcd векторное пространство $W$.
Обозначим
\ShowEq{set linear maps, drc vector space}
множество линейных отображений
\DrawEq{A:V->W}{}
\drc векторного пространства $V$
в \drc векторное пространство $W$.
\qed
\end{definition}

\begin{sloppypar}
%В литературе используется также обозначение $Hom_{D\RCstar}(V,W)$.
%Однако я предпочёл предложенное обозначение с точки зрения излагаемого материала.
Мы можем рассматривать тело $D$ как одномерное \rcd векторное пространство.
Соответственно мы можем рассматривать множества
$\mathcal L(\RCstar D;D;W)$ и $\LDVD$.
\end{sloppypar}

\begin{theorem}
\label{theorem: sum of linear maps, rcd vector spaces}
Предположим, что $V$, $W$ - \rcd векторные пространства.
Тогда множество
$\LDVW$
является абелевой группой
относительно закона композиции
\ShowEq{sum of maps, rcd vector space}
Линейное отображение $A+B$ называется
\AddIndex{суммой отображений}{sum of maps}
$A$ и $B$.
\end{theorem}
\begin{proof}
Нам надо показать, что отображение
\ShowEq{A+B:V->W}
определённое равенством \EqRef{sum of maps, rcd vector space},
- это линейное отображение \rcd векторных пространств.
Согласно определению
\xRef{0701.238}{definition: linear map of rcd vector spaces}
\ShowEq{sum of maps 1, rcd vector space}
Мы видим, что
\ShowEq{sum of maps 2, rcd vector space}
Нам надо показать так же, что эта операция коммутативна.
\ShowEq{sum of maps 3, rcd vector space}
\end{proof}

\begin{theorem}
\label{theorem: matrix of linear map of rcd vector spaces}
Пусть
\ShowEq{basis in vector space V}
- базис в \rcd векторном пространстве $V$
и
\ShowEq{basis in vector space W}
- базис в \rcd векторном пространстве $W$.
Пусть
\ShowEq{matrix of linear map}
- произвольная матрица.
Тогда отображение
\ShowEq{-A:V->W}
определённое равенством
\ShowEq{-A:V->W, presentation}
относительно выбранных базисов,
является линейным отображением \rcd векторных пространств.
\end{theorem}
\begin{proof}
Теорема \ref{theorem: matrix of linear map of rcd vector spaces}
является обратным утверждением теореме
\xRef{0701.238}{theorem: linear map of rcd vector space}.
Из равенства
\EqRef{-A:V->W, presentation}
следует, что
\ShowEq{linear map 2}
\end{proof}

\begin{theorem}
\label{theorem: product of linear map over scalar, rcd vector space}
Пусть \ShowEq{basis in vector space V}
- базис в \rcd векторном пространстве $V$
и \ShowEq{basis in vector space W}
- базис в \rcd векторном пространстве $W$.
Предположим линейное отображение $\Vector A$ имеет матрицу
\ShowEq{matrix of linear map}
относительно выбранных базисов.
Пусть $m\in D$.
Тогда матрица
\ShowEq{matrix mA of linear map}
определяет линейное отображение
\ShowEq{right action on linear map of rcd vector spaces}
которое мы будем называть
\AddIndex{левосторонним произведением отображения $A$ на скаляр}
{left-side product of map over scalar}.
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теоремы
\ref{theorem: matrix of linear map of rcd vector spaces}.
\end{proof}

\begin{theorem}
\label{theorem: linear maps of rcd vector space}
Множество $\LDVW$ является \drc векторным пространством.
\end{theorem}
\begin{proof}
Теорема \ref{theorem: sum of linear maps, rcd vector spaces} утверждает,
что $\LDVW$ - абелевая группа.
Из теоремы
\ref{theorem: product of linear map over scalar, rcd vector space} следует,
что элемент тела $D$
порождает левостороннее преобразование на абелевой группе
$\LDVW$.
Из теорем \ref{theorem: matrix of linear map of rcd vector spaces},
\xRef{0701.238}{theorem: Ts representation of the ring} и
\xRef{0701.238}{theorem: effective Ts representation of the division ring}
следует, что множество $\LDVW$ является $D\star$\Hyph векторным пространством.

\begin{sloppypar}
Выписывая элементы базиса $D\star$\Hyph векторного пространства $\LDVW$
в виде \subs строки или \sups строки, мы представим
$D\star$\Hyph векторное пространство $\LDVW$
как \dcr\ или \drc векторное пространство.
При этом надо иметь в виду, что выбор между \drc\ и \dcr линейной
зависимостью в $D\star$\Hyph векторном пространстве
$\LDVW$ не зависит от типа
векторных пространств $V$ и $W$.
\end{sloppypar}

Для того, чтобы выбрать тип векторного пространства
$\LDVW$
мы обратим внимание на следующее обстоятельство.
Допустим $V$ и $W$ - \rcd векторные пространства.
Допустим $\LDVW$ - \drc векторное пространство.
Тогда действие \sups строки \rcd линейных отображений ${}^jA$
на \subs строку векторов $f_i$ можно представить в виде матрицы
\ShowEq{linear maps of rcd vector space}
Эта запись согласуется с матричной записью действия \drc линейной комбинации
$a\RCstar A\ $ \rcd линейных отображений $A$.
\end{proof}

Мы можем также определить правостороннее произведение
\rcd линейного отображения $A$ на скаляр.
Однако, вообще говоря, это левостороннее представление тела $D$
в $D\star$\Hyph векторном пространстве
$\LDVW$ не может быть перенесено
в \rcd векторное пространство $W$. Действительно,
в случае правостороннего произведения мы имеем
\ShowEq{linear maps of rcd vector space, 1}
Поскольку произведение в теле не коммутативно, мы не можем выразить
полученное выражение как произведение $A\RCstar v$ на скаляр $m$.

Следствием теоремы \ref{theorem: linear maps of rcd vector space}
является неоднозначность записи
\ShowEq{linear maps of rcd vector space, 2}
Мы можем предположить, что смысл этой записи ясен из контекста.
Однако желательно неоднозначность избежать. Мы будем пользоваться для этой цели
скобками. Выражение
\ShowEq{linear maps of rcd vector space, 3}
означает, что \drc линейная комбинация \rcd линейных отображений ${}^iA$
отображает вектор $v$ в вектор $w$.
Выражение
\ShowEq{linear maps of rcd vector space, 4}
означает, что \RC произведение линейных отображений $A$ и $B$
отображает вектор $v$ в вектор $w$.

\section{\texorpdfstring{$1$}{1}\hyph форма
на \texorpdfstring{$\RCstar D$}{rcd}\hyph векторном пространстве}
\label{section: 1-Form on a Vector Space}

\begin{definition}
\AddIndex{$1$\Hyph форма}{1-form} на \rcd векторном пространстве $V$
- это линейное отображение
\ShowEq{1-form on rcd vector space}
\qed
\end{definition} 

Мы можем значение $1$\Hyph формы $b$, определённое для
вектора $a$, записывать в виде
\ShowEq{1-form on rcd vector space, 1}

\begin{theorem}
\label{theorem: L(RCstar D;V;D) is Dstar vector space}
Множество $\LDVD$ является $D\star$\Hyph векторным пространством.
\end{theorem}
\begin{proof}
\rcd векторное пространство размерности 1 эквивалентно телу $D$
\end{proof}

\begin{theorem}
\label{theorem: presentation of 1-form relative frame}
Пусть $\Basis e$ - базис в \rcd векторном пространстве $V$.
$1$\Hyph форма $\Vector b$ имеет представление
\ShowEq{1-form on rcd vector space, presentation}
относительно выбранного базиса, где вектор $a$ имеет разложение
\ShowEq{1-form on rcd vector space, 2}
и
\ShowEq{1-form and vector of basis}
\end{theorem}
\begin{proof}
Так как $\Vector b$ - $1$\Hyph форма,
из \EqRef{1-form on rcd vector space, 2} следует, что
\ShowEq{1-form and vector a}
\EqRef{1-form on rcd vector space, presentation} следует из
\EqRef{1-form and vector a} и \EqRef{1-form and vector of basis}.
\end{proof}

\begin{theorem}
\label{theorem: 1-form is uniquely defined}
Пусть $\Basis e$ - базис в \rcd векторном пространстве $V$.
$1$\Hyph форма
\ShowEq{-1-form on rcd vector space}
однозначно определена
значениями \EqRef{1-form and vector of basis},
в которые $1$\Hyph форма $\Vector b$ отображает вектора базиса.
\end{theorem}
\begin{proof}
Утверждение является следствием теорем
\ref{theorem: presentation of 1-form relative frame} и
\xRef{0701.238}{theorem: expansion relative basis, vector space}.
\end{proof}

\begin{theorem}
Пусть $\Basis e$ - базис в \rcd векторном пространстве $V$.
Множество $1$\Hyph форм
\ShowEq{basis d}
таких, что
\ShowEq{basis of dual vector space}
является базисом $\Basis d$ \drc векторного пространства $\LDVD$.
\end{theorem}
\begin{proof}
$1$\Hyph форма ${}^{\gij}d=\Vector b$ существует
для данного $\gij$ согласно теореме
\ref{theorem: 1-form is uniquely defined},
если положить
\ShowEq{basis of dual vector space, 1}.
Если предположить, что существует $1$\Hyph форма
\ShowEq{basis of dual vector space, 2}
то
\ShowEq{basis of dual vector space, 3}
Согласно равенству
\EqRef{basis of dual vector space}
\ShowEq{basis of dual vector space, 4}
Следовательно, $1$\Hyph формы
${}^{\gij}d$ линейно независимы.
\end{proof}

\begin{definition}
Пусть $V$ - \rcd векторное пространство.
\drc векторное пространство
\ShowEq{dual space of rcd vector space}
называется \AddIndex{дуальным пространством к \rcd векторному пространству}
{dual space of rcd vector space}
$V$.
Пусть $\Basis e$ - базис в \rcd векторном пространстве $V$.
Базис $\Basis d$ \drc векторного пространства $V^*$,
удовлетворяющий равенству \EqRef{basis of dual vector space},
называется \AddIndex{базисом, дуальным базису}
{basis dual to basis} $\Basis e$.
\qed
\end{definition}

\begin{theorem}
\begin{sloppypar}
Пусть $A$ - пассивное преобразование многообразия базисов
$\mathcal{B}(V,\RCGL nD)$.
Допустим базис
\ShowEq{dual space, image of basis}
является образом базиса $\Basis e$.
Пусть $B$ - пассивное преобразование многообразия базисов
$\mathcal{B}(V^*,\RCGL nD)$ такое, что базис
\ShowEq{dual space, image of dual basis}
дуален базису.
Тогда
\begin{equation}
B=A^{\RCInverse}
\EqLabel{dual space, dual passive transformation}
\end{equation}
\end{sloppypar}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{basis of dual vector space},
\EqRef{dual space, image of basis},
\EqRef{dual space, image of dual basis}
следет
\ShowEq{dual space, passive transformations}
Равенство \EqRef{dual space, dual passive transformation}
следует из равенства \EqRef{dual space, passive transformations}.
\end{proof}

\section{Парные представления тела}

\begin{theorem}
\label{theorem: right-side product of rcd vector over scalar}
\begin{sloppypar}
В любом \rcd векторном пространстве можно определить структуру
$D*$\Hyph векторного пространства, определив
правостороннее произведение вектора на скаляр равенством
\ShowEq{right-side product of rcd vector over scalar}
\end{sloppypar}
\end{theorem}
\begin{proof}
Непосредственная проверка доказывает, что отображение
\[
f:D\rightarrow V^*
\]
определённое равенством
\[
f(m)=m\delta
\]
определяет \Ts{D}представление.
\end{proof}

Мы можем иначе
сформулировать теорему
\ref{theorem: right-side product of rcd vector over scalar}.

\begin{theorem}
\label{theorem: twin representations of division ring}
%\begin{sloppypar}
Если мы определили эффективное правостороннее представление $f$ тела $D$
на абелевой группе $V$,
то мы можем однозначно определить эффективное левостороннее представление $h$ тела $D$
на абелевой группе $V$
такое, что диаграмма
\ShowEq{twin representations of division ring}
коммутативна для любых $a$, $b\in D$.
\qed
%\end{sloppypar}
\end{theorem}
%\begin{proof}
%\end{proof}

Мы будем называть представления $f$ и $h$
\AddIndex{парными представлениями тела}{twin representations of division ring} $D$.

\begin{theorem}
\label{theorem: twin representations, vector space}
В векторном пространстве
$V$ над телом $D$ мы
можем определить $D\star$\Hyph произведение и $\star D$\Hyph произведение вектора на скаляр.
Согласно теореме \ref{theorem: twin representations of division ring} эти операции 
удовлетворяют равенству
\begin{equation}
(am)b=a(mb)
\EqLabel{associative law for twin representations}
\end{equation}
\end{theorem}
Равенство \EqRef{associative law for twin representations}
представляет \AddIndex{закон ассоциативности для парных представлений}
{associative law}.
Это позволяет нам писать подобные выражения не пользуясь скобками.
\begin{proof}
В разделе \ref{section: rcd Linear Map} дано определение
правостороннего произведения линейного отображения $A$ \rcd векторного пространства на скаляр.
Согласно теореме \ref{theorem: right-side product of rcd vector over scalar},
\Ts{D}представление в абелевой группе
$\LDVV$ может быть перенесено
в \rcd векторное пространство $V$ согласно правилу
\ShowEq{twin representations, vector space}
\end{proof}

Аналогия с векторными пространствами над полем заходит столь далеко,
что мы можем предположить существование концепции базиса, который
годится для левостороннего и правостороннего произведения вектора на скаляр.

\begin{theorem}
\label{theorem: rcd dcr basis, vector space}
Многообразие базисов \drc векторного пространства $V$
и многообразие базисов \crd векторного пространства $V$ отличны
\[
\mathcal{B}(V,D\RCstar)\ne\mathcal{B}(V,\CRstar D)
\]
\end{theorem}
\begin{proof}
При доказательстве этой теоремы мы будем пользоваться стандартным представлением
матрицы. Не нарушая общности, мы проведём доказательство в координатном векторном
пространстве $D^n$.

Пусть
\ShowEq{e=delta}
множество векторов векторного пространства $D^{\gin}$.
Очевидно, $\Basis e$ является одновременно базисом \drc векторного пространства
и базисом \crd векторного пространства.
Для произвольного множества векторов
\ShowEq{set of vectors f}
\drc координатная матрица 
\ShowEq{set of vectors f 1}
относительно базиса $\Basis e$ совпадает с \crd координатной матрицей
относительно базиса $\Basis e$.

Если множество векторов
\ShowEq{set of vectors f}
- базис \rcd векторного пространства,
то согласно \xRef{0701.238}{theorem: coordinate matrix of basis}
матрица \EqRef{set of vectors f 1} - \RC невырожденная матрица.

Если множество векторов
\ShowEq{set of vectors f}
- базис \crd векторного пространства,
то согласно теореме \xRef{0701.238}{theorem: coordinate matrix of basis}
матрица \EqRef{set of vectors f 1} - \CR невырожденная матрица.

Следовательно, если множество векторов
\ShowEq{set of vectors f}
порождают базис \drc векторного пространства и базис \crd векторного пространства,
их координатная матрица \EqRef{set of vectors f 1}
является \RC невырожденной и \CR невырожденной матрицей.
Утверждение следует из теоремы \xRef{0701.238}{theorem: CR RC singular matrix}.
\end{proof}

Из теоремы \ref{theorem: rcd dcr basis, vector space} следует, что
существует базис $\Basis e$ \drc векторного пространства $V$,
который не является базисом \crd векторного пространства $V$.

\section{\texorpdfstring{$D$}{D}\hyph векторное пространство}
\label{section: D Vector Space}

При изучении многих задач мы вполне можем ограничиться рассмотрением
$D\star$\Hyph векторного пространства либо $\star D$\Hyph векторного пространства.
Однако есть задачи, в которых мы вынуждены отказаться от простой модели
и одновременно рассматривать обе структуры векторного пространства.

Парное представление тела $D$
в абелевой группе $V$
определяет структуру
\AddIndex{$D$\hyph векторного пространства}{D vector space}.
Из этого определения следует, что если
$v$, $w\in V$, то для любых $a$, $b$, $c$, $d\in D$
\ShowEq{D linear combination}
Выражение
\EqRef{D linear combination}
называется
\AddIndex{линейной комбинацией векторов}
{linear combination of  vectors} $D$\hyph векторного пространства $V$.

\begin{definition}
\label{definition: linearly independent, D vector space}
Векторы
\ShowEq{Vector A subs row 02}
$D$\Hyph векторного пространства
$V$ \AddIndex{линейно независимы}
{linearly independent vectors},
если из равенства
\ShowEq{D linearly independent}
следует
\ShowEq{D linearly independent 1}
В противном случае, векторы $a_i$
\AddIndex{линейно зависимы}{linearly dependent vectors}.
\qed
\end{definition}

\begin{definition}
Мы называем множество векторов
\ShowEq{basis, D vector space}
\AddIndex{базисом $D$\Hyph векторного пространства}{basis, D vector space},
если векторы $e_{\gii}$
линейно независимы и, добавив к этой системе любого другого вектора,
мы получим новую систему, которая является линейно зависимой.
\qed
\end{definition}

\begin{theorem}
\label{theorem: D vector space has dcr basis}
Базис $D$\Hyph векторного пространства $V$
является базисом \dcr векторного пространства $V$.
\end{theorem}
\begin{proof}
Пусть векторы
$a_i$, $i\in I$ линейно зависимы в \dcr векторном пространстве.
Тогда существует \subs строка
\ShowEq{D dimension 0}
такая, что
\ShowEq{D dimension 1}
Из равенства
\EqRef{D dimension 1},
следует, что
\ShowEq{D dimension 2}
Согласно определению
\ref{definition: linearly independent, D vector space},
векторы $a_i$
линейно зависимы в $D$\Hyph векторном пространстве.

Пусть \dcr размерность векторного пространства $V$ равна $\gin$.
Пусть $\Basis e$ - базис \dcr векторного пространства.
Пусть
\[
\begin{pmatrix}
1&...&0
\\...&...&...\\
0&...&1
\end{pmatrix}
\]
координатная матрица базиса $\Basis e$.
Очевидно, что мы не можем
представить вектор $e_{\gin}$ как
$D$\Hyph линейную комбинацию векторов $e_{\giA}$,
..., $e_{\gi{n-1}}$.
%\[(c_0^{ki}\otimes c_1^{ki})f_k\]
%
%\[c_{0\cdot ki}=c_{0\cdot ki}^ne_n\]
%\[c_{1\cdot ki}=c_{1\cdot ki}^me_m\]
%\[e_ne_m=C_{nm}^pe_p\]
%\[f_k=h_k^rf_{kr}\]
%
%\[=>\]
%
%\[a^{ki}c_{0\cdot ki}^nc_{1\cdot ki}^mC_{nm}^pe_ph_k^rf_{kr}\]
\end{proof}

Для нас несущественно, является ли множество векторов
\ShowEq{ei, i in I}
базисом \rcd векторного пространства
или базисом \dcr векторного пространства.
Поэтому при записи координат вектора мы индексы будем записывать
в стандартном формате.
Рассматривая базис $D$\Hyph векторного пространства $V$ мы,
опираясь на теорему
\ref{theorem: D vector space has dcr basis},
будем рассматривать его как базис \dcr векторного пространства $V$.



==> Polymodule.Russian.tex <==
%auto-ignore
\input{Polymodule.Eq}
\chapter{Произведение представлений}
 
\section{Бимодуль}
\label{section: bimodule}

\begin{definition}
$\Vector V$ -
\AddIndex{($S\star$, $\star T$)\hyph бимодуль}{(Sstar,starT)-bimodule},
если на множестве $\Vector V$ определены структуры $S\star$\hyph векторного пространства  и
$\star T$\hyph векторного пространства.\footnote{Напомню, что в наших обозначениях
$S\star$\hyph векторное пространство означает левое $S$\hyph векторное пространство и
$\star T$\hyph векторное пространство означает правое $T$\hyph векторное пространство.}
\qed
\end{definition}

Мы также пользуемся записью \symb{{}_S\Vector V_T}{S T bimodule}1,
когда мы хотим сказать, что $\Vector V$ - ($S$, $T$)\hyph бимодуль.

\begin{example}
\label{example: (D CRstar, RCstar D)-vector space}
В разделе \ref{section: D Vector Space}
мы рассмотрели
$D$\Hyph векторное пространство,
в котором можно определить структуру
($D\CRstar$, $\RCstar D$)\hyph бимодуля.
\qed
\end{example}

\begin{example}
Множество $n\times m$ матриц порождает
($D\star$, $\star D$)\hyph бимодуль.
$D\star$\hyph базис можно представить в виде множества матриц
${_i}{^j}e=(\delta_i^l\delta_k^j)$.
\qed
\end{example}

\begin{example}
Чтобы увидеть пример ($S\RCstar$, $\RCstar T$)\hyph бимодуля,
мы можем взять множество матриц
\begin{equation}
\left(
 \begin{array}{ccc}
(A_1,{}^1B) &...& (A_1,{}^mB)\\
... & ... & ... \\
(A_n,{}^1B) &...&(A_n,{}^mB)
\end{array}\right)
\EqLabel{S RCstar, RCstar T vector space}
\end{equation}
Формально мы можем представить эту матрицу в виде
\[
\left(
 \begin{array}{ccc}
(A_1,{}^1B) &...& (A_1,{}^mB)\\
... & ... & ... \\
(A_n,{}^1B) &...&(A_n,{}^mB)
\end{array}\right)
=
\left(
 \begin{array}{ccc}
A_1\\
...  \\
A_n
\end{array}\right)
\RCstar
\left(
 \begin{array}{ccc}
{}^1B &...& {}^mB
\end{array}\right)
\]
Это представление ясно показывает, что $S\RCstar$\hyph размерность
($S\RCstar$, $\RCstar T$)\hyph бимодуля равна $n$ и $\RCstar T$\hyph размерность равна $m$.
Однако в отличии от примера \ref{example: (D CRstar, RCstar D)-vector space}
мы не можем построить $S\RCstar$\Hyph базис или $\RCstar T$\Hyph базис, который
порождал бы ($S\RCstar$, $\RCstar T$)\hyph бимодуль.
На самом деле базис ($S\RCstar$, $\RCstar T$)\hyph бимодуля имеет вид
$({}^a\Vector e,\Vector f_b)$, и любой вектор ($S\RCstar$, $\RCstar T$)\hyph бимодуля
имеет разложение
\begin{equation}
(\Vector A,\Vector{B})=A_a({}^a\Vector e,\Vector f_b){}^bB
\EqLabel{S RCstar, RCstar T vector space, expansion}
\end{equation}
коэффициенты которого порождают матрицу \EqRef{S RCstar, RCstar T vector space}.
\qed
\end{example}

Мы можем записать равенство \EqRef{S RCstar, RCstar T vector space, expansion} в виде
\ShowEq{S RCstar, RCstar T vector space, expansion, 1}
Равенство \EqRef{S RCstar, RCstar T vector space, expansion, 1}
выглядит необычно, но оно становится понятным, если мы положим
\[
(\Vector A,\Vector{B})=(\Vector A,\Vector 0)+(\Vector 0,\Vector B)
\]
Соглашение \xRef{0701.238}{remark: left and right vector space notation} справедливо
для представления векторов $\RCstar T$\hyph векторного пространства
независимо от представления векторов $S\RCstar$\hyph векторного пространства.
Мы можем записать это равенство в виде
\ShowEq{S RCstar, RCstar T vector space, expansion, 2}
При этом координаты вектора $(\Vector A,\Vector{B})$ не порождают матрицы.
Однако это для нас сейчас не имеет значения.

Мы хотим записать компоненты $A$ и $B$
в равенстве \EqRef{S RCstar, RCstar T vector space, expansion}
с одной стороны по отношению к векторам
$({}^a\Vector e,\Vector f_b)$. На первый взгляд это кажется
невозможной задачей. Однако мы примем соглашение записывать это равенство в виде
\ShowEq{S RCstar, RCstar T vector space, expansion, 3}

Эта конструкция легко подаётся обобщению.

\section{Прямое произведение тел}
\label{section: Direct Product of Division Rings}

\begin{definition}
\label{definition: product of objects in category}
Пусть $\mathcal A$ - категория.
Пусть $\{B_i,\Ii\}$ - множество объектов из $\mathcal A$.
Объект
\ShowEq{product of objects in category}
и множество морфизмов
\[
\{\xymatrix{f_i:P\ar[r]&B_i},\Ii\}
\]
называется
\AddIndex{произведением объектов $\{B_i,\Ii\}$ в категории $\mathcal A$}
{product of objects in category}\footnote{Определение
дано согласно \citeBib{Serge Lang},
страница 45.}, если для любого объекта $R$ и множество морфизмов
\[
\{\xymatrix{g_i:R\ar[r]&B_i},\Ii\}
\]
существует единственный морфизм
\[
\xymatrix{h:R\ar[r]&P}
\]
такой, что диаграмма
\ShowEq{product of objects in category diagram}
коммутативна для всех $\Ii$.

Если $|I|=n$, то для произведения объектов
$\{B_i,\Ii\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product of objects in category, 1 n}
\qed
\end{definition}

\begin{example}
Пусть \(\mathcal S\) - категория множеств.\footnote{Смотри
также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\ref{definition: product of objects in category},
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
\qed
\end{example}

\begin{theorem}
Пусть произведение существует в категории \(\mathcal A\) \(\Omega\)\Hyph алгебр.
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\).
%семейства \(\Omega\)\Hyph алгебр
Тогда
\StartLabelItem
\begin{enumerate}
\item
Множество \(A\) является декартовым произведением
семейства множеств
\ShowEq{Ai iI}
\item
Гомоморфизм \(\Omega\)\Hyph алгебры
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
\item
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
\LabelItem{tuple represent A number}
\item
Пусть
\ShowEq{omega in}
- n\Hyph арная операция.
Тогда операция $\omega$ определена покомпонентно
\ShowEq{operation is defined componentwise}
где
\ShowEq{a=ai 1n}.
\LabelItem{operation is defined componentwise}
\end{enumerate}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение
семейства множеств
\ShowEq{Ai iI}
и, для каждого \iI, отображение 
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
Рассмотрим диаграмму морфизмов в категории множеств $\mathcal S$
\ShowEq{operation is defined componentwise, diagram}
где отображение $g_i$ определено равенством
\ShowEq{gi()=}
Согласно определению
\ref{definition: product of objects in category},
отображение $\omega$ определено однозначно из множества диаграмм
\EqRef{operation is defined componentwise, diagram}
\ShowEq{omega(ai)=(omega ai)}
Равенство
\EqRef{operation is defined componentwise}
является следствием равенства
\EqRef{omega(ai)=(omega ai)}.
\ifx\texFuture\Defined

\begin{lemma}
\label{lemma: tuple represent A number}
{\it
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{projection on i factor}
является произведением в категории \(\mathcal A\).
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
}
\end{lemma}

{\sc Доказательство.}
Пусть
\ShowEq{a ne b}
- такие \(A\)\Hyph числа, что для любого \iI
\ShowEq{p(a)=p(b)}
Если предположить, что неравные \(A\)\Hyph числа
имеют равные разложения в виде кортежа,
то мы можем определить отношение эквивалентности,
фактор по которому скорее кандидат на произведение.
\hfill\(\odot\)

Из равенства
\ShowEq{pj(a)=aj}
следует, что отображение \(p_j\) является проекцией.
\fi
\end{proof}

\begin{definition}
Пусть произведение существует в категории \(\Omega\)\Hyph алгебр.
Если \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\),
то \(\Omega\)\Hyph алгебра \(A\) называется
\AddIndex{прямым}{direct product of Omega algebras}
или
\AddIndex{декартовым произведением \(\Omega\)\Hyph алгебр}{Cartesian product of Omega algebras}
\ShowEq{Ai iI}.
\qed
\end{definition}

\begin{example}
Пусть $\{G_i,\Ii\}$ - множество групп.
Пусть
\ShowEq{Cartesian product of groups}
декартово произведение множеств $G_i$, $\Ii$.
Мы определим на $G$ групповую структуру посредством
покомпонентного умножения.
Если $x=(x_i,\Ii)\in D$ и $y=(y_i,\Ii)\in D$,
мы определим их произведение
\[xy=(x_iy_i,\Ii)\]
Если $x=(x_i,\Ii)\in D$,
мы определим обратный элемент
\[x^{-1}=(x_i^{-1},\Ii)\]
Множество $G$ называется
\AddIndex{декартовым произведением групп}{Cartesian product of groups}\footnote{Определение
дано согласно \citeBib{Serge Lang}, страницы 47, 48.}
$G_i$, $\Ii$.

Если $|I|=n$,
то для декартова произведения групп $G_1$, ..., $G_n$
мы так же будем пользоваться записью
\ShowEq{Cartesian product of groups, 1 n}
\qed
\end{example}

\begin{theorem}
\label{theorem: Product of Abelian group}
Декартово произведение абелевых групп является абелевой группой.
\end{theorem}
\begin{proof}
Пусть $x=(x_i,\Ii)\in G$ и $y=(y_i,\Ii)\in G$.
Тогда
\[
x+y=(x_i+y_i,\Ii)=(y_i+x_i,\Ii)=y+x
\]
\end{proof}

\begin{example}
Пусть $\{D_i,\Ii\}$ - множество тел.
Пусть
\ShowEq{direct product of division rings}
произведение аддитивных групп тел $D_i$, $\Ii$.
Если $x=(x_i,\Ii)\in D$ и $y=(y_i,\Ii)\in D$,
мы определим их произведение покомпонентно
\[xy=(x_iy_i,\Ii)\]
Мультипликативная единица - это $e=(e_i,\Ii)\in D$, где $e_i$,
$\Ii$ - мультипликативная единица тела $D_i$.
Множество $D$ называется
\AddIndex{прямым произведением тел}{direct product of division rings}\footnote{Определение
дано согласно
предложению 1 из \citeBib{Serge Lang},
стр. 79} $D_i$, $\Ii$.
 
Если $|I|=n$,
то для прямого произведения тел $D_1$, ..., $D_n$
мы так же будем пользоваться записью
\ShowEq{direct product of division rings, 1 n}
\qed
\end{example}

Прямое произведение тел  $D_i$, $\Ii$, вообще говоря, не является телом.
Например, пусть $x_1\in D_1$, $x_1\ne 0$, $x_2\in D_2$, $x_2\ne 0$. Тогда
\[
(x_1,0)(0,x_2)=(0,0)
\]
Однако прямое произведение тел является кольцом.
Следовательно, прямое произведение не определенно в категории
тел, но прямое произведение тел определено в категории колец.

\begin{theorem}
\label{theorem: map from product into product}
Пусть множество \(A\) является
декартовым произведением множеств
\ShowEq{Ai iI}
и множество \(B\) является
декартовым произведением множеств
\ShowEq{Bi iI}.
Для каждого \iI, пусть
\ShowEq{f:A->B i}
является отображением множества $A_i$ в множество $B_i$.
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras diagram}
где отображения
\ShowEq{pi p'i}
являются проекцией на \(i\)\Hyph й множитель.
Множество коммутативных диаграмм
\EqRef{homomorphism of Cartesian product of Omega algebras diagram}
однозначно определяет отображение
\ShowEq{f:A->B}
\DrawEq{f:A->B=}{}
\end{theorem}
\begin{proof}
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras}
Пусть \(a\in A\).
Согласно утверждению
\RefItem{tuple represent A number},
\(A\)\Hyph число \(a\)
может быть представлено в виде кортежа \(A_i\)\Hyph чисел
\ShowEq{a=p(a)i}
Пусть
\ShowEq{b=f(a)}
Согласно утверждению
\RefItem{tuple represent A number},
\(B\)\Hyph число \(b\)
может быть представлено в виде кортежа \(B_i\)\Hyph чисел
\ShowEq{b=p(b)i}
Из коммутативности диаграммы $(1)$
и из равенств
\EqRef{b=f(a)},
\EqRef{b=p(b)i}
следует, что
\ShowEq{b=g(a)i}
Из коммутативности диаграммы $(2)$
и из равенства
\EqRef{a=p(a)i}
следует, что
\ShowEq{b=f(a)i}
\end{proof}

\begin{theorem}
\label{theorem: homomorphism of Cartesian product of Omega algebras}
Пусть \(\Omega\)\Hyph алгебра \(A\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}
и \(\Omega\)\Hyph алгебра \(B\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Bi iI}.
Для каждого \iI,
пусть отображение
\ShowEq{f:A->B i}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
Тогда отображение
\ShowEq{f:A->B}
определённое равенством
\DrawEq{f:A->B=}{homomorphism}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{omega in}
- n\Hyph арная операция.
Пусть
\ShowEq{a=ai 1n} и
\ShowEq{b=bi 1n}.
Из равенств
\EqRef{operation is defined componentwise},
\eqRef{f:A->B=}{homomorphism}
следует, что
\ShowEq{f:A->B omega}
\end{proof}

\begin{remark}
Утверждение, обратное утверждениям теорем
\ref{theorem: map from product into product},
\ref{theorem: homomorphism of Cartesian product of Omega algebras},
вообще говоря, неверно.
Рассмотрим, например, $R$\Hyph векторное пространство $V$ размерности $2$
и линейное отображение
\ShowEq{linear map dimension 2}
Векторное пространство $V$ - это абелева группа, которая является
декартовым произведением абелевых групп
\ShowEq{V=RxR}
Отображение $f$ является гомоморфизмом абелевой группы $V$.
Однако соответствие
\ShowEq{x2->x'2}
зависит от значения переменной $x^1$
и поэтому не является отображением.
\qed
\end{remark}

\section{Прямое произведение \texorpdfstring{\drc}{drc-}векторных пространств}
\label{section: direct product, drc vector space}

\begin{lemma}
\label{lemma: product of *algebras is *algebra}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение семейства \(\Omega_1\)\Hyph алгебр
\ShowEq{Ai iI}.
Для каждого \iI, пусть множество ${}^*A_i$
является \(\Omega_2\)\Hyph алгеброй.
Тогда множество
\ShowEq{f in *A =}
является декартовым произведением \(\Omega_2\)\Hyph алгебр ${}^*A_i$.
\end{lemma}
\begin{proof}
Согласно определению
\EqRef{f in *A =},
мы можем представить отображение
\ShowEq{f in *A}
в виде кортежа
\ShowEq{f=(fi)}
отображений
\ShowEq{fi in *Ai}
Согласно определению
\EqRef{f in *A =},
\ShowEq{(fi)(ai)=}
Пусть
\ShowEq{omega in}
- n\Hyph арная операция.
Мы определим операцию $\omega$
на множестве
\ShowEq{circ A}
равенством
\ShowEq{circ A omega}
\end{proof}

\begin{theorem}
\label{theorem: product of single transitive representations}
Допустим категория $\mathcal A_1$ $\Omega_1$\Hyph алгебр имеет произведение.
Допустим категория $\mathcal A_2$ $\Omega_2$\Hyph алгебр имеет произведение.
Тогда в категории\footnote{Смотри определение
\xRef{0701.238}{definition: category of representations of F algebra from category}}
\ShowEq{(A1*)A2}
существует произведение
однотранзитивных левосторонних представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре.
\end{theorem}
\begin{proof}
Для
\ShowEq{j=12}
пусть
\ShowEq{P=xBi}
произведение семейства $\Omega_j$\Hyph алгебр
\ShowEq{Bi}
и для любого $\Ii$ отображение
\EqParm{ti:P->Bi}{P=P}
является проекцией на множитель $i$.
Для каждого $\Ii$, пусть
\EqParm{F:P->*P}{P=B}
однотранзитивное \Ts{B_{1i}}представление в \(\Omega_2\)\Hyph алгебре $B_{2i}$.

Пусть
\(b_1\in P_1\).
Согласно утверждению
\RefItem{tuple represent A number},
\(P_1\)\Hyph число \(b_1\)
может быть представлено в виде кортежа \(B_{1i}\)\Hyph чисел
\ShowEq{b=t(b)1i}
Пусть
\(b_2\in P_2\).
Согласно утверждению
\RefItem{tuple represent A number},
\(P_2\)\Hyph число \(b_2\)
может быть представлено в виде кортежа \(B_{2i}\)\Hyph чисел
\ShowEq{b=t(b)2i}

\begin{lemma}
Для каждого $\Ii$, рассмотрим диаграмму отображений
\ShowEq{define product of single transitive representations}
Пусть отображение
\ShowEq{g:P1->*P2}
определено равенством
\ShowEq{g(b1)(b2)=}
Тогда отображение \(g\) является
однотранзитивным \Ts{P_1}представлением в \(\Omega_2\)\Hyph алгебре $P_2$
\EqParm{F:P->*P}{P=P}
Отображение
\ShowEq{ti12}
является морфизмом представления \(g\) в представление \(h_i\).
\end{lemma}

{\sc Доказательство.}
\StartLabelItem
\begin{enumerate}
\item
Согласно определениям
\ref{definition: transformation of universal algebra},
\ref{definition: left-side representation of algebra},
отображение $h_i(b_{1i})$ является гомоморфизмом
\(\Omega_2\)\Hyph алгебры $B_{2i}$.
Согласно теореме
\ref{theorem: homomorphism of Cartesian product of Omega algebras},
из коммутативности диаграммы $(1)$ для каждого \iI,
следует, что отображение
\ShowEq{g(b):P->P}
определённое равенством
\EqRef{g(b1)(b2)=}
является гомоморфизмом
\(\Omega_2\)\Hyph алгебры $P_2$.
\LabelItem{g(b) is homomorphism of Omega2 algebra P2}
\item
Согласно определению
\ref{definition: left-side representation of algebra},
множество
\ShowEq{*B2i}
является $\Omega_1$\Hyph алгеброй.
Согласно лемме
\ref{lemma: product of *algebras is *algebra},
множество
\ShowEq{*P2}
является $\Omega_1$\Hyph алгеброй.
\item
Согласно определению
\ref{definition: left-side representation of algebra},
отображение
\ShowEq{h:B1->*B2 i}
является гомоморфизмом
\(\Omega_1\)\Hyph алгебры.
Согласно теореме
\ref{theorem: homomorphism of Cartesian product of Omega algebras},
отображение
\ShowEq{g:P1->*P2}
определённое равенством
\ShowEq{g(b1)=}
является гомоморфизмом
\(\Omega_1\)\Hyph алгебры.
\LabelItem{g is homomorphism of Omega1 algebra P1->*P2}
\end{enumerate}

Согласно утверждениям
\RefItem{g(b) is homomorphism of Omega2 algebra P2},
\RefItem{g is homomorphism of Omega1 algebra P1->*P2}
и определению
\ref{definition: left-side representation of algebra},
отображение $g$ является \Ts{P_1}представлением
в $\Omega_2$\Hyph алгебре $P_2$.

Пусть
\ShowEq{b2 12 in P2}
Согласно утверждению
\RefItem{tuple represent A number},
\(P_2\)\Hyph числа
\ShowEq{b2 12}
может быть представлено в виде кортежей \(B_{2i}\)\Hyph чисел
\ShowEq{b=t(b)2i 12}
Согласно теореме
\ref{theorem: Representation is single transitive iff},
поскольку представление $h_i$ однотранзитивно,
то существует единственное \(B_{1i}\)\Hyph число $b_{1i}$ такое, что
\ShowEq{b22=h(b1)b21}
Согласно определениям
\EqRef{b=t(b)1i},
\EqRef{g(b1)(b2)=},
\EqRef{b=t(b)2i 12},
существует единственное \(P_1\)\Hyph число $b_1$ такое, что
\ShowEq{b22=g(b1)b21}
Согласно теореме
\ref{theorem: Representation is single transitive iff},
представление $g$ однотранзитивно.

Из коммутативности диаграммы $(1)$ и определения
\ref{definition: morphism of representations of F algebra}
следует, что отображение
\ShowEq{ti12}
является морфизмом представления \(g\) в представление \(h_i\).
\hfill\(\odot\)

Пусть
\ShowEq{d=g(b)(b)}
Из равенств
\EqRef{g(b1)(b2)=},
\EqRef{d=g(b)(b)}
следует, что
\ShowEq{d=h(b)(b)}

Для
\ShowEq{j=12}
пусть $R_j$ другой объект категории $\mathcal A_j$. Для любого $\Ii$, пусть
\EqParm{ti:P->Bi}{P=R1}
морфизм из $\Omega_1$\Hyph алгебра $R_1$ в
$\Omega_1$\Hyph алгебру $B_{1i}$.
Согласно определению
\ref{definition: product of objects in category},
существует единственный морфизм $\Omega_1$\Hyph алгебры
\ShowEq{s:R->P,1}
такой, что коммутативна диаграмма
\ShowEq{t*s=r1}
Пусть
\ShowEq{a in R1}
Пусть
\ShowEq{b=s(a)1}
Из коммутативности диаграммы
\EqRef{t*s=r1}
и утверждений
\EqRef{b=s(a)1},
\EqRef{b=t(b)1i}
следует, что
\ShowEq{b=r(a)1i}

Пусть
\EqParm{F:P->*P}{P=R}
однотранзитивное \Ts{R_1}представление в \(\Omega_2\)\Hyph алгебре $R_2$.
Согласно теореме
\ref{theorem: unique morphism of representations of F algebra},
морфизм $\Omega_2$\Hyph алгебры
\EqParm{ti:P->Bi}{P=R2}
такой, что отображение
\ShowEq{(r12)}
является морфизмом
представлений из $f$ в $h_i$,
определён однозначно
с точностью до выбора образа $R_2$\Hyph числа $a_2$.
Согласно замечанию
\ref{remark: morphism of representations of F algebra},
в диаграмме отображений
\ShowEq{r12 product of single transitive representations}
диаграмма $(2)$ коммутативна. 
Согласно определению
\ref{definition: product of objects in category},
существует единственный морфизм $\Omega_2$\Hyph алгебры
\ShowEq{s:R->P,2}
такой, что коммутативна диаграмма
\ShowEq{t*s=r2}
Пусть
\ShowEq{a in R2}
Пусть
\ShowEq{b=s(a)2}
Из коммутативности диаграммы
\EqRef{t*s=r2}
и утверждений
\EqRef{b=s(a)2},
\EqRef{b=t(b)2i}
следует, что
\ShowEq{b=r(a)2i}
Пусть
\ShowEq{c=f(a)(a)}
Из коммутативности диаграммы $(2)$ и равенств
\EqRef{d=h(b)(b)},
\EqRef{b=r(a)2i},
\EqRef{c=f(a)(a)}
следует, что
\ShowEq{d=r(c)2i}
Из равенств
\EqRef{d=h(b)(b)},
\EqRef{d=r(c)2i}
следует, что
\ShowEq{d=s(c)2}
что согласуется с коммутативносью диаграмы
\EqRef{t*s=r2}.

Для каждого $\Ii$, мы объединим диаграммы отображений
\EqRef{define product of single transitive representations},
\EqRef{t*s=r1},
\EqRef{t*s=r2},
\EqRef{r12 product of single transitive representations}
\ShowEq{product of single transitive representations}
Из равенств
\EqRef{d=g(b)(b)}
\EqRef{b=s(a)2}
и из равенств
\EqRef{c=f(a)(a)},
\EqRef{d=s(c)2},
следует коммутативность диаграммы $(3)$.
Следовательно, отображение
\ShowEq{(s12)}
является морфизмом
представлений из $f$ в $g$.,
Согласно теореме
\xRef{0701.238}{theorem: unique morphism of representations of F algebra},
морфизм
\ShowEq{(s12)}
определён однозначно,
так как мы требуем
\EqRef{d=s(c)2}.

Согласно определению
\ref{definition: product of objects in category},
представление $g$
и семейство морфизмов представления
\ShowEq{ti12, family}
является произведением в категории
\ShowEq{(A1*)A2}.
\end{proof}

\begin{theorem}
В категории $\mathcal G*$ левосторонних представлений группы
существует произведение
эффективных левосторонних представлений группы.
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\ref{theorem: product of single transitive representations}
и \xRef{0701.238}{theorem: Free representation is single transitive}
\end{proof}

\begin{definition}
Пусть $\{V_i,\Ii\}$ - множество \Di векторных пространств.
Левостороннее представление кольца $\displaystyle D=\prod_{\Ii}D_i$
в абелевой группе
\ShowEq{V=xVi}
называется \AddIndex{прямым произведением
\ShowEq{direct product, rcd vector space}
\Di векторных пространств}
{direct product, rcd vector space}\footnote{Определение
дано согласно \citeBib{Serge Lang},
стр. 98} $V_i$, $\Ii$.
\qed
\end{definition}

Если $|I|=n$, то для прямого произведения
\Di векторных пространств $V_1$, ..., $V_n$
мы так же будем пользоваться записью
\ShowEq{direct product, drc vector space, 1 n}

Согласно определению представление кольца $D$ в абелевой группе $V$
определенно покомпонентно. 
Если $a=(a_i,\Ii)\in D$ и
\ShowEq{v=(vi)}
мы определим правостороннее представление, соответствующее элементу $a$
\ShowEq{representation in direct product, rcd vector space}
Мы рассматриваем соглашение,
описанное в замечании
\xRef{0701.238}{remark: left and right matrix notation},
покомпонентно.
Линейную комбинацию \rcd векторов $\Vector v_k$ мы будем записывать в виде
\ShowEq{linear combination 1, direct product, rcd vector space}
Мы так же будем пользоваться записью
\ShowEq{Linear combination 2, direct product, rcd vector space}
Если $|I|=n$, то равенство
\EqRef{Linear combination 2, direct product, rcd vector space}
можно записать в виде
\ShowEq{Linear combination 3, direct product, rcd vector space}

Так как прямое произведение тел не является телом, то
прямое произведение
\Di векторных пространств,
вообще говоря, является модулем.
Однако структура этого модуля близка к структуре
\rcd векторного пространства.

\begin{theorem}
Пусть $V_1$, ..., $V_n$ - множество \Di векторных пространств.
Пусть $\Basis e_i$ - \Di базис векторного пространства $V_i$.
Множество векторов
\ShowEq{basis,n vector space}
порождает базис прямого произведения
\ShowEq{V=V1x...xVn}
\end{theorem}
\begin{proof}
Мы докажем утверждение теоремы индукцией по $n$.

При $n=1$ утверждение очевидно.

Допустим утверждение справедливо при $n=k-1$.
Мы можем представить пространство $V$ в виде\footnote{Вообще говоря,
мы должны рассматривать более широкий класс модулей вида
\[V_1\times...\times V_k\]
включая ассоциативность произведения.}
\ShowEq{V1x...xVk=()xVk}
Соответственно, произвольный вектор
\ShowEq{(v1k)}
можно представить в виде
\ShowEq{Linear combination, direct product, 1}
\ShowEq{(v1k-1)}
и согласно предположению индукции
\ShowEq{Linear combination, direct product, 2}
Из равенств \EqRef{Linear combination, direct product, 1}
и \EqRef{Linear combination, direct product, 2}
следует
\ShowEq{Linear combination, direct product, 3}
Следовательно утверждение справедливо при $n=k$.
\end{proof}

Если $V_1$, ..., $V_n$ -
$D$\hyph векторные пространства,
то прямое произведение называется
\AddIndex{прямым произведением $D$\Hyph векторных пространств}
{direct product of D vector spaces}.

\begin{theorem}
%\label{theorem: product of single transitive representations}
Допустим категория $\mathcal A$ $\Omega$\Hyph алгебр имеет произведение.
Тогда в категории $A*$\footnote{Смотри определение
\xRef{0701.238}{definition: category of left-side representations of Omega1 algebra}},
где $A$ - $\Omega$\Hyph алгебра,
существует произведение
однотранзитивных \Ts{A}представлений.
\end{theorem}
\begin{proof}
Доказательство теоремы похоже на доказательство теоремы
\ref{theorem: product of single transitive representations}
с той разницей, что мы пользуемся диаграммой
\[
\xymatrix{
&&N\ar[rrrrr]^{T_i}\ar@{}[drrrrr]|{(3)}&&\ar@{}[dddddll]|{(2)}&
&&K_i
\\
&&&&&&&
\\
A\ar[r]^{id}\ar@/^2pc/@{=>}[urrr]^g&
A\ar@{=>}[urrrrr]^(.4){h_i}&&&
N\ar[r]^{T_i}\ar[lluu]_{g(a)}&
K_i\ar[rruu]_(.3){h_i(a)}
\\
A\ar[u]^{id}\ar@/_2pc/[ur]_{id}\ar@/_2pc/@{=>}[drrr]^f
&&&&
M\ar[u]^S\ar@{}[ur]|{(1)}\ar[ddll]^(.3){f(a)}\ar@/_1pc/[ru]_{R_i}
\\
&&&&&&&
\\
&&M\ar[uuuuu]^S\ar@/_5pc/[rrrrruuuuu]_{R_i}
}
\]
\end{proof}

Рассмотрим связь между
произведением
однотранзитивных левосторонних представлений $\Omega$\Hyph алгебры $A$
в категории $\mathcal A*$ и
произведением
однотранзитивных левосторонних представлений $\Omega$\Hyph алгебры $A$
в категории $A*$.
Пусть для каждого $\Ii$ определено представление $\Omega$\Hyph алгебры $A$
на множестве $K_i$.
Для каждого $\Ii$ рассмотрим диаграмму
\[
\xymatrix{
\prod_{\Ii}A\ar[r]^{f_i}&A
\\
A\ar[u]^g\ar[ur]_{id}
}
\]
где $g$ - отображение алгебры $A$ на диагональ в
$\displaystyle \prod_{\Ii}A$ и
$f_i$ - проекция на множитель $i$.
Из диаграммы следует, что отображения
$g$ и $f_i$ инъективны.
Следовательно оба произведения эквивалентны.

\section{Морфизмы прямого произведения \texorpdfstring{\rcd}{rcd-}векторных пространств}

Пусть $V_i$, $\Ii$,
$W_j$, $\Jj$
- \rcd векторные пространства.
Положим
\ShowEq{V=xV W=xW}
Линейное отображение
\ShowEq{Morphisms of Direct Product of rcd Vector Spaces}
сохраняет линейные операции.
Так как операции в модуле $W$
мы выполняем покомпонентно, то мы можем
представить отображение $f$ в виде
\ShowEq{f=(fj)}
Пусть
\ShowEq{I:Vi->V}
вложение $V_i$ в $V$.
Тогда для любого вектора
\ShowEq{v=(vi)}
справедливо
\ShowEq{fj(v)=+fj(vi)}
Следовательно, отображение
\EqRef{Morphisms of Direct Product of rcd Vector Spaces}
можно представить в виде матрицы \rcd линейных отображений
\ShowEq{f:Vi->Wj}


==> Preface.0701.238.English.tex <==
%auto-ignore
\input{Preface.0701.238.Eq}
\chapter{Preface}

\ePrints{0701.238}
\ifx\Semafor\ValueOn
\section{Preface to Version 1}
\else
\section{Preface}
\fi

Starting a new journey you do not know in the beginning what to expect down the road.
I started studying noncommutative algebra just out of curiosity.
In the case of a module over a ring it is impossible to give
the definition of basis in the way we do it in the case of a vector space over a field.
I wanted to understand how the picture changes when I use division ring
instead of a field.

I started from the study of systems of linear equations. I started
from system of two equations in two unknowns. Even I solved system without problem, 
it was impossible to express this solution as the ratio of two determinants.

I understood that this problem might be interesting not only for me.
I started to search for the mathematicians, who are interested in the same problem.
Professor Retakh
introduced me papers \citeBib{math.QA-0208146,q-alg-9705026}
dedicated to theory of quasideterminants. It was beginning of my research in theory
of vector space.

I dedicated chapter \ref{chapter: Biring of Matrices} to biring of matrices. There are
two reasons why I study this algebra. 

Suppose we are given basis in vector space. Then we can describe transformation
of vector space
using a matrix. Product of matrices corresponds to the product of transformations.
In contrast to commutative case it is not each time possible to represent this product
as the product of rows of first matrix over columns of second one.
The same time representation of matrix as
\[
A=\left(
\begin{array}{ccc}
A^1_1&...&A^1_n\\
...&...&...\\
A^n_1&...&A^n_n
\end{array}
\right)
\]
depends on convention.
Without loss of generality we can represent matrix as
\[
A=\left(
\begin{array}{ccc}
A^1_1&...&A^n_1\\
...&...&...\\
A^1_n&...&A^n_n
\end{array}
\right)
\]
However in this case the algorithm to find product changes.

Structures like biring are known in algebra. In lattice we define
operations $a\vee b$ and $a\wedge b$ which exchange places
when order on the set reverses. The symmetry between \RC product
and \CR product is phrased as duality principle. Subsequently
I extend the duality principle to representation theory and theory of
vector spaces.
Without considering the duality principle the book would be four times its size,
let alone the fact that endless reiterations would make the text hard to read.

According to each
product we can extend the definition of a quasideterminant given
in \citeBib{math.QA-0208146,q-alg-9705026}
and introduce two different
types of a quasideterminant.

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
The chapter \ref{chapter: Representation of Algebra}
is review of representation theory and is basis for following
chapters.
We extend to representation theory convention
described in remark
\ref{remark: left and right matrix notation}.
\else
The chapter \ref{chapter: Representation of Group}
is review of theory of representation of group
and is basis for following
chapters.
\fi
Theorem about an existence of twin representations in homogeneous space finishes the
chapter.

In the chapter \ref{chapter: Vector Space Over Division Ring}
I study a few concepts of linear algebra over division ring $D$.
I recall definitions of a vector space and a basis in the beginning.\footnote{You
can see definitions also in \citeBib{Carl Faith 1}.}
Linear algebra over a division ring is more diverse
than linear algebra over a field.
In contrast to vector space over a field,
we can define left and right vector space over an arbitrary division ring $D$.
To make the definition of a basis stronger I turn to theory
of an arbitrary system of linear equations (section
\ref{section: System of Linear Equations})
for each type of vector space.
However, in spite of this
diversity statements from linear algebra over a division ring
are very similar to statements
from linear algebra
over a field.

Because I apply statements of this chapter
in geometry, I will follow
the same notation as we use in geometry.
To write coordinates of a vector and elements of a matrix
we follow the convention described in section
\ref{section: Concept of Generalized Index}.

We identify the vector and the set of its coordinates relative
selected basis. However, they are different objects. To underscore
this difference, I returned to traditional notation of
vector as $\Vector a$,
when vector and its coordinates are present in the same equation;
at the same time we will use notation
$a^b$ for coordinates of vector $\Vector a$.
We use the same root letter for notation of a basis and vectors
which form it. To distinguish a vector and a basis, we will
use notation $\Basis e$ for the basis and notation
$\Vector e_a$ for vectors which form the basis $\Basis e$.
Studying theory of vector space we use convention
described in remark
\ref{remark: left and right matrix notation}
and in section
\xRef{math.OA-0612137}{section: Representation of Group}.

Chapter \ref{chapter: Basis Manifold} is dedicated to the theory of linear representation.
The studying of a homogenous space of a group of symmetry of a \drc vector space
leads us to the definition of a basis of this \drc vector space
and a basis manifold.
We introduce two types of transformation of a basis manifold:
active and passive transformations. The difference between them is
that the active transformation can be expressed as a transformation of
an original space.
As it is shown in \citeBib{Rashevsky} passive transformation
gives ability to define
concepts of invariance and of geometric object.
Based on this theory I study
basis manifold, passive and active transformations
in section \ref{section: Basis Manifold for Vector Space}.
I study geometric object of the \drc vector space
in section \ref{section: Geometric Object of Vector Space}.

We have two opposite points of view about a geometric object.
On the one hand we determine coordinates of the geometric object
relative to a given basis and introduce the law of transition of
coordinates during transformation of the basis.
At the same time we study the set of coordinates
of the geometric object relative to different bases
as a single whole. This gives us an opportunity
to study the geometric object without using coordinates.

\ePrints{0701.238}
\ifx\Semafor\ValueOn
Chapter \ref{chapter: rcd Linear Map}
is dedicate to linear map of \rcd vector spaces over division ring.
This statement is basis for development of theory of twin representations of ring $D$.
The notation that I introduced for the theory of vector space
seems ponderous. However this notation is guided by the existence of twin representations.

Linear algebra over a division ring is more diverse than linear algebra over
a field. 
Noncommutativity compels us to take care about a proper order of factors in
an expression. This leads not only to diversity of concepts, but also helps more
clear see statements of commutative algebra.

\begin{flushright}
January, 2007
\end{flushright}

\section{Preface to Version 2}
\epigraph
{Any criminal once a while makes mistake.
//
When detective discovered my cap on the table, he became furious.
Next time there was rain, and I left a wet track on the floor.
Needless to say, I had to start from the scratch again.
And I started again and again. The Tunguska Cosmic Body, an unplanned solar eclipse, ...
However, \ finally detective did not find \ defects in the design.
//
- Tic-tac-toe, - detective sought sorrowfully. - You were not
tired to code this game? It is time to start something more deep.}
{Author is unknown. The art of programming.}

Science research sometimes reminds programming. Complex and large project
gradually becomes surrounded by code. Everything seems to be simple and clear. However, suddenly
the bug appears. Fix of this bug demands to alter nearly half of the code. As the wise man observed
in any software there is at least one bug, though.

When I started the research in the field of vector spaces over division ring, I saw that
I stepped to terra incognita. The concept of quasideterminant
extremely lightened my task. The opportunity to solve a system of linear equations
made this theory very similar to theory of vector spaces over field.
This gave ability to define basis and extent the concept of geometric object.

Tensors of order $2$ appeared on the scene as dark cloud.
Non commutability seemed to be putting on the structure of tensor
insurmountable constrains. However at this time I discovered
light in the tunnel.

\input{Preface.Additive.English}

$D$\Hyph vector space is the best candidate
for building of tensor algebra. However one more important structure was required here.

When we study rings, we study not only left or right module over ring,
but bimodule also. Division ring is no exception.
However if we add up the concept of the biring,
it becomes obvious that it does not matter from what side we multiply.
As consequence it appears
that bivector space is particular case of 
direct product of \drc vector spaces.
%multivector spaces.
We cannot define
polylinear map.
However consideration of
polyadditive maps of direct product of \drc vector spaces leads
to definition of tensor product.
Such way we can build tensors of arbitrary
structure.

I designed this paper such way that it allows reproduce my not simple and interesting adventure
in the world of tensors over division ring.

\begin{flushright}
March, 2009
\end{flushright}

\section{Preface to Version 3}

\input{Preface.Linear.English}

\section{Preface to Version 5}
\epigraph
{Passenger: ... We will be late at the train station!
//
Little Engine: ... But if we do not see the first lily of the valley,
then we will be late for the entire spring! 
//
...
//
Passenger: ... We will be too late!
//
Little Engine: Yes. But if we do not hear the first nightingales,
then we will be late for the entire summer! 
//
...
//
Little Engine: Dawn! ... every sunrise is the only in our life! 
... It is time to ride. After all we will be late.
//
Passenger: Yes. But if we do not see the dawn, we may be late for the whole life!
}
{Gennadi Tsyferov, Little Engine from Romashkovo.}

Young man John departed from point A to point B.
Two hours later his friend Peter went on a bicycle from point $B$
in the direction to the point $A$.
How fast did Peter ride, if they met in an hour?..

This is the familiar problem of school problem book.
But the problem is not so simple as it is formulated.
When Peter was near the pond he saw swans and stopped to
make picture. John stopped in the grove to hear the nightingales.
There they met.

Very often I tempted to take a look at the end of the problem book.
The solution is almost there, just a jiffy away.
However some uncertainty remains when you see the printed answer. 
I already see in general the theory that I am looking for.
However I understand that I have a long way ahead of me before I will be able
to tell about this to others.
Besides, my experience tells ne that when you stroll along unfamiliar terrain,
suddenly see such an amazing landscape that unintentionally stay there longer,
to explore this place better.

However, once I could not resist and, in the paper \citeBib{0906.0135},
I tried to analyze how it may look like geometry over division ring.
Although the paper was premature, the results
formed the basis of my subsequent research.

\[
\xymatrix{
\ar@{-}[rr]& &
}
\]

In the paper \citeBib{1003.1544}, I explored the system of additive equations
in $\Omega$\hyph algebra where the operation of addition is defined.
The format of notation of equations in \citeBib{1003.1544} is
determined by the format of operations in $\Omega$\hyph algebra.
This format is different from format accepted in this book by default.
The theory of additive equations is generalization of the theory of \rcd linear
equations and uses the same methods. 
Different order of variable and coefficient in equation
made it difficult to compare results in both books.
However it is not important for me  whether I consider a system of \dcr linear
equations or a system of \rcd linear equations. This stimulated
me to edit text of this book and to consider the system
of \rcd linear equations by default.

Besides, I realized that the notion of a set of additive mappings is
artificial in the study of linear algebra over division ring.
That is why I removed corresponding definitions and theorems from this version.
Now I am directly considering a linear mapping over a given field.

The main difference of linear mappings over division ring is
that I cannot represent a linear mapping as product of element
of division ring over variable. In papers \citeBib{1001.4852,1003.1544},
I found way to functionally separate variable and mapping.
This allows me to represent a notation of linear mapping in the familiar form.
However in this book I keep the previous notation.
It has several reasons for this.

First of all, both forms of notation are correct. We can use any of these
forms of notation choosing the one that seems more appropriate.
It also enables the reader to compare both forms of notation.
In addition, in \citeBib{1003.1544}, I consider linear mapping of algebras
in parallel with their tensor product, since these two topics are
inseparable.
In this book, I decided to follow the same path that I covered
when I worked on the second version of this book
and present the tensor product as distinctive peak to
ascend at the end of the book.

However, the road covered after the last version was
reflected on last chapters of the book.
For instance, since division ring is algebra over field, I decided to use
the standard representation of indexes.
The key changes are attributed
with my perception of $D$\Hyph vector spaces.
Let us take a closer look at this subject in greater detail
since this subject remains outside of the scope of the book.

$D$\Hyph vector space appeared as corollary of theorem
about twin representations of division ring in Abelian group (theorems
\ref{theorem: twin representations of division ring},
\ref{theorem: twin representations, vector space}).
Initially I considered $D$\Hyph vector space
as consolidation of structures of \dcr vector space and \rcd
vector space. Correspondingly I considered \dcr basis
and \rcd basis.

Let
$\Basis p$ be basis of \rcd vector space $V$
and basis $\Basis r$ be basis of \dcr vector space $V$.
Vector ${}_ir$ of basis $\Basis r$
has expansion
\ShowEq{vector expansion, basis 1 2, D vector space}
relative to basis $\Basis p$.
Vector $p_j$ of basis $\Basis p$
has expansion
\ShowEq{vector expansion, basis 2 1, D vector space}
relative to basis $\Basis r$.

It is easy to see from design that $R$ is
coordinate matrix of basis $\Basis r$
relative to basis $\Basis p$.
Columns of matrix $R$ are \dcr linearly independent.

In the same way, $P$ is
coordinate matrix of basis $\Basis p$
relative to basis $\Basis p$.
Columns of matrix $P$ are \rcd linearly independent.

From equations \EqRef{vector expansion, basis 1 2, D vector space}
and \EqRef{vector expansion, basis 2 1, D vector space} it follows
\ShowEq{vector expansion, rcd basis, D vector space}
From equation \EqRef{vector expansion, rcd basis, D vector space}
we see that order of brackets is important.

Though matrices $P$ and $R$ are not inter inverse,
we see that equation \EqRef{vector expansion, rcd basis, D vector space}
represents identical transformation of $D$\Hyph vector space.
It is possible to write this transformation as
\ShowEq{vector expansion, dcr basis, D vector space}

From comparison of equations \EqRef{vector expansion, rcd basis, D vector space}
and \EqRef{vector expansion, dcr basis, D vector space}
it follows that change of order of brackets changes order
of summation. These equations express the symmetry in choice of
bases $\Basis p$ and $\Basis r$.

\ifx\texFuture\Defined
Vector $q\in V$ has expansion
\ShowEq{vector expansion, D vector space}
Let us substitute \EqRef{vector expansion, basis 1 2, D vector space} into
\EqRef{vector expansion, D vector space}
\ShowEq{vector expansion, D vector space, 1}
Let us substitute \EqRef{vector expansion, D vector space} into
\EqRef{vector expansion, rcd basis, D vector space}
\ShowEq{vector expansion, rcd vector, D vector space}
\fi

A non-trivial presentation of identity
map like expression \EqRef{vector expansion, rcd basis, D vector space}
or
\EqRef{vector expansion, dcr basis, D vector space}
was a complete surprise to me.

There is another interesting statement that I saved for later
analysis, namely the theorem \ref{theorem: rcd dcr basis, vector space},
which states existence of \dcr basis which is not
\rcd basis. We will make a pause here.

In \citeBib{0912.3315}, I explored the theory of representations of $\Omega$\Hyph algebra.
According to this theory,
$D$\Hyph vector space is representation of algebra
$D\otimes D$ in Abelian group.
Therefore, choice of basis is determined neither by \Ds linear  dependence
or by \sD linear  dependence, but by dependence like in expression
\[
a_{s\cdot 0}^i \Vector e_i a_{s\cdot 1}^i
\]
Therefore, \dcr basis is not also basis of $D$\Hyph vector space
if it is not \rcd bais.
However, it is easy to see that the set of transformations of basis
forms a group.
This structure of basis  leads to the fact that the difference
between right and left bases disappears. This is why for $D$\Hyph vector
space, I use standard representation of index.

However, even more surprising statement follows from this.
Coordinates of vector of $D$\Hyph vector space belong
to algebra $D\otimes D$.
Few questions arise.
\begin{itemize}
\item Can a basis of $D$\Hyph vector space
be \rcd basis?
\item What is relation between dimensions of $D$\Hyph vector space
and \rcd vector space?
\item What is the structure of $1$\Hyph
dimensional $D$\Hyph vector space?
\end{itemize}
I intend to explore these questions for free modules over arbitrary
algebra. This is the main reason why this topic is outside the scope
of this book.

But we can already say that the set of
\rcd linearly dependent vectors cannot be the basis of $D$\Hyph vector space.
Therefore  dimension of $D$\Hyph vector space
does not exceed dimension of corresponding \drc vector space.
Therefore, I gave in this book proper
description of $D$\hyph vector space.

Well, I could not resist, and once again looked at the end of the problem book.

\begin{flushright}
August, 2010
\end{flushright}
\fi


==> Preface.0701.238.Eq.tex <==
%auto-ignore

\DefEquation
{
\begin{matrix}
{}_ir=p_j\ {}^j_iR
&
{}_ir= p\RCstar {}_iR
\end{matrix}
}
{vector expansion, basis 1 2, D vector space}

\DefEquation
{
\begin{matrix}
p_j=P^i_j\ {}_ir
&
p_j=P_j\CRstar r
\end{matrix}
}
{vector expansion, basis 2 1, D vector space}

\DefEquation
{
\begin{split}
{}_ir&=p_j\ {}^j_iR
=P^k_j\ {}_kr\ {}^j_iR
\\
{}_ir&=p\RCstar {}_iR
=(P\CRstar r)\RCstar {}_iR
\end{split}
}
{vector expansion, rcd basis, D vector space}

\DefEquation
{
\begin{split}
q&=q_r^i\ {}_ir=p_j\ {}^jq_p
\\
q&=q_r\CRstar r=p\RCstar q_p
\end{split}
}
{vector expansion, D vector space}

\DefEquation
{
\begin{matrix}
q_r^i\ p_j\ {}^j_iR=p_j\ {}^jq_p
&
q_r\CRstar(p\RCstar R)=p\RCstar q_p
\end{matrix}
}
{vector expansion, D vector space, 1}

\DefEquation
{
\begin{array}{lll}
q_r^i\ {}_ir&=q_r^i\ p_j\ {}^j_iR
&=q_r^i\ P^k_j\ {}_kr\ {}^j_iR
\\
q_r\CRstar p&=q_r\CRstar(p\RCstar R)
&=q_r\CRstar((P\CRstar p)\RCstar R)
\end{array}
}
{vector expansion, rcd vector, D vector space}

\DefEquation
{
\begin{split}
p_j&=P^i_j\ {}_ir
=P^i_j\ (p_k\ {}^k_iR)
\\
p_j&=P_j\CRstar r
=P_j\CRstar (p\RCstar R)
\end{split}
}
{vector expansion, dcr basis, D vector space}


==> Preface.0701.238.Russian.tex <==
%auto-ignore
\input{Preface.0701.238.Eq}
\chapter{Предисловие}

\ePrints{0701.238}
\ifx\Semafor\ValueOn
\section{Предисловие к изданию 1}
\else
\section{Предисловие}
\fi
Отправляясь в новое путешествие, не знаешь вначале, что ждёт тебя в пути.
Знакомство с некоммутативной алгеброй началось с простого любопытства.
В случае модуля над кольцом нельзя дать определение базиса
подобно тому, как мы это делаем в случае векторного пространства над полем.
Я хотел понять, как изменится картина, если вместо поля я буду рассматривать тело.

Прежде всего мне надо было научиться решать системы линейных уравнений. Я начал
с системы двух уравнений с двумя неизвестными. Хотя решение было найдено легко, 
это решение нельзя выразить как отношение двух определителей.

Я понимал, что эта проблема интересует не только меня. Я начал искать
математиков, интересующихся подобными задачами. Профессор Ретах
познакомил меня со статьями \citeBib{math.QA-0208146,q-alg-9705026}
по теории квазидетерминантов. Это было началом моего исследования в теории
векторных пространств.

Глава \ref{chapter: Biring of Matrices} посвящена бикольцу матриц. Существует две причины,
почему я рассматриваю эту алгебру. 

Если в векторном пространстве задан базис, то преобразование
векторного пространства можно описать
с помощью матрицы. Произведению преобразований соответствует произведение
матриц. В отличии от коммутативного случая мы не всегда можем представить
это произведение в виде произведения строк первой матрицы на столбцы второй.
В то же время запись элементов матрицы в виде
\[
A=\left(
\begin{array}{ccc}
A^1_1&...&A^1_n\\
...&...&...\\
A^n_1&...&A^n_n
\end{array}
\right)
\]
является вопросом соглашения.
Не нарушая общности, мы можем записать матрицу в виде
\[
A=\left(
\begin{array}{ccc}
A^1_1&...&A^n_1\\
...&...&...\\
A^1_n&...&A^n_n
\end{array}
\right)
\]
Но тогда изменяется правило умножения матриц.

Конструкции подобные бикольцу известны в алгебре. В структуре определены
операции $a\vee b$ и $a\wedge b$, которые меняются местами, если порядок на множестве
меняется на противоположный. Симметрия между \RC произведением
и \CR произведением сформулирована в форме принципа двойственности. Впоследствии
я распространяю принцип двойственности на теорию представлений и теорию векторных
пространств. Без учёта принципа двойственности эта книга была бы в четыре раза больше,
не говоря о том, что бесконечные повторения текста сделали бы чтение текста невозможным.

Согласно каждому виду произведения мы можем
расширить определение квазидетерминанта, данное
в \citeBib{math.QA-0208146,q-alg-9705026},
и определить два разных
вида квазидетерминанта.

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
Глава \ref{chapter: Representation of Algebra} является
обзором теории представлений и является базой для последующих
глав.
Мы распространим на представление алгебры соглашение,
описанное в замечании
\ref{remark: left and right matrix notation}.
\else
Глава \ref{chapter: Representation of Group} является
обзором теории представлений групп
и является базой для последующих
глав.
\fi
Теорема о существовании парных представлений в однородном
пространстве завершает главу.

В главе \ref{chapter: Vector Space Over Division Ring}
я изучаю
несколько концепций линейной алгебры над телом $D$.
Сперва я напоминаю определения векторного пространства и базиса.\footnote{Определения
можно найти также в \citeBib{Carl Faith 1}.}
Линейная алгебра над телом более богата фактами
по сравнению с
линейной алгеброй над полем.
В отличии от векторных пространств над полем,
мы можем определить левое и правое векторное пространство над
произвольным телом $D$.
Чтобы дать более строгое определение базиса, я излагаю теорию
произвольной системы линейных уравнений (раздел
\ref{section: System of Linear Equations})
для каждого типа векторного пространства.
Тем не менее, не смотря на это
разнообразие, утверждения линейной алгебры над телом очень похожи
на утверждения из линейной алгебры
над полем.

Так как я пользуюсь утверждениями этой главы
в геометрии, я следую той же форме записи, что мы
используем в геометрии.
При записи координат вектора и элементов матрицы
мы будем следовать
соглашению, описанному в разделе
\ref{section: Concept of Generalized Index}.

Мы отождествляем вектор с набором его координат относительно
некоторого базиса. Тем не менее, это различные объекты. Чтобы
подчеркнуть это различие, я вернулся к традиционному обозначению
вектора в форме $\Vector a$,
когда вектор и его координаты присутствуют в одном и том же равенстве;
в тоже время мы будем пользоваться записью
$a^b$ для координат вектора $\Vector a$.
Мы используем одну и туже корневую букву для обозначения базиса и
составляющих его векторов. Чтобы отличить вектор и базис, мы будем
пользоваться обозначением $\Basis e$ для базиса и обозначением
$\Vector e_a$ для векторов, составляющих базис $\Basis e$.
Изучая теорию векторных пространств мы будем пользоваться соглашением,
описанным в замечании
\ref{remark: left and right matrix notation}
и в разделе
\xRef{math.OA-0612137}{section: Representation of Group}.

Глава \ref{chapter: Basis Manifold} посвящена теории линейных представлений.
Изучение однородного пространства группы симметрий \drc векторного пространства
ведёт нас к определению базиса этого \drc векторного пространства
и многообразия базисов.
Мы вводим два типа преобразований многообразия базисов:
активные и пассивные преобразования. Различие между ними состоит в том,
что активное преобразование может быть выражено как преобразование
исходного пространства.
Как показано в \citeBib{Rashevsky}, пассивное преобразование
даёт возможность определить
понятия инвариантности и геометрического объекта.
Опираясь на эту теорию, я изучаю
многообразие базисов, пассивные и активные преобразования
в разделе \ref{section: Basis Manifold for Vector Space}.
Я рассматриваю геометрический объект в \drc векторном пространстве
в разделе \ref{section: Geometric Object of Vector Space}.

Мы имеем
две противоположные точки зрения на геометрический объект.
С одной стороны мы фиксируем координаты геометрического объекта
относительно заданного базиса и указываем закон преобразования
координат при замене базиса. В то же время мы рассматриваем
всю совокупность координат геометрического объекта
относительно различных базисов как единое целое. Это
даёт нам возможность бескоординатного
изучения геометрического объекта.

\ePrints{0701.238}
\ifx\Semafor\ValueOn
Глава \ref{chapter: rcd Linear Map} посвящена линейным отображениям
\rcd векторных пространств над телом.
Это явилось основой построения парных представлений кольца D.
Несмотря на кажущуюся громоздкость, обозначения, которыми я пользуюсь в
теории векторных пространств, опираются на существование парных представлений.

Линейная алгебра над телом более разнообразна по сравнению с линейной алгеброй над полем. 
Некоммутативность заставляет нас позаботиться о правильном порядке множителей в
выражении. Это порождает не только разнообразие понятий, но также помогает лучше
понять утверждения коммутативной алгебры.

\begin{flushright}
Январь, 2007
\end{flushright}

\section{Предисловие к изданию 2}
\epigraph
{Любой преступник рано или поздно совершает ошибку.
//
Когда детектив нашёл мою кепку на столе, он пришёл в ярость.
В следующий раз был дождь, и я оставил мокрые следы на полу.
Нечего говорить, опять пришлось начать сначала.
И я начинал снова и снова. То тунгуский метеорит, то незапланированное затмение Солнца...
Но в конце концов детектив не нашёл изъянов в дизайне.
//
- Крестики и нолики, - печально вздохнул детектив. - Вам не
надоело кодироать эту игру? Пора уже заняться чем-то более серьёзным.}
{Автор неизвестен. Искуство программирования.}

Научный поиск иногда напоминает программирование. Сложный и большой проект
постепенно обрастает кодами. Всё кажется просто и понятно. Но вдруг появляется
баг, исправление которого требует переделать почти половину кода. Впрочем, как заметил
мудрец, в любой программе есть по крайней мере один баг.

Когда я начал исследование в области векторных пространств над телами, я понимал,
что я ступаю на terra incognita. Концепция квазидетерминанта
весьма облегчила мою задачу. Возможность решить систему линейных уравнений
сделала эту теорию весьма похожей на теорию векторных пространств над полями.
Это дало возможность построить базис и расширить концепцию геометрического объекта.

Тёмным облаком встали на горизонте двухвалентные тензоры. Казалось, некоммутативность
накладывает на их структуру непреодолимые ограничения. Но именно в эту минуту я увидел
свет в тунеле.

\input{Preface.Additive.Russian}

$D$\Hyph векторное пространство является наиболее удачным претендентом
для построения тензорной алгебры. Однако здесь потребовалась ещё одна важная конструкция.

Когда мы имеем дело с кольцами, мы изучаем не только модули, левые или правые,
но и бимодули. Тело не является исключением.
Но если добавить сюда концепцию бикольца,
становится очевидным, что мне без разницы, с какой стороны умножать.
Как следствие, оказывается,
что бивекторное пространство - это частный случай
прямого произведения \drc векторных пространств.
%мультивекторных пространств.
Мы не можем определить полилинейное отображение.
Однако рассмотрение
полиадитивных отображений прямого произведения \drc векторных пространств приводит
к определению тензорного произведения.
Таким образом,
можно построить тензора произвольной природы.

Статья эта построена таким образом, чтобы воспроизвести моё непростое и интересное путешествие
в мир тензоров над телом.

\begin{flushright}
Март, 2009
\end{flushright}

\section{Предисловие к изданию 3}

\input{Preface.Linear.Russian}

\newpage

\section{Предисловие к изданию 5}
\epigraph
{Пассажир: ... Мы же опоздаем на станцию!
//
Паровозик: ... Но если мы не увидим первых ландышей,
то мы опоздаем на всю весну! 
//
...
//
Пассажир: ... Мы же совсем опоздаем!
//
Паровозик: Да. Но если мы не услышим первых соловьёв,
то мы опоздаем на всё лето! 
//
...
//
Паровозик: Рассвет! ... каждый рассвет единственный в жизни! 
... Ехать пора. Ведь мы опоздаем.
//
Пассажир: Да. Но если мы не увидим рассвет, мы можем опоздать на всю жизнь!
}
{Геннадий Цыферов, Паровозик из Ромашково.}

Молодой человек по имени Женя вышел из пункта $A$ в пункт $B$.
Через два часа его товарищ Петя выехал из пункта $B$
на велосипеде по направлению к пункту $A$.
С какой скоростью ехал Петя, если они встретились через час?..

Знакомая задача из школьного задачника.
Но задача не столь проста как она сформулирована.
Петя проезжал мимо пруда, увидел лебедей и остановился, чтобы их
сфотографировать. А Женя остановился в роще послушать соловьёв.
Там они и встретились.

Очень часто хочется заглянуть в конец задачника. Вот оно решение,
уже близко.
Однако что-то непознанное останется за рамками готового ответа.
Я уже сейчас вижу в общих чертах теорию, которую я ищу.
Но я понимаю, что прежде я смогу рассказать об этом другим, мне предстоит
пройти длинный путь.
Кроме того, мой опыт мне подсказывает, что когда бредёшь по незнакомой
местности, внезапно увидишь столь удивительный ландшафт, что невольно задержишься,
чтобы познакомиться с ним получше.

Впрочем, один раз я не удержался и в статье \citeBib{0906.0135}
попытался проанализировать, как может выглядеть геометрия над телом.
И хотя статья выглядела незавершенной, её результаты легли в основу
моих последующих исследований.

\[
\xymatrix{
\ar@{-}[rr]& &
}
\]

В статье \citeBib{1003.1544} я рассматриваю систему аддитивных уравнений
в $\Omega$\hyph алгебре, в которой определена операция сложения.
Формат записи уравнений в \citeBib{1003.1544} определён форматом операций в
$\Omega$\hyph алгебре.
Этот формат отличался от формата принятому в этой книге по умолчанию.
Теория аддитивных уравнений является обобщением теории \rcd линейных
уравнений и пользуется теми же методами.
Другой порядок переменной и коэффициента в уравнении
затруднял сравнение результатов в обеих книгах.
Однако для меня не имеет значения, рассматриваю ли я систему \dcr линейных
уравнений или систему \rcd линейных уравнений. Это побудило
меня отредактировать текст этой книги и рассматривать систему
\rcd линейных уравнений по умолчанию.

Кроме того я понял, что множество аддитивных отображений является
понятием искусственным при изучении линейной алгебры над телом.
Поэтому я при переработке этого издания удалил соответствующие определения
и теоремы и рассматриваю непосредственно линейное отображение над
заданным полем.

Основное отличие линейных отображений над телом состоит в том,
что я не могу представить линейное отображение в виде произведения элемента
тела на переменную. В статьях \citeBib{1001.4852,1003.1544}
я нашёл способ функционального разделения переменной и отображения.
Это позволяет представить запись линейного отображения в знакомой форме.
Однако в этой книге я сохранил прежнюю форму записи.
Причин этому несколько.

Прежде всего, обе формы записи верны. Мы можем пользоваться любой из
этих форм записи, выбирая ту, которая кажется более адекватной.
Это даёт также возможность читателю сопоставлять обе формы записи.
Кроме того, в \citeBib{1003.1544} я рассматриваю линейное отображение алгебр
параллельно с их тензорным произведением, так как эти две темы
неразделимы.
В этой книге я решил сохранить тот путь, который я прошёл
при написании второго издания этой книги
и сохранить тензорное произведение как своеобразную вершину, к которой я
подымаюсь в конце книги.

Тем не менее, путь, пройденный после последнего издания,
отразился на последних главах книги.
Например, поскольку тело является алгеброй над полем, я решил перейти к
стандартному представлению индексов. Основные изменения коснулись
моего понимания $D$\Hyph векторных пространств.
Я остановлюсь на этом вопросе немного подробнее,
поскольку эта тема осталась за пределами книги.

$D$\Hyph векторное пространство возникло как следствие теоремы
о парных представлениях тела в абелевой группе (теоремы
\ref{theorem: twin representations of division ring},
\ref{theorem: twin representations, vector space}).
Вначале я рассматривал $D$\Hyph векторное пространство
как объединение структур \dcr векторного пространства и \rcd
векторного пространства. Соответственно я рассматриваю \dcr базис
и \rcd базис.

Допустим, что
$\Basis p$ - базис \rcd векторного пространства $V$
и $\Basis r$ - базис \dcr векторного пространства $V$.
Вектор ${}_ir$ базиса $\Basis r$
имеет разложение
\ShowEq{vector expansion, basis 1 2, D vector space}
относительно базиса $\Basis p$.
Вектор $p_j$ базиса $\Basis p$
имеет разложение
\ShowEq{vector expansion, basis 2 1, D vector space}
относительно базиса $\Basis r$.

Нетрудно видеть из построения, что $R$ -
координатная матрица базиса $\Basis r$
относительно базиса $\Basis p$.
Столбцы матрицы $R$ \dcr линейно независимы.

Аналогично, $P$ -
координатная матрица базиса $\Basis p$
относительно базиса $\Basis r$.
Столбцы матрицы $P$ \rcd линейно независимы.

Из равенств \EqRef{vector expansion, basis 1 2, D vector space}
и \EqRef{vector expansion, basis 2 1, D vector space} следует
\ShowEq{vector expansion, rcd basis, D vector space}
Из равенства \EqRef{vector expansion, rcd basis, D vector space}
видно, что порядок скобок существенен.

Хотя матрицы $P$ и $R$ не являются взаимно обратными,
мы можем сказать, что равенство \EqRef{vector expansion, rcd basis, D vector space}
описывает тождественное преобразование $D$\Hyph векторного пространства.
Это преобразование можно записать также в виде
\ShowEq{vector expansion, dcr basis, D vector space}

Из сравнения равенств \EqRef{vector expansion, rcd basis, D vector space}
и  \EqRef{vector expansion, dcr basis, D vector space}
следует, что изменение порядка скобок приводят к изменению порядка
суммирования. Эти равенства выражают симметрию в выборе
базисов $\Basis p$ и $\Basis r$.

\ifx\texFuture\Defined
Вектор $q\in V$ имеет разложение
\ShowEq{vector expansion, D vector space}
Подставим \EqRef{vector expansion, basis 1 2, D vector space} в
\EqRef{vector expansion, D vector space}
\ShowEq{vector expansion, D vector space, 1}
Подставим \EqRef{vector expansion, D vector space} в
\EqRef{vector expansion, rcd basis, D vector space}
\ShowEq{vector expansion, rcd vector, D vector space}
\fi

Нетривиальная запись тождественного
отображения в виде \EqRef{vector expansion, rcd basis, D vector space}
либо
\EqRef{vector expansion, dcr basis, D vector space}
явилась для меня полнейшей неожиданностью.

Другое интересное утверждение, которое я сохранил для последующего
анализа - это теорема \ref{theorem: rcd dcr basis, vector space},
которая утверждает существование \dcr базиса, который не является
\rcd базисом. Здесь мы сделаем остановку.

Согласно теории представлений $\Omega$\Hyph алгебры,
рассмотренной в \citeBib{0912.3315},
$D$\Hyph векторное пространство является представлением алгебры
$D\otimes D$ в абелевой группе.
Следовательно, выбор базиса определяется не \Ds линейной зависимостью
или \sD линейной зависимостью, а зависимостью вида
\[
a_{s\cdot 0}^i \Vector e_i a_{s\cdot 1}^i
\]
Следовательно, \dcr базис, который не является \rcd базисом,
не является также базисом $D$\Hyph векторного пространства.
Тем не менее не трудно убедиться, что множество преобразований базиса
порождает группу.
Эта структура базиса приводит к тому, что исчезает разница
между правым и левым базисами. Поэтому я для $D$\Hyph векторного
пространства пользуюсь стандартным представлением индекса.

Однако из этого следует ещё более удивительное утверждение.
Координаты вектора $D$\Hyph векторного пространства принадлежат
алгебре $D\otimes D$.
Сразу появляются вопросы.
\begin{itemize}
\item Может ли базис $D$\Hyph векторного пространства
быть \rcd базисом?
\item Каково соотношение размерностей $D$\Hyph векторного
пространства и \rcd векторного пространства?
\item Какова структура $1$\Hyph
мерного $D$\Hyph векторного пространства?
\end{itemize}
Я планирую рассмотреть эти вопросы для свободных модулей над произвольной
алгеброй. Это основная причина почему эта тема лежит вне
рамок этой книги.

Однако уже сейчас можно сказать, что множество векторов,
которое \rcd линейно зависимо, не может быть базисом $D$\Hyph векторного
пространства. Поэтому размерность $D$\Hyph векторного пространства
не превышает размерность соответствующего \drc векторного
пространства. А следовательно описание $D$\hyph векторного пространства,
предложенное в данной книге остаётся верным.

Что ж. Я не удержался, и заглянул в конец задачника.

\begin{flushright}
Август, 2010
\end{flushright}
\fi


==> Preface.Additive.English.tex <==
%auto-ignore
The considering of \drc linear maps leads to the concept
of twin representations of division ring in Abelian group.
Abelian group, in which we define twin representation of division ring $D$,
is called $D$\Hyph vector space.
Since we define multiplication over elements of division ring $D$ from left,
as well as right, then homomorphisms of $D$\Hyph vector spaces
cannot keep this operation. This leads to concept
of additive map which is morphism of $D$\Hyph vector
space.\footnote{Design of additive mapping which I made proving theorem
\ref{theorem: linear map, D vector space},
is instructive methodically. From the time when I
started to learn differential geometry, I accepted
the fact that we can everything express using tensor,
that we enumerate components of tensor by
indexes and this relationship is permanent.
Once I saw that it was not the case,
I found myself unprepared to recognize it
It got month before I was able to write down expression that I saw by my eyes.
The problem was because I tried to write down this expression in
tensor form.}


==> Preface.Additive.Russian.tex <==
%auto-ignore
Изучение \drc линейных отображений приводит к концепции
парных представлений тела в абелевой группе.
Абелева группа, в которой определено парное представление тела $D$,
называется $D$\Hyph векторным пространством.
Поскольку умножение на элементы тела $D$ определено и слева,
и справа, гомоморфизмы $D$\Hyph векторных пространств
не могут сохранять эту операцию. Это приводит к концепции
аддитивного отображения, которое является морфизмом $D$\Hyph векторных
пространств.\footnote{Построение аддитивного отображения, выполненное при доказательстве теоремы
\ref{theorem: linear map, D vector space},
весьма поучительно методически. С того самого момента,
когда я начал изучать дифференциальную геометрию, я признал
факт, что всё сводится к тензорам, что компоненты тензора нумеруются с
помощью индексов и эта связь неразрывна.
В тот момент, когда это оказалось не так, я оказался не готов признать это.
Понадобился месяц прежде, чем я смог записать выражение, которое я видел глазами,
но которое я не мог записать до этого, так как пытался выразить его в тензорной
или операторной форме.}


==> Preface.Linear.English.tex <==
%auto-ignore

Quaternion algebra is the simplest example of division ring.
This is why I verify
theorems in quaternion algebra to see how they work.
Quaternion algebra is similar to complex field
and so it is natural to search some parallel.

In real field any additive map automatically turns out to be
linear over real field. This statement is caused by statement that real
field is completion of rational field and is corollary of
theorem \ref{theorem: linear map, division ring, rational}.

However the statement changes for complex field.
Not every additive map of complex field is
linear over complex field. Conjugation is the simplest example of
such map.
As soon as I discovered this extremely interesting statement, I returned to question about
analytical representation of additive map.

Exploring additive maps, I realized that I too abruptly
expanded the set of linear maps while switching from field to division ring.
The reason for this was not a very clear understanding
of how to overcome the noncommutativity of the product.
However during the process of research it became more evident
that any additive map is linear over some field.
For the first time I used this concept when constructing the
tensor product
and the concept took shape in a subsequent study.

During constructing the tensor product of division rings $D_1$, ..., $D_n$
I assumed existence of field $F$ such that additive
map of division ring $D_i$ is linear over this field for any $i$. If all division rings
have characteristic $0$, then according to theorem
\ref{theorem: linear map, division ring, rational}
such field always exists. However
dependence of tensor product on selected field $F$ arises here.
To get rid of this dependence, I assume
that field $F$ is maximal field that possesses stated property.

If $D_1=...=D_n=D$, then such field is center $Z(D)$
of division ring $D$.
If the product in division ring $D$ is commutative\footnote{In other words,
division ring is field.}, then $Z(D)=D$.
So, starting with additive map, I arrive at concept
of linear map, which is generalization of linear map over field.

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
%The set of additive maps contains disjoint subsets
%of additive maps generated by one generator, as well as
%maps that are linear combination of maps of first group.
%The set  of generators depends on division ring, however
%always includes identity map.

%My decision to explore additive map generated only by identity
%map was influenced by following.

%\item Additive map is morphism of representations of division ring $D$ in
%$D$\Hyph vextor space. We explore additive map of division ring $D$
%considering division ring $D$ as one dimensional $D$\Hyph vector space.
%If division $D$ is field, then additive map has
%to be linear. As we noted above, conjugation is
%not linear map of complex field.

My decision to explore the G\^ateaux derivative as linear map
was influenced by following.

\begin{itemize}

\item Linear map of field is homogeneous polynomial of
degree one.
%Complex polynomial depends on $z$, however it does not depend on $\overline z$.
%Like linear map, additive map is coordinated with structure of
%polynomial.

\item For continuous field derivative of function of field is homogeneous
polynomial of degree one that is good approximation to change of function.
The same time we explore the derivative as linear map of
field. At the transition to division ring we can save the same link
between derivative and additive map.

\end{itemize}

%Because additive map generated by identity map is the main object of our course
%I do not introduce new terminology and when I use
%termin additive map I have in mind additive map
%generated by identity map.
\fi

Research in area of complex numbers and quaternions
revealed one more interesting phenomenon. In spite of the fact that
complex field is extension of real
field, the structure of linear map over complex
field is different from the structure of linear map
over real field. This difference leads to the statement
that conjugation of complex numbers is additive map
but not linear map over complex field.

Similarly, the structure of linear map over division ring of
quaternions is different from the structure of linear map
over complex field.
The source of difference is statement that the center of quaternion algebra
has more simple structure than complex field.
This difference leads to the statement that
conjugation of quaternion satisfies to equation
\[
\overline p =-\frac 12 (p+ipi+jpj+kpk) 
\]
Consequently, the problem  to find a mapping satisfying
to a theorem similar to the Riemann theorem
(theorem \ref{theorem: complex field over real field}),
is a nontrivial task for quaternions.

\begin{flushright}
August, 2009
\end{flushright}


==> Preface.Linear.Russian.tex <==
%auto-ignore

Алгебра кватернионов - самый простой пример тела. Поэтому я проверяю
полученные мной теоремы в алгебре кватернионов, чтобы увидеть как они работают.
Алгебра кватернионов похожа на поле комплексных чисел
и поэтому естественно искать некоторые параллели.

В поле действительных чисел любое аддитивное отображение автоматически оказывается
линейным над полем действительных чисел. Это связано с тем, что поле действительных
чисел является пополнением поля рациональных чисел и является следствием
теоремы \ref{theorem: linear map, division ring, rational}.

Однако в случае комплексных чисел ситуация меняется.
Не всякое аддитивное отображение поля комплексных чисел оказывается
линейным над полем комплексных чисел. Операция сопряжения - простейший пример
такого отображения.
Когда я обнаружил этот крайне интересный факт, я вернулся к вопросу об
аналитическом представлении аддитивного отображения.

Изучая аддитивные отображения, я понял, что я слишком резко
расширил множество линейных отображений при переходе от поля к телу.
Причиной этому было не вполне ясное понимание как преодолеть
некоммутативность произведения.
Однако в процессе построений становилось всё более очевидным,
что любое аддитивное отображение линейно над некоторым полем.
Впервые эта концепция появилась при построении
тензорных произведений
и отчётливо проявилась в
последующем исследовании.

При построении тензорного произведения тел $D_1$, ..., $D_n$
я предполагаю существование поля $F$, над которым аддитивное
преобразование тела $D_i$ линейно для любого $i$. Если все тела
имеют характеристику $0$, то согласно теореме
\ref{theorem: linear map, division ring, rational}
такое поле всегда существует. Однако здесь возникает
зависимость тензорного произведения от выбранного поля $F$.
Чтобы избавиться от этой зависимости, я предполагаю,
что поле $F$ - максимальное поле, обладающее указанным свойством.

Если $D_1=...=D_n=D$, то такое поле является центром $Z(D)$
тела $D$.
Если произведение в теле $D$ коммутативно\footnote{Иными словами,
тело является полем.}, то $Z(D)=D$.
Следовательно, начав с аддитивного отображения, я пришёл к концепции
линейного отображения, которая является обобщением линейного отображения над полем.

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
%Множество аддитивных отображений содержит непересекающиеся классы
%аддитивных отображений, порождаемых одной образующией, а также
%отображения, являющиеся линейной комбинацией отображений первой группы.
%Множество образующих зависит от тела, но всегда включает тождественное отображение.

%На моё решение изучать аддитивные отображения, порождаемые только тождественным
%отображением, повлияли следующие обстоятельства.

%\item Аддитивное отображение - это морфизм представлений тела $D$ в
%$D$\Hyph векторном пространстве. Мы изучаем аддитивное отображение тела $D$,
%рассматривая тело $D$ как одномерное $D$\Hyph векторное пространство.
%Если тело $D$ является полем, то аддитивное отображение должно
%стать линейным. Как мы заметили выше, операция сопряжения не
%является линейным отображением поля комплексных чисел.

На моё решение изучать производную Гато как линейное отображение
повлияли следующие обстоятельства.

\begin{itemize}

\item Линейное отображение поля - это в тоже время однородный многочлен
первой степени.
%Комплексный многочлен зависит от $z$, но не зависит от $\overline z$.
%Так же как и линейное отображение, аддитивное отображение должно быть согласовано со структурой
%многочлена.

\item Для непрерывных полей производная функции поля - это однородный
многочлен первого порядка, аппроксимирующий изменение функции.
Одновременно мы рассматриваем производную как линейное отображение
поля. При переходе к телу мы можем сохранить ту же связь
производной и аддитивного отображения.

\end{itemize}

%Так как основным объектом нашего изучения являются аддитивные отображения,
%порождённые тождественным отображением, я не ввожу новой терминологии и,
%употребляя термин аддитивное отображение, имею в виду аддитивное отображение,
%порождённое тождественным отображением.
\fi

Исследование в области комплексных чисел и кватернионов
проявили ещё одно интересное явление. Несмотря на то,
что поле комплексных чисел является расширением поля
действительных чисел, структура линейного отображения над полем
комплексных чисел отличается от структуры линейного отображения
над полем действительных чисел. Это различие приводит к тому,
что операция сопряжения комплексных чисел является аддитивным отображением,
но не является линейным отображением над полем комплексных чисел.

Аналогично, структура линейного отображения над телом
кватернионов отличается от структуры линейного отображения
над полем комплексных чисел.
Причина различия в том, что центр алгебры кватернионов
имеет более простую структуру, чем поле комплексных чисел.
Это отличие приводит к тому, что операция сопряжения
кватерниона удовлетворяет равенству
\[
\overline p =-\frac 12 (p+ipi+jpj+kpk) 
\]
Вследствие этого задача найти отображения, удовлетворяющие
теореме подобной теореме Римана
(теорема \ref{theorem: complex field over real field}),
является нетривиальной задачей для кватернионов.

\begin{flushright}
Август, 2009
\end{flushright}


==> Quaternion.Russian.tex <==
%auto-ignore
\ePrints{1003.1544,8433-5163}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\Chapter{Алгебра с делением}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
В этом разделе мы рассмотрим равенства, которые следуют из теоремы
\ref{theorem: Gateaux differential and jacobian, algebra}.
Мы рассмотрим
поля комплексных чисел, алгебру кватернионов и алгебру октонионов.
Хотя в разделе \ref{chapter: Differentiable maps}
мы изучали дифференцируемые отображения в ассоциативную алгебру,
однако, как было отмечено в разделе
\ref{Section: Linear Map into Nonassociative Algebra},
равенства, которые мы записываем в неассоциативной алгебре,
незначительно отличаются от равенств, которые мы записываем в ассоциативной алгебре.
\fi%Calculus.Paper
\else%1003.1544,8433-5163,Calculus.Paper
\Chapter{Алгебра кватернионов}
\label{chapter: Quaternion Algebra}
\fi%1003.1544,8433-5163,Calculus.Paper

\input{\FilePrefix Complex.Number.Russian}

\input{\FilePrefix Quaternion.Eq}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
\Section{Линейная функция алгебры кватернионов}

\begin{theorem}
\label{theorem: Quaternion over real field}
Положим
\ShowEq{basis of quaternion}
базис алгебры кватернионов $H$.
Тогда в базисе \EqRef{basis of quaternion} структурные константы имеют вид
\ShowEq{structural constants, quaternion}
\end{theorem}
\begin{proof}
Значение структурных констант следует из таблицы умножения
\EqRef{product of quaternions}.
\end{proof}

Так как вычисления в этом разделе занимают много места,
я собрал в одном месте ссылки на теоремы в этом разделе.
\begin{description}
\item [Теорема \ref{theorem: Standard components of linear function, quaternion},
страница \pageref{theorem: Standard components of linear function, quaternion}]
определение координат линейного отображения
алгебры кватернионов $H$
через стандартные компоненты этого отображения.
\item [Равенство \EqRef{quaternion, 3, B->A},
страница \pageref{eq: quaternion, 3, B->A}]
матричная форма зависимости координат линейного отображения
алгебры кватернионов $H$
от стандартных компонент этого отображения.
\item [Равенство \EqRef{quaternion, 3, A->B},
страница \pageref{eq: quaternion, 3, A->B}]
матричная форма зависимости стандартных компонент линейного отображения
алгебры кватернионов $H$
от координат этого отображения.
\item [Теорема \ref{theorem: coordinates of linear function, quaternion},
страница \pageref{theorem: coordinates of linear function, quaternion}]
зависимость стандартных компонент линейного отображения
алгебры кватернионов $H$
от координат этого отображения.
\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\item [Равенство \EqRef{quaternion conjugation},
страница \pageref{eq: quaternion conjugation}]
сопряжения кватернионов - линейное отображение
\fi
\end{description}

\begin{theorem}
\label{theorem: Standard components of linear function, quaternion}
Стандартные компоненты линейной функции
алгебры кватернионов $H$ относительно базиса
\EqRef{basis of quaternion}
и координаты соответствующего линейного преобразования
удовлетворяют соотношениям
\ShowEq{quaternion linear system, 1}
\end{theorem}
\begin{proof}
Пользуясь равенством
\ePrints{1003.1544,8433-5163}
\ifx\Semafor\ValueOn
\EqRef{coordinates of map A}
\else%1003.1544,8433-5163
\EqRef{linear map over field, division ring, relation}
\fi%1003.1544,8433-5163
получаем соотношения
\ShowEq{Standard components of linear function, 1, quaternion}

Уравнения
\ShowEq{quaternion linear system ref, 0}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 0}.

Уравнения
\ShowEq{quaternion linear system ref, 1}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 1}.

Уравнения
\ShowEq{quaternion linear system ref, 2}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 2}.

Уравнения
\ShowEq{quaternion linear system ref, 3}
формируют систему линейных уравнений
\EqRef{quaternion linear system, 1, 3}.
\end{proof}

\begin{theorem}
\label{theorem: Quaternion over real field, matrix}
Рассмотрим алгебру кватернионов $H$ с базисом
\EqRef{basis of quaternion}.
Стандартные компоненты линейной функции над полем $F$
и координаты этой функции над полем $F$
удовлетворяют соотношениям
\ShowEq{quaternion, 3}
где
\ShowEq{quaternion, 3, 1}
\end{theorem}
\begin{proof}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
Утверждение теоремы является следствием теорем
\ref{theorem: coordinates of map A1 A2, algebra},
\ref{theorem: Quaternion over real field}.
\else
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 0}
в виде произведения матриц
\ShowEq{quaternion matrix 0}
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 1}
в виде произведения матриц
\ShowEq{quaternion matrix 1}
Из равенства \EqRef{quaternion matrix 1}
следует
\ShowEq{quaternion over real field, 3, 1}
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 2}
в виде произведения матриц
\ShowEq{quaternion matrix 2}
Из равенства \EqRef{quaternion matrix 2}
следует
\ShowEq{quaternion over real field, 3, 2}
Запишем систему линейных уравнений
\EqRef{quaternion linear system, 1, 3}
в виде произведения матриц
\ShowEq{quaternion matrix 3}
Из равенства \EqRef{quaternion matrix 3}
следует
\ShowEq{quaternion over real field, 3, 3}
Мы объединяем равенства
\EqRef{quaternion matrix 0},
\EqRef{quaternion over real field, 3, 1},
\EqRef{quaternion over real field, 3, 2},
\EqRef{quaternion over real field, 3, 3}
в равенстве
\EqRef{quaternion, 3, B->A}.
\fi
\end{proof}

\begin{theorem}
\label{theorem: coordinates of linear function, quaternion}
Стандартные компоненты линейной функции
алгебры кватернионов $H$ относительно базиса
\EqRef{basis of quaternion}
и координаты соответствующего линейного преобразования
удовлетворяют соотношениям
\ShowEq{quaternion over real field}
\end{theorem}
\begin{proof}
Системы линейных уравнений
\EqRef{quaternion over real field, 2, 0},
\EqRef{quaternion over real field, 2, 1},
\EqRef{quaternion over real field, 2, 2},
\EqRef{quaternion over real field, 2, 3}
получены
в результате перемножения матриц в равенстве
\EqRef{quaternion, 3, A->B}.
\end{proof}

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\begin{theorem}
\label{theorem: quaternion conjugation}
Сопряжение кватернионов удовлетворяет равенству
\ShowEq{quaternion conjugation}
\end{theorem}
\begin{proof}
Сопряжение кватернионов является линейным отображением с матрицей
\ShowEq{quaternion conjugation, matrix}
Утверждение теоремы следует из равенства
\EqRef{quaternion, 3, A->B}
и утверждения \eqref{f in L(A,A), 2, associative algebra}
теоремы \ref{theorem: linear map in L(A,A), associative algebra}.
\end{proof}
\fi
\fi%Calculus.Paper

\ePrints{0812.4763,0908.3307}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\Section{Дифференцируемое отображение тела кватернионов}
\label{section: Differentiable Map of Division Ring of Quaternions}
\fi

\begin{theorem}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
Рассмотрим алгебру кватернионов $H$ с базисом
\ShowEq{basis of quaternion}
\fi
Если матрица
$\displaystyle
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi i}}{\partial x^{\gi j}}
\end{pmatrix}
$
является матрица Якоби функции
$
x\rightarrow y
$
тела кватернионов над полем действительных чисел,
то
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ShowEq{quaternion over real field, derivative}
\else
\ShowEq{quaternion over real field, Jacobian matrix}
\fi
\end{theorem}
\begin{proof}
Следствие теоремы
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
\ref{theorem: Standard components of linear function, quaternion}.
\else%0812.4763,0908.3307
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\xRef{8433-5163}{theorem: Quaternion over real field, matrix}.
\else%Calculus.Paper
\ref{theorem: Quaternion over real field, matrix}.
\fi%Calculus.Paper
\fi%0812.4763,0908.3307
\end{proof}

\begin{theorem}
\label{theorem: quaternion conjugation, derivative}
Отображение кватернионов
\[
f(x)=\overline x
\]
имеет производную Гато
\ShowEq{quaternion conjugation, derivative}
\end{theorem}
\begin{proof}
\ePrints{0812.4763,0908.3307}
\ifx\Semafor\ValueOn
Матрица Якоби отображения $f$ имеет вид
\ShowEq{quaternion conjugation, matrix}
Из равенств
\EqRef{quaternion over real field, derivative, 2, 0}
следует
\begin{equation}
\EqLabel{quaternion conjugation, derivative, 1}
\SP 00=
\SP 11=
\SP 22=
\SP 33=
-\frac 12
\end{equation}
Из равенств
\EqRef{quaternion over real field, derivative, 2, 1},
\EqRef{quaternion over real field, derivative, 2, 2},
\EqRef{quaternion over real field, derivative, 2, 3}
следует
\begin{equation}
\EqLabel{quaternion conjugation, derivative, 2}
\SP ij=0
\ \ \ \gi i\ne\gi j
\end{equation}
Равенство
\EqRef{quaternion conjugation, derivative}
следует из равенств
\EqRef{Gateaux derivative, division ring, standard representation},
\EqRef{quaternion conjugation, derivative, 1},
\EqRef{quaternion conjugation, derivative, 2}.
\else
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
Матрица Якоби отображения $f$ имеет вид
\ShowEq{quaternion conjugation, matrix}
Утверждение теоремы следует из равенств
\EqRef{Gateaux derivative, algebra, standard representation},
\EqRef{Jacobian, A->B},\EqRef{quaternion conjugation, matrix}.
\else%Calculus.Paper
Следствие теорем
\ref{theorem: Gateaux derivative of linear map},
\ref{theorem: quaternion conjugation}.
\fi%Calculus.Paper
\fi
\end{proof}

\begin{theorem}
Норма кватерниона удовлетворяет равенствам\footnote{Утверждение
теоремы аналогично примеру X,
\citeBib{Hamilton Elements of Quaternions 1}, с. 455.}
\ShowEq{norm of quaternion, derivative}
\end{theorem}
\begin{proof}
Равенство
\EqRef{norm2 of quaternion, derivative} следует из
\ePrints{0812.4763}
\ifx\Semafor\ValueOff
равенств
\EqRef{Gateaux derivative, fg, algebra},
\EqRef{Gateaux derivative, fx=axb, algebra},
\EqRef{norm of quaternion},
\EqRef{quaternion conjugation, derivative}.
\else
теоремы
\ref{theorem: quaternion conjugation, derivative}
и равенств
\EqRef{norm of quaternion},
\EqRef{Gateaux derivative of product, division ring}.
Так как $\NormX\in R$,
то равенство
\EqRef{norm of quaternion, derivative}
следует из равенства
\EqRef{norm2 of quaternion, derivative}.
\fi
\end{proof}
\fi

\ePrints{0812.4763}
\ifx\Semafor\ValueOn
\begin{theorem}
В теле кватернионов над полем действительных чисел $H$
с базисом
\EqRef{basis of quaternion}
стандартное \Ds представление дифференциала Гато отображения $x^2$
имеет вид
\[
\partial x^2(a)=(x+x_1)a+x_2ai+x_3aj+x_4ak
\]
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: Gateaux Dstar derivative, division ring}.
\end{proof}
\fi

\ePrints{1003.1544,8433-5163}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOff
\begin{theorem}
Мы можем отождествить кватернион
\ShowEq{quaternion a}
и матрицу
\ShowEq{quaternion product ax, Jacobian}
\end{theorem}
\begin{proof}
Произведение кватернионов
\EqRef{quaternion a} и
\ShowEq{quaternion x}
имеет вид
\ShowEq{quaternion product ax}
Следовательно, функция $f_a(x)=ax$ имеет матрицу Якоби
\EqRef{quaternion product ax, Jacobian}.
Очевидно, что $f_a\circ f_b=f_{ab}$. Аналогичное равенство
верно для матриц
\ShowEq{quaternion ab, Jacobian product}
Следовательно, мы можем отождествить кватернион $a$ и матрицу $J_a$.
\end{proof}
\fi


==> Rcd.Basis.Russian.tex <==
%auto-ignore
\input{Rcd.Basis.Eq}
\chapter{Многообразие базисов}
\label{chapter: Basis Manifold}

\section{Линейное представление группы}
\label{section: Linear Representation of Group}

Пусть $V$ - \rcd векторное пространство.
Мы доказали в теореме
\ref{theorem: automorphism of vector space},
что любой автоморфизм \rcd векторного пространства $V$ можно отождествить
с некоторой матрицей.
Мы доказали в теореме
\ref{theorem: Automorphisms of vector space form a group},
что автоморфизмы \rcd векторного пространства порождают группу.
Поэтому, когда мы изучаем представления в \rcd векторном пространстве, нас
интересуют линейные отображения \rcd векторного пространства.

\begin{definition}
Пусть $V$ - \rcd векторное пространство.\footnote{Изучая
представление группы в \rcd векторном пространстве, мы будем следовать соглашению,
описанному в замечании
\ref{remark: left and right matrix notation}.}
Мы будем называть левостороннее представление\footnote{Согласно теореме
\ref{theorem: Automorphisms of vector space form a group},
линейное отображение правого векторного пространства
является левосторонним преобразованием.
}
$f$ группы $G$ в \rcd векторном пространстве $V$
\AddIndex{линейным \Ts{G}представлением}{linear G* representation}.
%если $f(a)$ - автоморфизм \rcd векторного пространства $V$ для любого $a\in G$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: active transformations, vector space}
Автоморфизмы \rcd векторного пространства порождают линейное
эффективное \Ts{\RCGL nD}представление.
\end{theorem}
\begin{proof}
Если даны два автоморфизма $\Vector A$ и $\Vector B$, то мы можем записать
\ShowEq{active transformations, vector space}
Следовательно, результирующий автоморфизм имеет матрицу
\ShowEq{active transformations, vector space, 1}

Нам осталось показать,
что ядро неэффективности состоит только
из единичного элемента. Тождественное преобразование
удовлетворяет равенству
\ShowEq{active transformations, vector space, 2}
Выбирая значения координат в форме
\ShowEq{active transformations, vector space, 3}, где
$k$ задано, мы получим
\ShowEq{identity transformation, vector space}
Из \EqRef{identity transformation, vector space} следует
\ShowEq{identity transformation, vector space, 1}
Поскольку $k$ произвольно, мы приходим к заключению $A=\delta$.
\end{proof}

\begin{theorem}
\label{theorem: representation of linear map relative different bases}
Пусть $\Basis f$, $\Basis g$ - базисы \rcd векторного пространства $\Vector V$.
Пусть $\Basis e$, $\Basis h$ - базисы \rcd векторного пространства $\Vector W$.
Пусть $A_1$ - матрица линейного отображения
\DrawEq{A:V->W}{different bases}
относительно базисов $\Basis f$ и $\Basis e$ и
$A_2$ - матрица линейного отображения
\eqRef{A:V->W}{different bases}
относительно базисов $\Basis g$ и $\Basis h$.
Если базис $\Basis f$ имеет координатную матрицу $B$ относительно
базиса $\Basis g$
\ShowEq{coordinate matrix, f, g}
и $\Basis e$ имеет координатную матрицу $C$ относительно
базиса $\Basis h$
\ShowEq{coordinate matrix, e, h}
то матрицы $A_1$ и $A_2$ связаны соотношением
\ShowEq{representation of rcd linear map relative different bases}
\end{theorem}
\begin{proof}
Вектор $\Vector a\in V$ имеет разложение
\ShowEq{expansion of vector a}
относительно базисов $\Basis f$ и $\Basis g$.
Так как $A$ - линейное отображение, то мы можем записать его в форме
\ShowEq{representation of linear map relative different bases, 1}
относительно базисов $\Basis f$ и $\Basis e$ и
\ShowEq{representation of linear map relative different bases, 2}
относительно базисов $\Basis g$ и $\Basis h$.
В силу теоремы
\ref{theorem: coordinate matrix of basis}
матрица $C$ имеет \RC обратную и из равенства
\EqRef{coordinate matrix, e, h} следует
\ShowEq{coordinate matrix, h, e}
Подставив \EqRef{coordinate matrix, h, e} в равенство
\EqRef{representation of linear map relative different bases, 2}, получим
\ShowEq{representation of linear map relative different bases, 3}
В силу теоремы
\ref{theorem: expansion relative basis, vector space}
сравнение равенств
\EqRef{representation of linear map relative different bases, 1}
и \EqRef{representation of linear map relative different bases, 3} даёт
\ShowEq{representation of linear map relative different bases, 4}
Так как вектор $a$ - произвольный вектор, из теоремы
\ref{theorem: active transformations, vector space} и равенства
\EqRef{representation of linear map relative different bases, 4}
следует утверждение теоремы.
\end{proof}

\begin{theorem}
\label{theorem: representation of automorphism relative different bases}
Пусть $\Vector A$ - автоморфизм
\rcd векторного пространства.
Пусть $A_1$ - матрица этого автоморфизма, заданная
относительно базиса $\Basis f$, и
$A_2$ - матрица того же автоморфизма, заданная
относительно базиса $\Basis g$.
Если базис $\Basis f$ имеет координатную матрицу $B$ относительно
базиса $\Basis g$
\ShowEq{coordinate matrix, f, g}
то матрицы $A_1$ и $A_2$ связаны соотношением
\ShowEq{representation of automorphism relative different bases}
\end{theorem}
\begin{proof}
Утверждение следует из теоремы
\ref{theorem: representation of linear map relative different bases},
так как в данном случае $C=B$.
\end{proof}

\section{Многообразие базисов \texorpdfstring{\rcd}{rcd-}векторного пространства}
\label{section: Basis Manifold for Vector Space}

\begin{theorem}
\label{theorem: active transformations, basis, vector space}
Автоморфизм $A$, действуя на каждый вектор базиса в \rcd векторном пространстве,
отображает базис в другой базис.
\end{theorem}
\begin{proof}
Пусть $\Basis e$ - базис в \rcd векторном пространстве $V$.
Согласно теореме
\ref{theorem: automorphism of vector space},
вектор $e_a$ отображается в вектор $e'_a$
\ShowEq{automorphism, vector space, 1}
Если векторы $e'_a$ линейно зависимы,
то в линейной комбинации
\ShowEq{automorphism, vector space, 2}
$\lambda\ne 0$.
Из равенств \EqRef{automorphism, vector space, 1}
и \EqRef{automorphism, vector space, 2} следует, что
\ShowEq{automorphism, vector space, 3}
и $\lambda\ne 0$. Это
противоречит утверждению, что векторы $e_a$ линейно независимы.
Следовательно, векторы $e'_a$ линейно независимы
и порождают базис.
\end{proof}

Таким образом, мы можем распространить
линейное \Ts{\RCGL nD}представление
на множество базисов.
Мы будем называть преобразование этого левостороннего представления
\AddIndex{активным преобразованием}{active transformation, vector space}
потому, что линейное отображение векторного пространства породило это преобразование
(\citeBib{Korn}).
Активное преобразование не является линейным преобразованием, так как
на множестве базисов не определена линейная операция.
Соответственно определению мы будем записывать действие
активного преобразования $A\in \RCGL nD$ на базис $\Basis e$ в форме
\ShowEq{active transformation}
Мы будем называть гомоморфизм группы $G$ в группу $\RCGL nD$
активных преобразований
\AddIndex{активным \sT{G}представлением}{active representation, vector space}.

\begin{theorem}
\label{theorem: active representation is single transitive}
Активное \Ts{\RCGL nD}представление на множестве базисов
однотранзитивно.
\end{theorem}
\begin{proof}
Чтобы доказать теорему, достаточно показать, что для любых двух базисов
определено по крайней мере одно преобразование левостороннего представления
и это преобразование единственно.
Гомоморфизм $A$, действуя на базис $\Basis e$ имеет вид
\ShowEq{homomorphism on rcd basis}
где $g_i$ - координатная матрица вектора $\Vector g_i$
и $e_i$ - координатная матрица вектора $\Vector e_i$
относительно базиса $\Basis h$.
Следовательно, координатная матрица образа базиса равна
\RC произведению координатной матрицы исходного базиса и матрицы автоморфизма
\ShowEq{homomorphism on rcd basis, 1}
В силу теоремы
\ref{theorem: coordinate matrix of basis},
матрицы $g$ и $e$ невырождены. Следовательно, матрица
\ShowEq{homomorphism on rcd basis, 2}
является матрицей автоморфизма, отображающего базис $\Basis e$
в базис $\Basis g$.

Допустим элементы $g_1$, $g_2$ группы $G$ и базис $\Basis e$ таковы, что
\ShowEq{two transformations on basis manifold, 1}
В силу теорем
\ref{theorem: coordinate matrix of basis}
и
\ref{theorem: two products equal}
справедливо равенство $g_1=g_2$.
Отсюда следует утверждение теоремы.
\end{proof}

Если на векторном пространстве $V$ определена дополнительная структура,
не всякое линейное отображение сохраняет свойства заданной структуры.
В этом случае нас интересует подгруппа
$G$ группы $\RCGL nD$, которая порождает
линейные отображения, сохраняющие свойства заданной структуры.
Мы обычно будем называть группу $G$
\AddIndex{группой симметрии}{SymmetryGroup}.
Не нарушая общности, мы будем отождествлять элемент $g$ группы $G$
с соответствующим преобразованием представления
и записывать его действие на вектор $v\in V$
в виде $g\RCstar v$.

Не всякие два базиса могут быть связаны
преобразованием группы симметрии
потому, что не всякое невырожденное линейное преобразование принадлежит
представлению группы $G$. Таким образом, множество базисов
можно представить как объединение орбит группы $G$.

\begin{definition}
\label{definition: basis manifold of vector space}
Мы будем называть орбиту
\ShowEq{basis manifold of vector space}
выбранного базиса $\Basis e$
\AddIndex{многообразием базисов
\ShowEq{basis manifold of rcd vector space}
\rcd векторного пространства}{basis manifold of rcd vector space}
$V$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: representation on basis manifold, vector space}
Активное \Ts{G}представление на многообразии базисов
однотранзитивно.
\end{theorem}
\begin{proof}
Это следствие теоремы
\ref{theorem: active representation is single transitive}
и определения
\ref{definition: basis manifold of vector space}.
\end{proof}

Из теоремы \ref{theorem: representation on basis manifold, vector space} следует,
что многообразие базисов $\mathcal{B}(V,G)$
является однородным пространством группы $G$.
Согласно теореме
\xRef{math.OA-0612137}{theorem: two representations of group},
на многообразии базисов существует
\sT{G}представление, перестановочное с активным.
Как мы видим из замечания \xRef{math.OA-0612137}{remark: one representation of group}
преобразование
\sT{G}представления отличается от активного преобразования
и не может быть сведено к
преобразованию пространства $V$.
Чтобы подчеркнуть различие, это преобразование называется
\AddIndex{пассивным преобразованием}{passive transformation, vector space}
многообразия базисов $\mathcal{B}(\Vector V,G)$,
а \sT{G}представление называется
\AddIndex{пассивным \sT{G}представлением}{passive *G representation}.
Согласно определению мы будем записывать пассивное преобразование базиса $\Basis e$,
порождённое элементом $A\in G$, в форме
\ShowEq{passive transformation}

\begin{remark}
Я привёл примеры пассивных и активных представлений
в таблице \ref{table:Passive and Active Representations}.
\qed
\end{remark}

\begin{table}[h]
\caption{Активное и пассивное представления}
\label{table:Passive and Active Representations}
\begin{tabular}{|c|c|c|c|}
\hline
векторное пространство&группа&активное&пассивное\\
&представления&представление&представление\\
\hline
\rcd векторное пространство&$\RCGL nD$&
левостороннее&правостороннее\\
\hline
\crd векторное пространство&$\CRGL nD$&
левостороннее&правостороннее\\
\hline
\drc векторное пространство &$\RCGL nD$&
правостороннее&левостороннее\\
\hline
\dcr векторное пространство &$\CRGL nD$&
правостороннее&левостороннее\\
\hline
\end{tabular}
\end{table}

Согласно теореме
\xRef{math.OA-0612137}{theorem: single transitive representation of group}
мы можем определить на $\mathcal{B}(V,G)$
две формы координат, определённые на группе $G$.
Так как мы определили два представления группы $G$ на $\mathcal{B}(V,G)$,
то мы для определения координат пользуемся пассивным \sT{G}представлением.
Наш выбор основан на следующей теореме.

\begin{theorem}
\label{theorem: coordinate matrix of basis and passive transformation}
Координатная матрица базиса $\Basis g$ относительно базиса $\Basis e$
\rcd векторного пространства $V$ совпадает с матрицей пассивного преобразования, отображающего
базис $\Basis e$ в базис $\Basis g$.
\end{theorem}
\begin{proof}
Согласно конструкции, изложенной в примере
\ref{example: rcd vector space},
координатная матрица базиса $\Basis g$ относительно базиса $\Basis e$
состоит из \sups строк, являющихся координатными матрицами векторов
$g_i$ относительно базиса $\Basis e$. Следовательно,
\ShowEq{coordinate matrix of basis and passive transformation, 1}
В тоже время пассивное преобразование $A$, связывающее два базиса, имеет вид
\ShowEq{coordinate matrix of basis and passive transformation, 2}
В силу теоремы
\ref{theorem: expansion relative basis, vector space},
\ShowEq{coordinate matrix of basis and passive transformation, 3}
для любого $i$. Это доказывает теорему.
\end{proof}

Координаты представления называются
\AddIndex{стандартными координатами базиса}{standard coordinates of basis}.
Эта точка зрения позволяет определить два типа координат
для элемента $g$ группы $G$. Мы можем либо пользоваться координатами,
определёнными на группе, либо определить координаты как
элементы матрицы соответствующего преобразования.
Первая форма координат более эффективна, когда мы изучаем
свойства группы $G$. Вторая форма координат
содержит избыточную информацию,
но бывает более удобна,
когда мы изучаем представление группы $G$.
Мы будем называть вторую форму координат
\AddIndex{координатами представления}{coordinates of representation, drc vector space}.

\section{Геометрический объект в \texorpdfstring{$\RCstar D$}{Rcd}\Hyph векторном пространстве}
\label{section: Geometric Object of Vector Space}

Активное преобразование изменяет базисы и векторы согласовано
и координаты вектора относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к изменению
координат вектора относительно базиса.

Допустим пассивное преобразование $A\in G$ отображает
базис $\Basis e\in\mathcal{B}(V,G)$
в базис $\Basis e'\in\mathcal{B}(V,G)$
\ShowEq{passive transformation of vector space}
Допустим вектор $v\in V$ имеет разложение
\ShowEq{vector expansion in vector space, basis e}
относительно базиса $\Basis e$ и имеет разложение
\ShowEq{vector expansion in vector space, basis eprim}
относительно базиса $\Basis e'$.
Из \EqRef{passive transformation of vector space}
и \EqRef{vector expansion in vector space, basis eprim} следует, что
\ShowEq{vector expansion in vector space, basis e, 1}
Сравнивая \EqRef{vector expansion in vector space, basis e}
и \EqRef{vector expansion in vector space, basis e, 1} получаем, что
\ShowEq{coordinate transformation in vector space, 1}
Так как $A$ - \RC невырожденная матрица, то
из \EqRef{coordinate transformation in vector space, 1} следует
\ShowEq{coordinate transformation in vector space}
Преобразование координат \EqRef{coordinate transformation in vector space}
не зависит от вектора $\Vector v$ или базиса $\Basis e$, а
определенно исключительно координатами вектора $\Vector v$
относительно базиса $\Basis e$.

\begin{theorem}
\label{theorem: coordinate transformations form representation, vector space}
Преобразования координат \EqRef{coordinate transformation in vector space}
порождают эффективное линейное
\Ts{G}представление, называемое
\AddIndex{координатным представлением в \rcd векторном пространстве}
{coordinate representation, rcd vector space}.
\end{theorem}
\begin{proof}
Допустим мы имеем два последовательных пассивных преобразования
$A$ и $B$. Преобразование координат
\EqRef{coordinate transformation in vector space}
соответствует пассивному преобразованию $A$.
Преобразование координат
\ShowEq{coordinate transformation in vector space, b}
соответствует пассивному преобразованию $B$. Произведение
преобразований координат \EqRef{coordinate transformation in vector space}
и \EqRef{coordinate transformation in vector space, b} имеет вид
\ShowEq{coordinate transformation in vector space, ab}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\ShowEq{coordinate transformation in vector space, ab 1}
Это доказывает, что преобразования координат
порождают линейное \Ts{G}представление.

Если координатное преобразование не изменяет векторы $\delta_k$,
то ему соответствует единица группы $G$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
\end{proof}

Предположим,
что отображение группы $G$ в
группу пассивных преобразований
\rcd векторного пространства $N$ согласовано с группой симметрий
\rcd векторного пространства $V$.\footnote{Мы пользуемся одним и тем же
символом типа векторного пространства для векторных пространств $N$
и  $V$. Тем не менее они могут иметь различный тип.}
Это означает, что пассивному преобразованию $a$
\rcd векторного пространства $V$
соответствует пассивное преобразование $A(a)$
\rcd векторного пространства $N$.
\ShowEq{passive transformation of vector space N}
Тогда координатное преобразование в $N$ принимает вид
\ShowEq{coordinate transformation, vector space N}

\begin{definition}
\label{definition: geometric object, coordinate representation, vector space}
Мы будем называть орбиту
\ShowEq{geometric object, coordinate rcd vector space}%
\AddIndex{геометрическим объектом в координатном представлении,
определённом в \rcd векторном пространстве}
{geometric object, coordinate rcd vector space}
$V$.
Для любого базиса
\ShowEq{geometric object 1, coordinate rcd vector space}
соответствующая точка \EqRef{coordinate transformation, vector space N}
орбиты  определяет
\AddIndex{координаты геометрического объекта в координатном \rcd векторном пространстве}
{coordinates of geometric object, coordinate rcd vector space}
относительно базиса $\Basis e'_V$.
\qed
\end{definition}

\begin{definition}
\label{definition: geometric object, vector space}
Мы будем называть орбиту
\ShowEq{geometric object, rcd vector space}%
\AddIndex{геометрическим объектом, определённым в \rcd векторном пространстве}
{geometric object, rcd vector space}
$V$.
Для любого базиса
\ShowEq{geometric object 1, rcd vector space}
соответствующая точка \EqRef{coordinate transformation, vector space N}
орбиты  определяет
\AddIndex{координаты геометрического объекта в \rcd векторном пространстве}
{coordinates of geometric object, rcd vector space}
относительно базиса $\Basis e'_V$
и соответствующий вектор
\ShowEq{geometric object 2, rcd vector space}%
называется
\AddIndex{представителем геометрического объекта в \drc векторном пространстве}
{representative of geometric object, drc vector space}
$V$ в базисе $\Basis e'_V$.
\qed
\end{definition}

Так как геометрический объект - это орбита представления,
то согласно теореме
\xRef{math.OA-0612137}{theorem: proper definition of orbit}
определение геометрического объекта корректно.

Мы будем также говорить, что $\Vector w$ - это
\AddIndex{геометрический объект типа $A$}{geometric object of type A, vector space}

Определение \ref{definition: geometric object, coordinate representation, vector space}
строит геометрический объект в координатном пространстве.
Определение \ref{definition: geometric object, vector space} предполагает,
что мы выбрали базис в векторном пространстве $W$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.

Вопрос как велико разнообразие геометрических объектов
хорошо изучен в случае векторных пространств. Однако он
не столь очевиден в случае \rcd векторных пространств. Как видно из таблицы
\ref{table:Passive and Active Representations}
\drc векторное пространство и \rcd векторное пространство
имеют общую группу симметрии $\RCGL nD$. Это позволяет,
рассматривая пассивное представление в \rcd векторное пространство,
изучать геометрический объект в \drc векторном пространстве.
Можем ли мы одновременно
изучать геометрический объект в \crd пространстве?
На первый взгляд, в силу теоремы
\ref{theorem: CR RC singular matrix}
ответ отрицательный. Однако, равенство
\ref{eq: rcstar transpose}
устанавливает искомое линейное отображение между $\RCGL nD$ и $\CRGL nD$.

\begin{theorem}[принцип инвариантности]
\label{theorem: invariance principle}
\label{index: invariance principle}
Представитель геометрического объекта не зависит от выбора
базиса $\Basis e'_V$.
\end{theorem}
\begin{proof}
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Basis e_V$,
базис
$\Basis e_W$
и координаты геометрического объекта
$w^\alpha$. Соответствующий представитель геометрического
объекта имеет вид
\ShowEq{invariance principle 1}
Предположим базис $\Basis e'_V$ связан с базисом
$\Basis e_V$ пассивным преобразованием
\ShowEq{invariance principle 2}
Согласно построению это порождает пассивное преобразование
\EqRef{passive transformation of vector space N}
и координатное преобразование
\EqRef{coordinate transformation, vector space N}. Соответствующий
представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
\end{proof}

\begin{definition}
\label{definition: sum of geometric objects}
Пусть
\ShowEq{sum of geometric objects, 1}
геометрические объекты одного и того же типа,
определённые в \rcd векторном пространстве $V$.
Геометрический объект
\ShowEq{sum of geometric objects, 2}
называется \AddIndex{суммой
\ShowEq{sum of geometric objects, 3}
геометрических объектов}{sum of geometric objects}
$\Vector w_1$ и $\Vector w_2$.
\qed
\end{definition}

\begin{definition}
\label{definition: product of geometric object and constant}
Пусть
\ShowEq{product of geometric object and constant, 1}
геометрический объект,
определённый в \rcd векторном пространстве $V$.
Геометрический объект
\ShowEq{product of geometric object and constant, 2}
называется \AddIndex{произведением
\ShowEq{product of geometric object and constant, 3}
геометрического объекта $\Vector w_1$ и константы $k\in D$}
{product of geometric object and constant}.
\qed
\end{definition}

\begin{theorem}
Геометрические объекты типа $A$,
определённые в \rcd векторном пространстве $V$,
образуют \rcd векторное пространство.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из непосредственной проверки
свойств векторного пространства.
\end{proof}


==> Rcd.Morphism.Russian.tex <==
%auto-ignore
\input{Rcd.Morphism.Eq}

\section{Линейное отображение \texorpdfstring{$\RCstar D$}{Rcd}\hyph векторных пространств}
\label{section: Linear Map of Vector Spaces}

\begin{definition}
\label{definition: rcs rct linear map of vector spaces}
Пусть $V$ - $\RCstar S$\Hyph векторное пространство.
Пусть $U$ - $\RCstar T$\Hyph векторное пространство.
Мы будем называть морфизм
\ShowEq{S->T V->U}
правых представлений тела
в абелевой группе
\AddIndex{линейным отображением}{linear map}
$\RCstar S$\Hyph векторного пространства $V$
в $\RCstar T$\Hyph векторное пространство $U$.
\qed
\end{definition}

Согласно теореме
\ePrints{4776-3181,4993-2400}
\ifx\Semafor\ValueOn
\xRef{0912.3315}{theorem: decompositions of morphism of representations}
\else
\ref{theorem: decompositions of morphism of representations}
\fi
при изучении линейного отображения
мы можем ограничиться случаем $S=T$.

\begin{definition}
\label{definition: linear map of rcd vector spaces}
Пусть $V$ и
$W$ - \rcd векторные пространства.
Мы будем называть отображение
\DrawEq{A:V->W}{}
\AddIndex{линейным отображением}{linear map}
\rcd векторного пространства,
если\footnote{Выражение
\ShowEq{linear map of rcd vector spaces, product on scalar, 1}
означает выражение
\ShowEq{linear map of rcd vector spaces, product on scalar, 2}
}
\ShowEq{linear map of rcd vector spaces, product on scalar}
для любых
\ShowEq{product on scalar, 1}
\qed
\end{definition}

\begin{theorem}
\label{theorem: linear map of rcd vector space}
Пусть
\ShowEq{rcd vector space Basis f}
базис в \rcd векторном пространстве $V$
и
\ShowEq{rcd vector space Basis e}
базис в \rcd векторном пространстве $U$.
Тогда линейное отображение
\DrawEq{A:V->W}{rcd linear}
\rcd векторных пространств имеет представление
\DrawEq{A:V->W, presentation}{rcd linear}
относительно заданных базисов. Здесь
\begin{itemize}
\item $a$ - координатная матрица вектора
$\Vector a$ относительно базиса $\Basis f$.
\item $b$ - координатная матрица вектора
$$\Vector b=\Vector A(\Vector a)$$ относительно базиса $\Basis e$.
\item $A$ - координатная матрица множества векторов
\ShowEq{Vector A(f)}
относительно базиса $\Basis e$.
Мы будем называть матрицу $A$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
относительно базисов $\Basis f$ и $\Basis e$.
\end{itemize}
\end{theorem}
\begin{proof}
Вектор $\Vector a\in V$ имеет разложение
\ShowEq{rcd linear map, 1}
относительно базиса $\Basis f$.
Вектор $\Vector b\in U$ имеет разложение
\ShowEq{rcd linear map, 2}
относительно базиса $\Basis e$.

Так кaк $\Vector A$ - линейное отображение, то на основании
\EqRef{linear map of rcd vector spaces, product on scalar} следует,
что
\ShowEq{rcd linear map, 3}
\ShowEq{rcd linear map, 3i}
является вектором \rcd векторного пространства $U$ и имеет
разложение
\RcdMap{rcd linear map, 4}
относительно базиса $\Basis e$.
Комбинируя \EqRef{rcd linear map, 3}
и \EqRef{rcd linear map, 4}, мы получаем
\ShowEq{rcd linear map, 5}
\eqRef{A:V->W, presentation}{rcd linear}  следует
из сравнения \EqRef{rcd linear map, 2}
и \EqRef{rcd linear map, 5} и
теоремы \xRef{0701.238}{theorem: expansion relative basis, vector space}.
\end{proof}

На основании теоремы \ref{theorem: linear map of rcd vector space}
мы идентифицируем линейное отображение \eqRef{A:V->W}{rcd linear}
\rcd векторных пространств и
матрицу его представления \eqRef{A:V->W, presentation}{rcd linear}.

\begin{theorem}
\label{theorem: product of linear maps, rcd vector space}
Пусть
\ShowEq{rcd vector space Basis f}
базис в \rcd векторном пространстве $V$,
\ShowEq{rcd vector space Basis e}
базис в \rcd векторном пространстве $U$,
и
\ShowEq{rcd vector space Basis g}
базис в \rcd векторном пространстве $W$.
Предположим, что мы имеем
коммутативную диаграмму отображений
\ShowEq{product of linear maps, rcd vector space}
где линейное отображение $A$ имеет представление
\ShowEq{product of linear maps, rcd, A}
относительно заданных базисов
и линейное отображение $B$ имеет представление
\ShowEq{product of linear maps, rcd, B}
относительно заданных базисов.
Тогда отображение $C$ является линейным и имеет представление
\ShowEq{product of linear maps, rcd, C}
относительно заданных базисов.
\end{theorem}
\begin{proof}
Отображение $C$ является линейным, так как
\ShowEq{product of linear maps, 1, rcd vector space}
Равенство
\EqRef{product of linear maps, rcd, C}
следует из подстановки
\EqRef{product of linear maps, rcd, A}
в \EqRef{product of linear maps, rcd, B}.
\end{proof}

Записывая линейное отображение в форме \RC произведения, мы можем переписать
\EqRef{linear map of rcd vector spaces, product on scalar} в виде
\ShowEq{linear map of rcd vector spaces, product on scalar, image}
Утверждение теоремы
\ref{theorem: product of linear maps, rcd vector space}
мы можем записать в виде
\ShowEq{product of rcd linear maps, vector spaces, image}
Равенства
\EqRef{linear map of rcd vector spaces, product on scalar, image} и
\EqRef{product of rcd linear maps, vector spaces, image}
представляют собой
\AddIndex{закон ассоциативности для линейных отображений \rcd векторных пространств}
{associative law}.
Это позволяет нам писать подобные выражения не пользуясь скобками.

Равенство \eqRef{A:V->W, presentation}{rcd linear}
является координатной записью линейного отображения.
На основе теоремы \ref{theorem: linear map of rcd vector space}
бескоординатная запись также может быть представлена с помощью \RC произведения
\ShowEq{linear map of rcd vector spaces, presentation, 5}
Если подставить равенство
\EqRef{linear map of rcd vector spaces, presentation, 5} в теорему
\ref{theorem: product of linear maps, rcd vector space},
то мы получим цепочку равенств
\ShowEq{rcd linear map, 6}

\ePrints{4993-2400}
\ifx\Semafor\ValueOff
\begin{remark}
\label{remark: drc linear map}
На примере линейных отображений легко видеть
насколько теорема 
\ePrints{4776-3181}
\ifx\Semafor\ValueOn
\xRef{0912.3315}{theorem: decompositions of morphism of representations}
\else
\ref{theorem: decompositions of morphism of representations}
\fi
облегчает наши рассуждения при изучении морфизма представлений
$\Omega$\Hyph алгебры.
Договоримся в рамках этого замечания
теорию линейных отображений называть сокращённой теорией,
а теорию, излагаемую в этом замечании, называть расширенной теорией.

Пусть $V$ - $\RCstar S$\Hyph векторное пространство.
Пусть $U$ - $\RCstar T$\Hyph векторное пространство.
Пусть
\ShowEq{rcs rct linear map of vector spaces, presentation}
линейное отображение
$\RCstar S$\Hyph векторного пространства $V$
в $\RCstar T$\Hyph векторное пространство $U$.
Пусть
\ShowEq{rcd vector space Basis f}
базис в $\RCstar S$\Hyph векторном пространстве $V$
и
\ShowEq{rcd vector space Basis e}
базис в $\RCstar T$\Hyph векторном пространстве $U$.

Из определений
\ref{definition: rcs rct linear map of vector spaces} и
\ref{definition: morphism of representations of F algebra}
следует
\ShowEq{rcs rct linear map of vector spaces, presentation, 1}
\ShowEq{rcd linear map, 3i}
также вектор векторного пространства $U$ и имеет
разложение
\RcdMap{rcs rct linear map of vector spaces, presentation, 2}
относительно базиса $\Basis e$.
Комбинируя \EqRef{rcs rct linear map of vector spaces, presentation, 1}
и \EqRef{rcs rct linear map of vector spaces, presentation, 2}, мы получаем
\ShowEq{rcs rct linear map of vector spaces, presentation, 3}

Пусть $W$ - \rcd векторное пространство.
Пусть
\ShowEq{linear map of rct rcd vector spaces, presentation}
линейное отображение
$\RCstar T$\Hyph векторного пространства $U$
в \rcd векторное пространство $W$.
Пусть
\ShowEq{rcd vector space Basis g}
базис в \rcd  векторном пространстве $W$.
Тогда, согласно
\EqRef{rcs rct linear map of vector spaces, presentation, 3},
произведение 
линейного отображения $(r,\Vector A)$ и
линейного отображения $(p,\Vector B)$
имеет вид
\ShowEq{rcs rct linear map of vector spaces, presentation, 4}
Сопоставление равенств
\EqRef{product of linear maps, rcd, C} и
\EqRef{rcs rct linear map of vector spaces, presentation, 4}
показывает насколько рассширеная теория линейных отображений
сложнее сокращённой теории.

При необходимости мы можем пользоваться рассширеной теорией,
но мы не получим новых результатов по сравнению со случаем
сокращённой теорией. В то же время обилие деталей
делает картину менее ясной и требует постоянного внимания.
\qed
\end{remark}
\fi


==> Ring.Linear.Map.Russian.tex <==
%auto-ignore
\input{Ring.Linear.Map.Eq}

\ifx\PrintBook\undefined
\else
\chapter{Линейное отображение тела}
\label{chapter: Linear map, Division Ring}
\fi

\section{Линейное отображение тела}
\label{section: linear map of division ring}

Согласно замечанию
\xRef{0701.238}{remark: Geometry of Division Ring over Field},
мы рассматриваем тело $D$ как алгебру над полем \FZD.

\begin{definition}
\label{definition: linear map of division ring}
Пусть $D_1$, $D_2$ - тела.
Пусть $F$ - поле такое, что
\ShowEq{field division ring d1 d2}
Линейное отображение
\ShowEq{f d1 d2}
$F$\Hyph векторного пространства $D_1$
в $F$\Hyph векторное пространство $D_2$
называется
\AddIndex{линейным отображением
тела $D_1$ в тело $D_2$}{linear map of division ring}.
\qed
\end{definition} 

Согласно определению \ref{definition: linear map of division ring},
линейное отображение $f$ тела $D_1$ в тело $D_2$
удовлетворяет свойству
\ShowEq{linear map of division ring}

\begin{theorem}
\label{theorem: linear map, division ring, integer}
Пусть отображение
\ShowEq{f d1 d2}
является линейным отображением
тела $D_1$ характеристики $0$ в тело $D_2$ характеристики $0$.
Тогда\footnote{Допустим
\ShowEq{f d1 d2}
является линейным отображением
тела $D_1$ характеристики $2$ в тело $D_2$ характеристики $3$.
Тогда для любого $a\in D_1$, $2a=0$, хотя $2 f(a)\ne 0$.
Следовательно, если мы предположим, что характеристика тела $D_1$ больше
$0$, то мы должны потребовать, чтобы характеристика тела $D_1$
равнялась характеристике тела $D_2$.}
\[
f(nx)=nf(x)
\]
для любого целого $n$.
\end{theorem}
\begin{proof}
Мы докажем теорему индукцией по $n$.
При $n=1$ утверждение очевидно, так как
\[
f(1x)=f(x)=1f(x)
\]
Допустим уравнение справедливо при $n=k$. Тогда
\[
f((k+1)x)=f(kx+x)=f(kx)+f(x)=kf(x)+f(x)=(k+1)f(x)
\]
\end{proof}

\begin{theorem}
\label{theorem: linear map, division ring, rational}
Пусть отображение
\ShowEq{f d1 d2}
является линейным отображением
тела $D_1$ характеристики $0$ в тело $D_2$ характеристики $0$.
Тогда
\[
f(ax)=af(x)
\]
для любого рационального $a$.
\end{theorem}
\begin{proof}
Запишем $a$ в виде $a=\frac pq$.
Положим $y=\frac 1qx$. Тогда
согласно теореме \ref{theorem: linear map, division ring, integer}
\begin{equation}
f(x)=f(qy)=qf(y)=qf\left(\frac 1qx\right)
\EqLabel{additive map, division ring, rational, 1}
\end{equation}
Из равенства \EqRef{additive map, division ring, rational, 1}
следует
\begin{equation}
\frac 1qf(x)=f\left(\frac 1qx\right)
\EqLabel{additive map, division ring, rational, 2}
\end{equation}
Из равенства \EqRef{additive map, division ring, rational, 2}
следует
\[
f\left(\frac pqx\right)=pf\left(\frac 1qx\right)=\frac pqf(x)
\]
\end{proof}

Мы не можем распространить утверждение теоремы
\ref{theorem: linear map, division ring, rational}
на произвольное подполе центра $Z(D)$ тела $D$.

\begin{theorem}
\label{theorem: exists linear map not linear over center, division ring}
Пусть тело $D$ является алгеброй над полем \FZD.
Если $F\ne Z(D)$, то существует линейное отображение
\ShowEq{f D D}
которое нелинейно над полем $Z(D)$.
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно рассмотреть поле
комплексных чисел $C$ так как $C=Z(C)$.
Так как поле комплексных чисел является алгеброй над полем вещественных чисел,
то функция
\[
z\rightarrow \overline z
\]
линейна. Однако равенство
\[
\overline{az}=a\overline z
\]
неверно.
\end{proof}

Из теоремы
\ref{theorem: exists linear map not linear over center, division ring}
возникает вопрос.
Для чего мы рассматриваем линейные отображения над полем $F\ne Z(D)$,
если это приводит к резкому рассширению множества линейных отображений?
Ответом на этот вопрос служит богатый опыт
теории функции комплексного переменного.

\begin{theorem}
\label{theorem: sum of linear maps, division ring}
Пусть отображения
\ShowEq{f d1 d2}
\ShowEq{g d1 d2}
являются линейными отображениями
тела $D_1$ в тело $D_2$.
Тогда отображение $f+g$ также является линейным.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\ShowEq{sum of maps, division ring}
\end{proof}

\begin{theorem}
\label{theorem: linear map times constant, division ring}
Пусть отображение \ShowEq{f d1 d2}
является линейным отображением
тела $D_1$ в тело $D_2$.
Тогда отображения $af$, $fb$, $a$, $b\in R_2$, также являются линейными.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\ShowEq{linear map times constant, division ring}
\end{proof}

\begin{definition}
Обозначим
\ShowEq{set linear maps, division ring}
множество линейных отображений
\ShowEq{f d1 d2}
тела $D_1$ в тело $D_2$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: linear map, division ring, morphism}
Мы можем представить линейное отображение
\ShowEq{f d1 d2}
тела $D_1$ в тело $D_2$ в виде
\ShowEq{linear map, division ring, morphism}
где $(G_{k}, k\in K)$ - множество аддитивных отображений
тела $D_1$ в тело $D_2$.\footnote{Здесь и в дальнейшем
мы будем предполагать
сумму по индексу, который встречается в произведении несколько раз.
Равенство \EqRef{linear map, division ring, morphism}
является рекурсивным определением и есть надежда, что мы можем
его упростить.}
Выражение
\ShowEq{component of linear map, division ring}
в равенстве \EqRef{linear map, division ring, morphism}
называется
\AddIndex{компонентой линейного отображения}{component of linear map} $f$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из теорем
\ref{theorem: sum of linear maps, division ring} и
\ref{theorem: linear map times constant, division ring}.
\end{proof}

Если в теореме
\ref{theorem: linear map, division ring, morphism}
$|K|=1$,
то равенство
\EqRef{linear map, division ring, morphism}
имеет вид
\ShowEq{linear map, division ring, morphism G}
и отображение $f$ называется
\AddIndex{линейным отображением, порождённым отображением}
{linear map generated by map} $G$.
Отображение $G$ мы будем называть
\AddIndex{образующей линейного отображения}
{generator of linear map}.

\begin{theorem}
\label{theorem: linear map based G, standard form, division ring}
Пусть $D_1$, $D_2$ - тела характеристики $0$.
Пусть $F$, $F\subset Z(D_1)$, $F\subset Z(D_2)$, - поле.
Пусть $G$ - линейное отображение.
Пусть $\Basis e$ - базис тела $D_2$ над полем $F$.
\AddIndex{Стандартное представление линейного отображения}
{linear map, standard representation}
\EqRef{linear map, division ring, morphism G}
имеет вид\footnote{Представление линейного отображения тела с помощью
компонент линейного отображения
неоднозначно. Чисто алгебраическими методами мы можем
увеличить либо уменьшить число слагаемых.
Если размерность тела $D_2$ над полем $F$ конечна, то стандартное представление
линейного отображения гарантирует конечность множества
слагаемых в представлении отображения.}
\ShowEq{standard component of linear map}
\ShowEq{linear map, division ring, G, standard representation}
Выражение
$\ShowSymbol{standard component of linear map}{G}$
в равенстве \EqRef{linear map, division ring, G, standard representation}
называется
\AddIndex{стандартной компонентой линейного отображения}
{standard component of linear map} $f$.
\end{theorem}
\begin{proof}
Компоненты линейного отображения $f$
имеют разложение
\ShowEq{linear map, division ring, components extention}
относительно базиса $\Basis e$.
Если мы подставим \EqRef{linear map, division ring, components extention}
в \EqRef{linear map, division ring, morphism G},
мы получим
\ShowEq{linear map, division ring, G, standard representation, 1}
Подставив в равенство \EqRef{linear map, division ring, G, standard representation, 1}
выражение
\ShowEq{linear map, division ring, G, standard representation, 2}
мы получим равенство \EqRef{linear map, division ring, G, standard representation}.
\end{proof}

\begin{theorem}
\label{theorem: linear map, G, coordinates and components, division ring}
Пусть $D_1$, $D_2$ - тела характеристики $0$.
Пусть $F$, $F\subset Z(D_1)$, $F\subset Z(D_2)$, - поле.
Пусть $G$ - линейное отображение.
Пусть $\Basis e_1$ - базис тела $D_1$ над полем $F$.
Пусть $\Basis e_2$ - базис тела $D_2$ над полем $F$.
Пусть
\ShowEq{structural constants, division ring D2}
- структурные константы тела $D_2$.
Тогда линейное отображение
\EqRef{linear map, division ring, morphism G},
порождённое линейным отображением $G$,
можно записать в виде
\ShowEq{linear map, G, coordinates and components, division ring}
\end{theorem}
\begin{proof}
Выберем отображение
\ShowEq{linear map D1 D2 generator}
Согласно теореме \xRef{0701.238}{theorem: linear map of rcd vector space}
линейное отображение $f(a)$ относительно базисов $\Basis e_1$ и
$\Basis e_2$ принимает вид
\EqRef{linear map, G, coordinates and components, division ring}.
Из равенств \EqRef{linear map, division ring, G, standard representation}
и \EqRef{linear map D1 D2 generator}
следует
\ShowEq{division ring, F linear map G, standard representation}
Из равенств \EqRef{linear map, G, coordinates and components, division ring}
и \EqRef{division ring, F linear map G, standard representation}
следует
\ShowEq{linear map, G, coordinates and components, division ring, 1}
Так как векторы $e_{2.\gi r}$ линейно независимы над полем $F$ и величины
$a^{\gik}$ произвольны, то из равенства
\EqRef{linear map, G, coordinates and components, division ring, 1}
следует равенство
\EqRef{linear map, G, coordinates and components, division ring, relation}.
\end{proof}

При рассмотрении отображений
\ShowEq{linear map, division ring}
мы будем полагать $G(x)=x$.

\begin{theorem}
\label{theorem: linear map, division ring, canonical morphism}
Пусть $D$ является телом характеристики $0$.
Линейное отображение
\EqRef{linear map, division ring}
имеет вид
\ShowEq{linear map, division ring, canonical morphism}
\end{theorem}

\begin{theorem}
\label{theorem: linear map, standard form, division ring}
Пусть $D$ - тело характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над полем $F\subset Z(D)$.
Стандартное представление линейного отображения
\EqRef{linear map, division ring, canonical morphism}
тела
имеет вид
\ShowEq{linear map, division ring, standard representation}
\end{theorem}

\begin{theorem}
\label{theorem: linear map over field, division ring}
Пусть $D$ является телом характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над полем $F\subset Z(D)$.
Тогда линейное отображение
\EqRef{linear map, division ring}
можно записать в виде
\ShowEq{linear map over field, division ring}
\end{theorem}

\begin{theorem}
\label{theorem: linear map over field, division ring, determinant}
Рассмотрим матрицу
\ShowEq{linear map over field, division ring, matrix}
строки которой пронумерованы индексом
\ShowEq{linear map over field, division ring, row of matrix}
и столбцы пронумерованы индексом
\ShowEq{linear map over field, division ring, column of matrix}
Если
\ShowEq{linear map over field, division ring, determinant},
то для заданных координат линейного преобразования $f_{\gi i}^{\gi j}$
система линейных уравнений
\EqRef{linear map over field, division ring, relation}
относительно стандартных компонент этого преобразования
$f^{\gi{kr}}$ имеет единственное
решение.
Если
\ShowEq{linear map over field, division ring, determinant=0},
то условием существования решения
системы линейных уравнений
\EqRef{linear map over field, division ring, relation}
является равенство
\ShowEq{linear map over field, division ring, determinant=0, 1}
В этом случае система линейных уравнений
\EqRef{linear map over field, division ring, relation}
имеет бесконечно много решений и существует линейная
зависимость между величинами $f_{\gi i}^{\gi j}$.
\end{theorem}
\begin{proof}
Равенство
\EqRef{linear map, division ring, canonical morphism}
является частным случаем равенства
\EqRef{linear map, division ring, morphism G}
при условии $G(x)=x$.
Теорема
\ref{theorem: linear map, standard form, division ring}
является частным случаем теоремы
\ref{theorem: linear map based G, standard form, division ring}
при условии $G(x)=x$.
Теорема
\ref{theorem: linear map over field, division ring}
является частным случаем теоремы
\ref{theorem: linear map, G, coordinates and components, division ring}
при условии $G(x)=x$.
Утверждение теоремы
\ref{theorem: linear map over field, division ring, determinant}
является следствием
теории линейных уравнений над полем.
\end{proof}

\begin{theorem}
\label{theorem: identity map, division ring}
Стандартные компоненты тождественного отображения имеют вид
\ShowEq{identity map, division ring}
\end{theorem}
\begin{proof}
Равенство
\EqRef{identity map, division ring}
является следствием равенства
\ShowEq{identity map 0, division ring}
Убедимся, что стандартные компоненты
\EqRef{identity map, division ring}
линейного преобразования удовлетворяют уравнению
\ShowEq{identity map 1, division ring}
которое следует из уравнения
\EqRef{linear map over field, division ring, relation}
если $f=\delta$.
Из равенств
\EqRef{identity map, division ring},
\EqRef{identity map 1, division ring}
следует
\ShowEq{identity map 2, division ring}
Равенство
\EqRef{identity map 2, division ring}
верно, так как из равенств
\ShowEq{identity map 3, division ring}
следует
\ShowEq{identity map 4, division ring}
Если
\ShowEq{linear map over field, division ring, determinant},
то решение
\EqRef{identity map, division ring}
единственно.
Если
\ShowEq{linear map over field, division ring, determinant=0},
то система линейных уравнений
\EqRef{identity map 1, division ring}
имеет бесконечно много решений.
Однако нас интересует по крайней мере одно.
\end{proof}

\begin{theorem}
\label{theorem: zero map, division ring}
Если
\ShowEq{linear map over field, division ring, determinant},
то стандартные компоненты нулевого отображения
\ShowEq{zero map, division ring}
определены однозначно и имеют вид
\ShowEq{zero map, division ring, 1}
Если
\ShowEq{linear map over field, division ring, determinant=0},
то множество стандартных компонент нулевого отображения
порождает векторное пространство.
\end{theorem}
\begin{proof}
Теорема верна, поскольку стандартные компоненты $z^{\gi{ij}}$
являются решением однородной системы линейных уравнений
\ShowEq{zero map, division ring, 2}
\end{proof}

\begin{remark}
\label{remark: zero map, division ring}
Рассмотрим равенство
\ShowEq{linear maps a=b, division ring}
Из теоремы \ref{theorem: zero map, division ring}
следует, что только при условии
\ShowEq{linear map over field, division ring, determinant}
из равенства
\EqRef{linear maps a=b, division ring}
следует
\ShowEq{linear maps a=b, 1, division ring}
В противном случае мы должны предполагать равенство
\ShowEq{linear maps a=b, 2, division ring}
%Это означает, что векторы
%\ShowEq{linear maps a=b, 3, division ring}
%линейно зависимы.
Несмотря на это, мы и в случае
\ShowEq{linear map over field, division ring, determinant=0}
будем пользоваться стандартным представлением
так как в общем случае указать множество линейно
независимых векторов - задача достаточно сложная.
Если мы хотим определить операцию над линейными отображениями,
записанными в стандартном представлении,
то также как в случае теоремы
\ref{theorem: identity map, division ring}
мы будем выбирать представитель из множества возможных представлений.
\qed
\end{remark}

\begin{theorem}
Выражение
\ShowEq{fkr is tensor}
является тензором над полем $F$
\ShowEq{fkr is tensor, division ring, transformation}
\end{theorem}
\begin{proof}
$D$\Hyph линейное отображение относительно базиса $\Basis e$
имеет вид
\EqRef{linear map over field, division ring}.
Пусть $\Basis e{}'$ - другой базис. Пусть
\ShowEq{fkr is tensor, division ring, change basis}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e{}'$.
Так как линейное отображение $f$ не меняется, то
\ShowEq{fkr is tensor, division ring, transformation, 1}
Подставим \xEqRef{0701.238}{division ring over field, change basis, 3},
\EqRef{fkr is tensor, division ring, change basis}
в равенство \EqRef{fkr is tensor, division ring, transformation, 1}
\ShowEq{fkr is tensor, division ring, transformation, 2}
Так как векторы $e_{\gi j}$ линейно независимы и
компоненты вектора $x^{\gi i}$ произвольны, то равенство
\EqRef{fkr is tensor, division ring, transformation}
следует
из равенства
\EqRef{fkr is tensor, division ring, transformation, 2}.
Следовательно, выражение
$f_k^r$
является тензором над полем $F$.
\end{proof}

\ePrints{0908.3307}%
\ifx\Semafor\ValueOff%
\begin{definition}
Множество
\ShowEq{kernel of linear map, division ring}
называется
\AddIndex{ядром линейного отображения}{kernel of linear map}
\ShowEq{f d1 d2}
тела $D_1$
в тело $D_2$.
\qed
\end{definition}

\begin{theorem}
Ядро линейного отображения
\ShowEq{f d1 d2}
является подгруппой аддитивной группы тела $D_1$.
\end{theorem}
\begin{proof}
Пусть $a$, $b\in\text{ker}f$. Тогда
\begin{align*}
f(a)&=0
\\
f(b)&=0
\\
f(a+b)=f(a)+f(b)&=0
\end{align*}
Следовательно, $a+b\in\text{ker}f$.
\end{proof}

\begin{definition}
Линейное отображение
\ShowEq{f d1 d2}
тела $D_1$
в тело $D_2$
называется
\AddIndex{вырожденным}{singular linear map},
если
\[\text{ker}f\ne\{0\}\]
\qed
\end{definition}
\fi

\begin{theorem}
\label{theorem: product of linear map, D D D}
Пусть $D$ - тело характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над центром $Z(D)$ тела $D$.
Пусть
\ShowEq{product of additive map, D D D}
линейные отображения тела $D$.
Отображение
\begin{equation}
h(x)=gf(x)=g(f(x))
\EqLabel{D linear map, division ring, h1}
\end{equation}
является линейным отображением
\ShowEq{D linear map, division ring, h2}
где
\ShowEq{D linear map, division ring, h gf}
\end{theorem}
\begin{proof}
Отображение \EqRef{D linear map, division ring, h1}
линейно так как
\ShowEq{product of additive map, D D D, 1}

Если мы подставим
\EqRef{D linear map, division ring, f} и
\EqRef{D linear map, division ring, g} в
\EqRef{D linear map, division ring, h1},
то мы получим
\ShowEq{additive map, division ring, h3}
Сравнивая \EqRef{additive map, division ring, h3}
и \EqRef{D linear map, division ring, h2},
мы получим \EqRef{D linear map, division ring, h gf, 0},
\EqRef{D linear map, division ring, h gf, 1}.

Если мы подставим
\EqRef{D linear map, division ring, standard representation, f} и
\EqRef{D linear map, division ring, standard representation, g} в
\EqRef{D linear map, division ring, h1},
то мы получим
\ShowEq{D linear map, division ring, standard representation, h3}
Сравнивая \EqRef{D linear map, division ring, standard representation, h3}
и \EqRef{D linear map, division ring, standard representation, h2},
мы получим \EqRef{D linear map, division ring, standard representation, h gf}.
\end{proof}

\ePrints{0812.4763}
\ifx\Semafor\ValueOn

\begin{definition}
\label{definition: map projective over commutative ring, ring}
Пусть коммутативное кольцо $P$ является подкольцом центра $Z(R)$ кольца $R$.
Отображение
\[f:R\rightarrow R\]
кольца $R$
называется
\AddIndex{проективным над коммутативным кольцом}
{map projective over commutative ring} $P$, если
\[
f(px)=f(x)
\]
для любого $p\in P$. Множество
\[
Px=\{px:p\in P,x\in R\}
\]
называется
\AddIndex{направлением $x$ над коммутативным кольцом}
{direction over commutative ring}\footnote{Направление
над коммутативным кольцом $P$ является подможеством кольца $R$.
Однако мы будем обозначать направление $Px$ элементом
$x\in R$, когда это не приводит к неоднозначности.
Мы будем говорить о направлении над коммутативным кольцом $Z(R)$,
если мы явно не указываем коммутативное кольцо $P$.} $P$.
\qed
\end{definition}

\begin{example}
\label{example: map projective over commutative ring, ring}
Если отображение $f$
кольца $R$ линейно над коммутативным кольцом $P$,
то отображение
\[
g(x)=x^{-1}f(x)
\]
проективно над коммутативным кольцом $P$.
\qed
\end{example}
\fi

\section{Полилинейное отображение тела}

\begin{definition}
\label{definition: map polylinear over commutative ring, ring}
Пусть $R_1$, ..., $R_n$, $P$ - кольца характеристики $0$.
Пусть $S$ - модуль над кольцом $P$.
Пусть $F$ - коммутативное кольцо, которое для любого $i$ является подкольцом центра
кольца $R_i$.
Отображение
\[
f:R_1\times...\times R_n\rightarrow
S
\]
называется \AddIndex{полилинейным над коммутативным кольцом $F$}
{map polylinear over commutative ring, ring},
если
\ShowEq{map polylinear over commutative ring}
для любого $i$, $1\le i\le n$, и любых $p_i$, $q_i \in R_i$, $b\in F$.
Обозначим
\ShowEq{set polylinear maps, ring}
множество полилинейных отображений
колец
$R_1$, ..., $R_n$
в модуль
$S$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: polylinear map, division ring}
Пусть $D$ - тело характеристики $0$.
Полилинейное отображение
\ShowEq{polylinear map, division ring}
имеет вид
\ShowEq{polylinear map, division ring, canonical morphism}
$\sigma_s$ - перестановка множества переменных
$\{d_1,...,d_n\}$
\ShowEq{transposition of set of variables, division ring}
\end{theorem}
\begin{proof}
Мы докажем утверждение индукцией по $n$.

При $n=1$ доказываемое утверждение является следствием теоремы
\ref{theorem: linear map, division ring, canonical morphism}.
При этом мы можем отождествить\footnote{В представлении
\EqRef{polylinear map, division ring, canonical morphism}
мы будем пользоваться следующими правилами.
\begin{itemize}
\item Если область значений какого-либо индекса - это множество,
состоящее из одного элемента, мы будем опускать соответствующий
индекс.
\item Если $n=1$, то $\sigma_s$ - тождественное преобразование.
Это преобразование можно не указывать в выражении.
\end{itemize}}
\ShowEq{polylinear map, division ring, 1, canonical morphism}

Допустим, что утверждение теоремы справедливо при $n=k-1$.
Тогда отображение
\EqRef{polylinear map, division ring}
можно представить в виде
\ShowEq{polylinear map, induction on n, 1, division ring}
Согласно предположению индукции полилинейное отображение
$h$ имеет вид
\ShowEq{polylinear map, induction on n, 2, division ring}
Согласно построению $h=g(d_k)$.
Следовательно, выражения $h\pC{t}{p}$
являются функциями $d_k$.
Поскольку $g(d_k)$ - линейная функция $d_k$,
то только одно выражение $h\pC{t}{p}$
является линейной функцией переменной $d_k$, и остальные выражения
$\pC{t}{q}h$
не зависят от $d_k$.

Не нарушая общности, положим $p=0$.
Согласно равенству
\EqRef{linear map, division ring, canonical morphism}
для заданного $t$
\ShowEq{polylinear map, induction on n, 3, division ring}
Положим $s=tr$ и определим перестановку $\sigma_s$ согласно правилу
\ShowEq{polylinear map, induction on n, 4, division ring}
Положим
\ShowEq{polylinear map, induction on n, 5, division ring}
Мы доказали шаг индукции.
\end{proof}

\begin{definition}
\begin{sloppypar}
Выражение
\ShowEq{component of polylinear map, division ring}
в равенстве \EqRef{polylinear map, division ring, canonical morphism}
называется \AddIndex{компонентой полилинейного отображения $f$}
{component of polylinear map, division ring}.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: standard representation of polylinear map, division ring}
Пусть $D$ - тело характеристики $0$.
Допустим $\Basis e$
- базис тела $D$ над полем \FZD.
\AddIndex{Стандартное представление полилинейного отображения}
{polylinear map, standard representation} тела
имеет вид
\ShowEq{standard component of polylinear map}
\ShowEq{polylinear map, division ring, standard representation}
Индекс $t$ нумерует всевозможные перестановки
$\sigma_t$ множества переменных
$\{d_1,...,d_n\}$.
Выражение
$\ShowSymbol{standard component of polylinear map}{ring}$
в равенстве \EqRef{polylinear map, division ring, standard representation}
называется \AddIndex{стандартной компонентой полилинейного отображения}
{standard component of polylinear map} $f$.
\end{theorem}
\begin{proof}
Компоненты полилинейного отображения $f$
имеют разложение
\ShowEq{polylinear map, division ring, components extention}
относительно базиса $\Basis e$.
Если мы подставим \EqRef{polylinear map, division ring, components extention}
в \EqRef{polylinear map, division ring, canonical morphism},
мы получим
\ShowEq{polylinear map, division ring, standard representation, 1}
Рассмотрим выражение
\ShowEq{polylinear map, division ring, standard representation, 2}
В правой части подразумевается сумма тех слагаемых с индексом $s$,
для которых перестановка $\sigma_s$ совпадает. Каждая такая сумма
будет иметь уникальный индекс $t$.
Подставив в равенство
\EqRef{polylinear map, division ring, standard representation, 1}
выражение
\EqRef{polylinear map, division ring, standard representation, 2}
мы получим равенство \EqRef{polylinear map, division ring, standard representation}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map over field, division ring}
Пусть $\Basis e$ - базис тела $D$ над полем \FZD.
Полилинейное отображение
\EqRef{polylinear map, division ring}
можно представить в виде $D$-значной формы степени $n$
над полем \FZD\footnote{Теорема доказана по аналогии
с теоремой в \citeBib{Rashevsky}, с. 107, 108}
\ShowEq{polylinear map over field, division ring}
где
\ShowEq{polylinear map over field, coordinates, division ring}
и величины $f_{\gi{i_1...i_n}}$
являются координатами $D$-значного ковариантнго тензора над полем $F$.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: map polylinear over commutative ring, ring}
равенство
\EqRef{polylinear map over field, division ring}
следует из цепочки равенств
\ShowEq{polylinear map over field, 1, division ring}
Пусть $\Basis e'$ - другой базис. Пусть
\ShowEq{polylinear map over field, division ring, change basis}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e'$.
Из равенств \EqRef{polylinear map over field, division ring, change basis}
и \EqRef{polylinear map over field, coordinates, division ring}
следует
\ShowEq{polylinear map over field, division ring, change coordinates}
Из равенства \EqRef{polylinear map over field, division ring, change coordinates}
следует тензорный закон преобразования координат полилинейного отображения.
Из равенства \EqRef{polylinear map over field, division ring, change coordinates}
и теоремы \xRef{0701.238}{theorem: division ring over field, change basis}
следует, что значение отображения $f(a_1,...,a_n)$ не зависит от выбора
базиса.
\end{proof}

Полилинейное отображение
\EqRef{polylinear map, division ring}
\AddIndex{симметрично}
{polylinear map symmetric, division ring}, если
\[
f(d_1,...,d_n)=f(\sigma(d_1),...,\sigma(d_n))
\]
для любой перестановки $\sigma$ множества $\{d_1,...,d_n\}$.

\begin{theorem}
\label{theorem: polylinear map symmetric, division ring}
Если полилинейное отображение $f$ симметрично,
то
\ShowEq{polylinear map symmetric, division ring}
\end{theorem}
\begin{proof}
Равенство
\EqRef{polylinear map symmetric, division ring}
следует из равенства
\ShowEq{polylinear map symmetric, 1, division ring}
\end{proof}

Полилинейное отображение
\EqRef{polylinear map, division ring}
\AddIndex{косо симметрично}{polylinear map skew symmetric}, если
\[
f(d_1,...,d_n)=|\sigma|f(\sigma(d_1),...,\sigma(d_n))
\]
для любой перестановки $\sigma$ множества $\{d_1,...,d_n\}$.
Здесь
\[
|\sigma|=
\left\{
\begin{matrix}
1&\textrm{перестановка }\sigma\textrm{ чётная}
\\
-1&\textrm{перестановка }\sigma\textrm{ нечётная}
\end{matrix}
\right.
\]

\begin{theorem}
\label{theorem: polylinear map skew symmetric, division ring}
Если полилинейное отображение $f$ косо симметрично,
то
\ShowEq{polylinear map skew symmetric, division ring}
\end{theorem}
\begin{proof}
Равенство
\EqRef{polylinear map skew symmetric, division ring}
следует из равенства
\ShowEq{polylinear map skew symmetric, 1, division ring}
\end{proof}

\begin{theorem}
\label{theorem: coordinates of polylinear map, division ring over field}
Координаты полилинейного над полем $F$ отображения
\EqRef{polylinear map, division ring}
и его компоненты относительно базиса $\Basis e$
удовлетворяют равенству
\ShowEq{coordinates of polylinear map, division ring over field}
\end{theorem}
\begin{proof}
В равенстве \EqRef{polylinear map, division ring, standard representation}
положим
\ShowEq{coordinates of polylinear map, 1, division ring over field}
Тогда равенство \EqRef{polylinear map, division ring, standard representation}
примет вид
\ShowEq{polylinear map, division ring, standard representation, 1a}
Из равенства \EqRef{polylinear map over field, division ring}
следует
\ShowEq{polylinear map over field, division ring, 1a}
Равенство
\EqRef{coordinates of polylinear map, division ring over field}
следует из сравнения равенств
\EqRef{polylinear map, division ring, standard representation, 1a}
и
\EqRef{polylinear map over field, division ring}.
Равенство
\EqRef{coordinates of polylinear map, division ring over field, 1}
следует из сравнения равенств
\EqRef{polylinear map, division ring, standard representation, 1a}
и
\EqRef{polylinear map over field, division ring, 1a}.
\end{proof}


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {единичный интервал}%
   {unit interval}%

\SetIndexSpace%A%0
\Symb%
   {минорная матрица}%
   {A from b a}%
\Symb%
   {минорная матрица}%
   {A from columns T}%
\Symb%
   {минорная матрица}%
   {A from rows S}%
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
\Symb%
   {минорная матрица}%
   {A without column a}%
\Symb%
   {минорная матрица}%
   {A without columns T}%
\Symb%
   {минорная матрица}%
   {A without row b}%
\Symb%
   {минорная матрица}%
   {A without rows S}%
\Symb%
   {активное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {активное представление группы $G(\Vector  f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {\crd вектор}%
   {crd vector}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
\Symb%
   {левая дробь}%
   {left fraction}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
\Symb%
   {$A$\Hyph модуль однородных многочленов над $D$\Hyph алгеброй $A$}%
   {module of homogeneous polynomials over algebra}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
\Symb%
   {главный идеал}%
   {principal ideal}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {симплекс}%
   {simplex}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
\Symb%
   {замыкание множества}%
   {closure of set}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {открытый шар}%
   {open ball}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {правая дробь}%
   {right fraction}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
\Symb%
   {тензорное произведение представлений}%
   {tensor product of representations}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
\Symb%
   {структурные константы}%
   {structural constants}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, scalar}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Symb%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {матрица Якоби левого сдвига}%
   {aE, quaternion, Jacobian matrix}%
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис модуля}%
   {basis for module}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Symb%
   {базис $D$\Hyph векторного пространства}%
   {basis, D vector space}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма функционала}%
   {norm of functional}%
\Symb%
   {норма отображения}%
   {norm of map}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
\Symb%
   {норма представления}%
   {norm of representation}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Symb%
   {сумма отображений}%
   {sum of maps}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита эффективного \sT{G}представления}%
   {orbit of effective *G representation}%
\Symb%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%
   {орбита эффективного \Ts{G}представления}%
   {orbit of effective G* representation}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
\Symb%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
\Symb%
   {множество правосторонних преобразований множества $M$}%
   {set of right-side transformations}%
\Symb%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb%
   {пространство орбит эффективного \sT{G}представления}%
   {space of orbits of effective *G representation}%
\Symb%
   {пространство орбит эффективного \Ts{G}представления}%
   {space of orbits of effective G* representation}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита \Ts{G}представления группы}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {пассивное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {passive representation in basis manifold}%
\Symb%
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
\Symb%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%
\Symb%
   {тензорное произведение колец}%
   {tensor product of rings}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {интеграл отображения \(f\)}%
   {integral of map}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Symb%
   {образ базиса $X$ при пассивном преобразовании $S$}%
   {passive transformation of basis, representation}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of left-side representations of Omega1 algebra from category}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb%
   {векторное пространство}%
   {V}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to generating set, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Symb%
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
\Symb%
   {суперпозиция координат эндоморфизма представления $f$ и точки $m$}%
   {superposition of coordinates, representation}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%M%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Symb%
   {степень меры}%
   {power of measure}%
\Symb%
   {произведение мер}%
   {product of measures}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%

\SetIndexSpace%O%1
\Symb%
   {норма операции}%
   {norm of operation}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex


==> Tensor.Russian.tex <==
%auto-ignore
\input{Tensor.Eq}
\ifx\PrintBook\undefined
\else
\chapter{Тензорное произведение}
\label{chapter: Tensor Product}
\fi

\section{Тензорное произведение колец}

\begin{theorem}
\label{theorem: free module with semigroup basis}
Пусть $G$ - полугруппа.
Пусть $M$ - свободный модуль с базисом $G$ над коммутативным кольцом $F$.
Тогда на $M$ определена структура кольца таким образом,
что $F$ является подкольцом центра $Z(M)$ кольца $M$.
\end{theorem}
\begin{proof}
Произвольные векторы $a$, $b$, $c\in M$ имеют единственное разложение
\begin{align*}
a&=a^ig_i
&b&=b^jg_j 
&c&=c^kg_k 
\end{align*}
относительно базиса $G$.
$i\in I$, $j\in J$, $k\in K$, где $I$, $J$, $K$ - конечные множества.
Не нарушая общности, мы можем положить $i$, $j$, $k\in I\cup J\cup K$.

Для $a$ и $b$ определим произведение равенством
\begin{equation}
ab=(a^ib^j)(g_ig_j)
\EqLabel{free module, basis ring, 1}
\end{equation}
Из цепочки равенств
\begin{align*}
(a+b)c&=((a^i+b^i)g_i)(c^jg_j)
\\
&=((a^i+b^i)c^j)(g_ig_j)
\\
&=(a^ic^j+b^ic^j)(g_ig_j)
\\
&=(a^ic^j)(g_ig_j)+(b^ic^j)(g_ig_j)
\\
&=(a^ig_i)(c^jg_j)+(b^ig_i)(c^jg_j)
\\
&=ac+bc
\end{align*}
следует, что предложенное произведение дистрибутивно справа
по отношению к сложению.
Аналогично доказывается,
что предложенное произведение дистрибутивно слева
по отношению к сложению.
Из цепочки равенств
\begin{align*}
(ab)c&=((a^ig_i)(b^jg_j))(c^kg_k)
\\
&=((a^ib^j)(g_ig_j))(c^kg_k)
\\
&=((a^ib^j)c^k)((g_ig_j)g_k)
\\
&=(a^i(b^jc^k))(g_i(g_jg_k))
\\
&=(a^ig_i)((b^jc^k)(g_jg_k))
\\
&=(a^ig_i)((b^jg_j)(c^kg_k))
\\
&=a(bc)
\end{align*}
следует, что предложенное произведение ассоциативно.

Пусть $e\in G$ - единица полугруппы $G$. Из равенства
\[
ae=(a^ig_i)e=a^i(g_ie)=a^ig_i=a
\]
следует, что $e$ является единицей кольца $M$.

Отображение
\[
f:p\in F\rightarrow pe\in M
\]
является гомоморфным вложением кольца $F$ в кольцо $M$,
откуда следует, что кольцо $F$ содержится в центре $Z(M)$ кольца $M$.
\end{proof}

\ifx\texFuture\Defined
\begin{definition}
Рассмотрим категорию $\mathcal A$, объектами которой
являются отображения множества $S$ в кольцо, содержащее
коммутативное кольцо $F$.
Если $f:S\rightarrow R$ и $f':S\rightarrow R'$ - объекты категории $\mathcal A$,
то под морфизмом из $f$ в $f'$ мы понимаем гомоморфизм $g:R\rightarrow R'$,
для которого диаграмма
\[
\xymatrix{
&R\ar[dd]_g
\\
S\ar[ru]^f\ar[rd]_{f'}
\\
&R'
}
\]
коммутативна.
Универсальный объект называется
%добавить в индекс
\AddIndex{свободным кольцом, определённым множеством $S$ и коммутативным кольцом $F$}
{free ring determined by set and commutative ring}.\footnote{Я определяю
свободное кольцо
по аналогии с определением в \citeBib{Serge Lang}, с. 49.}
\qed
\end{definition}

\begin{theorem}
Свободное кольцо, определённое множеством $S$ и коммутативным кольцом $F$ существует.
Отображение $f$ инъективно и порождает кольцо $R$.
\end{theorem}
\begin{proof}
Согласно предложению 7, \citeBib{Serge Lang}, с. 49,
существует мультипликативная группа $G$ порождённая множеством $S$.
Пусть $M$ - свободный модуль над коммутативным кольцом $F$,
порождённый базисом $G$.
Рассмотрим следующую диаграмму
\[
\xymatrix{
S\ar[r]^k\ar[rd]_{k'}\ar@/^2pc/[rr]^f\ar@/_3pc/[rrd]_f
&G\ar[d]_m\ar[r]^n\ar[dr]^l&M\ar[d]
\\
&G'\ar[r]&N
}
\]
\end{proof}

Пусть $R_1$, ..., $R_n$ -
кольца характеристики $0$.
Пусть $F$ - коммутативное кольцо, являющееся подкольцом центра $Z(R_i)$, $i=1$,...,$n$.\footnote{Такое кольцо
всегда существует. Например, кольцо целых чисел.}
\fi

Пусть $R_1$, ..., $R_n$ -
кольца характеристики $0$.\footnote{Я определяю
тензорное произведение колец
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.}
Пусть $F$ - максимальное коммутативное кольцо, являющееся подкольцом центра $Z(R_i)$
для любого i, $i=1$,...,$n$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
полилинейные над коммутативным кольцом $F$ отображения
\EqParm{category of polylinear maps}{V=R}
%где $S_1$, $S_2$ - кольца характеристики $0$,
%центры которых содержат кольцо $F$.
где $S_1$, $S_2$ - модули над кольцом $F$.
Мы определим морфизм $f\rightarrow g$
как линейное над коммутативным кольцом $F$ отображение $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\EqParm{fg:V1n->W h}{V=R}
Универсальный объект
\ShowEq{tensor product of rings}
категории $\mathcal A$ называется
\AddIndex{тензорным произведением колец $R_1$, ..., $R_n$ над коммутативным кольцом $F$}
{tensor product of rings}.

\begin{theorem}
\label{theorem: tensor product of rings is module}
Тензорное произведение колец существует.
\end{theorem}
\begin{proof}
Пусть $M$ - модуль над кольцом $F$, порождённый
произведением
\EqParm{V1x...xVn}{V=R}
мультипликативных полугрупп колец $R_1$, ..., $R_n$.
Инъекция
\EqParm{i:V1n->M}{V=R}
определена по правилу
\DrawEqParm{map i, tensor product}{d=d}{ring}
и является гомоморфизмом мультипликативной полугруппы
кольца $R_1\times...\times R_n$ на базис модуля $M$.
Следовательно, произведение векторов базиса определено покомпонентно
\begin{equation}
(d_1,...,d_n)(c_1,...,c_n)=(d_1c_1,...,d_nc_n)
\EqLabel{product in basis, ring, tensor product}
\end{equation}
Пусть $N\subset M$ - подмодуль, порождённый элементами вида
\DrawEqParm{kernel, tensor product}{d=d}{ring}
где
\EqParm{kernel where, tensor product}{d=d,V=R}
Пусть
\ShowEq{j:M->M/N}
каноническое отображение на фактормодуль.
Рассмотрим коммутативную диаграмму
\DrawEqParm{diagram top, tensor product}{V=R}{ring}
Поскольку элементы
\eqRefParm{kernel, tensor product}{d=d}{ring}
принадлежат ядру линейного отображения $j$,
то из равенства
\eqRefParm{map i, tensor product}{d=d}{ring}
следует
\DrawEqParm{f, tensor product}{d=d}{ring}
Из равенств
\eqRefParm{f, tensor product}{d=d}{ring}
следует, что отображение $f$ полилинейно над полем $F$.
Поскольку $M$ - модуль с базисом
$R_1\times...\times R_n$, то согласно теореме \citeBib{Serge Lang}-1,
на с. 104
для любого модуля $V$ и любого
полилинейного над $F$ отображения
\EqParm{g:V1n->V}{V=R}
существует единственный гомоморфизм
\ShowEq{k:M->V}
для которого коммутативна следующая диаграмма
\DrawEqParm{diagram bottom, tensor product}{V=R}{ring}
Так как $g$ - полилинейно над $F$, то
\ShowEq{kerk<N}
Согласно утверждению 
на с. \citeBib{Serge Lang}-94
отображение $j$ универсально в категории гомоморфизмов
векторного пространства $M$,
ядро которых содержит $N$.
Следовательно, определён гомоморфизм
\ShowEq{h:M/N->V}
для которого коммутативна диаграмма
\DrawEq{diagram right, tensor product}{ring}
Объединяя диаграммы
\eqRefParm{diagram top, tensor product}{V=R}{ring},
\eqRefParm{diagram bottom, tensor product}{V=R}{ring},
\eqRef{diagram right, tensor product}{ring},
получим коммутативную диаграмму
\EqParm{diagram, tensor product}{V=R}
Так как $\mathrm{Im}f$ порождает $M/N$,
то отображение $h$ однозначно определено.
\end{proof}

Согласно доказательству теоремы
\ref{theorem: tensor product of rings is module}
\EqParm{oxR=M/N}{V=R}
Для $d_i\in R_i$ будем записывать
\DrawEqParm{map j, tensor product}{d=d}{ring}
Из равенств
\eqRefParm{map i, tensor product}{d=d}{ring} и
\eqRefParm{map j, tensor product}{d=d}{ring}
следует
\EqParm{map f, tensor product}{d=d}%Draw{ring}
Равенства
\eqRefParm{f, tensor product}{d=d}{ring}
можно записать в виде
\DrawEqParm{tensors, tensor product}{d=d}{ring}

\begin{theorem}
Тензорное произведение $\oxn R$ колец
$R_1$, ..., $R_n$ характеристики $0$ над кольцом $F$ является кольцом.
\end{theorem}
\begin{proof}
Согласно доказательству теоремы
\ref{theorem: tensor product of rings is module}
базис модуля $M$ над кольцом $F$
является полугруппой.
Согласно теореме
\ref{theorem: free module with semigroup basis}
в модуле $M$ определена структура кольца.
Подмодуль $N$ является двусторонним идеалом кольца $M$.
Каноническое отображение на фактормодуль
\ShowEq{j:M->M/N}
является также каноническим гомоморфизмом в факторкольцо.
Следовательно, в модуле $M/N=R_1\otimes...\otimes R_n$
определена структура кольца.
Из равенства
\EqRef{product in basis, ring, tensor product}
следует
\ShowEq{product of tensors, ring, tensor product}
Из равенства
\eqRefParm{tensors, tensor product}{d=d}{ring},
следует
\begin{align*}
&d_1\otimes...\otimes d_i\otimes...\otimes d_n
\\
=&d_1\otimes...\otimes (d_i+0)\otimes...\otimes d_n
\\
=&d_1\otimes...\otimes d_i\otimes...\otimes d_n
+d_1\otimes...\otimes 0\otimes...\otimes d_n
\end{align*}
Следовательно, мы можем отождествить тензор $d_1\otimes...\otimes 0\otimes...\otimes d_n$
с нулём $0\otimes...\otimes 0$.
В силу условия теоремы произведение равно $0\otimes...\otimes 0$
только, если один из сомножителей равен $0\otimes...\otimes 0$.
Единицей произведения служит тензор $e_1\otimes...\otimes e_n$.
%Справедливо так же равенство
%\[
%(a_1\otimes...\otimes a_n)^{-1}=(a_1)^{-1}\otimes...\otimes (a_n)^{-1}
%\]
\end{proof}

\section{Тензорное произведение тел}
\label{section: Tensor Product of Division Rings}

Пусть $D_1$, ..., $D_n$ -
тела характеристики $0$.
Пусть $F$ - поле, являющееся подкольцом центра $Z(D_i)$
для любого i, $i=1$,...,$n$.
Тензор
\[a_1\otimes...\otimes a_n\in D_1\otimes...\otimes D_n\]
имеет обратный
\[
(a_1\otimes...\otimes a_n)^{-1}=(a_1)^{-1}\otimes...\otimes (a_n)^{-1}
\]
Однако \AddIndex{тензорное произведение
\ShowEq{tensor product of division rings}
тел $D_1$, ..., $D_n$}
{tensor product of division rings},
вообще говоря, не является телом,
так как мы не можем сказать,
является ли обратим элемент
\[p(a_1\otimes...\otimes a_n)+q(b_1\otimes...\otimes b_n)\]

\begin{remark}
\label{remark: representation of tensor, ring}
Представление тензора в виде
\ShowEq{tensor representation, ring}
неоднозначно.
Если $r\in F$, то
\[
(d_1 r)
\otimes
d_2
=d_1
\otimes
(rd_2 )
\]
Чисто алгебраическими методами мы можем
увеличить либо уменьшить число слагаемых.
К числу допустимых преобразований относится
\begin{align*}
&d_1
\otimes
d_2
+c_1
\otimes
c_2
\\
=&d_1
\otimes
(d_2-c_2+c_2)
+c_1
\otimes
c_2
\\
=&d_1
\otimes
(d_2-c_2)
+d_1
\otimes
c_2
+c_1
\otimes
c_2
\\
=&d_1
\otimes
(d_2-c_2)
+(d_1
+c_1)
\otimes
c_2
\end{align*}
\qed
\end{remark}

В качестве иллюстрации замечания
\ref{remark: representation of tensor, ring} рассмотрим
следующую теорему.

\begin{theorem}
\label{theorem: singular additive map, division ring}
Если в теле $D$ характеристики $0$ существуют элементы
$a$, $b$, $c$, произведение которых не коммутативно,
то существует нетривиальная запись нулевого тензора.%
\ePrints{0812.4763}%
\ifx\Semafor\ValueOn%
\footnote{Утверждение теоремы \ref{theorem: singular additive map, division ring}
и её доказательство тривиальны.
Однако это утверждение важно при изучении аддитивных отображений
расслоенных тел (\citeBib{0702.561}).}
\fi
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочки равенств
\begin{align*}
0\otimes 0=&a\otimes a-a\otimes a+b\otimes b-b\otimes b
\\
=&(a+c)\otimes a-c\otimes a-a\otimes (a-c)-a\otimes c
\\
&+(b-c)\otimes b+c\otimes b-b\otimes (b+c)+b\otimes c
\\
=&(a+c)\otimes a-a\otimes (a-c)+(b-c)\otimes b
\\
&+c\otimes (b-a)-b\otimes (b+c)+(b-a)\otimes c
\end{align*}
\end{proof}

Неоднозначность представления тензора
приводит к тому, что мы должны найти
каноническое представление тензора.
Мы можем найти решение поставленной задачи в случае тензорного произведения тел.
Допустим тело $D_i$ является векторным пространством над
полем $F\subset Z(D_i)$.
Допустим это векторное пространство имеет конечный базис
\ShowEq{finite basis i vector space}
Следовательно, любой элемент $f_i$ тела $D_i$ можно представить в виде
\ShowEq{expansion in basis i vector space}
В этом случае тензор
\EqRef{tensor representation, ring}
можно записать в виде
\ShowEq{tensor canonical representation 1, ring}
где $a^s$, ${}_sf^{s_1}_1\in F$.
Мы можем упростить выражение
\EqRef{tensor canonical representation 1, ring}
\ShowEq{tensor canonical representation 2, ring}
Положим
\ShowEq{tensor canonical representation 3, ring}
Тогда равенство \EqRef{tensor canonical representation 2, ring}
примет вид
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation 4, ring}
Выражение \EqRef{tensor canonical representation 4, ring}
определенно однозначно с точностью до выбора базиса.
Мы будем называть
выражение
$\ShowSymbol{standard component of tensor}{ring}$
\AddIndex{стандартной компонентой тензора}{standard component of tensor}.

\ifx\texFuture\Defined
Положим $D_i=D$
либо $D_i=D^*$, где $D^*$ дуальное тело к телу $D$.
Для определённости положим $D_1=...=D_p=D$, $D_{p+1}=...=D_{p+q}=D^*$, $p+q=n$.
Положим $\Basis d$ - базис тела $D$ над полем $F$ и
$\Basis c$ - дуальный базис.
Определенно \Ts представление группы $GL(F,m)$ в теле $D$.
Определенно \sT представление группы $GL(F,m)$ в теле $D^*$.

Мы распространим представление группы $GL(F,m)$ на представление этой группы
в тензорном произведении $D_1\otimes...\otimes D_m$.
Мы будем следовать построению, выполненному в секции
\xRef{0701.238}{section: Geometric Object of Vector Space}.

\begin{theorem}
\label{theorem: additive map is tensor, division ring}
Компоненты аддитивного отображения тела $D$ характеристики $0$
порождают тензор типа ${}^*D\otimes D^*$.
\end{theorem}
\begin{proof}
Если $a\in F$, то отображения
\[
f(x)=(a\ \pC{s}{0}f)\ x\ \pC{s}{1}f
\]
и
\[
g(x)=\pC{s}{0}f\ x\ (a\ \pC{s}{1}f)
\]
совпадают.
Если даны аддитивные отображения
\[
f_1(x)=\pC{s}{0}f\ x\ \pC{s}{1}f_1
\]
\[
f_2(x)=\pC{s}{0}f\ x\ \pC{s}{1}f_2
\]
то отображение
\[
f(x)=\pC{s}{0}f\ x\ (\pC{s}{1}f_1+\pC{s}{1}f_2)
\]
также является аддитивным.
Закон преобразования компонент тензора следует из теоремы
\ref{theorem: product of linear map, D D D}.
\end{proof}
\fi

\section{Тензорное произведение \texorpdfstring{$D\RCstar$}{Drc}-векторных пространств}

Пусть $D_1$, ..., $D_n$ - тела характеристики $0$.\footnote{Я определяю
тензорное произведение \drc векторных пространств
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.}
Пусть $V_i$ - $D_i\RCstar$\hyph векторное пространство, $i=1$, ..., $n$.
Рассмотрим категорию $\mathcal A$, объектами которой являются
полилинейные отображения
\EqParm{category of polylinear maps}{V=V}
где $W_1$, $W_2$ - \Ds модули над кольцом
$D_1\otimes...\otimes D_n$.
Мы определим морфизм $f\rightarrow g$
как аддитивное отображение
\ShowEq{h:W1->W2}
для которого коммутативна диаграмма
\EqParm{fg:V1n->W h}{V=V}
Универсальный объект
\ShowEq{tensor product of Dstar vector spaces}
категории $\mathcal A$
называется \AddIndex{тензорным произведением \Ds векторных пространств}
{tensor product of Dstar vector spaces}
$V_1$, ..., $V_n$.

\begin{theorem}
\label{theorem: tensor product of Dstar vector spaces}
Тензорное произведение \Ds векторных пространств существует.
\end{theorem}
\begin{proof}
Пусть $F$ - поле, являющееся подкольцом центра $Z(D_i)$
для любого i, $i=1$,...,$n$.

Пусть $D$ - свободное векторное пространство над кольцом $F$, порождённое
произведением $D_1\times...\times D_n$
мультипликативных полугрупп тел $D_1$, ..., $D_n$.
Инъекция
\[
\xymatrix{
i':D_1\times...\times D_n
\ar[r]&D
}
\]
определена по правилу
\begin{equation}
\EqLabel{map iprim, Dstar vector spaces, tensor product}
i'(d_1,...,d_n)=(d_1,...,d_n)
\end{equation}
и является гомоморфизмом мультипликативной полугруппы
кольца $D_1\times...\times D_n$ на базис модуля $D$.
Следовательно, произведение векторов базиса определено покомпонентно
\begin{equation}
(d_1,...,d_n)(c_1,...,c_n)=(d_1c_1,...,d_nc_n)
\EqLabel{product in basis, ring, Dstar vector spaces, tensor product}
\end{equation}
Согласно теореме \ref{theorem: free module with semigroup basis}
на векторном пространстве $D$ определена структура кольца.

Рассмотрим прямое произведение $F\times D$ поля $F$ и кольца $D$.
Мы будем отождествлять элемент $(f,e)$ с элементом $f\in F$ и
элемент $(1,d)$ с элементом $d\in D$.

Пусть $M$ - свободный модуль над кольцом $F\times D$, порождённый
декартовым произведением
\EqParm{V1x...xVn}{V=V}.
Если
\ShowEq{v in V1n}
то соответствующий вектор из $M$ мы будем обозначать
$(v_1,...,v_n)$.
Пусть
\EqParm{i:V1n->M}{V=V}
инъекция, определённая по правилу
\DrawEqParm{map i, tensor product}{d=v}{Dstar vector spaces}
Пусть $N\subset M$ - векторное подпространство, порождённое элементами вида
\DrawEqParm{kernel, tensor product}{d=v}{Dstar vector spaces}
%(a_1,..., a_n)(v_1,...,v_n)-(a_1v_1,...,a_nv_n), $a_i\in D_i$
где
\EqParm{kernel where, tensor product}{d=v,V=V}
Пусть
\ShowEq{j:M->M/N}
каноническое отображение на фактормодуль.
Рассмотрим коммутативную диаграмму
\DrawEqParm{diagram top, tensor product}{V=V}{Dstar vector spaces}
Поскольку элементы
\eqRefParm{kernel, tensor product}{d=v}{Dstar vector spaces}
принадлежат ядру линейного отображения $j$,
то из равенства
\eqRefParm{map i, tensor product}{d=v}{Dstar vector spaces}
следует
\DrawEqParm{f, tensor product}{d=v}{Dstar vector spaces}
Из равенств
\eqRefParm{f, tensor product}{d=v}{Dstar vector spaces}
следует, что отображение $f$ полилинейно над полем $F$.
Поскольку $M$ - модуль с базисом
$V_1\times...\times V_n$, то согласно теореме \citeBib{Serge Lang}-1,
на с. 104
для любого модуля $V$ и любого
полилинейного над $F$ отображения
\EqParm{g:V1n->V}{V=V}
существует единственный гомоморфизм
\ShowEq{k:M->V}
для которого коммутативна следующая диаграмма
\DrawEqParm{diagram bottom, tensor product}{V=V}{Dstar vector spaces}
Так как $g$ - полилинейно над $F$, то
\ShowEq{kerk<N}
Согласно утверждению 
на с. \citeBib{Serge Lang}-94
отображение $j$ универсально в категории гомоморфизмов
модуля $M$,
ядро которых содержит $N$.
Следовательно, определён гомоморфизм
\ShowEq{h:M/N->V}
для которого коммутативна диаграмма
\DrawEq{diagram right, tensor product}{Dstar vector spaces}
Объединяя диаграммы
\eqRefParm{diagram top, tensor product}{V=V}{Dstar vector spaces},
\eqRefParm{diagram bottom, tensor product}{V=V}{Dstar vector spaces},
\eqRef{diagram right, tensor product}{Dstar vector spaces},
получим коммутативную диаграмму
\EqParm{diagram, tensor product}{V=V}
Так как $\mathrm{Im}f$ порождает $M/N$,
то отображение $h$ однозначно определено.
\end{proof}

Согласно доказательству теоремы
\ref{theorem: tensor product of Dstar vector spaces}
\EqParm{oxR=M/N}{V=V}
Для $v_i\in V_i$ будем записывать
\DrawEqParm{map j, tensor product}{d=v}{Dstar vector spaces}
Из равенств
\eqRefParm{map i, tensor product}{d=v}{Dstar vector spaces} и
\eqRefParm{map j, tensor product}{d=v}{Dstar vector spaces}
следует
\EqParm{map f, tensor product}{d=v}%Draw{Dstar vector spaces}
Равенства
\eqRefParm{f, tensor product}{d=v}{Dstar vector spaces},
можно записать в виде
\DrawEqParm{tensors, tensor product}{d=v}{}%{Dstar vector spaces}

\begin{theorem}
\label{theorem: tensor product of Dstar vector spaces, module}
Тензорное произведение $\oxn V$
является модулем над тензорным произведением $\oxn D$.
\end{theorem}
\begin{proof}
Для доказательства утверждения теоремы необходимо доказать, что действие
\ShowEq{(ox d)(ox v)=(d)ox v}
кольца $\oxn D$ на модуле $\oxn V$
определено корректно. Это следует из цепочек равенств
\ShowEq{tensor product of Dstar vector spaces, module}
\end{proof}

\section{Тензорное произведение \texorpdfstring{$D$}{D}-векторных пространств}

Пусть $D_1$, ..., $D_n$ - тела характеристики $0$.\footnote{Я определяю
тензорное произведение $D$\Hyph векторных пространств
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.}
Пусть $V_i$ -
$D_i$\Hyph векторное пространство, $i=1$, ..., $n$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
полилинейные отображения
\EqParm{category of polylinear maps}{V=V}
где $W_1$, $W_2$ - модули над кольцом
$D_1\otimes...\otimes D_n$.
Мы определим морфизм $f\rightarrow g$
как линейное отображение
\ShowEq{h:W1->W2}
для которого коммутативна диаграмма
\EqParm{fg:V1n->W h}{V=V}
Универсальный объект
\ShowEq{tensor product of D vector spaces}
категории $\mathcal A$
называется \AddIndex{тензорным произведением $D$\Hyph векторных пространств}
{tensor product of D vector spaces}
$V_1$, ..., $V_n$.

\begin{theorem}
\label{theorem: tensor product of D vector spaces}
Тензорное произведение $D$\Hyph векторных пространств существует.
\end{theorem}
\begin{proof}
Пусть $F$ - поле, являющееся подкольцом центра $Z(D_i)$
для любого i, $i=1$,...,$n$.

Пусть $D$ - свободное векторное пространство над кольцом $F$, порождённое
произведением $D_1\times...\times D_n$
мультипликативных полугрупп тел $D_1$, ..., $D_n$.
Инъекция
\[
\xymatrix{
i':D_1\times...\times D_n
\ar[r]&D
}
\]
определена по правилу
\begin{equation}
\EqLabel{map iprim, D vector spaces, tensor product}
i'(d_1,...,d_n)=(d_1,...,d_n)
\end{equation}
и является гомоморфизмом мультипликативной полугруппы
кольца $D_1\times...\times D_n$ на базис модуля $D$.
Следовательно, произведение векторов базиса определено покомпонентно
\begin{equation}
(d_1,...,d_n)(c_1,...,c_n)=(d_1c_1,...,d_nc_n)
\EqLabel{product in basis, ring, D vector spaces, tensor product}
\end{equation}
Согласно теореме \ref{theorem: free module with semigroup basis}
на векторном пространстве $D$ определена структура кольца.

Рассмотрим прямое произведение $F\times D$ поля $F$ и кольца $D$.
Мы будем отождествлять элемент $(f,e)$ с элементом $f\in F$ и
элемент $(1,d)$ с элементом $d\in D$.

Пусть $M$ - свободный модуль над кольцом $F\times D$, порождённый
декартовым произведением
\EqParm{V1x...xVn}{V=V}.
Если
\ShowEq{v in V1n}
то соответствующий вектор из $M$ мы будем обозначать
$(v_1,...,v_n)$.
Пусть
\EqParm{i:V1n->M}{V=V}
инъекция, определённая по правилу
\DrawEqParm{map i, tensor product}{d=v}{D vector spaces}
Пусть $N\subset M$ - векторное подпространство, порождённое элементами вида
\DrawEqParm{kernel, tensor product}{d=v}{D vector spaces}
%(a_1,..., a_n)(v_1,...,v_n)-(a_1v_1,...,a_nv_n)
%(v_1,...,\v_n)(a_1,..., a_n)-(v_1a_1,...,v_na_n)
где
\EqParm{kernel where, tensor product}{d=v,V=V}
Пусть
\ShowEq{j:M->M/N}
каноническое отображение на фактормодуль.
Рассмотрим коммутативную диаграмму
\DrawEqParm{diagram top, tensor product}{V=V}{D vector spaces}
Поскольку элементы
\eqRefParm{kernel, tensor product}{d=v}{D vector spaces}
принадлежат ядру линейного отображения $j$,
то из равенства
\eqRefParm{map i, tensor product}{d=v}{D vector spaces}
следует
\DrawEqParm{f, tensor product}{d=v}{D vector spaces}
Из равенств
\eqRefParm{f, tensor product}{d=v}{D vector spaces}
следует, что отображение $f$ полилинейно над полем $F$.
Поскольку $M$ - модуль с базисом
$\xn V$, то согласно теореме \citeBib{Serge Lang}-1,
на с. 104
для любого модуля $V$ и любого
полилинейного над $F$ отображения
\EqParm{g:V1n->V}{V=V}
существует единственный гомоморфизм
\ShowEq{k:M->V}
для которого коммутативна следующая диаграмма
\DrawEqParm{diagram bottom, tensor product}{V=V}{D vector spaces}
Так как $g$ - полилинейно над $F$, то
\ShowEq{kerk<N}
Согласно утверждению 
на с. \citeBib{Serge Lang}-94
отображение $j$ универсально в категории гомоморфизмов
модуля $M$,
ядро которых содержит $N$.
Следовательно, определён гомоморфизм
\ShowEq{h:M/N->V}
для которого коммутативна диаграмма
\DrawEq{diagram right, tensor product}{D vector spaces}
Объединяя диаграммы
\eqRefParm{diagram top, tensor product}{V=V}{D vector spaces},
\eqRefParm{diagram bottom, tensor product}{V=V}{D vector spaces},
\eqRef{diagram right, tensor product}{D vector spaces},
получим коммутативную диаграмму
\EqParm{diagram, tensor product}{V=R}
Так как $\mathrm{Im}f$ порождает $M/N$,
то отображение $h$ однозначно определено.
\end{proof}

Согласно доказательству теоремы
\ref{theorem: tensor product of D vector spaces}
\EqParm{oxR=M/N}{V=V}
Для $v_i\in V_i$ будем записывать
\DrawEqParm{map j, tensor product}{d=v}{D vector spaces}
Из равенств
\eqRefParm{map i, tensor product}{d=v}{D vector spaces} и
\eqRefParm{map j, tensor product}{d=v}{D vector spaces}
следует
\EqParm{map f, tensor product}{d=v}%Draw{D vector spaces}
Равенства
\eqRefParm{f, tensor product}{d=v}{D vector spaces}
можно записать в виде
\DrawEqParm{tensors, tensor product}{d=v}{}%{D vector spaces}

\begin{theorem}
\label{theorem: tensor product of D vector spaces, module}
Тензорное произведение $\oxn V$
является бимодулем над тензорным произведением $\oxn D$.
\end{theorem}
\begin{proof}
Доказательство утверждения теоремы аналогично
доказательству утверждения теоремы \ref{theorem: tensor product of Dstar vector spaces, module}.
\end{proof}


==> Tstar.Representation.Russian.tex <==
%auto-ignore
\input{Tstar.Representation.Eq}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\chapter{Представление универсальной алгебры}
\label{chapter: Representation of Algebra}
\else
\chapter{Представление группы}
\label{chapter: Representation of Group}
\fi

\section{Представление универсальной алгебры}

\begin{definition}
\label{definition: transformation of universal algebra}
\ePrints{0906.0135}
\ifx\Semafor\ValueOn
Пусть\footnote{Определения и теоремы из этой главы
включены также в главы
\xRef{8443-0072}{chapter: Representation of Algebra},
\xRef{8443-0072}{chapter: Basis of Representation of Universal Algebra}.
}
\else
Пусть
\fi
на множестве $M$ определена структура $\Omega_2$\Hyph алгебры
(\citeBib{Burris Sankappanavar,Cohn: Universal Algebra}).
Эндоморфизм
$\Omega_2$\Hyph алгебры
\ShowEq{t:M->M}
называется \AddIndex{преобразованием универсальной алгебры}
{transformation of universal algebra} $M$.\footnote{Если множество
операций $\Omega_2$\Hyph алгебры пусто, то
\ShowEq{t:M->M}
является отображением.}
\qed
\end{definition}

Мы будем обозначать
\symb{\delta}{identical transformation}1
тождественное преобразование.

\begin{definition}
\label{definition: left-side representation of algebra} 
Пусть
\ShowEq{set of left-side transformations}
- множество
\AddIndex{левосторонних преобразований}{left-side transformation}
\[
u'=t u
\]
$\Omega_2$\Hyph алгебры $M$.
Пусть на множестве ${}^*M$ определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{left-side representation of algebra}
$\Omega_1$\Hyph алгебры $A$ в
$\Omega_1$\Hyph алгебру ${}^*M$
называется
\AddIndex{левосторонним представлением $\Omega_1$\Hyph алгебры $A$}
{left-side representation of algebra}
или
\AddIndex{\Ts{A}представлением}{A* representation of algebra}
в $\Omega_2$\Hyph алгебре $M$.
\qed
\end{definition}

\begin{definition}
\label{definition: right-side representation of algebra} 
Пусть
\ShowEq{set of right-side transformations}
- множество
\AddIndex{правосторонних преобразований}{right-side transformation}
\[
u'= ut
\]
$\Omega_2$\Hyph алгебры $M$.
Пусть на множестве $M^*$ определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{right-side representation of algebra}
$\Omega_1$\Hyph алгебры $A$ в
$\Omega_1$\Hyph алгебру $M^*$
называется
\AddIndex{правосторонним представлением $\Omega_1$\Hyph алгебры $A$}
{right-side representation of algebra} или
\AddIndex{\sT{A}представлением}{*A representation of algebra}
в $\Omega_2$\Hyph алгебре $M$.
\qed
\end{definition}

\ePrints{4993-2400}
\ifx\Semafor\ValueOff
Мы распространим на теорию представлений соглашение,
описанное в замечании
\ePrints{0803.2620,0906.0135,0912.3315}
\ifx\Semafor\ValueOn
\xRef{0701.238}{remark: left and right matrix notation}.
\else
\ePrints{0501.237}
\ifx\Semafor\ValueOn
\xRef{0612.111}{remark: left and right matrix notation}.
\else
\ref{remark: left and right matrix notation}.
\fi
\fi
Мы можем записать принцип двойственности в следующей форме
\fi

\begin{theorem}[принцип двойственности]
\label{theorem: duality principle, algebra representation}
Любое утверждение, справедливое для
левостороннего представления $\Omega_1$\Hyph алгебры $A$,
будет справедливо для правостороннего представления $\Omega_1$\Hyph алгебры $A$.
\end{theorem}

\begin{remark}
\label{remark: duality principle, algebra representation}
Существует две формы записи преобразования $\Omega_2$\Hyph алгебры $M$.
Если мы пользуемся операторной записью, то преобразование $A$
записывается в виде $Aa$ или $aA$, что соответствует
левостороннему преобразованию или правостороннему преобразованию.
Если мы пользуемся функциональной записью, то преобразование $A$
записывается в виде $A(a)$ независимо от того, это
левостороннее или правостороннее преобразование.
Эта запись согласована с принципом двойственности.

Это замечание является основой следующего соглашения.
Когда мы пользуемся функциональной записью, мы не различаем
левостороннее и правостороннее преобразование.
Мы будем обозначать
\symb{{}^* M}{set of transformations}1
множество преобразований $\Omega_2$\Hyph алгебры $M$.
Пусть на множестве ${}^* M$ определена структура $\Omega_1$\Hyph алгебры.
Пусть $A$ является $\Omega_1$\Hyph алгеброй.
Мы будем называть гомоморфизм
\begin{equation}
f:A\rightarrow {}^* M
\EqLabel{representation of algebra}
\end{equation}
\AddIndex{представлением $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$}
{representation of algebra}.
Мы будем также пользоваться записью
\ShowEq{representation A in M}
для обозначения представления $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.

Соответствие между операторной записью и функциональной записью однозначно.
Мы можем выбирать любую форму записи, которая удобна для изложения конкретной темы.
\qed
\end{remark}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
Существует несколько способов описать представление.
Мы можем указать отображение $f$, имея в виду что область определения -
это $\Omega_1$\Hyph алгебра $A$ и область значений - это $\Omega_1$\Hyph алгебра ${}^*M$.
Либо мы можем указать $\Omega_1$\Hyph алгебру $A$
и $\Omega_2$\Hyph алгебру $M$, имея в виду что нам известна структура
отображения $f$.\footnote{Например, мы рассматриваем векторное пространство $\Vector V$ над
полем $D$ (
\ePrints{0906.0135}
\ifx\Semafor\ValueOn
определение \xRef{0701.238}{definition: Tstar vector space}
\else
\ePrints{4993-2400,0701.238}
\ifx\Semafor\ValueOff
подраздел \ref{subsection: Vector Space}
\else
definition \ref{definition: Tstar vector space}
\fi
\fi
).
}

Диаграмма
\[
\xymatrix{
M\ar[rr]^{f(a)}&&M\\
&A\ar@{=>}[u]^f&
}
\]
означает, что мы рассматриваем представление $\Omega_1$\Hyph алгебры $A$.
Отображение $f(a)$ является образом $a\in A$.
\fi

\begin{definition}
\label{definition: effective representation of algebra}
Мы будем называть представление $\Omega_1$\Hyph алгебры $A$
\AddIndex{эффективным}{effective representation of algebra},
если отображение \EqRef{representation of algebra} -
изоморфизм $\Omega_1$\Hyph алгебры $A$ в ${}^* M$.
\qed
\end{definition}

\begin{remark}
\label{remark: notation for effective representation of algebra}
Если левостороннее представление $\Omega_1$\Hyph алгебры эффективно, мы можем отождествлять
элемент $\Omega_1$\Hyph алгебры с его образом и записывать левостороннее преобразование,
порождённое элементом $a\in A$,
в форме
\[v'=av\]
Если правостороннее представление $\Omega_1$\Hyph алгебры эффективно, мы можем отождествлять
элемент $\Omega_1$\Hyph алгебры с его образом и записывать правостороннее преобразование,
порождённое элементом $a\in A$,
в форме
\[v'=va\]
\qed
\end{remark}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{definition}
\label{definition: transitive representation of algebra}
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},
если для любых $a, b \in V$ существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и эффективно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
\label{theorem: Representation is single transitive iff}
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in M$
существует одно и только одно $g\in A$ такое, что $a=f(g)(b)$
\end{theorem}
\begin{proof}
Следствие определений \ref{definition: effective representation of algebra}
и \ref{definition: transitive representation of algebra}.
\end{proof}

\section{Морфизм представлений
универсальной алгебры}

\begin{theorem}
Пусть $A$ и $B$ - $\Omega_1$\Hyph алгебры.
Представление $\Omega_1$\Hyph алгебры $B$
\[
g:B\rightarrow {}^\star M
\]
и гомоморфизм $\Omega_1$\Hyph алгебры
\begin{equation}
h:A\rightarrow B
\EqLabel{homomorphism of algebra F}
\end{equation}
определяют представление $f$ $\Omega_1$\Hyph алгебры $A$
\[
\xymatrix{
A\ar[dr]^h\ar[rr]^f&&{}^* M\\
&B\ar[ur]^g&
}
\]
\end{theorem}
\begin{proof}
Отображение $f$ является гомоморфизмом $\Omega_1$\Hyph алгебры $A$ в
$\Omega_1$\Hyph алгебру ${}^* M$,
так как отображение $g$ является гомоморфизмом $\Omega_1$\Hyph алгебры $B$ в
$\Omega_1$\Hyph алгебру ${}^* M$.
\end{proof}

Если мы изучаем представление $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебрах $M$ и $N$, то нас интересуют отображения
из $M$ в $N$, сохраняющие структуру представления.
\fi

\begin{definition}
\label{definition: morphism of representations of F algebra}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$ и 
\ShowEq{g:B->*N}
представление $\Omega_1$\Hyph алгебры $B$
в $\Omega_2$\Hyph алгебре $N$.
Пара отображений
\ShowEq{morphism of representations of F algebra, definition, 1}
таких, что
\begin{itemize}
\item $r$ - гомоморфизм $\Omega_1$\Hyph алгебры
\item $R$ - гомоморфизм $\Omega_2$\Hyph алгебры
\item
\ShowEq{morphism of representations of F algebra, definition, 2}
\end{itemize}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
\qed
\end{definition}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{remark}
Мы можем рассматривать пару отображений $r$, $R$ как отображение
\[
F:A\cup M\rightarrow B\cup N
\] такое, что
\[
F(A)=B \ \ \ \ F(M)=N
\]
Поэтому в дальнейшем мы будем говорить, что дано отображение $(r,R)$.
\qed
\end{remark}

\begin{definition}
Если представления $f$ и $g$ совпадают, то морфизм представлений $(r,R)$ называется
\AddIndex{морфизмом представления $f$}{morphism of representation f}.
\qed
\end{definition}

Для произвольного $m\in M$ равенство
\EqRef{morphism of representations of F algebra, definition, 2}
имеет вид
\ShowEq{morphism of representations of F algebra, definition, 2m}

\ePrints{8443-0072}
\ifx\Semafor\ValueOff
\begin{remark}
Рассмотрим морфизм представлений
\EqRef{morphism of representations of F algebra, definition, 1}.
Мы можем обозначать элементы множества $B$, пользуясь буквой по образцу $b\in B$.
Но если мы хотим показать, что $b$ является образом элемента $a\in A$,
мы будем пользоваться обозначением $\RedText{r(a)}$.
Таким образом, равенство
\[
\RedText{r(a)}=r(a)
\]
означает, что $\RedText{r(a)}$ (в левой части равенства)
является образом $a\in A$ (в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $N$ в виде $\BlueText{R(m)}$.
Мы будем следовать этому соглащению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами, где определены
соответствующие представления.
\qed
\end{remark}
\fi

\begin{remark}
\label{remark: morphism of representations of F algebra}
Мы можем интерпретировать
\EqRef{morphism of representations of F algebra, definition, 2m}
двумя способами
\begin{itemize}
\item Пусть преобразование $\BlueText{f(a)}$ отображает $m\in M$
в $\BlueText{f(a)}(m)$.
Тогда преобразование $g(\RedText{r(a)})$ отображает
$\BlueText{R(m)}\in N$ в $\BlueText{R(f(a)(m))}$.
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\ShowEq{morphism of representations of F algebra, definition, 2m 1}
Из \EqRef{morphism of representations of F algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
\qed
\end{remark}

\begin{theorem}
\label{theorem: morphism of representations and algebra}
Рассмотрим представление
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ 
и представление
\ShowEq{g:B->*N}
$\Omega_1$\Hyph алгебры $B$.
Морфизм
\[
\xymatrix{
h:A\ar[r]&B&H:M\ar[r]&N
}
\]
представлений из $f$ в $g$
удовлетворяет соотношению
\ShowEq{morphism of representations of F algebra, 1}
для произвольной $n$-арной операции $\omega$ $\Omega_1$\Hyph алгебры.
\end{theorem}
\begin{proof}
Так как $f$ - гомоморфизм, мы имеем
\ShowEq{morphism of representations of F algebra, 2}
Из \EqRef{morphism of representations of F algebra, definition, 2} и
\EqRef{morphism of representations of F algebra, 2} следует
\ShowEq{morphism of representations of F algebra, 3}
Так как $h$ - гомоморфизм, из
\EqRef{morphism of representations of F algebra, 3} следует
\ShowEq{morphism of representations of F algebra, 4}
Так как $g$ - гомоморфизм, из
\EqRef{morphism of representations of F algebra, 4} следует
\EqRef{morphism of representations of F algebra, 1}.
\end{proof}

\begin{theorem}
\label{theorem: morphism of representations and homomorphism of algebra}
Пусть отображение
\[
\xymatrix{
h:A\ar[r]&B&H:M\ar[r]&N
}
\]
является морфизмом из представления
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ в представление
\ShowEq{g:B->*N}
$\Omega_1$\Hyph алгебры $B$.
Если представление $f$ эффективно, то отображение
\[
{}^*H:{}^* M\rightarrow{}^* N
\]
определённое равенством
\ShowEq{morphism of representations, star morphism}
является гомоморфизмом $\Omega_1$\Hyph алгебры.
\end{theorem}
\begin{proof}
Так как представление $f$ эффективно, то для выбранного преобразования
$\BlueText{f(a)}$ выбор элемента $a$ определён однозначно.
Следовательно, преобразование $\RedText{g(h(a))}$
в равенстве \EqRef{morphism of representations, star morphism}
определено корректно.

Так как $f$ - гомоморфизм, мы имеем
\begin{equation}
{}^*H(\omega(f(a_1),...,f(a_n)))={}^*H(f(\omega(a_1,...,a_n)))
\EqLabel{morphism of representations, star morphism, 2}
\end{equation}
Из \EqRef{morphism of representations, star morphism} и
\EqRef{morphism of representations, star morphism, 2} следует
\begin{equation}
{}^*H(\omega(f(a_1),...,f(a_n)))=g(h(\omega(a_1,...,a_n)))
\EqLabel{morphism of representations, star morphism, 3}
\end{equation}
Так как $h$ - гомоморфизм, из
\EqRef{morphism of representations, star morphism, 3} следует
\begin{equation}
{}^*H(\omega(f(a_1),...,f(a_n)))=g(\omega(h(a_1),...,h(a_n)))
\EqLabel{morphism of representations, star morphism, 4}
\end{equation}
Так как $g$ - гомоморфизм,
\[
{}^*H(\omega(f(a_1),...,f(a_n)))=\omega(g(h(a_1)),...,g(h(a_n)))
=\omega({}^*H(f(a_1)),...,{}^*H(f(a_n)))
\]
следует из \EqRef{morphism of representations, star morphism, 4}.
Следовательно, отображение ${}^*H$ является гомоморфизмом $\Omega_1$\Hyph алгебры.
\end{proof}

\begin{theorem}
\label{theorem: morphism of representations of F algebra}
Если представление
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ однотранзитивно и представление
\ShowEq{g:B->*N}
$\Omega_1$\Hyph алгебры $B$ однотранзитивно,
то существует морфизм
\ShowEq{morphism representation hH}
представлений из $f$ в $g$.
\end{theorem}
\begin{proof}
Выберем гомоморфизм $h$.
Выберем элемент $m\in M$
и элемент $n\in N$. 
Чтобы построить отображение $H$, рассмотрим следующую диаграмму
\[
\xymatrix{
&M\ar[dd]^(.3)a\ar[rr]^H&&N\ar[dd]_(.3){h(a)}\\
&\ar @{}[rr]|{(1)}&&\\
&M\ar[rr]^H&&N\\
A\ar[rr]^h\ar@{=>}[uur]^(.3)f&&B\ar@{=>}[uur]^(.3)g
}
\]
Из коммутативности диаграммы $(1)$ следует
\[
H(am)=h(a)H(m)
\]
Для произвольного $m'\in M$ однозначно определён $a\in A$ такой,
что $m'=am$. Следовательно, мы построили отображении $H$,
которое удовлетворяет равенству
\EqRef{morphism of representations of F algebra, definition, 2}.
\end{proof}

\begin{theorem}
\label{theorem: unique morphism of representations of F algebra}
Если представление
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ однотранзитивно и представление
\ShowEq{g:B->*N}
$\Omega_1$\Hyph алгебры $B$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\[
\xymatrix{
h:A\ar[r]&B
}
\]
гомоморфизм $\Omega_2$\Hyph алгебры
\[
\xymatrix{
H:M\ar[r]&N
}
\]
такой, что $(h,H)$ является морфизмом
представлений из $f$ в $g$,
определён однозначно
с точностью до выбора образа $n=H(m)\in N$
заданного элемента $m\in M$.
\end{theorem}
\begin{proof}
Из доказательства теоремы
\ref{theorem: morphism of representations of F algebra}
следует, что выбор гомоморфизма $h$ и элементов
$m\in M$, $n\in N$ однозначно определяет отображение $H$.
\end{proof}

\begin{theorem}
Если представление
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ однотранзитивно,
то для любого эндоморфизма $h$ $\Omega_1$\Hyph алгебры $A$ существует морфизм
представления $f$
\ShowEq{morphism representation hH}
\end{theorem}
\begin{proof}
Рассмотрим следующую диаграмму
\ShowEq{morphism representation hH diagram}
Утверждение теоремы является следствием теоремы
\ref{theorem: morphism of representations of F algebra}.
\end{proof}

\begin{theorem}
\label{theorem: product of morphisms of representations of F algebra}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$,
\ShowEq{g:B->*N}
представление $\Omega_1$\Hyph алгебры $B$,
\[
h:C\rightarrow {}^* L
\]
представление $\Omega_1$\Hyph алгебры $C$.
Пусть определены морфизмы представлений $\Omega_1$\Hyph алгебры
\[
\xymatrix{
p:A\ar[r]&B&P:M\ar[r]&N
}
\]
\[
\xymatrix{
q:B\ar[r]&C&Q:N\ar[r]&L
}
\]
Тогда определён морфизм представлений $\Omega_1$\Hyph алгебры
\[
\xymatrix{
r:A\ar[r]&C&R:M\ar[r]&L
}
\]
где $r=qp$, $R=QP$.
Мы будем называть морфизм $(r,R)$ представлений из $f$ в $h$
\AddIndex{произведением морфизмов $(p,P)$ и $(q,Q)$
представлений универсальной алгебры}
{product of morphisms of representations of universal algebra}.
\end{theorem}
\begin{proof}
Мы можем представить утверждение теоремы,
пользуясь диаграммой
\ShowEq{product of morphisms of representations of F algebra}
Отображение $r$ является гомоморфизмом $\Omega_1$\Hyph алгебры $A$ в
$\Omega_1$\Hyph алгебру $C$.
Нам надо показать, что пара отображений $(r,R)$ удовлетворяет
\EqRef{morphism of representations of F algebra, definition, 2}:
\ShowEq{product of morphisms of representations of F algebra, 1}
\end{proof}

\begin{definition}
\label{definition: category of representations of F algebra from category}
Допустим $\mathcal A$ категория $\Omega_1$\Hyph алгебр.
Мы определим \AddIndex{категорию
\symb{\mathcal A*}
{category of left-side representations of Omega1 algebra from category}1
$\ $ левосторонних представлений универсальной алгебры
из категории $\mathcal A$}
{category of left-side representations of Omega1 algebra from category}.
Объектами этой категории являются левосторонние представлениями $\Omega_1$\Hyph алгебры.
Морфизмами этой категории являются морфизмы левосторонних представлений $\Omega_1$\Hyph алгебры.
\qed
\end{definition}

\begin{definition}
\label{definition: transformation coordinated with equivalence}
Пусть на множестве $M$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия
\ShowEq{m1 m2 modS}
следует
$f(m_1)\equiv f(m_2)(\mathrm{mod}\ S)$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: transformation correlated with equivalence}
Пусть на множестве $M$ определена эквивалентность $S$.
Пусть на множестве ${}^* M$ определена $\Omega_1$\Hyph алгебра.
Если любое преобразование $f\in{}^* M$ согласованно с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве ${}^*(M/S)$.
\end{theorem}
\begin{proof}
Пусть $h=\mathrm{nat}\ S$. Если
\ShowEq{m1 m2 modS},
то $h(m_1)=h(m_2)$. Поскольку
$f\in{}^* M$ согласованно с эквивалентностью $S$,
то $h(f(m_1))=h(f(m_2))$. Это позволяет определить
преобразование $F$ согласно правилу
\ShowEq{morphism of representations and equivalence, 0}

Пусть $\omega$ - n\Hyph арная операция $\Omega_1$\Hyph алгебры.
Пусть $f_1$, ..., $f_n\in{}^\star M$ и
\ShowEq{morphism of representations and equivalence}
Согласно условию теоремы, преобразование
\ShowEq{morphism of representations and equivalence, 1}
согласованно с эквивалентностью $S$.
Следовательно, из условия
\ShowEq{m1 m2 modS}
и определения
\ref{definition: transformation coordinated with equivalence}
следует
\ShowEq{morphism of representations and equivalence, 2}
Следовательно, мы можем определить операцию $\omega$ на множестве ${}^\star(M/S)$ по правилу
\ShowEq{morphism of representations and equivalence, 3}
Из определения
\EqRef{morphism of representations and equivalence, 0}
и равенства
\EqRef{morphism of representations and equivalence, 2}
следует, что мы корректно определили
операцию $\omega$ на множестве ${}^\star(M/S)$.
\end{proof}

\begin{theorem}
\label{theorem: decompositions of morphism of representations}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$,
\ShowEq{g:B->*N}
представление $\Omega_1$\Hyph алгебры $B$.
Пусть
\[
\xymatrix{
r:A\ar[r]&B&R:M\ar[r]&N
}
\]
морфизм представлений из $f$ в $g$.
Положим
\begin{align*}
s&=rr^{-1}&S&=RR^{-1}
\end{align*}
Тогда для отображений $r$, $R$ существуют разложения,
которые можно описать диаграммой
\ShowEq{decompositions of morphism of representations, diagram}
\begin{enumerate}
\item $s=\mathrm{ker}\ r$ является конгруэнцией на $A$.
Существует разложение гомоморфизма $r$
\ShowEq{morphism of representations of algebra, homomorphism, 1}
$j=\mathrm{nat}\ s$ - естественный гомоморфизм
\ePrints{8443-0072}
\ifx\Semafor\ValueOff
\ShowEq{morphism of representations of algebra, homomorphism, 2}
\else
\newline
\fi
$t$ - изоморфизм
\ShowEq{morphism of representations of algebra, homomorphism, 3}
$i$ - вложение
\ShowEq{morphism of representations of algebra, homomorphism, 4}
\item $S=\mathrm{ker}\ R$ является эквивалентностью на $M$.
Существует разложение отображения $R$
\begin{equation}
R=ITJ
\EqLabel{morphism of representations of algebra, map, 1}
\end{equation}
$J=\mathrm{nat}\ S$ - сюръекция
\ePrints{8443-0072}
\ifx\Semafor\ValueOff
\ShowEq{morphism of representations of algebra, map, 2}
\else
\newline
\fi
$T$ - биекция
\ShowEq{morphism of representations of algebra, map, 3}
$I$ - вложение
\ShowEq{morphism of representations of algebra, map, 4}
\item $F$ - левостороннее представление $\Omega_1$\Hyph алгебры $A/s$ в $M/S$
\item $G$ - левостороннее представление $\Omega_1$\Hyph алгебры $rA$ в $RM$
\item $(j,J)$ - морфизм представлений $f$ и $F$
\label{theorem: (j,J) is morphism of representations}
\item $(t,T)$ - морфизм представлений $F$ и $G$
\label{theorem: (t,T) is morphism of representations}
\item $(t^{-1},T^{-1})$ - морфизм представлений $G$ и $F$
\label{theorem: (t-1,T-1) is morphism of representations}
\item $(i,I)$ - морфизм представлений $G$ и $g$
\label{theorem: (i,I) is morphism of representations}
\item Существует разложение морфизма представлений
\ShowEq{decompositions of morphism of representations}
\label{theorem: exists decompositions of morphism of representations}
\end{enumerate} 
\end{theorem}
\begin{proof}
Существование диаграмм $(1)$ и $(2)$ следует из теоремы II.3.7
(\citeBib{Cohn: Universal Algebra}, с. 74).
%Существование диаграммы $(2)$ следует из теоремы I.3.1
%(\citeBib{Cohn: Universal Algebra}, с. 28).

Мы начнём с диаграммы $(4)$.

Пусть $m_1\equiv m_2(\mathrm{mod}\ S)$.
%Тогда $J(m_1)=J(m_2)$,
Следовательно,
\ShowEq{morphism of representations of algebra, (4), 1}
%$JT(m_1)=JT(m_2)$,
%так как $JT$ - отображение на $MR$.
Если $a_1\equiv a_2(\mathrm{mod}\ s)$, то
\ShowEq{morphism of representations of algebra, (4), 2}
Следовательно,
$j(a_1)=j(a_2)$.
Так как $(r,R)$ - морфизм представлений, то
\ShowEq{morphism of representations of algebra, (4), 3 4}
Из \EqRef{morphism of representations of algebra, (4), 1},
\EqRef{morphism of representations of algebra, (4), 2},
\EqRef{morphism of representations of algebra, (4), 3},
\EqRef{morphism of representations of algebra, (4), 4}
следует
\ShowEq{morphism of representations of algebra, (4), 5}
Из \EqRef{morphism of representations of algebra, (4), 5}
следует
\begin{equation}
f(a_1)(m_1)\equiv f(a_2)(m_2)(\mathrm{mod}\ S)
\EqLabel{morphism of representations of algebra, (4), 6}
\end{equation}
и, следовательно,
\ShowEq{morphism of representations of algebra, (4), 7}
Из \EqRef{morphism of representations of algebra, (4), 7}
следует, что отображение
\ShowEq{morphism of representations of algebra, (4), 8}
определено корректно и является преобразованием множества $M/S$.

Из равенства
\EqRef{morphism of representations of algebra, (4), 6}
(в случае $a_1=a_2$) следует, что для любого $a$ преобразование
согласованно с эквивалентностью $S$.
Из теоремы
\ref{theorem: transformation correlated with equivalence} следует,
что на множестве ${}^*(M/S)$ определена структура $\Omega_1$\Hyph алгебры.
Рассмотрим $n$\Hyph арную операцию $\omega$ и $n$
преобразований
\ShowEq{transformation correlated with equivalence, 1}
пространства $M/S$. Мы положим
\ShowEq{morphism of representations of algebra, (4), 9}
Следовательно, отображение $F$ является представлением
$\Omega_1$\Hyph алгебры $A/s$.

Из \EqRef{morphism of representations of algebra, (4), 8}
следует, что $(j,J)$ является морфизмом представлений $f$ и $F$
(утверждение \eqref{theorem: (j,J) is morphism of representations}
теоремы).

Рассмотрим диаграмму $(5)$.

Так как $T$ - биекция, то мы можем отождествить элементы множества
$M/S$ и множества $MR$, причём это отождествление имеет вид
\ShowEq{morphism of representations of algebra, (5), 1}
Мы можем записать преобразование $F(\RedText{j(a)})$
множества $M/S$ в виде
\ShowEq{morphism of representations of algebra, (5), 2}
Так как $T$ - биекция, то мы можем определить преобразование
\ShowEq{morphism of representations of algebra, (5), 3}
множества $RM$. Преобразование
\EqRef{morphism of representations of algebra, (5), 3}
зависит от $\RedText{j(a)}\in A/s$.
Так как $t$ - биекция, то мы можем отождествить элементы множества
$A/s$ и множества $rA$, причём это отождествление имеет вид
\ShowEq{morphism of representations of algebra, (5), 6}
Следовательно, мы определили отображение
\[
G:rA\rightarrow{}^\star RM
\]
согласно равенству
\ShowEq{morphism of representations of algebra, (5), 4}

Рассмотрим $n$\Hyph арную операцию $\omega$ и $n$
преобразований
\ShowEq{morphism of representations of algebra, (5), 7}
пространства $RM$. Мы положим
\ShowEq{morphism of representations of algebra, (5), 5}
Согласно \EqRef{morphism of representations of algebra, (5), 4}
операция $\omega$ корректно определена на множестве ${}^\star RM$.
Следовательно, отображение $G$ является представлением
$\Omega_1$\Hyph алгебры.

Из \EqRef{morphism of representations of algebra, (5), 4}
следует, что $(t,T)$ является морфизмом представлений $F$ и $G$
(утверждение \eqref{theorem: (t,T) is morphism of representations}
теоремы).

Так как $T$ - биекция, то из равенства
\EqRef{morphism of representations of algebra, (5), 1}
следует
\ShowEq{morphism of representations of algebra, (5), 1a}
Мы можем записать преобразование $G(\RedText{r(a)})$
множества $RM$ в виде
\ShowEq{morphism of representations of algebra, (5), 2a}
Так как $T$ - биекция, то мы можем определить преобразование
\ShowEq{morphism of representations of algebra, (5), 3a}
множества $M/S$. Преобразование
\EqRef{morphism of representations of algebra, (5), 3a}
зависит от $\RedText{r(a)}\in rA$.
Так как $t$ - биекция, то из равенства
\EqRef{morphism of representations of algebra, (5), 6}
следует
\ShowEq{morphism of representations of algebra, (5), 6a}
Так как по построению диаграмма $(5)$ коммутативна, то преобразование
\EqRef{morphism of representations of algebra, (5), 3a}
совпадает с преобразованием
\EqRef{morphism of representations of algebra, (5), 2}.
Равенство
\EqRef{morphism of representations of algebra, (5), 5}
можно записать в виде
\ShowEq{morphism of representations of algebra, (5), 5a}
Следовательно, $(t^{-1},T^{-1})$ является морфизмом представлений $G$ и $F$
(утверждение \eqref{theorem: (t-1,T-1) is morphism of representations}
теоремы).

Диаграмма $(6)$ является самым простым случаем в нашем доказательстве.
Поскольку отображение $I$ является вложением и диаграмма $(2)$
коммутативна, мы можем отождествить $n\in N$ и $\BlueText{R(m)}$,
если $n\in\textrm{Im}R$. Аналогично, мы можем отождествить
соответствующие преобразования.
\ShowEq{morphism of representations of algebra, (6), 1}
Следовательно,
$(i,I)$ является морфизмом представлений $G$ и $g$
(утверждение \eqref{theorem: (i,I) is morphism of representations}
теоремы).

Для доказательства утверждения
\eqref{theorem: exists decompositions of morphism of representations}
теоремы осталось показать, что определённое
в процессе доказательства представление $g'$ совпадает
с представлением $g$, а операции над преобразованиями совпадают
с соответствующими операциями на ${}^* N$.
\ShowEq{morphism of representations of algebra, (6), 2}
\end{proof}

\begin{definition}
\label{definition: isomorphism of repesentations of Omega algebra}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$,
\ShowEq{g:B->*N}
представление $\Omega_1$\Hyph алгебры $B$.
Пусть
\[
\xymatrix{
r:A\ar[r]&B&R:M\ar[r]&N
}
\]
морфизм представлений из $r$ в $R$ такой, что
$f$ - изоморфизм $\Omega_1$\Hyph алгебры и $g$
- изоморфизм $\Omega_2$\Hyph алгебры.
Тогда отображение $(r,R)$ называется
\AddIndex{изоморфизмом представлений}
{isomorphism of repesentations of Omega algebra}.
\qed
\end{definition}

\begin{theorem}
В разложении
\EqRef{decompositions of morphism of representations}
отображение $(t,T)$ является изоморфизмом представлений $F$ и $G$.
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: isomorphism of repesentations of Omega algebra}
и утверждений \eqref{theorem: (t,T) is morphism of representations}
и \eqref{theorem: (t-1,T-1) is morphism of representations}
теоремы \ref{theorem: decompositions of morphism of representations}.
\end{proof}

Из теоремы \ref{theorem: decompositions of morphism of representations}
следует, что мы можем свести задачу изучения морфизма представлений
$\Omega_1$\Hyph алгебры
к случаю, описываемому диаграммой
\ShowEq{morphism of representations of algebra, reduce, 1}

\begin{theorem}
\label{theorem: morphism of representations of algebra, reduce}
Диаграмма \EqRef{morphism of representations of algebra, reduce, 1}
может быть дополнена представлением $F_1$
$\Omega_1$\Hyph алгебры $A$ в множестве $M/S$ так,
что диаграмма
\ShowEq{morphism of representations of algebra, reduce, 2}
коммутативна. При этом множество преобразований представления $F$ и
множество преобразований представления $F_1$ совпадают.
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно положить
\[F_1(a)=F(\RedText{j(a)})\]
Так как отображение $j$ - сюрьекция, то $\mathrm{Im}F_1=\mathrm{Im}F$.
Так как $j$ и $F$ - гомоморфизмы $\Omega_1$\Hyph алгебры, то $F_1$
- также гомоморфизм $\Omega_1$\Hyph алгебры.
\end{proof}

Теорема \ref{theorem: morphism of representations of algebra, reduce}
завершает цикл теорем, посвящённых структуре морфизма представлений
$\Omega_1$\Hyph алгебры.
Из этих теорем следует, что мы можем упростить задачу изучения морфизма представлений
$\Omega_1$\Hyph алгебры и ограничиться морфизмом представлений вида
\[
\xymatrix{
id:A\ar[r]&A&R:M\ar[r]&N
}
\]
В этом случае мы можем отождествить морфизм $(\id,R)$ представлений
$\Omega_1$\Hyph алгебры и соответствующий гомоморфизм $R$ $\Omega_2$\Hyph алгебры
и пользоваться одной и тойже буквой $R$ для обозначения
этих отображений.
Мы будем пользоваться диаграммой
\ShowEq{morphism id,R of representations}
для представления морфизма $(\id,R)$ представлений
$\Omega_1$\Hyph алгебры.
Из диаграммы следует
\ShowEq{morphism of representations of F algebra}

Мы дадим следующее определение
по аналогии с определением
\ref{definition: category of representations of F algebra from category}.

\begin{definition}
\label{definition: category of left-side representations of Omega1 algebra}
Мы определим \AddIndex{категорию
\symb{A*}{category of left-side representations of Omega1 algebra}1
$\ $ левосторонних представлений $\Omega_1$\Hyph алгебры $A$}
{category of left-side representations of Omega1 algebra}.
Объектами этой категории являются
левосторонними представлениями $\Omega_1$\Hyph алгебры $A$.
Морфизмами этой категории являются морфизмы $(id,R)$
левосторонних представлений $\Omega_1$\Hyph алгебры $A$.
\qed
\end{definition}

\section{Автоморфизм представления универсальной алгебры}

\begin{definition}
\label{definition: endomorphism of representation of F algebra}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Морфизм представлений $\Omega_1$\Hyph алгебры
\ShowEq{morphism of representation of A in M}
такой, что $R$ - эндоморфизм $\Omega_2$\Hyph алгебры
называется
\AddIndex{эндоморфизмом представления}
{endomorphism of representation} $f$.
\qed
\end{definition}

\begin{theorem}
Если представление
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ однотранзитивно,
то для любых $p$, $q\in M$ существует единственный эндоморфизм
\ShowEq{endomorphism representation H}
представления $f$
такой, что $H(p)=q$.
\end{theorem}
\begin{proof}
Рассмотрим следующую диаграмму
\ShowEq{endomorphism representation H diagram}
Существование эндоморфизма является следствием теоремы
\ref{theorem: morphism of representations of F algebra}.
Единственность эндоморфизма для заданных $p$, $q\in M$
является следствием теоремы
\ref{theorem: unique morphism of representations of F algebra},
когда $h=\id$.
\end{proof}

\begin{theorem}
Эндоморфизмы представления $f$ порождают полугруппу.
\end{theorem}
\begin{proof}
Из теоремы
\ref{theorem: product of morphisms of representations of F algebra}
следует, что произведение эндоморфизмов $(p,P)$, $(r,R)$ представления $f$
является эндоморфизмом $(pr,PR)$ представления $f$.
\end{proof}

\begin{definition}
\label{definition: automorphism of representation of F algebra}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Морфизм представлений $\Omega_1$\Hyph алгебры
\ShowEq{morphism of representation of A in M}
такой, что $R$ - автоморфизм $\Omega_2$\Hyph алгебры
называется
\AddIndex{автоморфизмом представления}
{automorphism of representation} $f$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: group of automorphisms of representation}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Множество автоморфизмов представления $f$
порождает \AddIndex{группу}{group of automorphisms of representation}
\ShowEq{group of automorphisms of representation}.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{automorphisms R P}
- автоморфизмы представления $f$.
Согласно определению
\ref{definition: automorphism of representation of F algebra},
отображения $R$, $P$
являются автоморфизмами
$\Omega_2$\Hyph алгебры $M$.
Согласно теореме II.3.2,
(\citeBib{Cohn: Universal Algebra}, c. 60),
отображение $R\circ P$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$.
Из теоремы
\ref{theorem: product of morphisms of representations of F algebra}
и определения
\ref{definition: automorphism of representation of F algebra}
следует, что произведение автоморфизмов
$R\circ P$ представления $f$ является автоморфизмом представления $f$.

Пусть
\ShowEq{automorphisms R P Q}
- автоморфизмы представления $f$.
Из цепочки равенств
\ShowEq{associativity of product of automorphisms of representation}
следует ассоциативность произведения для отображений $R$, $P$, $Q$.\footnote{При
доказательстве ассоциативности произведения
я следую примеру полугруппы
из \citeBib{Kurosh: General Algebra}, с. 20, 21.}

Пусть $R$ - автоморфизм представления $f$.
Согласно определению
\ref{definition: automorphism of representation of F algebra}
отображение $R$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$.
Следовательно, отображение $R^{-1}$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$.
Для автоморфизма $R$ представления справедливо равенство
\EqRef{morphism of representations of F algebra, definition, 2m}.
Положим $m'=R(m)$. Так как $R$ - автоморфизм $\Omega_2$\Hyph алгебры,
то $m=R^{-1}(m')$
и равенство
\EqRef{morphism of representations of F algebra, definition, 2m}
можно записать в виде
\ShowEq{morphism of representations of F algebra, definition, 2m-1}
Так как отображение $R$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$,
то из равенства
\EqRef{morphism of representations of F algebra, definition, 2m-1}
следует
\ShowEq{morphism of representations of F algebra, definition, 2m-1, 1}
Равенство
\EqRef{morphism of representations of F algebra, definition, 2m-1, 1}
соответствует равенству
\EqRef{morphism of representations of F algebra, definition, 2m}
для отображения $R^{-1}$.
Следовательно, отображение $R^{-1}$ является автоморфизмом
представления $f$.
\end{proof}

\ePrints{4993-2400,0701.238}
\ifx\Semafor\ValueOff
\section{Примеры представления универсальной алгебры}

\subsection{Векторное пространство}
\label{subsection: Vector Space}
Согласно определениям
\ref{definition: vector space 1},
\ref{definition: vector space 2},
эффективное представление поля $D$ в абелевой группе
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или \AddIndex{$D$\Hyph векторным пространством}{D-vector space}.
Аналогично эффективное представление ассоциативного кольца $R$
в абелевой группе называется \AddIndex{модулем над кольцом}{module over ring} $R$
или \AddIndex{$R$\Hyph модулем}{R- module}.

\subsection{Представление группы на множестве}
\label{subsection: representation of group on the set}
Пусть $G$ - абелевая группа, и $M$ - множество.
Рассмотрим эфективное представление группы $G$ на множестве $M$.
Для заданных $a\in G$, $A\in M$ положим
$A\rightarrow A+a$.
Мы будем также пользоваться
записью $a=\overset{\rightarrow}{AB}$, если
\ShowEq{representation of group on the set, 1}
Тогда действие группы можно представить в виде
\ShowEq{representation of group on the set, 2}
Поскольку представление эффективно, то из равенств
\EqRef{representation of group on the set, 1},
\EqRef{representation of group on the set, 2}
и равенства
\ShowEq{representation of group on the set, 3}
следует, что
\ShowEq{representation of group on the set, 4}
\fi
\else %4776-3181

Я рассматриваю
представление универсальной алгебры в книге
\citeBib{0912.3315}.
В этой главе я рассматриваю представление групп.
В главе
\ref{chapter: Vector Space Over Division Ring}
я рассматриваю представление тела в абелевой группе.
\fi


==> Vector.Linear.Map.Russian.tex <==
%auto-ignore
\ifx\PrintBook\undefined
\else
\chapter{Линейное отображение \texorpdfstring{$D$}{D}\hyph векторных пространств}
\label{chapter: Linear map, D Vector Space}
\fi

\input{Vector.Linear.Map.Eq}

\section{Линейное отображение
\texorpdfstring{$D$}{D}\hyph векторных пространств}

При изучении линейного отображения $D$\hyph векторных пространств
мы будем рассматривать тело $D$ как конечно мерную алгебру над полем $F$.

\begin{definition}
\label{definition: linear map, vector space}
Пусть поле $F$ является подкольцом центра $Z(D)$ тела $D$.
Пусть $V$ и
$W$ - $D$\Hyph векторные пространства.
Мы будем называть отображение
\ShowEq{map A from V to W, vector space}
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$
\AddIndex{линейным отображением}{linear map},
если
\ShowEq{linear map, vector space}
Обозначим
\ShowEq{set linear maps, D vector space}
множество линейных отображений
\ShowEq{map A from V to W, vector space}
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$.
\qed
\end{definition}

Очевидно, что линейное отображение \drc векторного пространства, так же как
линейное отображение \crd векторного пространства являются линейными отображениями.
Множество морфизмов $D$\Hyph векторного пространства
шире, чем множество морфизмов \drc векторного пространства.
Чтобы рассмотреть линейное отображение векторных пространств,
мы будем следовать методике, предложенной в разделе
\xRef{0701.238}{section: Linear Map of Vector Spaces}.

\begin{theorem}
\label{theorem: partial linear map of variable}
Пусть $D$ - тело характеристики $0$.
Пусть $V$, $W$ - $D$\Hyph векторные пространства.
Линейное отображение
\ShowEq{map A from V to W, vector space}
относительно базиса \eV V
\rcd векторного пространства $V$ и
базиса \eV W
\rcd векторного пространства $W$
имеет вид
\ShowEq{linear map in vector space}
где
\ShowEq{Aij(vi)}
линейно зависит от
одной переменной $v^{\gii}$ и не зависит от остальных
координат вектора $v$.
\end{theorem}
\begin{proof}
Согласно определению \ref{definition: linear map, vector space}
\ShowEq{vector expansion, linear map, D vector space, 1}
Для любого заданного $\gii$ вектор
\ShowEq{vector expansion, linear map, D vector space, 2}
имеет единственное разложение
\ShowEq{vector expansion, linear map, D vector space, 3}
относительно базиса \eV W \rcd векторного пространства.
Подставив \EqRef{vector expansion, linear map, D vector space, 3}
в \EqRef{vector expansion, linear map, D vector space, 1},
мы получим \EqRef{linear map in vector space}.
\end{proof}

\begin{definition}
\label{definition: partial linear map of variable}
Линейное отображение
\ShowEq{partial linear map of variable}
называется
\AddIndex{частным линейным отображением}{partial linear map}
переменной $v^{\gii}$.
\qed
\end{definition}

Мы можем записать линейное отображение в виде произведения матриц
\ShowEq{linear map as product of matrices, 1}
Определим произведение матриц
\ShowEq{linear map as product of matrices, 2}
где $A=\left(A_{\gii}^{\gij}\right)$ - матрица частных линейных отображений.
Используя равенство
\EqRef{linear map as product of matrices, 2},
мы можем записать равенство
\EqRef{linear map as product of matrices, 1}
в виде
\ShowEq{linear map as product of matrices, 3}

\begin{theorem}
\label{theorem: linear map, D vector space}
Пусть $D$ - тело характеристики $0$.
Линейное отображение
\ShowEq{vector expansion, linear map, D vector space}
относительно базиса \eV V
в $D$\Hyph векторном пространстве $V$ и
базиса \eV W
в $D$\Hyph векторном пространстве $W$\footnote{Координатная запись
отображения \EqRef{vector expansion, linear map, D vector space}
зависит от выбора базиса. Равенства изменят свой вид, если например
мы выберем \crd базис $\Basis r_*$ в $D$\Hyph векторном пространстве $W$.}
имеет вид
\ShowEq{linear map, D vector space, canonical morphism}
\end{theorem}
\begin{proof}
Согласно теореме \ref{theorem: partial linear map of variable}
линейное отображение $A(v)$ можно записать в виде
\EqRef{linear map in vector space}.
Так как для заданных индексов $\gii$, $\gij$
частное линейное отображение
\ShowEq{Aij(vi)}
линейно по переменной $v^{\gii}$,
то согласно \EqRef{linear map, division ring, canonical morphism}
выражение
\ShowEq{Aij(vi)}
можно представить в виде
\ShowEq{vector expansion, linear map, D vector space, 2a}
где индекс $s$ нумерует слагаемые.
Множество значений индекса $s$ зависит от индексов $\gii$ и $\gij$.
Комбинируя равенства
\EqRef{vector expansion, linear map, D vector space, 1} и
\EqRef{vector expansion, linear map, D vector space, 2a},
мы получим
\ShowEq{linear map, D vector space, canonical morphism 1}
В равенстве
\EqRef{linear map, D vector space, canonical morphism 1}
мы суммируем также по индексу $\gii$.
Равенство \EqRef{linear map, D vector space, canonical morphism}
следует из сравнения равенств
\EqRef{vector expansion, D vector space W} и
\EqRef{linear map, D vector space, canonical morphism 1}.
\end{proof}

\begin{definition}
\begin{sloppypar}
Выражение
\ShowEq{component of linear map, D vector space}
в равенстве \EqRef{vector expansion, linear map, D vector space, 3}
называется
\AddIndex{компонентой линейного отображения}{component of linear map} $A$.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: product of linear maps, D vector space}
Пусть $D$ - тело характеристики $0$.
Пусть \eV V - базис в $D$\Hyph векторном пространстве $V$,
\eV U - базис в $D$\Hyph векторном пространстве $U$,
и \eV W - базис в $D$\Hyph векторном пространстве $W$.
Предположим, что мы имеем коммутативную диаграмму отображений
\[
\xymatrix{
V\ar[rr]^{C}\ar[dr]^{A} & & W\\
&U\ar[ur]^{B} &
}
\]
где линейное отображение $A$ имеет представление
\ShowEq{product of linear maps, D vector spaces, A}
относительно заданных базисов
и линейное отображение $B$ имеет представление
\ShowEq{product of linear maps, D vector spaces, B}
относительно заданных базисов.
Тогда отображение $C$ линейно и имеет представление
\ShowEq{product of linear maps, D vector spaces, C}
относительно заданных базисов, где\footnote{Индекс
$u$ оказался составным индексом, $u=st$.
Однако не исключено, что некоторые слагаемые в
\EqRef{product of linear maps, D vector spaces}
могут быть объединены вместе.}
\ShowEq{product of linear maps, D vector spaces}
\end{theorem}
\begin{proof}
Отображение $C$ линейно, так как
\ShowEq{product of linear maps, D vector spaces, 1}
Равенство
\EqRef{product of linear maps, D vector spaces, C}
следует из подстановки
\EqRef{product of linear maps, D vector spaces, A}
в \EqRef{product of linear maps, D vector spaces, B}.
\end{proof}

\begin{theorem}
Для линейного отображения $A$ существует
линейное отображение $B$ такое, что
\ShowEq{components of two linear maps, D vector space}
\end{theorem}
\begin{proof}
Отображение $B$ линейно, так как
\ShowEq{components of two linear maps, 1, D vector space}
Согласно равенству \EqRef{linear map, D vector space, canonical morphism}
\ShowEq{components of two linear maps, 2, D vector space}
\end{proof}

\begin{theorem}
\label{theorem: linear map, 0, D vector space}
Пусть $D$ - тело характеристики $0$.
Пусть
\ShowEq{map A from V to W, vector space}
линейное отображение
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$.
Тогда
\ShowEq{A(0)=0}
\end{theorem}
\begin{proof}
Следствие равенства
\ShowEq{A(0)=0 1}
\end{proof}

\begin{definition}
Множество
\ShowEq{kernel of linear map, D vector space}
называется
\AddIndex{ядром линейного отображения}{kernel of linear map}
\ShowEq{map A from V to W, vector space}
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$.
\qed
\end{definition}

\begin{definition}
Линейное отображение
\ShowEq{map A from V to W, vector space}
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$
называется
\AddIndex{вырожденным}{singular linear map},
если
\[\text{ker}A=V\]
\qed
\end{definition}

\section{Полилинейное отображение
\texorpdfstring{$D$}{D}\hyph векторного пространства}

\begin{definition}
Пусть поле $F$ является подкольцом центра $Z(D)$ тела $D$
характеристики $0$.
Пусть $V_1$, ..., $V_n$,
$W_1$, ..., $W_m$
- $D$\Hyph векторные пространства.
Мы будем называть отображение
\ShowEq{polylinear map of D vector spaces}
\AddIndex{полилинейным отображением}{polylinear map}
$\times$\hyph $D$\hyph векторного пространства
$V_1\times...\times V_n$
в $\times$\hyph $D$\hyph векторное пространство
$W_1\times...\times W_m$,
если
\ShowEq{polylinear map of D vector spaces, 1}
\qed
\end{definition}

\begin{definition}
Обозначим
\ShowEq{set polylinear maps, D vector space}
множество полилинейных отображений
$\times$\hyph $D$\hyph векторного пространства
$V_1\times...\times V_n$
в $\times$\hyph $D$\hyph векторное пространство
$W_1\times...\times W_m$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: polylinear map, D vector space}
Пусть $D$ - тело характеристики $0$.
Для каждого $k\in K=[1,n]$ допустим \eV{V_k}
- базис в $D$\Hyph векторном пространстве $V_k$ и
\ShowEq{polylinear map 1, D vector space}
Для каждого $l$, $1\le l\le m$, допустим \eV{W_l}
- базис в $D$\Hyph векторном пространстве $W_l$ и
\ShowEq{polylinear map 2, D vector space}
Полилинейное отображение
\EqRef{polylinear map of D vector spaces}
относительно базисов \eV{V_1}, ..., \eV{V_n},
\eV{W_1}, ..., \eV{W_m}
имеет вид
\ShowEq{polylinear map, D vector space, canonical morphism}
Область значений $S$ индекса $s$ зависит от значений индексов
$\gii_1$, ..., $\gii_n$.
$\sigma_s$ - перестановка множества переменных
$\{v^{\gii_1}_1,...,v^{\gii_n}_n\}$.
\end{theorem}
\begin{proof}
Так как отображение $A$
в $\times$\hyph $D$\hyph векторное пространство
$W_1\times...\times W_m$
можно рассматривать покомпонентно,
то мы можем ограничиться рассмотрением отображения
\ShowEq{polylinear map of D vector spaces, j}

Мы докажем утверждение индукцией по $n$.

При $n=1$ доказываемое утверждение является утверждением теоремы
\ref{theorem: linear map, D vector space}.
При этом мы можем отождествить\footnote{В представлении
\EqRef{polylinear map, D vector space, canonical morphism}
мы будем пользоваться следующими правилами.
\begin{itemize}
\item Если область значений какого-либо индекса - это множество,
состоящее из одного элемента, мы будем опускать соответствующий
индекс.
\item Если $n=1$, то $\sigma_s$ - тождественное преобразование.
Это преобразование можно не указывать в выражении.
\end{itemize}}
\ShowEq{polylinear map, D vector space, canonical morphism 1}

Допустим, что утверждение теоремы справедливо при $n=k-1$.
Тогда отображение
\EqRef{polylinear map of D vector spaces, j}
можно представить в виде
\ShowEq{polylinear map of D vector spaces, j 1}
Согласно предположению индукции полилинейное отображение
$B_l$ имеет вид
\ShowEq{polylinear map, D vector space, canonical morphism 2}
Согласно построению $B_l=C_l(v_k)$.
Следовательно, выражения
\ShowEq{polylinear map, D vector space, canonical morphism 3}
являются функциями $v_k$.
Поскольку $C_l(v_k)$ - линейная функция $v_k$,
то только одно выражение
\ShowEq{polylinear map, D vector space, canonical morphism 3}
является линейной функцией $v_k$, и остальные выражения
\ShowEq{polylinear map, D vector space, canonical morphism 4}
не зависят от $v_k$.

Не нарушая общности, положим $p=0$.
Согласно теореме
\ref{theorem: linear map, D vector space}
\ShowEq{polylinear map, D vector space, canonical morphism 5}
Положим $s=tr$ и определим перестановку $\sigma_s$ согласно правилу
\ShowEq{polylinear map, D vector space, canonical morphism sigma}
Положим
\ShowEq{polylinear map, D vector space, canonical morphism 6}
Мы доказали шаг индукции.
\end{proof}

\begin{definition}
\begin{sloppypar}
Выражение
\ShowEq{component of polylinear map, D vector space}
в равенстве \EqRef{polylinear map, D vector space, canonical morphism}
называется \AddIndex{компонентой полилинейного отображения}
{component of polylinear map} $A$.
\qed
\end{sloppypar}
\end{definition}


==> Vector.Space.Russian.tex <==
%auto-ignore
\input{Vector.Space.Eq}
\ifx\PrintBook\Defined
\chapter{Векторное пространство над телом}
\label{chapter: Vector Space Over Division Ring}
\fi

\section{Векторное пространство}
\label{section: Vector Space}

Чтобы определить левостороннее представление
\DrawEq{D->*M}{}
кольца $D$ в $\Omega$\Hyph алгебре $M$,
мы должны определить структуру кольца на множестве
${}^\star M$.
\footnote{Можно
ли определить операцию сложения на множестве
${}^\star M$, если эта операция не определена на множестве
$M$. Ответ на этот вопрос положительный.

Допустим $M=B\cup C$ и $F:B\rightarrow C$ - взаимно однозначное
отображение. Мы определим множество ${}^\star M$ левосторонних преобразований
множества $M$ согласно следующему правилу. Пусть $V\subseteq B$. левостороннее преобразованиие
$F_V$ имеет вид
\[
F_Vx=\left\{\begin{array}{lr}
x&x\in B\backslash V\\
Fx&x\in V  \\
x&x\in C\backslash F(V)\\
F^{-1}x&x\in F(V)  
\end{array}\right.
\]
Мы определим сложение левосторонних преобразований по правилу
\begin{align*}
F_V+F_W&=F_{V\bigtriangleup W}\\
V\bigtriangleup W&=(V\cup W)\backslash(V\cap W)
\end{align*}
Очевидно, что
\[
F_\emptyset+F_V=F_V
\]
\[F_V+F_V=F_\emptyset\]
Следовательно, отображение $F_\emptyset$ является нулём относительно
сложения, а множество ${}^\star M$ является абелевой группой.}

\begin{theorem}
\label{theorem: Ts representation of the ring}
Левостороннее представление $f$
кольца $D$ в $\Omega$\Hyph алгебре $M$ определенно тогда и только
тогда, когда определены левосторонние представления мультипликативной и аддитивной групп кольца $D$
и эти представления удовлетворяют соотношению
\[
f(a(b+c))=f(a)f(b)+f(a)f(c)
\]
\end{theorem}
\begin{proof}
Теорема следует из определения
\ref{definition: left-side representation of algebra}.
\end{proof}

\ePrints{4993-2400}
\ifx\Semafor\ValueOff
\begin{definition}
\label{definition: Tstar module}
Абелева группa $M$ является \AddIndex{$D*$\Hyph модулем}{D*-module},
если определено \Ts{D}представление
\DrawEq{D->*M}{}
\qed
\end{definition} 

Согласно нашим обозначениям $D*$\hyph модуль -
это \AddIndex{левый модуль нaд кольцом $D$}{left module over ring} и
\AddIndex{$*D$\hyph модуль}{starR-module} -
это \AddIndex{правый модуль нaд кольцом $D$}{right module over ring}.

Поле является частным случаем кольца. Поэтому векторное пространство над полем
имеет больше свойств чем модуль над кольцом.
Очень трудно, если вообще возможно,
распространить определения, работающие в векторном пространстве,
на модуль над произвольным кольцом.
Определение базиса и размерности векторного пространства тесно связаны с возможностью
найти решение линейного уравнения в кольце.
Свойства линейного уравнения в теле близки к свойствам
линейного уравнения в поле.
Поэтому мы надеемся что свойства векторного пространства над телом
близки к свойствам векторного пространства над полем.
\fi

\begin{theorem}
\label{theorem: effective Ts representation of the division ring}
Левостороннее представление тела $D$
\AddIndex{эффективно}{effective representation of division ring},
если эффективно левостороннее представление мультипликативной группы тела $D$.
\end{theorem}
\begin{proof}
Пусть
\DrawEq{D->*M}{}
левостороннее представление тела $D$. Если элементы $a$, $b$ мультипликативной группы
порождают одно и то же левостороннее преобразование, то
\ShowEq{Tstar representation of division ring}
для любого $m\in M$. Выполняя преобразование $f(a^{-1})$ над обеими частями
равенства \EqRef{Tstar representation of division ring}, мы получим
\[
m=f(a^{-1})(f(b)m)=f(a^{-1}b)m
\]
\end{proof}

Согласно замечанию
\ref{remark: notation for effective representation of algebra},
если представление тела эффективно,
мы отождествляем элемент тела и соответствующее
ему левостороннее преобразование.

\begin{definition}
\label{definition: Tstar vector space}
Пусть \(D\) является телом.
Абелева группa $V$ является
\AddIndex{$D*$\Hyph векторным пространством}{D* vector space},
если определено эффективное \Ts{D}представление
\DrawEq{D->*M}{Tstar vector space}
Абелева группa $V$ является
\AddIndex{$*D$\Hyph векторным пространством}{*D vector space},
если определено эффективное \sT{D}представление
\ShowEq{D->M*}
\qed
\end{definition} 

$D*$\hyph векторное пространство называется также
\AddIndex{левым $D$\hyph векторным пространством}{left vector space} или
левым векторным пространством нaд телом $D$.
$*D$\hyph векторное пространство называется также
\AddIndex{правым $D$\hyph векторным пространством}{right vector space} или
правым векторным пространством нaд телом $D$.

\begin{theorem}
\label{theorem: definition of vector space}
Элементы $D*$\Hyph векторного пространства $V$ удовлетворяют соотношениям
\begin{itemize}
\item 
\AddIndex{закону ассоциативности}{associative law}
\ShowEq{associative law, Dstar vector space}
\item 
\AddIndex{закону дистрибутивности}{distributive law}
\ShowEq{distributive law, Dstar vector space}
\item 
\AddIndex{закону унитарности}{unitarity law}
\ShowEq{unitarity law, Dstar vector space}
\end{itemize}
для любых
\ShowEq{a,b in D, m,n in V}
\end{theorem}
\begin{proof}
Равенство \EqRef{distributive law, Dstar vector space, 1} следует
из утверждения, что левостороннее преобразование $a$ является эндоморфизмом абелевой группы.
Равенство \EqRef{distributive law, Dstar vector space, 2} следует
из утверждения, что представление
\eqRef{D->*M}{Tstar vector space}
является гомоморфизмом аддитивной группы
тела $D$.
Равенства \EqRef{associative law, Dstar vector space} и
\EqRef{unitarity law, Dstar vector space} следуют
из утверждения, что представление
\eqRef{D->*M}{Tstar vector space}
является
левосторонним представлением мультипликативной группы тела $D$.
\end{proof}

Согласно нашим обозначениям $D*$\hyph векторное пространство -
это \AddIndex{левое $D$\hyph векторное пространство}{left vector space}.
Отображение
\ShowEq{DV->V}
порождённое \Ts{D}представлением
\eqRef{D->*M}{Tstar vector space},
называется
\AddIndex{левосторонним произведением вектора на скаляр}
{left-side product of vector over scalar}.

Согласно нашим обозначениям
\AddIndex{$*D$\hyph векторное пространство}{starD-vector space} -
это \AddIndex{правое $D$\hyph векторное пространство}{right vector space}.
Отображение
\ShowEq{VD->V}
порождённое \sT{D}представлением
\EqRef{D->M*},
называется
\AddIndex{правосторонним произведением вектора на скаляр}
{right-side product of vector over scalar}.

Любое утверждение, справедливое для
левого $D$\hyph векторного пространства,
справедливо для правого $D$\hyph векторного пространства,
если левостороннее произведение вектора на скаляр
заменить правосторонним произведением вектора на скаляр.

\begin{definition}
Пусть $V$ - $D*$\hyph векторное пространство нaд телом $D$.
Множество векторов $N$ -
\AddIndex{подпространство $D*$\hyph векторного пространства}
{subspace of Dstar vector space}
$V$, если
\ShowEq{subspace of Dstar vector space}
\qed
\end{definition}

\ePrints{4993-2400}
\ifx\Semafor\ValueOff
\begin{example}
\label{example: matrices vector space}
Определим на множестве
%\symb{D^m_n}{matrices vector space}1
\(D^m_n\)
$m\times n$ матриц над телом $D$
операцию сложения
\[
a+b=
\left(a_i^j\right)
+
\left(b_i^j\right)
=
\left(a_i^j+b_i^j\right)
\]
и умножения на скаляр
\[
da=
d\left(a_i^j\right)
=
\left(da_i^j\right)
\]
$a=0$ тогда и только тогда, когда $a_i^j=0$ для любых $i$, $j$.
Непосредственная проверка показывает, что
$D^m_n$ является $D*$\hyph векторным пространством,
если произведение действует слева.
В противном случае $D^m_n$
- $*D$\hyph векторное пространство.
Мы будем называть векторное пространство $D^m_n$
\AddIndex{$D*$\hyph векторным пространством матриц}{matrices vector space}.
\qed
\end{example}
\fi

\section{Тип векторного пространства}
\label{section: vector space type}

\ePrints{4993-2400}
\ifx\Semafor\ValueOff
Произведение вектора на скаляр асимметрично,
так как произведение определено для объектов разных множеств.
Однако различие между
\ePrints{4993-2400}
\ifx\Semafor\ValueOff
$D*$\hyph
\else
левым
\fi
и
\ePrints{4993-2400}
\ifx\Semafor\ValueOff
$*D$\hyph
\else
правым
\fi
векторным пространством появляется только тогда,
когда мы переходим к координатному представлению.
Говоря, векторное пространство является $D*$\hyph\ или $*D$\hyph, мы указываем,
с какой стороны, слева или справа, мы умножаем координаты
вектора на элементы тела.
\fi

\begin{definition}
Допустим $u$, $v$
- векторы $D*$\hyph векторного пространства $V$.
Мы будем говорить, что вектор $w$ является
\AddIndex{линейной комбинацией векторов}{linear composition of  vectors}
$u$ и $v$,
если мы можем записать
\ShowEq{w=au+bv}
где $a$ и $b$ - скаляры.
\qed
\end{definition}

Мы можем распространить понятие линейной комбинации на любое конечное семейство
векторов. Пользуясь обобщённым индексом для нумерации векторов, мы
можем представить семейство векторов в виде одномерной матрицы.
Мы пользуемся соглашением, что в заданном векторном пространстве мы представляем любое семейство
векторов либо в виде \subs строки
(матрицы строки), либо \sups строки
(матрицы столбца).
Это представление определяет характер записи линейной комбинации.
Рассматривая это представление в
$D*$\hyph
или
$*D$\hyph векторном пространстве, мы
получаем четыре разных модели векторного пространства,
рассмотренные в примерах
\ShowEq{models of vector space}

Чтобы иметь возможность,
не меняя записи указать, является векторное пространство
$D*$- или $*D$\hyph векторным пространством, мы вводим новое обозначение.
Символ \symb{D*}{vector space type}1\ называется
\AddIndex{типом векторного пространства}{vector space type} и
означает, что мы изучаем
$D*$\hyph векторное пространство.
Операция умножения в типе векторного пространства указывает на матричную операцию,
используемую в линейной комбинации.

\begin{example}
\label{example: drc vector space, definition}
Представим множество векторов
\ShowEq{sups row Vector A, 1}
$D*$\Hyph векторного пространства $V$
в виде
\sups строки (матрицы столбца)
\ShowEq{sups row Vector A}
и множество скаляров
\ShowEq{subs row c, 1},
в виде
\subs строки (матрицы строки)
\ShowEq{subs row c}
Тогда мы можем записать линейную комбинацию векторов $\pia$ в виде
\ShowEq{linear composition pVa}
Соответствующая реализация
$D*$\Hyph векторного пространства называется
\AddIndex{\drc векторным пространством}{drc vector space}
или
\AddIndex{левым $D$\Hyph векторным пространством строк}{left vector space of rows}.
\qed
\end{example}

\begin{example}
\label{example: dcr vector space, definition}
Представим множество векторов
\ShowEq{subs row Vector A, 1}
$D*$\Hyph векторного пространства $V$
в виде
subs строки (матрицы строки)
\ShowEq{subs row Vector A}
и множество скаляров
\ShowEq{sups row c, 1},
в виде
\sups строки (матрицы столбца)
\ShowEq{sups row c}
Тогда мы можем записать линейную комбинацию векторов $\bia$ в виде
\ShowEq{linear composition bVa}
Соответствующая реализация
$D*$\Hyph векторного пространства называется
\AddIndex{\dcr векторным пространством}{dcr vector space}
или
\AddIndex{левым $D$\Hyph векторным пространством столбцов}{left vector space of columns}.
\qed
\end{example}

\begin{example}
\label{example: crd vector space, definition}
Представим множество векторов
\ShowEq{Vector A sups row, 1}
$*D$\Hyph векторного пространства $V$
в виде
\sups строки (матрицы столбца)
\ShowEq{Vector A sups row}
и множество скаляров
\ShowEq{c subs row, 1},
в виде
\subs строки (матрицы строки)
\ShowEq{c subs row}
Тогда мы можем записать линейную комбинацию векторов $a^i$ в виде
\ShowEq{linear composition Vap}
Соответствующая реализация
$*D$\Hyph векторного пространства называется
\AddIndex{\crd векторным пространством}{crd vector space}
или
\AddIndex{правым $D$\Hyph векторным пространством строк}{right vector space of rows}.
\qed
\end{example}

\begin{example}
\label{example: rcd vector space, definition}
Представим множество векторов
\ShowEq{Vector A subs row, 1}
$*D$\Hyph векторного пространства $V$
в виде
\subs строки (матрицы строки)
\ShowEq{Vector A subs row}
и множество скаляров
\ShowEq{c sups row, 1},
в виде
\sups строки (матрицы столбца)
\ShowEq{c sups row}
Тогда мы можем записать линейную комбинацию векторов $a_i$ в виде
\ShowEq{linear composition Vab}
Соответствующая реализация
$*D$\Hyph векторного пространства называется
\AddIndex{\rcd векторным пространством}{rcd vector space}
или
\AddIndex{правым $D$\Hyph векторным пространством столбцов}
{right vector space of columns}.
\qed
\end{example}

\ePrints{4993-2400}
\ifx\Semafor\ValueOff
\begin{remark}
\label{remark: left and right vector space notation}
Мы распространим на векторное пространство и его тип соглашение,
описанное в замечании
\xRef{0612.111}{remark: left and right matrix notation}.
Например, в выражении
\[A\RCstar B\RCstar v\lambda\]
мы выполняем операцию умножения слева направо. Это соответствует
\rcd векторному пространству. Однако мы можем выполнять операцию умножения
справа налево. В традиционной записи это выражение примет вид
\[\lambda v\CRstar B\CRstar A\]
и будет соответствовать \dcr векторному пространству. Аналогично, читая выражение
снизу вверх мы получим выражение
\[A\CRstar B\CRstar v\lambda\]
соответствующего \crd векторному пространству.
\qed
\end{remark}
\fi

\section{Базис \texorpdfstring{$\RCstar D$}{rcD}-векторного пространства}
\label{section: Basis of Vector Space}

\begin{definition}
\label{definition: linearly independent vectors}
Векторы
\ShowEq{Vector A subs row, 1}
\rcd векторного пространства
$V$
\AddIndex{линейно независимы}{linearly independent vectors},
если $c=0$ следует из уравнения
\ShowEq{rcd linearly independent}
В противном случае, векторы $a_i$
\AddIndex{линейно зависимы}{linearly dependent vectors}.
\qed
\end{definition}

\begin{definition}
Множество векторов
\ShowEq{basis, vector space}
- \AddIndex{базис \rcd векторного пространства}{basis, rcd vector space},
если векторы $e_i$ линейно независимы и добавление
любого вектора к этой системе
делает эту систему линейно зависимой.
\qed
\end{definition}

\begin{theorem}
\label{theorem: expansion relative basis, vector space}
Если $\Basis e$ - базис \rcd векторного пространства $V$,
то любой вектор $\Vector v\in V$
имеет одно и только одно разложение
\ShowEq{expansion relative basis, vector space}
относительно этого базиса.
\end{theorem}
\begin{proof}
Так как система векторов $e_i$ является
максимальным множеством линейно независимых векторов,
система векторов
\ShowEq{expansion relative basis, vector space, 0}
- линейно зависима и в уравнении
\ShowEq{expansion relative basis, vector space, 1}
по крайней мере $b$ отлично от $0$. Тогда равенство
\ShowEq{expansion relative basis, vector space, 2}
следует из \EqRef{expansion relative basis, vector space, 1}.
\EqRef{expansion relative basis, vector space} следует
из \EqRef{expansion relative basis, vector space, 2}.

Допустим мы имеем другое разложение
\ShowEq{expansion relative basis, vector space, 3}
Вычтя \EqRef{expansion relative basis, vector space}
из \EqRef{expansion relative basis, vector space, 3},
мы получим
\ShowEq{expansion relative basis, vector space, 4}
Так как векторы $e_i$ линейно независимы, мы имеем
\[v'-v=0\]
\end{proof}

\begin{definition}
Мы будем называть матрицу
$v$ разложения \EqRef{expansion relative basis, vector space}
\AddIndex{координатной матрицей вектора}
{coordinate matrix of vector} $\Vector v$ в базисе $\Basis e$
и её элементы
\AddIndex{координатами вектора}{coordinates of vector}
$\Vector v$ относительно базиса $\Basis e$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: coordinate vector space}
Множество координат $a$ вектора $\Vector a$ в базисе $\Basis e$
\rcd векторного пространства
порождают \rcd векторное пространство
\ShowEq{coordinate rcd vector space},
изоморфное \rcd векторному пространству $V$.
Это \rcd векторное пространство называется
\AddIndex{координатным \rcd векторным пространством}
{coordinate rcd vector space},
а изоморфизм
\AddIndex{координатным изоморфизмом}{coordinate isomorphism}.
\end{theorem}
\begin{proof}
Допустим векторы $\Vector a$ и $\Vector b\in V$ имеют разложение
\ShowEq{coordinate vector space, 1}
в базисе $\Basis e$. Тогда
\ShowEq{coordinate vector space, 2}
для любого $m\in D$.
Таким образом, операции в векторном пространстве определены по координатно
\ShowEq{coordinate vector space, 3}
Это доказывает теорему.
\end{proof}

\begin{example}
\label{example: drc vector space}
Пусть
\ShowEq{drc vector space}
- \AddIndex{базис \drc векторного пространства}
{basis, drc vector space} $V$.
Согласно примеру
\ref{example: drc vector space, definition},
мы можем представить базис \(\Basis e\)
в виде \sups строки (матрицы столбца)
\ShowEq{basis, drc vector space}%
Координатная матрица
\ShowEq{drc vector}
вектора $\Vector a$ в базисе $\Basis e$
называется \AddIndex{\drc вектором}{drc vector}\footnote{\drc вектор
является аналогом вектор\hyph строки.
}
или
\AddIndex{$D*$\Hyph вектор строкой}{row D* vector}.

Пусть \sups строка
\ShowEq{drc vectors}
задаёт множество векторов.
Векторы $\piA$ имеют разложение
\ShowEq{drc vectors, 1}
Если мы подставим координатные матрицы вектора $\piA$ в
матрицу \EqRef{drc vectors}, мы получим матрицу
\ShowEq{drc vectors, 2}
Мы будем называть матрицу $A$
\AddIndex{координатной матрицей множества векторов}
{coordinate matrix of set of vectors}
$({}^i\Vector A,i\in I)$ в базисе $\Basis e$
и её элементы
\AddIndex{координатами множества векторов}{coordinates of set of vectors}
$({}^i\Vector A,i\in I)$ в базисе $\Basis e$.

Пусть \sups строка
\ShowEq{basis f, drc vector space}
является
базисом \drc векторного пространства $V$.
Мы будем говорить, что координатная матрица $f$ множества векторов
\ShowEq{basis f, drc vector space, 1}
определяет \AddIndex{координаты
\ShowEq{basis coordinates, drc vector space}
базиса}{coordinates of basis}
$\Basis f$ относительно базиса $\Basis e$.
\qed
\end{example}

\begin{example}
\label{example: dcr vector space}
Пусть
\ShowEq{dcr vector space}
- \AddIndex{базис \dcr векторного пространства}
{basis, dcr vector space} $V$.
Согласно примеру
\ref{example: dcr vector space, definition},
мы можем представить базис \(\Basis e\)
в виде \subs строки (матрицы строки)
\ShowEq{basis, dcr vector space}%
Координатная матрица
\ShowEq{dcr vector}
вектора $\Vector a$ в базисе $\Basis e$
называется \AddIndex{\drc вектором}{drc vector}\footnote{\drc вектор
является аналогом вектор\hyph строки.
}
или
\AddIndex{$D*$\Hyph вектор столбцом}{column D* vector}.

Пусть \subs строка
\ShowEq{dcr vectors}
задаёт множество векторов.
Векторы $\piA$ имеют разложение
\ShowEq{dcr vectors, 1}
Если мы подставим координатные матрицы вектора ${}_i\Vector A$ в
матрицу \EqRef{dcr vectors}, мы получим матрицу
\ShowEq{dcr vectors, 2}
Мы будем называть матрицу $A$
\AddIndex{координатной матрицей множества векторов}
{coordinate matrix of set of vectors}
$({}_i\Vector A,i\in I)$ в базисе $\Basis e$
и её элементы
\AddIndex{координатами множества векторов}{coordinates of set of vectors}
$({}_i\Vector A,i\in I)$ в базисе $\Basis e$.

Пусть \subs строка
\ShowEq{basis f, dcr vector space}
является
базисом \dcr векторного пространства $V$.
Мы будем говорить, что координатная матрица $f$ множества векторов
\ShowEq{basis f, dcr vector space, 1}
определяет \AddIndex{координаты
\ShowEq{basis coordinates, dcr vector space}
базиса}{coordinates of basis}
$\Basis f$ относительно базиса $\Basis e$.
\qed
\end{example}

\begin{example}
\label{example: crd vector space}
Пусть
\ShowEq{crd vector space}
- \AddIndex{базис \crd векторного пространства}
{basis, crd vector space} $V$.
Согласно примеру
\ref{example: crd vector space, definition},
мы можем представить базис \(\Basis e\)
в виде \sups строки (матрицы столбца)
\ShowEq{basis, crd vector space}%
Координатная матрица
\ShowEq{crd vector}
вектора $\Vector a$ в базисе $\Basis e$
называется \AddIndex{\crd вектором}{crd vector}\footnote{\rcd вектор
является аналогом вектор\hyph столбца.
}
или
\AddIndex{$*D$\Hyph вектор строкой}{row *D vector}.

Пусть \sups строка
\ShowEq{crd vectors}
задаёт множество векторов.
Векторы $\Vector A_j$ имеют разложение
\ShowEq{crd vectors, 1}
Если мы подставим координатные матрицы вектора $\Vector A_j$ в
матрицу \EqRef{crd vectors}, мы получим матрицу
\ShowEq{crd vectors, 2}
Мы будем называть матрицу $A$
\AddIndex{координатной матрицей множества векторов}
{coordinate matrix of set of vectors}
\ShowEq{Vector A sups row, 2}
в базисе $\Basis e$
и её элементы
\AddIndex{координатами множества векторов}
{coordinates of set of vectors}
\ShowEq{Vector A sups row, 2}
в базисе $\Basis e$.

Пусть \sups строка
\ShowEq{basis f, crd vector space}
является
базисом \crd векторного пространства $V$.
Мы будем говорить, что координатная матрица $f$ множества векторов
\ShowEq{basis f, crd vector space, 1}
определяет \AddIndex{координаты
\ShowEq{basis coordinates, crd vector space}
базиса}{coordinates of basis}
$\Basis f$ относительно базиса $\Basis e$.
\qed
\end{example}

\begin{example}
\label{example: rcd vector space}
Пусть
\ShowEq{rcd vector space}
- \AddIndex{базис \rcd векторного пространства}
{basis, rcd vector space} $V$.
Согласно примеру
\ref{example: rcd vector space, definition},
мы можем представить базис \(\Basis e\)
в виде \subs строки (матрицы строки)
\ShowEq{basis, rcd vector space}
Координатная матрица
\ShowEq{rcd vector}
вектора $\Vector a$ в базисе $\Basis e$
называется \AddIndex{\rcd вектором}{rcd vector}\footnote{\rcd вектор
является аналогом вектор\hyph столбца.
}
или
\AddIndex{$D*$\Hyph вектор столбцом}{column D* vector}.

Пусть \subs строка
\ShowEq{rcd vectors}
задаёт множество векторов.
Векторы $\Vector A_j$ имеют разложение
\ShowEq{rcd vectors, 1}
Если мы подставим координатные матрицы вектора $\Vector A_j$ в
матрицу \EqRef{rcd vectors}, мы получим матрицу
\ShowEq{rcd vectors, 2}
Мы будем называть матрицу $A$
\AddIndex{координатной матрицей множества векторов}
{coordinate matrix of set of vectors}
\ShowEq{Vector A sups row, 2}
в базисе $\Basis e$
и её элементы
\AddIndex{координатами множества векторов}
{coordinates of set of vectors}
\ShowEq{Vector A sups row, 2}
в базисе $\Basis e$.

Пусть \subs строка
\ShowEq{basis f, rcd vector space}
является
базисом \rcd векторного пространства $V$.
Мы будем говорить, что координатная матрица $f$ множества векторов
\ShowEq{basis f, rcd vector space, 1}
определяет \AddIndex{координаты
\ShowEq{basis coordinates, rcd vector space}
базиса}{coordinates of basis}
$\Basis f$ относительно базиса $\Basis e$.
\qed
\end{example}

\ePrints{4993-2400}
\ifx\Semafor\ValueOn
\else
Так как мы линейную комбинацию выражаем с помощью матриц, мы можем
распространить принцип двойственности на теорию векторных пространств.
Мы можем записать принцип двойственности в одной из следующих форм

\begin{theorem}[принцип двойственности]
\label{theorem: duality principle, vector space}
Пусть $\mathfrak{A}$ - истинное утверждение о векторных пространствах.
Если мы заменим одновременно
\begin{itemize}
\item \drc вектор и \dcr вектор
\item \rcd вектор и \crd вектор
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}

\begin{theorem}[принцип двойственности]
\label{theorem: duality principle, vector space, quasideterminants}
Пусть $\mathfrak{A}$ - истинное утверждение о векторных пространствах.
Если мы одновременно заменим
\begin{itemize}
\item \drc вектор и \rcd вектор или \dcr вектор и \crd вектор
\item \RC квазидетерминант и \CR квазидетерминант
\end{itemize}
то мы снова получим истинное утверждение.
\end{theorem}
\fi

\Input{Rcd.Morphism}

\ePrints{4993-2400}
\ifx\Semafor\ValueOff
\section{Система линейных уравнений}
\label{section: System of Linear Equations}

\begin{definition}
\label{definition: linear span, vector space}
Пусть $V$ - \rcd векторное пространство и
\ShowEq{rcd linear span}
- множество векторов.
\AddIndex{Линейная оболочка в \rcd векторном пространстве}{linear span, vector space}
- это множество
\ShowEq{linear span, vector space}
векторов, линейно зависимых от векторов $A_i$.
\qed
\end{definition}

\begin{theorem}
Пусть $\spanb$ - линейная оболочка в
\rcd векторном пространстве $V$.
Тогда $\spanb$
- подпространство \rcd векторного пространства $V$.
\end{theorem}
\begin{proof}
Предположим, что
\ShowEq{linear span, vector space, 1}
Согласно определению \ref{definition: linear span, vector space}
\ShowEq{linear span, vector space, 2}
Тогда
\ShowEq{linear span, vector space, 3}
Это доказывает утверждение.
\end{proof}

\begin{example}
Пусть $V$ - \rcd векторное пространство и
\subs строка
\ShowEq{rcd linear span, 0}
задаёт множество векторов.
Чтобы ответить на вопрос, или вектор
\ShowEq{rcd linear span, 1},
мы запишем линейное уравнение
\ShowEq{rcd linear span, 2}
где
\ShowEq{rcd linear span, 3}
\sups строка неизвестных коэффициентов разложения.
\ShowEq{rcd linear span, 1},
если уравнение \EqRef{rcd linear span, 2}
имеет решение.
Предположим, что
\ShowEq{rcd linear span, 5}
- базис.
Тогда векторы
\ShowEq{rcd linear span, 6}
имеют разложение
\ShowEq{rcd linear span, 7}
Если мы подставим \EqRef{rcd linear span, b}
и \EqRef{rcd linear span, ai}
в \EqRef{rcd linear span, 2}, мы получим
\ShowEq{rcd linear span, 8}
Применяя теорему \ref{theorem: expansion relative basis, vector space}
к \EqRef{rcd linear span, 8}, мы получим
\AddIndex{систему линейных уравнений}
{system of linear equations}
\ShowEq{system of rcd linear equations}

Мы можем записать систему линейных уравнений
\EqRef{system of rcd linear equations} в одной из следующих форм
\ShowEq{star rows system of linear equations}
\qed
\end{example}

\begin{example}
Пусть $V$ - \drc векторное пространство и
\sups строка
\ShowEq{drc linear span, 0}
задаёт множество векторов.
Чтобы ответить на вопрос, или вектор
\ShowEq{drc linear span, 1},
мы запишем линейное уравнение
\ShowEq{drc linear span, 2}
где
\ShowEq{drc linear span, 3}
\subs строка неизвестных коэффициентов разложения.
\ShowEq{drc linear span, 4},
если уравнение \EqRef{drc linear span, 2}
имеет решение.
Предположим, что
\ShowEq{drc linear span, 5}
- базис.
Тогда векторы
\ShowEq{drc linear span, 6}
имеют разложение
\ShowEq{drc linear span, 7}
Если мы подставим \EqRef{drc linear span, b}
и \EqRef{drc linear span, ai}
в \EqRef{drc linear span, 2}, мы получим
\ShowEq{drc linear span, 8}
Применяя теорему \ref{theorem: expansion relative basis, vector space}
к \EqRef{drc linear span, 8}, мы получим
\AddIndex{систему линейных уравнений}
{system of linear equations}\footnote{Читая систему
\rcd линейных уравнений \EqRef{system of rcd linear equations}
в \rcd векторном пространстве
снизу вверх
и слева направо,
мы получим систему линейных уравнений
\EqRef{system of drc linear equations}
в \drc векторном пространстве.}
\ShowEq{system of drc linear equations}

Мы можем записать систему линейных уравнений
\EqRef{system of drc linear equations} в одной из следующих форм
\ShowEq{star columns system of linear equations}
\qed
\end{example}

Чтобы найти решение системы линейных уравнений,
мы должны рассмотреть матрицу этой системы.
Из примеров
\ref{example: dcr vector space},
\ref{example: rcd vector space},
мы видим, что мы можем рассматривать столбец матрицы
как вектор левого или правого векторного пространства.
Чтобы сделать утверждения проще, мы будем указывать
тип векторного пространства перед словом линейный.
Например, утверждение

\begin{itemize}
\renewcommand{\labelitemi}{\ }
\item
Столбцы матрицы \dcr линейно зависимы.
\end{itemize}

\noindent
означает, что

\begin{itemize}
\renewcommand{\labelitemi}{\ }
\item
Столбцы матрицы являются векторами \dcr векторного пространства,
и соответствующие векторы линейно зависимы.
\end{itemize}

\noindent
В частности, система линейных уравнений
\EqRef{system of rcd linear equations}
в \rcd векторном пространстве называется
\AddIndex{системой \rcd линейных уравнений}
{system of rcd linear equations}
и система линейных уравнений
\EqRef{system of drc linear equations}
в \drc векторном пространстве называется
\AddIndex{системой \drc линейных уравнений}
{system of drc linear equations}.

\begin{definition}
Если $n\times n$ матрица $A$ имеет \RC обратную матрицу,
мы будем называть такую матрицу
\AddIndex{\RC невырожденной матрицей}{RC nonsingular matrix}.
В противном случае, мы будем называть такую матрицу
\AddIndex{\RC вырожденной матрицей}{RC singular matrix}.
\qed
\end{definition}

\begin{definition}
Предположим, что $A$
- \RC невырожденная матрица. Мы будем называть соответствующую систему
\rcd линейных уравнений
\ShowEq{nonsingular system of linear equations}
\AddIndex{невырожденной системой \rcd линейных уравнений}
{nonsingular system of linear equations}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: nonsingular system of linear equations}
Решение невырожденной системы \rcd линейных уравнений
\EqRef{nonsingular system of linear equations} определено однозначно
и может быть записано в любой из следующих форм\footnote{Мы можем найти решение системы
\EqRef{nonsingular system of linear equations}
в теореме
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=19}{1.6.1}.
Я повторяю это утверждение, так как я слегка изменил обозначения.
\label{footnote: nonsingular system of linear equations}}
\ShowEq{nonsingular system of linear equations, solution}
\end{theorem}
\begin{proof}
Умножая обе части равенства \EqRef{nonsingular system of linear equations}
слева на $A^{\RCInverse}$, мы получим
\EqRef{nonsingular system of linear equations, solution, matrix}.
Пользуясь определением
\xEqRef{0612.111}{j i RC-quasideterminant =},
мы получим \EqRef{nonsingular system of linear equations, solution, quasideterminant}.
Решение системы единственно в силу теоремы
\xRef{0612.111}{theorem: two products equal}.
\end{proof}

\section{Ранг матрицы}
\label{section: Rank of Matrix}

\begin{definition}
Мы будем называть матрицу\footnote{Мы
делаем следующие предположения в этом разделе
\begin{itemize}
\ShowEq{Rank of Matrix assumption 1}
\ShowEq{Rank of Matrix assumption 2}
- произвольная матрица.
\ShowEq{Rank of Matrix assumption 3 4}
\end{itemize}
\label{footnote: index assumption}}
$\SA T$ минорной матрицей порядка $k$.
\qed
\end{definition}

\begin{definition}
Если минорная матрица $\SA T$ - \RC невырожденная матрица,
то мы будем говорить, что
\RC ранг матрицы $A$ не меньше, чем $k$.
\AddIndex{\RC ранг матрицы $A$}{rc-rank of matrix}
\ShowEq{rc-rank of matrix}
- это максимальное значение $k$.
Мы будем называть соответствующую минорную матрицу
\AddIndex{\RC главной минорной матрицей}{RC-major minor}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: singular matrix and quasideterminant}
Пусть матрица $A$ - \RC вырожденная матрица и минорная матрица $\SA T$
- главный минорная матрица, тогда
\ShowEq{singular matrix and quasideterminant}
\end{theorem}
\begin{proof}
Чтобы понять, почему минорная матрица
\ShowEq{singular matrix and quasideterminant, 0}
не имеет \RC обратной матрицы,\footnote{Естественно ожидать связь между \RC вырожденностью матрицы
и её \RC квазидетерминантом, подобную связи, известной в коммутативном случае.
Однако \RC квазидетерминант определён не всегда. Например, если \RC обратная матрица
имеет слишком много элементов, равных $0$. Как следует из этой теоремы, не определён \RC квазидетерминант
также в случае, когда \RC ранг матрицы меньше $n-1$.}
мы предположим, что существует \RC обратная матрица
\ShowEq{B rc-1}
Запишем систему линейных уравнений
\xEqRef{0612.111}{inverse minor, 11},
\xEqRef{0612.111}{inverse minor, 12}
полагая
\ShowEq{I=r J=p}
(в этом случае
\ShowEq{[I]= [J]=})
\ShowEq{singular matrix and quasideterminant, 1}
и попробуем решить эту систему.
Мы умножим \EqRef{singular matrix and quasideterminant, 1} на
$\Bf$
\ShowEq{singular matrix and quasideterminant, 3}
Теперь мы можем подставить \EqRef{singular matrix and quasideterminant, 3} в
\EqRef{singular matrix and quasideterminant, 2}
\ShowEq{singular matrix and quasideterminant, 4}
Из \EqRef{singular matrix and quasideterminant, 4} следует
\ShowEq{singular matrix and quasideterminant, 5}
Выражение в скобках является квазидетерминантом
$\Bq$.
Подставляя это выражение в \EqRef{singular matrix and quasideterminant, 5},
мы получим
\ShowEq{singular matrix and quasideterminant, 6}
Тем самым мы доказали, что квазидетерминант $\Bq$
определён и условие его обращения в $0$ необходимое и достаточное условие
вырожденности матрицы $B$. Теорема доказана в силу соглашения
\EqRef{singular matrix and quasideterminant, 0}.
\end{proof}

\begin{theorem}
\label{theorem: rc rank of matrix, subs-rows}
Предположим, что $A$ - матрица\footref{footnote: index assumption},
$$\RCA=k<m$$
и $\SA T$ - \RC главная минорная матрица.
Тогда \subs строка ${}^pA$ является
\drc линейной комбинацией \subs строк ${}^SA$.
\ShowEq{rc rank of matrix, subs-rows}
\end{theorem}
\begin{proof}
Если матрица $A$ имеет $k$ \sups строк, то, полагая, что \subs строка ${}^pA$
- \drc линейная комбинация \EqRef{rc rank of matrix, subs-rows, 1}
\subs строк ${}^sA$ с коэффициентами $\pRs$,
мы получим систему \drc линейных уравнений
\EqRef{rc rank of matrix, subs-rows, 2}.
Согласно теореме \ref{theorem: nonsingular system of linear equations}
система \drc линейных уравнений
\EqRef{rc rank of matrix, subs-rows, 2}
имеет единственное решение\footnote{Мы положим,
что неизвестные переменные здесь - это $x_s=\pRs$
\label{footnote: xs=rps}}
и это решение нетривиально потому, что все \RC квазидетерминанты
отличны от $0$.

Остаётся доказать утверждение в случае, когда число \sups строк матрицы $A$
больше чем $k$.
Пусть нам даны \subs строка ${}^pA$ и \sups строка $A_r$.
Согласно предположению, минорная матрица
$\SATpr$ - \RC вырожденная матрица
и его \RC квазидетерминант
\ShowEq{rc rank of matrix, subs-rows, 3}
Согласно
\xEqRef{0612.111}{quasideterminant, 1}
равенство \EqRef{rc rank of matrix, subs-rows, 3} имеет вид
\ShowEq{rc rank of matrix, subs-rows, 4}
Матрица
\ShowEq{rc rank of matrix, subs-rows, 5}
не зависит от $r$. Следовательно, для любых $r\in N\setminus T$
\ShowEq{rc rank of matrix, subs-rows, 6}
Из равенства
\ShowEq{rc rank of matrix, subs-rows, 7}
следует, что
\ShowEq{rc rank of matrix, subs-rows, 8}
Подставляя \EqRef{rc rank of matrix, subs-rows, 5}
в \EqRef{rc rank of matrix, subs-rows, 8}, мы получим
\ShowEq{rc rank of matrix, subs-rows, 9}
\EqRef{rc rank of matrix, subs-rows, 6} и \EqRef{rc rank of matrix, subs-rows, 9}
завершают доказательство.
\end{proof}

\begin{corollary}
\label{corollary:rc rank of matrix, subs-rows}
Предположим, что $A$ - матрица,
$\RCA=k<m$.
Тогда \subs строки матрицы \drc линейно зависимы.
\DrawEq{rc rank of matrix, subs-rows drc linearly dependent}{}
\end{corollary}
\begin{proof}
Предположим, что \subs строка ${}^pA$ - \drc линейная комбинация
\EqRef{rc rank of matrix, subs-rows, 1}. Мы положим
\ShowEq{rc rank of matrix, subs-rows drc linearly dependent, 1}
и остальные
\ShowEq{rc rank of matrix, subs-rows drc linearly dependent, 2}
\end{proof}

\begin{theorem}
\label{theorem: rank of coordinate matrix}
Пусть
\ShowEq{rank of coordinate matrix}
семейство
\drc линейно независимых векторов. Тогда \RC ранг их
координатной матрицы равен $m$.
\end{theorem}
\begin{proof}
Пусть \(\Basis e\) - базис \drc векторного пространства.
Согласно конструкции, изложенной в примере \ref{example: drc vector space},
координатная матрица семейства векторов $({}^i\Vector A)$ относительно базиса $\Basis e$
состоит из \subs строк, являющихся координатными матрицами векторов
${}^i\Vector A$ относительно базиса $\Basis e$. Поэтому \RC ранг
этой матрицы не может превышать $m$.

Допустим \RC ранг
координатной матрицы меньше $m$.
Согласно следствию \ref{corollary:rc rank of matrix, subs-rows},
\subs строки матрицы \drc линейно зависимы
\DrawEq{rc rank of matrix, subs-rows drc linearly dependent}{coordinate matrix}
Положим $c=\lambda\RCstar A$.
Из равенства
\eqRef{rc rank of matrix, subs-rows drc linearly dependent}{coordinate matrix}
следует, что \drc линейная комбинация
\[
c\RCstar \Vector e=0
\]
векторов базиса равна $0$. Это противоречит утверждению, что векторы $\Vector e$ образуют
базис. Утверждение теоремы доказано.
\end{proof}

\begin{theorem}
\label{theorem: rc rank of matrix, sups-rows}
Предположим, что $A$ - матрица\footref{footnote: index assumption},
$$\RCA=k<n$$
и $\SA T$ - \RC главная минорная матрица.
Тогда \sups строка $A_r$ является
\rcd линейной композицией \sups строк $A_t$
\ShowEq{rc rank of matrix, sups-rows}
\end{theorem}
\begin{proof}
Если матрица $A$ имеет $k$ \subs строк, то, полагая, что \sups строка $A_r$
- \rcd линейная комбинация \EqRef{rc rank of matrix, sups-rows, 1}
\sups строк $A_t$ с коэффициентами $\tRr$,
мы получим систему \rcd линейных уравнений
\EqRef{rc rank of matrix, sups-rows, 2}.
Согласно теореме \ref{theorem: nonsingular system of linear equations}
система \rcd линейных уравнений
\EqRef{rc rank of matrix, sups-rows, 2}
имеет единственное решение\footnote{Мы положим,
что неизвестные переменные здесь - это ${}^tx=\tRr$
\label{footnote: xt=rtq}}
и это решение нетривиально потому, что все \RC квазидетерминанты
отличны от $0$.

Остаётся доказать утверждение в случае, когда число \subs строк матрицы $A$
больше чем $k$.
Пусть нам даны \sups строка $A_r$ и \subs строка ${}^pA$.
Согласно предположению, минорная матрица
$\SATpr$ - \RC вырожденная матрица
и его \RC квазидетерминант
\ShowEq{rc rank of matrix, sups-rows, 3}
Согласно
\xEqRef{0612.111}{quasideterminant, 1}
\EqRef{rc rank of matrix, sups-rows, 3} имеет вид
\ShowEq{rc rank of matrix, sups-rows, 5}
Матрица
\ShowEq{rc rank of matrix, sups-rows, 6}
не зависит от $p$, Следовательно, для любых $p\in M\setminus S$
\ShowEq{rc rank of matrix, sups-rows, 7}
Из равенства
\ShowEq{rc rank of matrix, sups-rows, 8}
следует, что
\ShowEq{rc rank of matrix, sups-rows, 9}
Подставляя \EqRef{rc rank of matrix, sups-rows, 6}
в \EqRef{rc rank of matrix, sups-rows, 9}, мы получим
\ShowEq{rc rank of matrix, sups-rows, 10}
\EqRef{rc rank of matrix, sups-rows, 7}
и \EqRef{rc rank of matrix, sups-rows, 10}
завершают доказательство.
\end{proof}

\begin{corollary}
\label{corollary:rc rank of matrix, sups-rows}
Предположим, что $A$ - матрица,
$\RCA=k<m$.
Тогда \sups строки матрицы \rcd линейно зависимы.
\[
A\RCstar \lambda=0
\]
\end{corollary}
\begin{proof}
Предположим, что \sups строка $A_r$ - правая линейная комбинация
\EqRef{rc rank of matrix, sups-rows, 1}. Мы положим
\ShowEq{rc rank of matrix, sups-rows rcd linearly dependent, 1}
и остальные
\ShowEq{rc rank of matrix, sups-rows rcd linearly dependent, 2}
\end{proof}

Опираясь на теорему \xRef{0612.111}{theorem: duality principle, quasideterminants},
мы можем записать подобные утверждения для \CR ранга матрицы.

\begin{theorem}
\label{theorem: cr rank of matrix, subs-rows}
Предположим, что $A$ - матрица,
\ShowEq{cr-rank of matrix}
и ${}_TA^S$ - \CR главная минорная матрица.
Тогда \subs строка $A^p$ является
\crd линейной композицией \subs строк $A^s$
\ShowEq{cr rank of matrix, subs-rows}
\end{theorem}

\begin{corollary}
\label{corollary: cr rank of matrix, subs-rows}
Предположим, что $A$ - матрица,
$\CRRank A=k<m$.
Тогда \subs строки матрицы \crd линейно зависимы.
\[
A\CRstar\lambda=0
\]
\end{corollary}

\begin{theorem}
\label{theorem: cr rank of matrix, sups-rows}
Предположим, что $A$ - матрица,
$$\CRRank A=k<n$$
и ${}_TA^S$ - \CR главная минорная матрица.
Тогда \sups строка ${}_rA$ является
\dcr линейной композицией \sups строк ${}_tA$
\ShowEq{cr rank of matrix, sups-rows}
\end{theorem}

\begin{corollary}
\label{corollary: cr rank of matrix, sups-rows}
Предположим, что $A$ - матрица,
$\CRRank a=k<m$.
Тогда \sups строки матрицы \dcr линейно зависимы.
\ShowEq{cr rank of matrix, sups-rows, 1}
\end{corollary}

\section{Система \texorpdfstring{$\RCstar D$}{rcD}\hyph линейных уравнений}

\begin{definition}
Предположим, что\footref{footnote: index assumption}
$A$ - матрица системы \drc линейных уравнений
\EqRef{star columns system of linear equations}.
Мы будем называть матрицу
\ShowEq{extended matrix, system of drc linear equations}
\AddIndex{расширенной матрицей}{extended matrix, system of drc linear equations} этой системы.
\qed
\end{definition}

\begin{definition}
Предположим, что\footref{footnote: index assumption}
$A$ - матрица системы \rcd линейных уравнений
\EqRef{star rows system of linear equations}.
Мы будем называть матрицу
\ShowEq{extended matrix, system of rcd linear equations}
\AddIndex{расширенной матрицей}{extended matrix, system of rcd linear equations} этой системы.
\qed
\end{definition}

\begin{theorem}
\label{theorem: star rows system of linear equations}
Система \rcd линейных уравнений \EqRef{star rows system of linear equations}
имеет решение тогда и только тогда, когда
\ShowEq{star rows system of linear equations, rank}
\end{theorem}
\begin{proof}
Пусть $\SA T$ - \RC главная минорная матрица матрицы $A$.

Пусть система \rcd линейных уравнений \EqRef{star rows system of linear equations}
имеет решение
\ShowEq{star rows system of linear equations, solution}
Тогда
\ShowEq{star rows system of linear equations, 1}
Уравнение \EqRef{star rows system of linear equations, 1} может быть записано в форме
\ShowEq{star rows system of linear equations, 2}
Подставляя \EqRef{rc rank of matrix, sups-rows} в
\EqRef{star rows system of linear equations, 2}, мы получим
\ShowEq{star rows system of linear equations, 3}
Из \EqRef{star rows system of linear equations, 3} следует, что \subs строка
$b$ является \rcd линейной комбинацией \subs строк $A_T$
\ShowEq{star rows system of linear equations, 4}
Это эквивалентно уравнению \EqRef{star rows system of linear equations, rank}.

Нам осталось доказать, что существование решения \rcd системы линейных уравнений
\EqRef{star rows system of linear equations} следует из
\EqRef{star rows system of linear equations, rank}.
Истинность \EqRef{star rows system of linear equations, rank} означает, что
$\SA T$ - так же \RC главная минорная матрица расширенной матрицы.
Из теоремы \ref{theorem: rc rank of matrix, sups-rows} следует, что \subs строка $b$
является \rcd линейной композицией \subs строк $A_T$
\ShowEq{star rows system of linear equations, 5}
Полагая
\ShowEq{star rows system of linear equations, 6},
мы получим
\ShowEq{star rows system of linear equations, 7}
Следовательно, мы нашли, по крайней мере, одно решение системы \rcd линейных уравнений
\EqRef{star rows system of linear equations}.
\end{proof}

\begin{theorem}
\label{theorem: star rows system of linear equations, solution}
Предположим, что \EqRef{star rows system of linear equations}
- система \rcd линейных уравнений,
удовлетворяющих \EqRef{star rows system of linear equations, rank}.
Если $\RCA=k\le m$,
то решение системы зависит
от произвольных значений $m-k$ переменных,
не включённых в \RC главную минорную матрицу.
\end{theorem}
\begin{proof}
Пусть $\SA T$ - \RC главную минорную матрицу матрицы $a$.
Предположим, что
\ShowEq{star rows system of linear equations, reduce, 1}
уравнение с номером $p$.
Применяя теорему \ref{theorem: rc rank of matrix, subs-rows}
к расширенной матрице \EqRef{extended matrix, system of drc linear equations}, мы получим
\ShowEq{star rows system of linear equations, reduce}
Подставляя \EqRef{star rows system of linear equations, reduce, 2}
и \EqRef{star rows system of linear equations, reduce, 3}
в \EqRef{star rows system of linear equations, reduce, 1}, мы получим
\ShowEq{star rows system of linear equations, reduce, 4}
\EqRef{star rows system of linear equations, reduce, 4} означает, что
мы можем исключить уравнение \EqRef{star rows system of linear equations, reduce, 1}
из системы \EqRef{star rows system of linear equations}
и новая система эквивалентна старой.
Следовательно, число уравнений может быть уменьшено до $k$.

В этом случае
у нас есть два варианта. Если число переменных также равно $k$, то
согласно теореме \ref{theorem: nonsingular system of linear equations} система имеет единственное решение
\EqRef{nonsingular system of linear equations, solution, quasideterminant}.
Если число переменных $m>k$, то мы можем передвинуть $m-k$ переменных, которые не
включены в \RC главную минорную матрицу в правой части.
Присваивая произвольные значения этим переменным, мы определяем значение
правой части и для этого значения мы получим единственное решение
согласно теореме \ref{theorem: nonsingular system of linear equations}.
\end{proof}

\begin{corollary}
\label{corollary:  nonsingular rows system of linear equations}
Система \rcd линейных уравнений \EqRef{star rows system of linear equations}
имеет единственное решение тогда и только тогда, когда
её матрица невырожденная.
\qed
\end{corollary}

\begin{theorem}
\label{theorem: Solutions homogenous system of linear equations}
Решения однородной системы \rcd линейных уравнений
\ShowEq{homogenous system of linear equations}
порождают \rcd векторное пространство.
\end{theorem}
\begin{proof}
Пусть $\Vector{X}$ - множество решений системы \rcd линейных уравнений
\EqRef{homogenous system of linear equations}.
Предположим, что
\ShowEq{homogenous system of linear equations x}
и
\ShowEq{homogenous system of linear equations y}
Тогда \[x^a\ _aa^b=0\] \[y^a\ _aa^b=0\]
Следовательно,
\ShowEq{homogenous system of linear equations x+y}
Таким же образом мы видим
\ShowEq{homogenous system of linear equations xb}
Согласно определению \ref{definition: Tstar vector space}
$\Vector{X}$ является \rcd векторным пространством.
\end{proof}

\section{Невырожденная матрица}

Предположим, что нам дана $n\times n$ матрица $A$.
Следствия \ref{corollary:rc rank of matrix, subs-rows}
и \ref{corollary:rc rank of matrix, sups-rows}
говорят нам, что если $\RCA<n$,
то \subs строки \drc линейно зависимы
и \sups строки \rcd линейно зависимы.\footnote{Это
утверждение похоже на утверждение
\citeBib{q-alg-9705026}-\href{http://arxiv.org/PS_cache/q-alg/pdf/9705/9705026.pdf\#Page=6}{1.2.5}.}

\begin{theorem}
\label{theorem: rc rank, sups rows}
Пусть $A$ - $n\times n$ матрица
и \sups строка $A_r$ - \rcd линейная комбинация других \sups строк.
Тогда $\RCA<n$.
\end{theorem}
\begin{proof}
Утверждение, что \sups строка $A_r$ является \rcd линейной комбинацией других \sups строк,
означает, что система \rcd линейных уравнений
\ShowEq{rc rank, sups rows}
имеет, по крайней мере, одно решение.
Согласно теореме \ref{theorem: star rows system of linear equations}
\ShowEq{rc rank, sups rows 1}
Так как число \sups строк меньше, чем $n$, то
\ShowEq{rc rank, sups rows 2}
\end{proof}

\begin{theorem}
\label{theorem: rc rank, subs rows}
Пусть $A$ - $n\times n$ матрица
и \subs строка ${}^pA$ - \drc линейная комбинация других \subs строк.
Тогда $\RCA<n$.
\end{theorem}
\begin{proof}
Доказательство утверждения похоже на доказательство теоремы
\ref{theorem: rc rank, sups rows}
\end{proof}

\begin{theorem}
Предположим, что $A$ и $B$ - $n\times n$ матрицы и
\begin{equation}
\EqLabel{RC product singular, 1}
C=A\RCstar B
\end{equation}
$C$ - \RC вырожденная матрица тогда и только тогда, когда
либо матрица $A$, либо матрица $B$ - \RC вырожденная матрица.
\end{theorem}
\begin{proof}
Предположим, что матрица $B$ - \RC вырожденная.
Согласно теореме \ref{theorem: rc rank of matrix, sups-rows}
\sups строки матрицы $B$
\rcd линейно зависимы. Следовательно,
\ShowEq{RC product singular, 2}
где $\lambda\ne 0$. Из
\EqRef{RC product singular, 1}
и \EqRef{RC product singular, 2} следует, что
\ShowEq{RC product singular, 3}
Согласно теореме \ref{theorem: rc rank, sups rows} матрица $C$
является \RC вырожденной.

Предположим, что матрица $B$ - не \RC вырожденная, но матрица $A$ - \RC вырожденная.
Согласно теореме \ref{theorem: rc rank of matrix, subs-rows}
\sups строки матрицы $A$
\rcd линейно зависимы. Следовательно,
\ShowEq{RC product singular, 4}
где $\mu\ne 0$. Согласно
теореме \ref{theorem: nonsingular system of linear equations} система
\ShowEq{RC product singular, 5}
имеет единственное решение, где $\lambda\ne 0$.
Следовательно,
\ShowEq{RC product singular, 6}
Согласно теореме \ref{theorem: rc rank, sups rows} матрица $C$ является \RC вырожденной.

Предположим, что матрица $C$ - \RC вырожденная матрица.
Согласно теореме \ref{theorem: rc rank of matrix, subs-rows}
\subs строки матрицы $C$
\rcd линейно зависимы. Следовательно,
\ShowEq{RC product singular, 7}
где $\lambda\ne 0$.
Из \EqRef{RC product singular, 1}
и \EqRef{RC product singular, 7} следует, что
\ShowEq{RC product singular, 8}
Если 
\ShowEq{RC product singular, 9}
выполнено, то матрица $B$ - \RC вырожденная. Предположим, что
матрица $B$ не \RC вырожденная. Положим
\ShowEq{RC product singular, 10}
где $\mu\ne 0$. Тогда
\ShowEq{RC product singular, 11}
Из \EqRef{RC product singular, 11} следует, что
матрица $A$ - \RC вырожденная.
\end{proof}

Опираясь на теорему \xRef{0612.111}{theorem: duality principle, quasideterminants},
мы можем записать подобные утверждения для \dcr линейной комбинации \subs строк
или \crd линейной комбинации \sups строк и \CR квазидетерминанта.

\begin{theorem}
\label{theorem: cr rank, rows}
Пусть $A$ - $n\times n$ матрица
и \sups строка ${}_rA$ - \crd линейная комбинация других \sups строк.
Тогда $\CRRank  A<n$.
\end{theorem}

\begin{theorem}
\label{theorem: cr rank, columns}
Пусть $A$ - $n\times n$ матрица
и \subs строка $A^p$ - \dcr линейная комбинация других \subs строк.
Тогда $\CRRank  A<n$.
\end{theorem}

\begin{theorem}
Предположим, что $A$ и $B$ - $n\times n$ матрицы и
$C=A\CRstar B$. $C$ - \CR вырожденная матрица тогда и только тогда, когда
либо матрица $A$, либо матрица $B$ - \CR вырожденная матрица.
\end{theorem}

\begin{definition}
\AddIndex{\RC матричная группа}{rc-matrix group}
\ShowEq{rc-matrix group}
- это группа
\RC невырожденных матриц, гле мы определяем
\RC произведение матриц
\xEqRef{0612.111}{rc-product of matrices}
и \RC обратную матрица
$A^{\CRInverse}$.
\qed
\end{definition}

\begin{definition}
\AddIndex{\CR матричная группа}{cr-matrix group}
\ShowEq{cr-matrix group}
- это группа
\CR невырожденных матриц
где мы определяем
\CR произведение матриц
\xEqRef{0612.111}{cr-product of matrices}
и \CR обратную матрицу
$A^{\CRInverse}$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: CR RC singular matrix}
\[
\RCGL nD\ne \CRGL nD
\]
\end{theorem}
\begin{remark}
Из теоремы
\xRef{0612.111}{theorem: RC-inverse matrix, delta}
следует, что
существуют матрицы, которые \CR невырожденны и \RC невырожденны.
Теорема \ref{theorem: CR RC singular matrix} означает, что множества
\CR невырожденных матриц и \RC невырожденных матриц
не совпадают. Например,
существует такая \RC невырожденная матрица, которая
\CR вырожденная матрица.
\qed
\end{remark}
\begin{proof}
Это утверждение достаточно доказать для $n=2$.
Предположим, что каждая \CR вырожденная матрица
\ShowEq{RC-singular matrix, 1}
является \RC вырожденной матрицей.
Из теоремы \ref{theorem: rc rank of matrix, sups-rows} и
теоремы \ref{theorem: rc rank of matrix, sups-rows} следует, что
\RC вырожденная матрица удовлетворяет условию
\ShowEq{RC, a22, 1}
Если мы подставим \EqRef{RC, column, 1 2, 1 1}
в \EqRef{RC, row, 2 2, 1 2}, мы получим
\ShowEq{RC, a22, 2}
$b$ и $c$ - произвольные элементы тела $D$ и \RC вырожденная матрица
\EqRef{RC-singular matrix, 1} имеет вид ($d={}^1A_1$)
\ShowEq{RC-singular matrix, 2}
Подобным образом мы можем показать, что \CR вырожденная матрица
имеет вид
\ShowEq{CR-singular matrix, 2}
Из предположения следует, что \EqRef{CR-singular matrix, 2}
и \EqRef{RC-singular matrix, 2} представляют одну и ту же матрицу.
Сравнивая \EqRef{CR-singular matrix, 2}
и \EqRef{RC-singular matrix, 2}, мы получим, что
для любых $d,c\in D$ существует такое $c'\in D$, которое не зависит от $d$ и
удовлетворяет уравнению
\[d c=c'd\]
Это противоречит утверждению, что $D$ - тело.
\end{proof}

\begin{example}
В случае тела кватернионов мы положим $b=1+k$, $c=j$, $d=k$.
Тогда мы имеем
\ShowEq{example rc singular matrix}

Система \rcd линейных уравнений
\ShowEq{example rc singular matrix, rcd}
имеет \RC вырожденную матрицу.
Мы можем записать систему \rcd линейных уравнений
\EqRef{example rc singular matrix, rcd} в виде
\ShowEq{example rc singular matrix, rcd 1}

Система \crd линейных уравнений
\ShowEq{example rc singular matrix, crd}
имеет \CR невырожденную матрицу.
Мы можем записать систему \crd линейных уравнений
\EqRef{example rc singular matrix, crd} в виде
\ShowEq{example rc singular matrix, crd 1}

Система \drc линейных уравнений
\ShowEq{example rc singular matrix, drc}
имеет \RC вырожденную матрицу.
Мы можем записать систему \drc линейных уравнений
\EqRef{example rc singular matrix, drc} в виде
\ShowEq{example rc singular matrix, drc 1}

Система \dcr линейных уравнений
\ShowEq{example rc singular matrix, dcr}
имеет \CR невырожденную матрицу.
Мы можем записать систему \dcr линейных уравнений
\EqRef{example rc singular matrix, dcr} в виде
\ShowEq{example rc singular matrix, dcr 1}
\qed
\end{example}
\fi

\section{Размерность \texorpdfstring{$\RCstar D$}{rcD}\hyph векторного пространства}
\label{section: Dimension of Vector Space}

\begin{theorem}
\label{theorem: basis of vector space}
Пусть $V$ - \rcd векторное пространство. Предположим, что $V$ имеет базисы
\ShowEq{basis e of V}
и
\ShowEq{basis g of V}
Если $|I|$ и $|J|$ - конечные числа, то $|I|=|J|$.
\end{theorem}
\begin{proof}
Предположим, что $|I|=m$ и $|J|=n$. Предположим, что
\begin{equation}
m<n
\EqLabel{basis of vector space, 0}
\end{equation}
Так как $\Basis e$ - базис, любой вектор
\ShowEq{basis g of V 1}
имеет разложение
\ShowEq{basis g of V 2}
Так как $\Basis{g}$ - базис,
\ShowEq{basis g of V 3}
следует из
\ShowEq{basis g of V 4}
Так как $\Basis e$ - базис, мы получим
\ShowEq{basis g of V 5}
Согласно \EqRef{basis of vector space, 0}
$\RCA\le m$ и система \EqRef{basis g of V 5}
имеет больше переменных, чем уравнений. Согласно теореме
\ePrints{4993-2400}
\ifx\Semafor\ValueOff
\ref{theorem: star rows system of linear equations, solution},
\else
\xRef{4776-3181}{theorem: star rows system of linear equations, solution},
\fi
$\lambda\ne 0$. Это противоречит
утверждению \EqRef{basis g of V 3}. 
Следовательно, утверждение $m<n$ неверно.

Таким же образом мы можем доказать, что утверждение $n<m$ неверно.
Это завершает доказательство теоремы.
\end{proof}

\begin{definition}
Мы будем называть
\AddIndex{размерностью \rcd векторного пространства}{dimension of vector space}
число векторов в базисе
\qed
\end{definition}

\begin{theorem}
\label{theorem: coordinate matrix of basis}
Координатная матрица \rcd базиса $\Basis{g}$ относительно \rcd базиса $\Basis e$
векторного пространства $V$ является \RC невырожденной матрицей.
\end{theorem}
\begin{proof}
Согласно лемме \ref{theorem: rank of coordinate matrix}
\rcd ранг координатной матрицы базиса $\Basis{g}$ относительно базиса $\Basis e$
равен размерности векторного пространства, откуда следует утверждение теоремы.
\end{proof}

\begin{definition}
Мы будем называть взаимно однозначное отображение
\DrawEq{A:V->W}{}
\AddIndex{изоморфизмом \rcd векторных пространств}{isomorphism of vector spaces},
если это отображение - линейное отображение
\rcd векторных пространств.
\qed
\end{definition}

\begin{definition}
\AddIndex{Автоморфизм \rcd векторного пространства}{automorphism of vector space}
$V$ - это изоморфизм $A:V\rightarrow V$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: automorphism of vector space}
Предположим, что $\Basis f$ - \rcd базис в векторном пространстве $V$.
Тогда любой автоморфизм $\Vector A$ \rcd векторного пространства
$V$ имеет вид
\ShowEq{automorphism, vector space}
где $A$ - \RC невырожденная матрица.
\end{theorem}
\begin{proof}
\EqRef{automorphism, vector space} следует из
теоремы \ref{theorem: linear map of rcd vector space}.
Так как $\Vector A$ - изоморфизм, то для каждого вектора $v'$ существует единственный вектор $v$ такой,
что $v'=v\RCstar \Vector A$.
Следовательно, система \rcd линейных уравнений \EqRef{automorphism, vector space}
имеет единственное решение. Согласно следствию \ref{corollary: nonsingular rows system of linear equations}
матрица $A$ невырожденна.
\end{proof}

\begin{theorem}
\label{theorem: Automorphisms of vector space form a group}
Автоморфизмы \rcd векторного пространства порождают группу $\RCGL nD$.
\end{theorem}
\begin{proof}
Если даны два автоморфизма $\Vector A$ и $\Vector B$, то мы можем записать
\ShowEq{Automorphisms of vector space}
Следовательно, результирующий автоморфизм имеет матрицу $B\RCstar A$.
\end{proof}

